Security, Fault Tolerance, and Communication Complexity in Distributed Systems

We present efficient and practical algorithms for a large, distributed system of processors to achieve reliable computations in a secure manner. Specifically, we address the problem of computing a general function of several private inputs distributed among the processors of a network, while ensuring the correctness of the results and the privacy of the inputs, despite accidental or malicious faults in the system. [...] Our algorithms maintain a low cost in local processing time, are the first to achieve optimal levels of fault-tolerance, and most importantly, have low communication complexity. In contrast to the best known previous methods, which require large numbers of rounds even for fairly simple computations, we devise protocols that use small messages and a constant number of rounds regardless of the complexity of the function to be computed. Through direct algebraic approaches, we separate the communication complexity of secure computing from the computational complexity of the function to be computed. We examine security under both the modern approach of computational complexity-based cryptography and the classical approach of unconditional, information-theoretic security. We [...] support formal proofs of claims to security, addressing an important deficiency in the literature. Our protocols are provably secure. In the realm of information-theoretic security, we characterize those functions which two parties can compute jointly with absolute privacy. We also characterize those functions which a weak processor can compute using the aid of powerful processors without having to reveal the instances of the problem it would like to solve. Our methods include a promising new technique called a locally random reduction, which has given rise not only to efficient solutions for many of the problems considered in this work but to several powerful new results in complexity theory.

==> abs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% abs.tex                    Abstract.
%
%                            Copyright @1989  Donald Beaver.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{center}
\bf Abstract
\end{center}

\vspace*{.2in}

We present efficient and practical algorithms for a large, distributed
system of processors to achieve reliable computations in a secure manner.
Specifically, we address the problem of computing a general function of
several private inputs distributed among the processors of a network,
while
ensuring the correctness of the results and the privacy of the inputs,
despite accidental or malicious faults in the system.  

Communication is often the most significant bottleneck in distributed
computing.
Our algorithms
maintain a low cost in local processing time, are the first to
achieve optimal levels of fault-tolerance, and most importantly, have low
communication complexity.  In contrast to the best known previous methods,
which require large numbers of rounds even for fairly simple computations,
we devise protocols that use small messages and a constant number of rounds
{\em regardless} of the complexity of the function to be computed.  Through
direct algebraic approaches, we separate the {\em communication complexity
of secure computing} from the {\em computational complexity} of the
function to be computed.

We examine security under both the modern approach of computational
complexity-based cryptography and the classical approach of unconditional,
information-theoretic security.  We develop a clear and concise set of
definitions that support formal proofs of claims to security, addressing an
important deficiency in the literature.  Our protocols are provably secure.

In the realm of information-theoretic security, we characterize those
functions which two parties can compute jointly with absolute privacy.  We
also characterize those functions which a weak processor can compute using
the aid of powerful processors without having to reveal the instances of
the problem it would like to solve.  Our methods include a promising new
technique called a {\em locally random reduction}, which has given rise not
only to efficient solutions for many of the problems considered in this
work but to several powerful new results in complexity theory.




==> ack.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ack.tex                    Acknowledgments.
%
%                            Copyright @1989  Donald Beaver.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{center}
{\bf Acknowledgments}
\end{center}

\bigskip

I would very much like to acknowledge the guidance and advice of
my advisor, Michael Rabin, and of my unofficial advisor, Joan
Feigenbaum, whose help and efforts on my behalf have been instrumental.
I would also like to thank 
Roger Brockett, 
Shafi Goldwasser, 
Mei Hsu, 
and
Les Valiant. 
Several institutions besides Harvard have provided formal and informal
support and a productive working environment, including 
Williams College, 
Cal Tech, 
the Hebrew University of Jerusalem, 
MIT,
the Deutsches Forschungszentrum f\"{u}r K\"{u}nstliche Intelligenz, 
and the New York Public Library.
This work was supported in part by NSF grant CCR-870-4513.

The great many colleagues and graduate students who have
made the past four years enjoyable, intellectually stimulating, or just
bearable are too many to mention, but in particular I would like to thank
Judit Bar-Ilan,
Stuart Haber,
Christos Kaklamanis,
Philip Klein,
Danny Krizanc,
Lisa Neal,
Rafail Ostrovsky,
Nir Shavit,
and
Thanasis Tsantilas.

I especially want to thank 
Susan Greenbaum,
Amanda Lathroum, 
Beralda Concei\c{c}ao de Lima,
and 
Gerry Waggett
for their unending support and inspiration.

And, of course, without two very important Professors, 
Don and Ollie Beaver, this effort would not have been possible.  
I dedicate this work to them, to all of my family,
and especially to my brother, James.





==> app.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% app.tex                    Anonymous Mail and Authentication.
%
%                            Copyright @1989  Donald Beaver.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{=======}
\typeout{app.tex}
\typeout{=======}


\chapter{Applications}       \label{chap-app}

\chapquote{
The artist possesses the ability to breathe soul into the lifeless
product of the machine.
}{
Walter Gropius}
% thanks to Emily Klotz, 5/3/90

The bulk of this dissertation has addressed formal specifications of
protocols for networks of players to compute arbitrary functions in a
distributed manner.  In this chapter we present efficient and
practical solutions for useful and important computations.

It would certainly be impractical to require multiparty protocols around
each distributed computation a collection of processors must make.  Some
computations, especially administrative and system-security oriented
computations, are of greater importance than others, but at the same time
need to be performed less often.  For example, authenticating a user or a
remote process must be correct and secure but are performed with lower
frequency than other computations.  Authorizing access to a file is another
example.

We propose very fast protocols for authentication\index{authentication},
authorization\index{authorization}, and anonymous mail\index{anonymous
mail}. These protocols are designed with specific goals in mind and
capitalize on properties that a general-purpose protocol-compiler (based
only on circuit specifications) ignores.

For the purposes of ensuring distributed system reliability, we envision a
{\em security kernel},\index{security kernel} in terms of processors and of
processes.  That is, not all the processors in a network need be involved
in ensuring the resilience of every computation.  A specific committee of,
say, seven processors would suffice, with the assurance that no more than
three are compromised.  These processors are tightly coupled with
high-speed secure communication lines.

With respect to the operations themselves, we propose that authentication
and authorization are infrequent yet essential computations, and that it is
reasonable to take special care to ensure the correct and secure operation
of a small body of desired processes.  Once a process has been
authenticated and authorized to read a file, the authorization need not be
repeated and the authentication can be omitted during repeated file access
requests.  

The Secure UNIX of Reeds and McElroy \cite{mr87,mr88-1,mr88-2,ree89} adopts
this sort of approach, allowing two remote processes to communicate over a
single pipe that excludes other processes and that fails as soon as one
process detaches.  While this does allow certain attacks to succeed --- a
corrupt operating system might capture an authorized line to a remote
system by running an authenticated process and substituting its own process
after the authentication with the remote host has occurred --- the attacks
are more difficult and complex.  Furthermore, a repeated authentication of
the {\em host} operating system, not each individual process at each
individual request, would serve as a more efficient safety check.  If the
host is continually authenticated then presumably its operations are valid
and the processes it runs cannot be substituted after their initial
authentication.  This is a reasonable trade-off of absolute security for
practicality.

Our efficient algorithms for specific tasks support the approach of
infrequent yet highly efficient and secure kernel operations.  We focus not
simply on achieving a constant number of rounds of interaction but on
achieving a {\em small} constant number of rounds, on the order of 2 or 3.

\section{On Strong Assumptions}
\label{sec-strong-ass}

In general, we assume a completely connected, synchronous network with
private lines\index{assumptions!noncryptographic}.  The robustness of
polynomial interpolation suggests the techniques developed here should be
adaptable to asynchronous models.  The fault-tolerance levels would be
lower, and many technical issues must be considered (such as the
availability of broadcast channels {\em vs.} Byzantine Agreement
subprotocols).  Because our protocols are robust against fail-stop faults,
their extension to problems of asynchronicity is natural.

A network without private lines\index{channel!private} can still use the
protocols developed here if suitable encryption of the lines is available.
Care must be taken to ensure that this approach of treating sub-issues in a
modular fashion does in fact treat each module independently --- for
example, to avoid unintended interaction between the design of the overall
protocol and the design of a communication line protection scheme, the same
encryption methods should not be used at all levels.  That is, if a
protocol assumes a private channel but also requires an encryption for
other reasons, the same encryption should not be used to replace the
private channel with an encrypted channel\index{channel!encrypted}.
Proofs of security remain necessary.

We have also assumed a complete network\index{network!complete}.  This
assumption is highly unlikely to hold except on a local-area network.  In
practical terms, however, it is not hard to achieve for a processor
security kernel with a small number of tightly-coupled processors.  In
theoretical terms, the issue of simulating a complete network using a
$t+1$-connected network is an interesting separate subproblem.

The modular treatment of the various subproblems provides optimism for the
design of very general protocols that are robust under very harsh
circumstances.  A word of caution must be interjected: as always, intuitive
claims to security require formal treatment.  But the modular approach
makes the analysis easier.



\section{Choice of Field}

For the purpose of implementation, we suggest a few natural finite fields.%
\index{field}

The first is $\gf(257),$ the set of integers modulo 257.  This field easily
encodes bytes using integers in the range 0---255.  Modular arithmetic is
fast and standard, though individual bit operations on the eight bits are
not quite so facile.  Two-byte words are supported by a modulus of
32771.

The other fields we suggest have characteristic 2: $\gf(256)=\gf(2^8),$
$\gf(65536)=\gf(2^{16}),$ $\gf(2^{32}),$ and $\gf(2^{64}),$
Field elements are represented as polynomials over $\gf(2)$ modulo an
irreducible polynomial (for example, $x^8+x^4+x^3+x^2+1$ for
$\gf(2^8),$ $x^{16}+x^{12}+x^3+x+1$ for $\gf(2^{16}),$ and 
$x^{32}+x^{22}+x^2+x+1$ for $\gf(2^{32})$).
% see Weldon Error Correct
% 2^64 a bit big to do by hand
Each coefficient is a single bit, so that the field elements themselves
correspond naturally to common word-sizes.  Addition over these fields is
quite simple and normally requires a single machine instruction: take the
bitwise exclusive-or.  Multiplication is somewhat more complicated,
requiring one to reduce the product modulo the appropriate irreducible
polynomial, but fast algorithms exist.

Generating random {\em bits} as the exclusive-or of random bits supplied by
many players is much easier using a field of characteristic 2 than one of
characteristic 257, since addition of random secret 0/1 values will
suffice.  In general, bitwise operations are facilitated by using
arithmetic over a field of characteristic 2.



\section{A Fast and Practical Password Scheme}
\label{sec-auth}

In the UNIX$^{tm}$ password\index{password} scheme for user authentication,
the passwords are not stored in a file on the system.  Rather, each
password is encrypted (using a DES-like encryption function) and the result
is stored in a password file.  Even if the password file is compromised, an
attacker cannot learn the passwords directly from the file.  When a user
would like to log in to the system, his attempted password is encrypted and
compared against the stored encryption.  If they match, the user is
authenticated.

One can imagine a generalization to the distributed environment in which
each host authenticates the user and the system as a whole considers the
user acceptable if a majority of the hosts have authenticated him.  An
immediate problem surfaces with password schemes: if the same password is
used for all the hosts, then a single corrupt host will learn the user's
global password when the user requests authentication.  This can be
circumvented by having a different password for each host (requiring some
nontrivial and probably security-prone bookkeeping by the user).
Nevertheless, there are many disadvantages, including the fundamental
problem that the encryption function itself is only {\em assumed} to be
unbreakable.

We propose a simple and efficient password scheme
\footnote{
This work was done while the author was on leave of absence from Harvard
University in the spring and summer of 1988.} 
%
discovered independently by Michael Rabin \cite{rab89-pc} that has some
similar properties but does not depend on the security of an encryption
function like DES.  That is, passwords cannot be obtained by capturing the
files on some fraction of the systems, and are certainly not compromised
during an execution in which {\em one} of the hosts is corrupt.  In order
to break the password directly, an attacker must corrupt a majority of the
hosts (we ignore dictionary searches and repeated attempts, which are
certainly valid issues for any password scheme but are orthogonal to the
problem of breaking the system directly).

The basic idea is as follows: a user secretly shares his password
$\password$ among the system at start-up.  Later, when he requests
authentication, he demonstrates his knowledge of the password by sharing it
again.  Let us call the second secret his attempt, $\attempt.$ The system
must compare $\password$ to $\attempt$ {\em without revealing $\password$}.

\boxfig{
\noindent{\bf \Proto{Initialize-Password}}
\index{password}
\begin{tabbing} \standtabs
%%%%%%%%%%%%%%%%%%
Let $E=\gf(2^{64}).$
Simultaneously: \\
      \> User shares $\password.$ \\
      \> \parbox[t]{4.7in}{
      Each host $i$ selects two uniformly random 64-bit elements $r_i,s_i,$
and shares them.} \\
      \> \parbox[t]{4.7in}{
      Run the \add protocol (non-interactively) to secretly compute }\\
      \>\>\> $r=\sum r_j, s=\sum s_j:$ \\
      \>\> --- More precisely, each host $i$ sets \\
      \>\>\>   $\piece_i(r) = \sum_j \piece_i(r_j)$ \\
      \>\>\>   $\piece_i(s) = \sum_j \piece_i(s_j)$ \\
\end{tabbing}
\caption{\label{fig-init-pass}
Protocol to initialize a user's password in a distributed system of
$n$ hosts.  
}}


It does not suffice to compute $(\password - \attempt)$ and reveal the
result, since knowing $\attempt$ would then reveal $\password.$ This
remains true even if the {\em user} is not supplied with the result; if the
user cooperates with just one corrupted host involved in the
authentication, then that host can reveal the result when it learns it.

One solution is to use Theorem~\ref{thm-nc1} to secretly compute
$\norm{\password - \attempt}$ in a constant number of rounds.  The protocol
most certainly is correct and uses only a few rounds, but we propose an
even simpler and more efficient protocol that is designed with the
particular password problem in mind.

The essential information that the system must compute is whether or not
$\password = \attempt.$ The result of the computation should specify
whether or not they are equal, but it need not be a deterministic result;
that is, the result need not be either 0 or 1.  What matters is that if the
values are not equal, the result of the computation should have the same
distribution regardless of what attempt is made and of what the password
is.  The problem of revealing information about the password through a
failed attempt is then solved.

The trick is the following: compute and then reveal $(\password -
\attempt)\cdot r,$ where $r$ is secret and uniformly random over $E -
\set{0}.$ If the attempt is correct, then the result is always 0.  But if
the attempt is invalid, then the result will be a uniformly distributed
nonzero random field element, for any $\password$ and $\attempt.$ Thus, no
information about $\password$ or $\attempt$ is revealed by the result, apart
from whether they are identical or not.  The system accepts the user if and
only if the result is 0;
each host outputs {\em accept} if the result is 0 and otherwise outputs
{\em reject}.

The only minor inefficiency is to generate a nonzero random field element.
The \randomsecret protocol will generate a uniformly random secret $r$ in
$E,$ but we should then have to normalize it in order to test if $r=0,$
returning us to the original problem.  One simple and acceptable approach
is simply to finesse the problem by using a large field $E$ so that the
chance that $r=0$ is negligible.  This would allow some very low
probability that a failed attempt will succeed.  In fact, the chance of
such an event is the same as guessing a valid password.  See
Figure~\ref{fig-authfast}.

\boxfig{
\noindent{\bf \authfast}
\index{authorization}
\begin{tabbing} \standtabs
%%%%%%%%%%%%%%%%%%
(A1) 
  \>  User shares $\attempt.$ \\
  \> \parbox[t]{4.7in}{
  Run the \add protocol (non-interactively) to secretly compute 
  $v=\password - \attempt.$} \\
  \>\> --- More precisely, each host $i$ sets \\
\>\>\>$\piece_i(v) = \piece_i(\password) - \piece_i(\attempt)$ \\
(A2) 
  \> \parbox[t]{4.7in}{
  To be ready for the {\em next} authentication,
  each host $i$ selects two uniformly random 64-bit elements
  $r_i^{new},s_i^{new},$ and shares them.  Each host $i$ sets} \\
      \>\>\>   $\piece_i(r^{new}) = \sum_j \piece_i(r_j^{new})$ \\
      \>\>\>   $\piece_i(s^{new}) = \sum_j \piece_i(s_j^{new})$ \\
  \>  Run the \mult protocol to secretly compute $w=v \cdot r.$ \\
  \>  \If $w=0$ \Then {\em accept} the user, \Else {\em reject} the user. 
\end{tabbing}
\caption{\label{fig-authfast}
\index{\authfast}
Protocol to authenticate user who has already shared password $\password.$  
}}


The chance that the scheme is broken through this error is less than that
of randomly selecting a password, and it is neither repeatable (the user
has no control over $r$) nor assisted by ulterior means (such as dictionary
lookups).  It therefore doubles at most the inherent chance of failure.
Figure~\ref{fig-authfast} describes the stripped-down scheme.  One round
suffices to share the attempt, and one to check it (with only fail-stop
errors).

A completely accurate solution is the following: generate a second random
secret, $s,$ and multiply it by $r.$ If the result is nonzero, then the
system has a proof that $r \not=0$ without revealing $r.$

The chance that randomly choosing $r$ and $s$ gives $r=0$ or that $r\not=
0$ and $s=0$ is small: $\frac{2 \mid E \mid -1}{\mid E\mid^2}.$ Otherwise,
with high probability the system has generated a uniformly random nonzero
secret $r,$ along with a (``zero-knowledge'') certificate that $r
\not= 0.$

For concreteness, let us use the field $\gf(2^{64})$ to handle passwords of
8 bytes.  The password set-up protocol is described in
Figure~\ref{fig-init-pass}.  The authentication protocol is described in
Figure~\ref{fig-auth}.  Note that in the authentication protocol, a failure
to obtain a nonzero secret $r$ requires that the network generate one; this
occurs with probability $2^{-64}$ and can essentially be ignored.




\boxfig{
\noindent{\bf \auth}
\index{authorization}
\begin{tabbing} \standtabs
%%%%%%%%%%%%%%%%%%
(A1) 
  \>  User shares $\attempt.$ \\
  \> \parbox[t]{4.7in}{
  Run the \add protocol (non-interactively) to secretly compute 
  $v=\password - \attempt.$} \\
  \>\> --- More precisely, each host $i$ sets \\
\>\>\>$\piece_i(v) = \piece_i(\password) - \piece_i(\attempt)$ \\
(A2) 
  \> \parbox[t]{4.7in}{
  To be ready for the {\em next} authentication,
  each host $i$ selects two uniformly random 64-bit elements
  $r_i^{new},s_i^{new},$ and shares them.  Each host $i$ sets} \\
      \>\>\>   $\piece_i(r^{new}) = \sum_j \piece_i(r_j^{new})$ \\
      \>\>\>   $\piece_i(s^{new}) = \sum_j \piece_i(s_j^{new})$ \\
  \>  Run the \mult protocol to secretly compute $w=v \cdot r.$ \\
  \>  Run the \mult protocol to secretly compute $u=r \cdot s.$ \\
(A3) 
  \>  (Refer to $r^{new}$ as $r$ and $s^{new}$ as $s.$) \\
  \>  Reconstruct $w$ and $u.$\\
  \>  \If $u \not= 0$ \Then: \\
  \>\>  \If $w=0$ \Then {\em accept} the user, \Else {\em reject} the user. \\
  \>  \If $u=0$ \Then repeat step (A2). \\
\end{tabbing}
\caption{\label{fig-auth}
Protocol to authenticate user who has already shared password $\password.$  
}}


\begin{theorem} \label{thm-auth}
For $2t<n,$ protocol \auth is statistically $t$-resilient and requires
a constant expected number of rounds.
\end{theorem}

\begin{proof}
Clearly, host $i$ outputs {\em accept} iff $r \not= 0$ and
$(\password-\attempt)\cdot r = 0,$ {\em i.e.} iff $\password = \attempt.$
If $\password=\attempt,$ the distribution on $(w,u)$ is 
\[
\set{r \leftarrow \uniform(E); s \leftarrow \uniform(E): (0,rs) },
\]
regardless of the values of $\password$ and $\attempt.$ 
If $\password \not= \attempt,$ the distribution on $(w,u)$ is the
distribution
\[
\set{r \leftarrow \uniform(E); s \leftarrow \uniform(E): 
((\password-\attempt) \cdot r,rs)}, 
\]
which for any (unequal) values of $\password$ and $\attempt,$ 
is fixed and identical to
\[
\set{r \leftarrow \uniform(E); s \leftarrow \uniform(E); 
w \leftarrow \uniform(E-\set{0}): (w,rs)}.
\]
\end{proof}

\begin{corollary} \label{cor-auth}
For $2t<n,$ Protocol \auth is $t$-resilient against passive (or even
fail-stop) adversaries and requires only $(3+\epsilon)$ expected rounds,
where $\epsilon=4/\abs{E}$ is small.
\end{corollary}

\begin{proof}
Follows from Theorem~\ref{thm-auth} and the observation that, when messages
are always correct, the number of rounds required for sharing and for
multiplying secrets is 1.  Step (A2) is repeated with probability 
$\frac{2 \mid E \mid -1}{\mid E\mid^2},$ which gives an expected time 
less than $4/\abs{E}$ when $\abs{E}\geq 7.$
\end{proof}


\noindent {\bf Remark:}  The secure authentication schemes we have
presented take the same amount of time as the simple method of having a
user authenticate itself to each processor separately and then taking a
vote.  They provide, on the other hand, a good deal more robustness.  For
example, once an intruder has recorded the message from a valid user to one
host in the voting scheme, that password can be re-used; the invader need
only accumulate enough attacks over time.  In our scheme, however, at least
half of the communications must be tapped {\em simultaneously} to obtain
{\em any} information at all.


\subsection{Unanimous Secret Ballots}

Secret ballots are fast and simple (\S\ref{sec-ballots}), and by
Theorem~\ref{thm-nc1}, checking whether a secret vote is {\em unanimous} or
not, without revealing the tally, also admits a protocol in constant
rounds.  The authorization techniques listed above suggest a faster and
more direct method: first compute $v=\sum_i x_i,$ where each $x_1$ is a
verified 0/1 secret vote, generate a random (nonzero) secret $r,$ and
secretly compute $vr.$ Reveal the result.  If the ballot is unanimous, the
result will be 0; otherwise it will be a uniformly distributed nonzero
number.


\section{Anonymous Mail}
\label{sec-anon}
\index{anonymous mail}\index{mail}

A mail system ought to provide privacy on two levels.  First, it should
hide the contents of each message from the general public, and certainly
from those involved in its delivery.  Second, it should not need to
identify the sender of the message, either to those involved in the
delivery or to the recipient.  It does not suffice simply to deliver a
message without attaching a sender's name in the header, since the name of
the originating host or workstation may be enough to reveal the sender.  In
fact, the delivery of anonymous messages in a network is powerful enough to
support general function computation \cite{bbr88}, though we shall not go
into the details here.  Delivering mail anonymously even when hosts are
identified is thus a powerful and a useful tool.

To be practical, however, a mail scheme must be efficient.  If the message
is an undivided unit, then it traverses some path from the sender S to the
receiver R.  If every host on that path is corrupt, then the receiver can
identify the origin.  Thus the path must be longer than the number $t$ of
corruptible hosts.  Already this is a very inefficient solution.
Furthermore, it requires that the message be encrypted in some form so that
the intermediate hosts cannot read the contents.

We adopt a different approach: divide the message in an appropriate manner
and send each portion via a different path.  If sufficiently few pieces are
captured, then nothing is learned about the contents.  Secretly sharing the
message and reconstructing it for the recipient suffices.  This is trivial
in a complete network with private channels, but in an incomplete network,
when two players may be forced to communicate via intermediate players,
secret sharing solves the problem of privacy robustly.  

Preserving the privacy of the sender, however, is a slightly more difficult
goal.  We must ensure that the paths to R do not identify S.  Thus, the
direct approach of as secretly sharing the message and reconstructing it
for R is suggestive, but not sufficient.  Every host knows {\em who} shared
the secret.

Consider the following situation: there is some secret permutation $\sigma$
on the elements $\set{1,\ldots,n},$ and each player $i$ knows $\sigma(i).$
Each player $i$ would like to send a message $M(i)$ to player $\sigma(i)$
without identifying itself.  We would like to compute a function $F$ such
that $F_{\sigma(i)}(M(1),\ldots,M(n),\sigma(1),\ldots,\sigma(n)) =M(i).$

One method to perform this computation would be to compute 
\[
F_j(M(1),\ldots,M(n),\sigma(1),\ldots,\sigma(n) =
\sum_{i=1}^n M(i) \delta(\sigma(i),j)\index{delta}
\]
Because the delta function is in $NC^1,$ Theorem~\ref{thm-nc1} implies
there is a constant-rounds protocol to compute $F.$  Note that we have
omitted a verification that the secrets $\sigma(1),\ldots,\sigma(n)$ do
indeed define a permutation; malicious players could upset the protocol.
An additional function that compares each pair of destinations and makes
sure no collisions occur is a necessary prerequisite.

A more efficient way is the following.  Each player, instead of sharing
$\sigma(i),$ shares a set of $n$ secrets $d(i,1),\ldots,d(i,n),$ such that
$d(i,\sigma(i))=1$ and the remaining secrets are 0.  It is trivial to check
privately that every $d(i,j)$ is 0 or 1 by computing and revealing
$d(i,j)(d(i,j)-1).$ It is also trivial to ensure that each player shares a
valid vector, by computing $\sum_j d(i,j)$ for each $i$ and revealing the
sums.  Thirdly, it is trivial to check for collisions by taking $\sum_i
d(i,j)$ for each $j$ and revealing the sums.  (Collisions give a sum
greater than 1, which reveals no information to the faulty processors that
changed their destinations.)  Thus there are three simple verifications to
perform in parallel, requiring the time of one multiplication and
reconstruction.

Given verified vectors, the final outputs are simply
\[
F_j(M(1),\ldots,M(n),d(1,1),\ldots,d(n,n)) =
\sum_{i=1}^n M(i) d(i,j).
\]

This construction gives an easy solution to the converse problem, {\em
limited espionage.}\index{espionage}%
%
\footnote{The terms {\em espionage} and {\em anonymous mail} were suggested
by M. Rabin.}
%
Like 1-out-of-2 Oblivious Transfer, in which the recipient chooses one of
two values to learn but the holder does not find out which, limited
espionage allows each player in the network to learn one secret from a list
of $N$ secrets without revealing which one it chose.  The protocol requires
each player to share a 0/1 vector specifying a 1 in the component
corresponding to the secret it desires, and the verifications are performed
as above before computing the simple weighted sum.  Note that in this case,
collisions need not be avoided; two players may look at the same secret.

The general problem of supporting arbitrary maps from sources to
destinations and multiple messages from a single player is somewhat more
involved.  Allow each player to send some number $N$ of messages to any
other player.  The set $\set{M(i,j,k) \mid i,j\in [n], k \in [N]}$
describes the list of all messages.  Player $i$ secretly shares each
$M(i,j,k)$ as a secret $s(j,(i-1)nN+k).$ The goal is to construct a random
secret permutation $\sigma \in {\cal S}_{nN}$ for each $j,$ and apply it to
the secrets $s(j,1),\ldots,s(j,nN)$ destined for player $j.$  The permuted
list of results hides the origins and is revealed directly to player $j.$
To generate a random secret permutation $X(j)$ on $nN$ indices, protocol
\randommatrix of \S\ref{sec-secret-matrices} suffices, using 0/1
matrices to represent permutations.  The permuted list of results for
player $j$ is computed by secretly multiplying the matrix $X(j)$ by the
vector of secrets $(s(j,1),\ldots,s(j,nN)).$

While mathematically correct, the size of the matrices makes this solution
prohibitive.  In a more practical vein, a different sort of approach is
preferable.  The approach used in delivering mail whose destinations are a
permutation of the sources is useful.  We provide each player $j$ with a
set of $n$ ``mailboxes,'' namely a fixed set of secrets $b(j,l).$ Each
mailbox has a corresponding set of flags $c(j,l)$ that indicate whether one
or more players have attempted to place a message in the mailbox.  The
protocol is simple: player $i$ sends a message $M(i,j,k)$ to player $j$ by
choosing a mailbox $(i,l)$ at random and sharing $M(i,j,k)$ as a secret
value $B(j,l,i)$ and sharing $C(j,l,i)=1.$ Other $C(j,l,i)$ values are
shared as 0.  The 0/1 verification is easy, and it is easy to bound the
number of messages sent by each player.  

Finally, the players secretly compute $b(j,l)= \sum_i B(j,l,i)$ and
$c(j,l)= \sum_i C(j,l,i).$ Each $b(j,l)$ and $c(j,l)$ is revealed to player
$j,$ who detects if there is a collision by virtue of $c(j,l)>1.$ Each
player announces the boxes containing collisions and the protocol is
repeated so that the senders can try again.  By choosing the number of
mailboxes sufficiently large for the expected traffic --- a practical issue
--- the expected number of repetitions is small.








==> aut.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% aut.tex                    Co-Authors.
%
%                            Copyright @1989  Donald Beaver.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{center}
{\bf Coauthors}
\end{center}

\bigskip


Some of the protocols appearing here represent joint work:
Chapter~\ref{chap-con} with Dr. Judit Bar-Ilan and Prof. Michael Rabin,
Chapter~\ref{chap-maj} with Prof. Shafi Goldwasser,
Chapter~\ref{chap-ccr} with Prof. Silvio Micali and Mr. Phillip Rogaway,
Chapters \ref{chap-ihs} and \ref{chap-lrr} with Dr. Joan Feigenbaum,
and
Chapters \ref{chap-zkp} and \ref{chap-mpp} with
Dr. Joan Feigenbaum, Dr. Joe Kilian, and Mr. Phillip Rogaway.
%All other chapters, including new definitions, represent individual work.

%Some of the algorithms appearing here represent joint work with
%Dr. Judit Bar-Ilan (Chapter~\ref{chap-con}), 
%Dr. Joan Feigenbaum (Chapters \ref{chap-ihs} and \ref{chap-lrr}), 
%Prof. Shafi Goldwasser (Chapter~\ref{chap-maj}),
%Dr. Joe Kilian (Chapters \ref{chap-zkp} and \ref{chap-mpp}), 
%Prof. Silvio Micali (Chapter~\ref{chap-ccr}), 
%and Mr. Phillip Rogaway (Chapters \ref{chap-zkp},
%\ref{chap-mpp}, and \ref{chap-ccr}).



==> bib.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% bib.tex                      Bibliography for thesis.
%
%                            Copyright @1989,90  Donald Beaver.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% have processed the following bibliographies
% bfkr.tex
% n2.tex
% priv.tex
% const.tex
% bg.tex




\begin{thebibliography}{ABC99}


%AAAaaa

\bibitem[AFK89]{afk89}
  M.\ Abadi, J.\ Feigenbaum, J.\ Kilian.
  ``On Hiding Information from an Oracle.''
  {\em J.\ Comput.\ Systems Sci.} {\bf 39} (1989), 21--50.

\bibitem[AV79]{av79}
  D.\ Angluin, L.\ Valiant.
  ``Fast Probabilistic Algorithms for Hamiltonian Paths and Matchings.''
  {\em J.\ Comput.\ Systems Sci.} {\bf 18} (1979), 155--193.

%BBBbbb

\bibitem[BFL90]{bfl90} L.\ Babai, L.\ Fortnow, C.\ Lund.
  ``Non-Deterministic Exponential Time has Two-Prover Interactive Proofs,''
%  Manuscript, January 16, 1990.
  Submitted to FOCS, IEEE, 1990. 

\bibitem[BM88]{bm88}
  L.\ Babai, S.\ Moran.
  ``Arthur-Merlin Games: A Randomized Proof System,
  and a Hierarchy of Complexity Classes.''
  {\em J.\ Comput.\ System Sci.}  {\bf 36} (1988), 254--276.
%mark check for original babai paper and check references in text


\bibitem[BB88]{bb88}
  J.\ Bar-Ilan, D.\ Beaver.
  ``Non-Cryptographic Fault-Tolerant Computing
  in a Constant Expected Number of Rounds of Interaction.''
  {\em Proceedings of PODC,} ACM, 1989, 201--209.

\bibitem[BBR88]{bbr88}
  J.\ Bar-Ilan, D.\ Beaver, M.\ Rabin.
  Personal communication, 1988.

\bibitem[Bar86]{bar86}
  D.\ Barrington,
  ``Bounded Width Polynomial Size Branching Programs 
  Recognize Exactly those Languages in  $NC^1.$ ''
  {\em Proceedings of the $18^{th}$ STOC,} ACM, 1986, 1--5.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BEAVER
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\bibitem[Bea88]{bea88-n2}
  D.\ Beaver.
  ``Distributed Computations Tolerating a Faulty Minority,
  and Multiparty Zero-Knowledge Proof Systems.''
  {\em J. Cryptology}, 1990.
  A preliminary version appeared as,
  ``Secure Multiparty Protocols Tolerating Half Faulty Processors,''
  in {\em Proceedings of Crypto,} ACM, 1989, and in Technical Report
  TR-19-88, Harvard University, September, 1988.

\bibitem[Bea89a]{bea89-priv}
  D.\ Beaver.
  ``Perfect Privacy for Two-Party Protocols.''
  {\em Proceedings of the DIMACS Workshop on 
  Distributed Computing and Cryptography,} Princeton, NJ, October, 1989,
  J. Feigenbaum, M. Merritt (eds.).
  Preliminary version in TR-11-89, Harvard University.

\bibitem[Bea89b]{bea89-def}
  D.\ Beaver.
  ``Formal Definitions for Secure Distributed Protocols.''
  {\em Proceedings of the DIMACS Workshop on 
  Distributed Computing and Cryptography,} Princeton, NJ, October, 1989,
  J. Feigenbaum, M. Merritt (eds.).

\bibitem[BCG89]{bcg89}
   D.\ Beaver, R.\ Cleve, S.\ Goldwasser.
   In preparation, 1989.

\bibitem[BF89a]{bf89-1} 
  D.\ Beaver, J.\ Feigenbaum.  
  ``Hiding Information from Several Oracles.''
  Harvard University Technical Report TR-10-89, May 1, 1989.

\bibitem[BF89b]{bf89-2} 
  D.\ Beaver, J.\ Feigenbaum.
  ``Encrypted Queries to Multiple Oracles.''
  AT\&T Bell Laboratories Technical Memorandum, August 14, 1989.

\bibitem[BF90]{bf90}
  D.\ Beaver, J.\ Feigenbaum.
  ``Hiding Instances in Multioracle Queries.''
  {\em Proceedings of the the $7^{th}$ STACS,} 
  Springer--Verlag LNCS {\bf 415}, 1990, 
  37--48.

\bibitem[BFKR89]{bfkr89} 
  D.\ Beaver, J.\ Feigenbaum, J.\ Kilian, P.\ Rogaway.
  ``Cryptographic Applications of Locally Random Reductions.''
  {\em Proceedings of Crypto 1990}.
  Also appeared as
  AT\&T Bell Laboratories Technical Memorandum, November 15, 1989.

\bibitem[BFS90]{bfs90}
  D.\ Beaver, J.\ Feigenbaum, V.\ Shoup.
  ``Hiding Instances in Zero-Knowledge Proof Systems.''
  {\em Proceedings of Crypto 1990}.

\bibitem[BG89]{bg89}
  D.\ Beaver, S.\ Goldwasser.
  ``Multiparty Computation with Faulty Majority.''
  {\em Proceedings of the $30^{th}$ FOCS,} IEEE, 1989, 468--473.

\bibitem[BGM89]{bgm89}
  D.\ Beaver, S.\ Goldwasser, Y.\ Mansour.  
  Personal communication, 1989.

\bibitem[BHY89]{bhy89-pc}
  D.\ Beaver, S.\ Haber, M.\ Yung.  
  In preparation, 1989.

\bibitem[BMR90]{bmr90} 
  D.\ Beaver, S.\ Micali, P.\ Rogaway.
  ``The Round Complexity of Secure Protocols.''
  {\em Proceedings of the $22^{st}$ STOC,} ACM, 1990, 503--513.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% from bfkr.tex
%via joe?
\bibitem[BBC]{bbc} C.\ Bennett, G.\ Brassard, C.\ Cr\'epeau.
  Personal communication, 1989.

\bibitem[BCG89]{BeCoGo89}
   M.\ Bellare, L.\ Cowen, S.\ Goldwasser.
  ``On the Power of Secret Key Exchange.''
   In preparation, 1989.

\bibitem[Ben87]{ben87}
  J.\ Benaloh.
  ``Verifiable Secret Ballot Elections''
  PhD Thesis, Yale University, 1987.

\bibitem[BC88]{bc88}
  M.\ Ben-Or, R.\ Cleve, ``Computing Algebraic Formulas
  Using a Constant Number of Registers.''
  {\em Proceedings of the $20^{th}$ STOC,} ACM, 1988, 254--257.

\bibitem[BGG88]{bgg88} 
  M.\ Ben-Or, O.\ Goldreich, S.\ Goldwasser, J.\ Hastad, 
  J.\ Kilian, S.\ Micali, P.\ Rogaway.
  ``Everything Provable is Provable in Zero-Knowledge.''
  {\em Proceedings of Crypto 1988,} Springer--Verlag, 1990.

\bibitem[BGMR85]{bgmr85}
  M.\ Ben-Or, O.\ Goldreich, S.\ Micali, R.\ Rivest. 
  ``Fair Contract Signing.''
  Proceedings of the ICALP (1985). 

\bibitem[BGKW88]{bgkw88} 
  M.\ Ben-Or, S.\ Goldwasser, J.\ Kilian, A.\ Wigderson.  
  ``Multi-Prover Interactive Proofs: How to Remove Intractability.''
  {\em Proceedings of the $20^{th}$ STOC,} ACM, 1988, 113--131.

\bibitem[BGW88]{bgw88}
  M.\ Ben-Or, S.\ Goldwasser, A.\ Wigderson.
  ``Completeness Theorems for Non-Cryptographic Fault-Tolerant
  Distributed Computation.''
  {\em Proceedings of the $20^{th}$ STOC,} ACM, 1988, 1--10.

\bibitem[BE88]{be88}
  M.\ Ben-Or, R.\ El-Yaniv,
  ``Interactive Consistency in Constant Expected Time.''
  Unpublished Manuscript, 1988.

\bibitem[Ber84]{ber84}
  S. Berkowitz.
  ``On Computing Determinant in Small Parallel Time Using a Small
  Number of Processors.''
  {\em Info.\ Proc.\   Letters} {\bf 18}:3 (1984), 147--150.

\bibitem[Bla81]{bla81}
  Blakley, 
  ``Security Proofs for Information Protection Systems.''
  {\em Proceedings of the the 1980 Symposium on Security and Privacy,}
  IEEE Computer Society Press, NY (1981), 79--88.

\bibitem[BK89]{bk89} 
  M.\ Blum, S.\ Kannan.
  ``Designing Programs that Check Their Work.''
  {\em Proceedings of the $21^{st}$ STOC,} ACM, 1989, 86--97.

\bibitem[BLL89]{bll89}
  M.\ Blum, L.\ Levin, M.\ Luby.
  ``If Permanent with the Uniform Distribution
  is in Average Polynomial Time then $\#$P $\subseteq$ ZPP.''
  Unpublished Manuscript, October 31, 1989.

\bibitem[BLR89a]{blr89} 
  M.\ Blum, M.\ Luby, R.\ Rubinfeld.
  ``Self-Testing/Correcting with Applications to Numerical Problems.''
  Preprint, November, 1989.

%blr2
\bibitem[BLR89b]{blr89-2} 
  M.\ Blum, M.\ Luby, R.\ Rubinfeld.
  ``Program Result Checking Against Adaptive Programs 
  and in Cryptographic Settings.''
  {\em Proceedings of the DIMACS Workshop on 
  Distributed Computing and Cryptography,} Princeton, October, 1989.

\bibitem[BLR90]{blr90} 
  M.\ Blum, M.\ Luby, R.\ Rubinfeld.
  ``Stronger Checkers and General Techniques for Numerical Problems,
  {\em Proceedings of the $22^{nd}$ STOC,} ACM, 1990, 73--83.

\bibitem[BM84]{bm84}  
  M.\ Blum, S.\ Micali.  
  ``How to Generate Cryptographically Strong
  Sequences of Pseudo-Random Bits.''
  {\em SIAM J.\ Comput.} {\bf 13} (1984), 850--864.

\bibitem[BCC88]{bcc88} 
  G.\ Brassard, D.\ Chaum, C.\ Cr\'epeau.
  ``Minimum Disclosure Proofs of Knowledge.''
  {\em J.\ Comput.\ System Sci.} {\bf 37} (1988), 156--189.


%CCCccc

\bibitem[CCD88]{ccd88} 
  D.\ Chaum, C.\ Cr\'epeau, I.\ Damgaard.
  ``Multiparty Unconditionally Secure Protocols.''  
  {\em Proceedings of the $20^{th}$ STOC,} ACM, 1988, 11--19.

\bibitem[CDG87]{cdg87}
  D.\ Chaum, I.\ Damgaard, J.\ van de Graaf.
  ``Multiparty Computations Ensuring Secrecy of Each Party's Input
  and Correctness of the Output.''
  {\em Proceedings of Crypto 1987,} Springer--Verlag, 1988.

\bibitem[Che52]{che52}
  H. Chernoff.
  ``A Measure of Asymptotic Efficiency for Tests of a Hypothesis
  Based on the Sum of Observations.''
  {\em Annals of Math. Statistics} {\bf 23} (1952), 493--507.

\bibitem[CGMA85]{cgma85}
  B.\ Chor, S.\ Goldwasser, S.\ Micali, B.\ Awerbuch.
  ``Verifiable Secret Sharing and
  Achieving Simultaneity in the Presence of Faults.''
  {\em Proceedings of the $17^{th}$ STOC,} ACM, 1985, 383--395.

\bibitem[CK89]{ck89}
  B.\ Chor, E.\ Kushilevitz.
  ``A Zero-One Law for Boolean Privacy,''
  {\em Proceedings of the $21^{st}$ STOC,} ACM, 1989, 62--72.

\bibitem[CR86]{cr86}
  B.\ Chor, M.\ Rabin.
  ``Achieving Independence in a Logarithmic Number of Rounds.''
  {\em Proceedings of the $6^{th}$ PODC,} ACM, 1987.
%mark page

\bibitem[Cle86]{cle86}
  R.\ Cleve.
  ``Limits on the Security of Coin Flips when Half the Processors are Faulty.''
  {\em Proceedings of the $18^{th}$ STOC,} ACM, 1986, 364--370.

\bibitem[Cle89]{cle89}
  R.\ Cleve.
  Personal communication, 1989.

%mark reference
\bibitem[CF85]{cf85}
  J.\ Cohen, M.\ Fischer.
  ``A Robust and Verifiable Cryptographically Secure Election.''

\bibitem[Con88]{c88} 
  A.\ Condon.
  ``Space Bounded Probabilistic Game Automata.''
  {\em Proceedings of the $3^{rd}$ Structure in Complexity Theory Conf.,}
  IEEE, 1988, 162--174.

\bibitem[CL89]{cl89} 
  A.\ Condon, R.\ J.\ Lipton.
  ``On the Complexity of Space-Bounded Interactive Proofs.''
  {\em Proceedings of the $30^{th}$ FOCS,} IEEE, 1989, 462--467.

\bibitem[Coo85]{coo85} 
  S. Cook.
  ``A Taxonomy of Problems with Fast Parallel Algorithms.''
  {\em Info.\ and Control} {\bf 64} (1985), 2--22.

\bibitem[CrK88]{crk88} 
  C. \crepeau, J. Kilian. 
  ``Achieving Oblivious Transfer Using Weakened Security Assumptions.''
  {\em Proceedings of the $29^{th}$ FOCS,} IEEE, 1988, 42--52.

%DDDddd

\bibitem[Den82]{den82}
  D. Denning,
  {\em Cryptography and Data Security.}
  Addison-Wesley, Reading, MA (1982).

\bibitem[DOD83]{dod83}
  {\em Department of Defense Trusted Computer System Evaluation
  Criteria.}
  US Department of Defense, Fort Meade, MD (August 15, 1983).

\bibitem[DH76]{dh76}
  W. Diffie, M. Hellman.
  ``New Directions in Cryptography.''
  {\em IEEE Transactions of Information Theory} {\bf IT-22} (November 1976),
  644--654.

\bibitem[DS88]{ds88} C. Dwork, L. Stockmeyer.
  ``Interactive Proof Systems with Finite State Verifiers.''
  IBM Research Report RJ 6262 (61659), May 26, 1988.
  Extended Abstract in 
  {\em Proceedings of Crypto 1988,} Springer--Verlag, 1990, 71--75.

\bibitem[Duf89]{duf89}
  T. Duff.
  ``Experience with Viruses on UNIX Systems.''
  {\em Computing Systems} {\bf 2}:2 (1989), 155--171.

%EEEeee

\bibitem[EGL82]{egl82}
  S. Even,  O. Goldreich,  A. Lempel.
  ``A Randomized Protocol for Signing Contracts.''
  {\em Proceedings of Crypto 1982,} Springer--Verlag, 1983, 205--210.

%FFFfff

\bibitem[Fel87]{fe87}
  P. Feldman.
  ``A practical scheme for Noninteractive Verifiable Secret Sharing.''
  {\em Proceedings of the $28^{th}$ FOCS,} IEEE, 1987, 427--437.

\bibitem[Fel88]{fel88}
  P. Feldman.
  ``One Can Always Assume Private Channels.''
  Unpublished Manuscript, 1988.

\bibitem[FM88]{fm88}
  P. Feldman, S. Micali.
  ``Optimal Algorithms for Byzantine Agreement.''
  {\em Proceedings of the $20^{th}$ STOC,} ACM, 1988, 148--161.

\bibitem[FKN89]{fkn89} 
  J. Feigenbaum, S. Kannan, N. Nisan.
  ``Lower Bounds on Random-Self-Reducibility.''
  AT\&T Bell Laboratories Technical Memorandum, December 4, 1989.

\bibitem[For87]{for87}
  L. Fortnow.
  ``The Complexity of Perfect Zero-Knowledge.''
  {\em Proceedings of the $19^{th}$ STOC,} ACM, 1987, 204--209.

\bibitem[FRS88]{frs} 
  L. Fortnow, J. Rompel, M. Sipser.
  ``On the Power of Multi-Prover Interactive Protocols.''
  {\em Proceedings of the $3^{rd}$ Structure in Complexity Theory Conf.,}
  IEEE, 1988, 156--161.


%GGGggg

%% \bibitem[GHY86]{ghy86}
%%  Z. Galil, S. Haber, M. Yung.
%%  ``Primitives for Designing Multi-Party Cryptographic Protocols
%%  from Specifications.''
%%  Unpublished manuscript, 1986.

%bfkr.tex
%ghy2
\bibitem[GHY87]{ghy87}
  Z. Galil, S. Haber, M. Yung.
  ``Cryptographic Computation: Secure Fault-Tolerant Protocols
  and the Public-Key Model.''
  {\em Proceedings of Crypto 1987,} Springer--Verlag, 1988, 135--155.

%bfkr.tex
%ghy1
\bibitem[GHY89]{ghy89} 
  Z. Galil, S. Haber, and M. Yung. 
  ``Minimum-Knowledge Interactive
  Proofs for Decision Problems.'' 
  {\em SIAM J.\ Comput.} {\bf 18} (1989), 711--739.

\bibitem[GGM86]{ggm86}
  O. Goldreich, S. Goldwasser, S. Micali.
  ``How to Construct Random Functions.''
  {\em JACM} {\bf 33}:4 (1986), 792--807.

\bibitem[GK89]{gk89} 
  O. Goldreich and H. Krawczyk.
  ``On the Composition of Zero-Knowledge Proofs.''
  Technical Report 570, Technion, Israel, June, 1989.

\bibitem[GL89]{gl89}
  O. Goldreich, L. Levin.
  ``A Hard-Core Predicate for All One-Way Functions.''
  {\em Proceedings of the $21^{st}$ STOC,} ACM, 1989, 25--32.

\bibitem[GMW86]{gmw86} O. Goldreich, S. Micali, A. Wigderson.
  ``Proofs that Yield Nothing but Their Validity and a 
  Methodology of Cryptographic Protocol Design.''
  {\em Proceedings of the $27^{th}$ FOCS,} IEEE, 1986, 174--187.

\bibitem[GMW87]{gmw87}
  O. Goldreich, S. Micali, A. Wigderson.
  ``How to Play Any Mental Game, or
  A Completeness Theorem for Protocols with Honest Majority.''
  {\em Proceedings of the $19^{th}$ STOC,} ACM, 1987, 218--229.

\bibitem[GV87]{gv87}
  O. Goldreich, R. Vainish.
  ``How to Solve any Protocol Problem -- An Efficiency Improvement.''
  {\em Proceedings of Crypto 1987,} Springer--Verlag, 1988, 73--86.

\bibitem[GM84]{gm84} 
  S. Goldwasser, S. Micali.
  ``Probabilistic Encryption.''
  {\em J. Comput. System Sci.} {\bf 28} (1984), 270--299.

\bibitem[GMR89]{gmr89}
  S. Goldwasser, S. Micali, C. Rackoff.
  ``The Knowledge Complexity of Interactive Proof Systems.'' 
  {\em SIAM J.\ Comput.} {\bf 18}:1 (1989), 186--208.

\bibitem[GS86]{gs86}
  S. Goldwasser, M. Sipser.
  ``Private Coins vs. Public Coins in Interactive Proof Systems.''
  {\em Proceedings of the $18^{th}$ STOC,} ACM, 1986, 59--68.



%HHHhhh

\bibitem[Hab88]{hab88}
  S. Haber.
  {\em Multi-Party Cryptographic Computation:
  Techniques and Applications},
  PhD Thesis, Columbia University, 1988.

%bg.tex
%\bibitem[HY89]{hy89}
%S. Haber, M. Yung.  Personal communication, 1989.

%bg.tex
\bibitem[HM87]{hm87}
  S. Haber, S. Micali.
  Personal communication, 1987.

\bibitem[HR83]{hr83}
  J. Halpern, M. Rabin.
  ``A Logic to Reason about Likelihood.''
  {\em Proceedings of the $15^{th}$ STOC,} ACM, 1983, 310--319.



%IIIiii

\bibitem[IL89]{il89}
  N. Immerman, S. Landau.
  ``The Complexity of Iterated Multiplication.''
  {\em Proceedings of the $4^{th}$ Structure in Complexity Theory Conf.,}
  IEEE, 1989, 104--111.

\bibitem[ILL89]{ill89}
  R. Impagliazzo, L. Levin, M. Luby.
  ``Pseudo-Random Generation from One-Way Functions.''
  {\em Proceedings of the $21^{st}$ STOC,} ACM, 1989, 12--24.

\bibitem[IR89]{ir89}
  R. Impagliazzo, S. Rudich.
  ``Limits on The Provable Consequences of One-Way Permutations.''
  {\em Proceedings of the $21^{st}$ STOC,} ACM, 1989, 44--62.

\bibitem[IY87]{iy87} 
  R. Impagliazzo, M. Yung.
  ``Direct Minimum-Knowledge Computation.''
  {\em Proceedings of Crypto 1987,} Springer--Verlag, 1988, 40--51.


%JJJjjj

%KKKkkk

\bibitem[Kil88a]{kil88-ot}
  J. Kilian.
  ``Founding Cryptography on Oblivious Transfer.''
  {\em Proceedings of the $20^{th}$ STOC,} ACM, 1988, 20--29.

\bibitem[Kil88b]{kil-n2}
  J. Kilian. Personal communication, 1988.

\bibitem[Kil88c]{k88-2} 
  J. Kilian.
  ``Zero-Knowledge with Log-Space Verifiers.''
  {\em Proceedings of the $29^{th}$ FOCS,} IEEE, 1988, 25--35.

\bibitem[KMR90]{kmr90}
  J. Kilian, S. Micali, P. Rogaway.
  ``The Notion of Secure Computation.''
  Unpublished Manuscript, 1990.

\bibitem[Kus89]{k89}
  E. Kushilevitz.
  ``Privacy and Communication Complexity.''
  {\em Proceedings of the $30^{th}$ FOCS,} IEEE, 1989, 416--421.


%LLLlll

\bibitem[Lip89]{lip89} 
  R. Lipton.
  ``New Directions in Testing.''
  Preprint, October, 1989.

\bibitem[LMR83]{lmr83}
  M. Luby, S. Micali, C. Rackoff.
  ``How to Simultaneously Exchange a Secret Bit
  by Flipping a Symmetrically Biased Coin.''
  {\em Proceedings of the $24^{th}$ FOCS,} IEEE, 1983, 11--21.

\bibitem[LFKN89]{lfkn89} 
  K. Lund, L. Fortnow, H. Karloff, N. Nisan.
  ``The Polynomial Time Hierarchy has Interactive Proofs.''
  Electronic mail announcement, December 13, 1989.

%MMMmmm

% bg.tex
%\bibitem[Man89]{m89}
%Y. Mansour.
%``Unbiased Protocols for Parity.'' Personal communication, 1989.

\bibitem[MR87]{mr87}
  D. McIlroy, J. Reeds.
  ``A Security Model for Files and Processes in the UNIX System.''
  AT\&T Bell Laboratories Technical Report, April 14, 1987.

\bibitem[MR88a]{mr88-1}
  D. McIlroy, J. Reeds.
  ``Multilevel Security with Fewer Fetters.''
  {\em Proceedings of the the Spring 1988 EUUG Conference, 
  European UNIX Users' Group,} London.

\bibitem[MR88b]{mr88-2}
  D. McIlroy, J. Reeds.
  ``Multilevel Windows on a Single-Level Terminal.''
  {\em Proceedings of the UNIX Security Workshop (1988),}
  USENIX, Portland, Oregon.

\bibitem[Mac89]{mac89}
  D. McIlroy.
  ``Virology 101.''
  {\em Computing Systems} {\bf 2}:2 (1989), 173--181.


%NNNnnn

\bibitem[Nis88]{nis88-pc} 
  N. Nisan. 
  Personal communication, 1988.

\bibitem[Nis89]{nis89-cosat} 
  N. Nisan.
  ``Co-SAT has Multiprover Interactive Proofs.''
  Preliminary draft, November, 1989.

\bibitem[NZ72]{nz} 
  I. Niven and H. Zuckerman.
  {\em An Introduction to the Theory of Numbers.}
  Wiley, New York, 1972.


%OOOooo

\bibitem[Ore87]{ore87}
  Y. Oren.
  ``On the Cunning Power of Cheating Verifiers:
  Some Observations about Zero  Knowledge Proofs.''
  {\em Proceedings of the $28^{th}$ FOCS,} IEEE, 1987, 462--471.



%PPPppp

\bibitem[PW72]{pw72}
  W. Peterson and E. Weldon.
  {\em Error Correcting Codes.}
  Second Ed., MIT Press (1972).

%QQQqqq



%RRRrrr

\bibitem[Rab78]{rab78}
  M. Rabin.
  ``Digitalized Signatures.''
  {\em Foundations of Secure Computations,} R. Demillo {\em et al}, Ed.
  Academic Press (1978), 155--165.

\bibitem[Rab79]{rab79}
  M. Rabin.
  ``Digitalized Signatures and Public-Key Functions as Intractable as
  Factorization.''
  Technical Report LCS/TR-212, MIT, January, 1979.

\bibitem[Rab88]{rab88-pc}
  M. Rabin.
  Personal communication, 1988.

\bibitem[Rab89]{rab89-pc}
  M. Rabin.
  Personal communication, 1989.

\bibitem[RT88]{tr88}
  T. Rabin.
  ``Robust Sharing of Secrets When the Dealer is Honest or Cheating.''
  Masters Thesis, Hebrew University, 1988.

%br
\bibitem[RB89]{br89} 
  T. Rabin, M. Ben-Or.
  ``Verifiable Secret Sharing and 
  Multiparty Protocols with Honest Majority.''
  {\em Proceedings of the $21^{st}$ STOC,} ACM, 1989, 73--85.

\bibitem[Ree89]{ree89}
  J. Reeds.
  ``Secure IX Network.''
  Proceedings of the DIMACS Workshop on 
  Distributed Computing and Cryptography, Princeton, NJ, October, 1989,
  J. Feigenbaum, M. Merritt (eds.).

\bibitem[Riv86]{riv86} 
  R. Rivest.
  Workshop on Communication and Computing, MIT, October, 1986.

\bibitem[RSA78]{rsa78} 
  R. Rivest, A. Shamir, L. Adleman.
  ``A Method for Obtaining Digital Signatures and Public Key
  Cryptosystems.''
  {\em Communications of the ACM} {\bf 21}:2 (1978), 120--126.

\bibitem[Rog89]{rog89}
  P. Rogaway, Personal Communication, 1989.

\bibitem[Rog90]{rog90}
  P. Rogaway.
  ``The Round Complexity of Secure Protocols.''
  PhD Thesis, Massachusetts Institute of Technology, 1990.


%bfkr.tex
% via joe?
\bibitem[Rud89]{ru} S. Rudich.
  Personal communication, 1989.


%SSSsss

\bibitem[Sha79]{sha79}
  A. Shamir.
  ``How to Share a Secret.''
   {\em Communications of the ACM,} {\bf 22} (1979), 612--613.

\bibitem[Sha89]{sha89} 
  A. Shamir. 
  ``IP = PSPACE.'' 
  Electronic mail announcement, December, 1989.

%TTTttt

\bibitem[Tod89]{tod89} 
  S. Toda.
  ``On the Computational Power of PP and $\oplus P$.''
  {\em Proceedings of the $30^{th}$ FOCS,} IEEE, 1989, 514--519.


\bibitem[TW87]{tw87} M. Tompa and H. Woll. 
  ``Random Self-Reducibility and Zero-Knowledge
  Proofs of Possession of Information.''
  {\em Proceedings of the $28^{th}$ FOCS,} IEEE, 1987, 472--482.


%UUUuuu



%VVVvvv


\bibitem[Val79]{val79}
  L. Valiant.
  ``The Complexity of Computing the Permanent.''
  {\em Theor. Comput. Sci.} {\bf 8} (1979), 189--201.


%WWWwww


%YYYyyy
\bibitem[Yao82a]{yao82} A.\ C.\ Yao. 
  ``Protocols for Secure Computations.''
  {\em Proceedings of the $23^{rd}$ FOCS,} IEEE, 1982, 160--164.

\bibitem[Yao82b]{yao82b} A.\ Yao,
  ``Theory and Applications of Trapdoor Functions,''
  {\em Proceedings of the $23^{rd}$ FOCS,} IEEE, 1982, 80--91.

\bibitem[Yao86]{yao86}
  A. Yao.
  ``How to Generate and Exchange Secrets.''
  {\em Proceedings of the $27^{th}$ FOCS,} IEEE, 1986, 162--167.

\bibitem[Yap83]{yap83} C. Yap.
  ``Some Consequences of Nonuniform Conditions on Uniform Classes.''
  {\em Theor. Comput. Sci.} {\bf 26} (1983), 287--300.

%ZZZzzz


\end{thebibliography}




==> ccr.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ccr.tex                    Cryptographic Constant Rounds.
%
%                            Copyright @1989  Donald Beaver.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{=======}
\typeout{ccr.tex}
\typeout{=======}

\chapter{Cryptographic Methods for Constant Rounds}
\label{chap-ccr}

We have seen that cryptographic assumptions of one sort or another
facilitate solutions where none are possible, according to
information theory.  The level of
fault-tolerance is vastly improved by assuming the existence of an
oblivious-transfer protocol; can other parameters be improved by making
cryptographic assumptions?

As it turns out, the number of rounds for any protocol can be reduced to a
constant, without any concomitant explosion in message size, if one is
willing to make the weakest sort of cryptographic assumption, namely that
there exists a one-way function.  No details about the structure of such a
function are needed for our protocols.  Thus, in turning to the
vulnerability of making unproven assumptions, we take the smallest possible
gamble.  Until such time as there is a proof that P$\not=\np$ and that
one-way functions exist, our techniques provide all the advantages of
complexity-based cryptography but at the least risk.

The solution is inspired by Yao's method for oblivious circuit evaluation,
in which one player supplies the other with an encrypted circuit and a
partial set of keys to decrypt it ({\em cf.} Chapter~\ref{chap-maj}).  The
encrypted circuit is evaluated locally, without any interaction.  Certainly
in the unbounded-resource models of Chapters \ref{chap-con} and
\ref{chap-min}, such an encryption is not possible with perfect,
information-theoretic security.  On the other hand, if we limit the
adversary to begin polynomial time, an encrypted circuit of the type
introduced by Yao can be computed itself as a result of a multiparty
protocol.  If the construction of the encrypted circuit requires constant
rounds, then the overall protocol will require only constant rounds, since
the encrypted circuits can be evaluated locally, without interaction.

There are crucial differences between the two-party
construction and the multiparty construction --- most notably the fact that
no single party actually knows how the circuit was constructed --- but the
important property is that, if the generalized Yao circuit can be
constructed, then it requires no interaction to evaluate it.
The encryption we describe here is more general and more involved than
that in Chapter~\ref{chap-maj} but is quite similar in other ways.

The complication arises from the need to combine pseudorandom
sequences generated by {\em all} the players in order to ensure that
no single player can fathom any part of the encrypted circuit not
corresponding to the restricted path of percolated keys.  Interestingly,
this approach would not work if general secret computation were needed
to construct the encrypted circuit, because the construction itself
must use constant rounds, and generating pseudorandom bits is a polynomial
time computation, not known to be in $NC^1,$ and hence not known to be
computable in constant rounds.  The second technique that allows the
solution to go through arises from the observation that each player
can compute pseudorandom sequences locally and {\em prove} to the network,
using methods of Chapter~\ref{chap-mzk}, that it shares these results
properly.  Proceeding from the pseudorandom outputs to the encrypted
circuit is an extremely fast and simple computation.

\section{Generalized Yao Gates}
\label{sec-yao-gate}

Fix $n,$ $m,$ and $F.$
Let $\gen(X)$ be a PRG that
outputs $(1+2n)\abs{X}$ bits (or to be pedantic, let $\gen(X)$ be the first
$(1+2n)\abs{X}$ bits produced by a PRG that outputs $3\abs{X}^2$ bits, with
$\abs{X} \geq n$).  Denote the first $\abs{X}$ bits by $\gentag(X),$ the
next $n\abs{X}$ bits by $\genmask(0,X),$ and the final $n\abs{X}$ bits by
$\genmask(1,X).$   In the sequel, all keys have the same length $k.$
Let $S \subseteq [n],$ and define the string $S(i)=0^{nk}$ if $i \not\in S$
and $S(i)=1^{nk}$ if $i \in S.$ The set $S$ will ultimately be used to zero
out components corresponding to faulty players.  If $\logand$ is the
bitwise logical AND, define the following strings, for $a \in \set{0,1}:$
\begin{eqnarray*}
\gentag(S,\vec{X}_{a}) & = & [\gentag(X_{a})\logand S(1)] \circ 
[\gentag(X_{a}^2)\logand S(2)] \circ \cdots \circ 
[\gentag(X_{a}^n)\logand S(n)] \\
%%%%%%%%%%%%%%%%%%
\gentag(S,\vec{Y}_{a}) & = & [\gentag(Y_{a})\logand S(1)] \circ 
[\gentag(Y_{a}^2)\logand S(2)] \circ \cdots \circ 
[\gentag(Y_{a}^n)\logand S(n)] 
\end{eqnarray*}
(The vector notation gives $X^i$ as the $i^{th}$ component of $\vec{X}.$)
Define the following strings for $a,b \in \set{0,1}:$
\begin{eqnarray*}
\genmask(S,a,\vec{X}_{b}) & = & 
[\genmask(a,X_{b}^1)\logand S(1)] \oplus \cdots
\oplus
[\genmask(a,X_{b}^n)\logand S(n)] \\
%%%%%%%%%%%%%%%%%%
\genmask(S,a,\vec{Y}_{b}) & = & 
[\genmask(a,Y_{b}^1)\logand S(1)] \oplus \cdots
\oplus
[\genmask(a,Y_{b}^n)\logand S(n)] \\
\end{eqnarray*}
Knowing any one of the keys will allow a player to match it to a tag (by
evaluating the PRG), but computing the masks requires knowledge of all
the keys.

The generalized Yao gate is the table consisting of four $3nk$-bit 
entries as follows: for $a=0,1$ and for $b=0,1,$
\begin{tabbing}  \standtabs
\>
$\encode(S,a,b,\vec{X}_0,\vec{X}_1,\omega_X,
\vec{Y}_0,\vec{Y}_1,\omega_Y,
\vec{Z}_0,\vec{Z}_1,\omega_Z) 
 = $ \\
\>\>\>\>
$\gentag(S,\vec{X}_{a}) \circ \gentag(S,\vec{Y}_{b}) \circ $ \\
\>\>\>\>
$[\genmask(S,b,\vec{X}_{a}) \oplus
\genmask(S,a,\vec{Y}_{b}) \oplus
\vec{Z}_{g(a \oplus \omega_X, b \oplus \omega_Y) \oplus \omega_Z}
]$
\end{tabbing}
We refer to the three $nk$-bit strings making up an entry of the table as
segments $\Yaogate_1(a,b),$ $\Yaogate_2(a,b),$ and $\Yaogate_3(a,b).$ The
entire table is thus:
\begin{tabbing}  \standtabs
\>
$\Yaogate(S,\vec{X}_0,\vec{X}_1,\omega_X,
\vec{Y}_0,\vec{Y}_1,\omega_Y,
\vec{Z}_0,\vec{Z}_1,\omega_Z)
= $\\
\>\>\>\>
$\encode(S,0,0,\vec{X}_0,\vec{X}_1,\omega_X,
\vec{Y}_0,\vec{Y}_1,\omega_Y,\vec{Z}_0,\vec{Z}_1,\omega_Z) \circ$ \\
\>\>\>\>
$\encode(S,0,1,\vec{X}_0,\vec{X}_1,\omega_X,
\vec{Y}_0,\vec{Y}_1,\omega_Y,\vec{Z}_0,\vec{Z}_1,\omega_Z) \circ$ \\
\>\>\>\>
$\encode(S,1,0,\vec{X}_0,\vec{X}_1,\omega_X,
\vec{Y}_0,\vec{Y}_1,\omega_Y,\vec{Z}_0,\vec{Z}_1,\omega_Z) \circ$ \\
\>\>\>\>
$\encode(S,1,1,\vec{X}_0,\vec{X}_1,\omega_X,
\vec{Y}_0,\vec{Y}_1,\omega_Y,\vec{Z}_0,\vec{Z}_1,\omega_Z)$
\end{tabbing}

Figure~\ref{fig-decode-multi-yao-gate} describes the the {\em decoding} of
a gate given input keys $\vec{X}$ and $\vec{Y}.$ 


\figstretch
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Figure:  Decode Generalized Yao Gate
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\boxfig{
\noindent{\bf \decodemygate}($S,\Yaogate,\vec{X},\vec{Y}$)
\begin{tabbing}  \standtabs
(DC1) \>
Compute $\gentag(S,\vec{X}),\gentag(S,\vec{Y}).$ \\
(DC2) \>
{\For $a = 0..1$ \Do} \\
\> \> Compute $\genmask(S,a,\vec{X}),\genmask(S,a,\vec{Y}).$ \\
(DC3) \>
Determine the least $\alpha,\beta$ such that \\
\> \> $\gentag(S,\vec{X}_\alpha) = \Yaogate_1(\alpha,\beta)$ and 
$\gentag(S,\vec{Y}_\beta)  = \Yaogate_2(\alpha,\beta)$ \\
(DC4) \>
Set $\vec{Z}\leftarrow \Yaogate_3(\alpha,\beta) \oplus
\genmask(S,\beta,\vec{X}) \oplus \genmask(S,\alpha,\vec{Y}).$   
\end{tabbing}
\caption{\label{fig-decode-multi-yao-gate}
Obtaining the output key $\vec{Z}$ from a generalized Yao gate, given the
encrypted table and two input keys $\vec{X}$ and $\vec{Y}.$ The set $S$
describes the indices of strings to consider as 0 when computing $\gentag,$
$\genmask.$ 
}}
\figstretchend


\subsection{Yao Circuit Construction}
\label{sec-general-yao}


Given the means to construct gates, constructing a circuit is
straightforward.   We use the notation for gates $g_{i,j}$
and input wires $\inp_0(i,j)$ and $\inp_1(i,j)$  as
described in \S\ref{sec-two-yao-ckt}.

We consider an array $\wires[i,j,l,I]$ of wire keys for $i \in
\set{0,\ldots,d},j\in \set{1,\ldots,w},$ $l\in \set{0,1},$ $I \in [n].$ The
keys $\wires[i,j,0,I]$ and $\wires[i,j,1,I])$ represent wire $(i,j),$ which
carries the output of gate $g_{i,j}.$ Keys $\wires[0,j,0,I]$ and
$\wires[0,j,1,I])$ represent inputs to the circuit.  Associated with each wire
$(i,j)$ is a {\em key translation bit} $\keytrans[i,j].$

Given $S,$ a set of components to void, and $\wires,$ the construction of
the circuit is as follows.  First, construct a table $\gentab$ of
$2dwn(1+2n)k$ pseudorandom bits, where
\[
\gentab = \gen(S,\wires)
\]
and where the function $\gen(S,\wires)$ gives
a table of $(2dwn)$ $((1+2n)k)$-bit strings defined by
\[
\gen(S,\wires)[i,j,l,I] = \gen(\wires[i,j,l,I]) \logand S(I).
\]
Second, convert this table to a circuit in the same fashion as the
gates are constructed.  That is, with respect to table $\gentab,$ define
the functions $\tabletag(\gentab,i,j,l,I)$ and 
$\tablemask(c,\gentab,i,j,l,I)$
($c\in\set{0,1}$) as the substrings of length $k$, $nk,$ and $nk$ of
$\gentab[i,j,l,I].$ 

The generalized Yao gate $\yaogate(\wires,\gentab,\keytrans,S,i,j)$ is then
constructed as in \S\ref{sec-yao-gate}, using $\tabletag$ and $\tablemask$
as the tag and mask functions.  The wire keys are as
follows.
\begin{eqnarray*}
\vec{X}_l & = & 
(\wires[\inp_0(i,j),l,1],
\wires[\inp_0(i,j),l,2]), \ldots, \wires[\inp_0(i,j),l,n]) \\
\vec{Y}_l & = & 
(\wires[\inp_1(i,j),l,1],
\wires[\inp_1(i,j),l,2]), \ldots, \wires[\inp_0(i,j),l,n]) \\
\vec{Z}_l & = & 
(\wires[i,j,l,1],
\wires[i,j,l,2]), \ldots, \wires[i,j,l,n])
\end{eqnarray*}
The key translations used to construct the gate are
$\keytrans_X=\keytrans[\inp_0(i,j)],$ $\keytrans_Y=\keytrans[\inp_1(i,j)],$
and $\keytrans_Z=\keytrans[i,j].$  As mentioned, a set $S$ of components to
be voided is used to place 0's over appropriate components.

The circuit thus constructed is denoted
$\yaocircuit(\wires,\gentab,\keytrans,S).$ Notice that the construction 
takes $\gentab$ into account independently of $\wires;$ it is well-defined
whether or not $\gentab$ arises from $\wires.$



\figstretch
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Figure:  Construct Generalized Yao Circuit
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\boxfig{
\noindent{\bf \makeyaocircuit}($\wires,\gentab,\keytrans,S$)
\begin{tabbing}  \standtabs
{\For $i=1..d$ \Do} \\
\> {\For $j=1..w$ \Do} \\
\>\>  $\yaocircuit(\wires,\gentab,\keytrans,S)[i,j] \leftarrow
\yaogate(\gentab,\keytrans,S,i,j);$ \\
\>\> more precisely, $\yaocircuit(\wires,\gentab,\keytrans,S)$ is the string \\
\>\>\>
$\yaogate(\wires,\gentab,\keytrans,S,1,1) \circ 
\yaogate(\wires,\gentab,\keytrans,S,1,2) \circ \cdots$ \\
\>\>\>
$\circ \yaogate(\wires,\gentab,\keytrans,S,d,w-1)
\circ \yaogate(\wires,\gentab,\keytrans,S,d,w)$
\end{tabbing}
\caption{\label{fig-make-yao-circuit}
How to construct a generalized Yao circuit from a table $\wires$ of keys,
a table
$\gentab$ of tags and masks, a set $\keytrans$ of key translations, and a
set $S \subseteq [n]$ of components to be voided.  
}}
\figstretchend

A set of inputs $\vec{x}=(x_1,\ldots,x_n)$ is written as a set of input
bits, $(x[1,1],\ldots,x[1,m],x[2,1],\ldots,x[2,m],
\ldots, x[n,1],\ldots,x[n,m]).$ The
{\em value} $\wireval[i,j]$ of wire $(i,j)$ is determined by the
input bits and the gates $g_{i,j}$ (in the natural fashion in which
a circuit is evaluated)
We use a bijection $L_0(J)=(J \Div m, J
\mod m)$ to map wire $(0,J)$ to input $x[L_0(J)].$

The input keys $\inkeys$ that must be revealed for the circuit to be
evaluable through key percolation are given by
\begin{eqnarray*}
\inkeys_I(\wires,\keytrans,\vec{x}) & = &
\{\wires[0,J,\keytrans[L_0(J)] \oplus x[L_0(J)],I]\}_{J \in [nm]} \\
\inkeys(\wires,\keytrans,\vec{x}) & = &
\{\inkeys_I\}_{I \in [n]}
\end{eqnarray*}
%The 0-1 indices of these keys are denoted $\inkeyind(\vec{x}) =
%\set{\keytrans[L_0(J)] \oplus x[L_0(J)]}_{J \in [nm]}.$  

Finally, the output key translations that must be revealed in order to
interpret the keys of the final level are
\[
B(\keytrans)=(\keytrans[w,1],\keytrans[w,2],\ldots,\keytrans[w,d]).
\]

The encrypted circuit is then 
\[
\hidecirc(\wires,\gentab,\keytrans,S,\vec{x})
=
\yaocircuit(\wires,\gentab,\keytrans,S) 
\circ 
B(\keytrans)
\circ
\inkeys(\wires,\keytrans,\vec{x}) 
\]


\section{Protocols in Constant Rounds}

\begin{theorem}  \label{thm-ccr-private}
Assume there exists a one-way function.  Let $F$ be a polynomial-time
function family.  Consider a complete broadcast network with private
channels, where each player is a probabilistic polynomial-time Turing
machine.  The adversary class consists of polynomial-size circuit families
and a fault class allowing $2t<n.$ Then there is a $t$-resilient protocol
for $F$ that runs in {\em constant} rounds and has polynomial message
complexity.
\end{theorem}

\begin{proof}   
\figstretch
\boxfig{
\noindent{\bf \ccrproto}\index{\ccrproto}
\begin{tabbing} \hspace{0.6in} \= \standtabs
(C1)
\>{\For $i=1..n$ \Dopar } \\
\>
Player $i$ shares input $x_{i}$ as secret bits 
$x[i1],\ldots,x[im].$
\\
(C2)
\>
Run \randombit to generate random bits 
$\set{\rho[i,j]}_{i\in [n],j \in [dwnk]}.$
\\
(C3)
\>
{\For $i=1..n$ \Dopar } \\
\>
Reveal $\rho[i,1],\ldots,\rho[i,dwnk]$ to player $i.$ \\
(C4.1)
\>
{\For $i=1..n$ \Do \for $j=1..dwn$ \Do} \\
\>
Player $i$ locally computes $G_{i,j}=\gen(\rho[i,jk+1]\cdots\rho[i,(j+1)k]).$
\\
(C4.2)
\>
{\For $i=1..n$ \Dopar \for $j=1..dwn$ \Dopar} \\
\>
Player $i$ shares $G_{i,j}.$ \\
(C5)
\>
{\For $i=1..n$ \Dopar \for $j=1..dwn$ \Dopar} \\
\>
Player $i$ proves 
$G_{i,j}=\gen(\rho_{i,jk+1}\cdots\rho_{i,(j+1)k})$
using \provepred. \\
(C6.1)
\>
Let $S$ be the set of players whose proof failed.  \\
(C6.2)
\>
Define $G_{i,j}=0^{(1+2n)k}$ for $i \in S$ and $j \in [dwn].$ \\
(C6.3)
\>
Compute $\yaocircuit(S,W),$ where $W$ is defined by the $G_{i,j}$ values. \\
(C7)
\>
Compute $\chi$ from $W,\vec{x}.$ \\
(C8)
\>
Reveal $\yaocircuit(S,W),\chi,B$ to all players.\\
\>   (Note that secrets in $B$ are contained in $W.$)\\
\>   Each player $i$ uses $\decodemygate$ to compute $F(\vec{x}).$
\end{tabbing}
\caption{\label{fig-proto-ccr}
Protocol to create a generalized Yao circuit $\yaocircuit$ and the
decrypting keys needed to evaluate it.  
}}
\figstretchend


The protocol is given in Figure~\ref{fig-proto-ccr}.  Constructing the
encrypted circuit requires constant rounds.  Revealing the encrypted
circuit reveals nothing more than the final outputs.  The resilience
of the protocol follows from Lemmas
\ref{lem-yc-ideal} (see \S\ref{sec-yao-pri-prf}), 
\ref{lem-ccr-yc} (see \S\ref{sec-ccr-res-prf}), 
and \ref{lem-resil-trans}.
\end{proof}   

\subsection{Generalized Yao Circuits Are Private}
\label{sec-yao-pri-prf}

Consider the following ideal protocol $\idealname(\hidecirc)$ to generate
% encrypted circuits. Each player supplies an input $(x_i,p_i)$ where $p_i  %drb2020
% \in \set{{\em participate},{\em quit}}.$ The trusted host sets   %drb2020
encrypted circuits. Each player supplies an input $(x_i,p_i)$ where $p_i
%\in \set{{\em participate},{\em quit}}.$ The trusted host sets   % drb2020
%$S=\set{i \mid p_i={\em quit}}$ and selects keys $\wires$ and key  % drb2020
\in \set{\mbox{\em participate},\mbox{\em quit}}.$ The trusted host sets 
$S=\set{i \mid p_i=\mbox{\em quit}}$ and selects keys $\wires$ and key
translations $\keytrans$ uniformly at random for all the indices $i \not\in
S.$ It computes $\gentab$ using $\gen$ and $\wires.$ It then constructs the
circuit and returns $\hidecirc(\wires,\gentab,\keytrans,S,\vec{x}).$ (By
\S\ref{sec-function} we can assume that each player learns every output
bit, so there is no need to return different subsets of output key
translations.)  
%It also gives each player the wire keys
%$\wires(I)=\set{\wires[i,j,0,I],\wires[i,j,1,I]}_{i \in [d],j\in [w]}.$
Finally, each player computes its output by percolating the keys from $B$
through the gates, using \decodemygate.


\begin{lemma}   \label{lem-yc-ideal}
Let the adversary class $\advclass$ include all nonuniform
polynomial-time Turing machines, consider only static adversaries, and let
$t \leq n-1.$ Then
\[
\idealname(\hidecirc)
\resilasFaC_{\advclass} 
\idf
\]
\end{lemma}

\begin{proof}
The bijection $L(m)=(m\Div w,m\mod w)$ between $[dw]$ and $[d]
\times [w]$   defines a natural ordering on pairs, namely $L(m) < L(m+1).$  
This row-major ordering extends directly to longer tuples.  In particular,
we consider the bijection $L(m)$ between
\mbox{$[d \cdot w \cdot 2 \cdot n]$} and
\mbox{$[d] \times [w] \times \set{0,1} \times [n]$}.
The tuple $(i,j,l,I)$ corresponds to a particular wire key and to one level
of the tag and mask table, $\gentab.$  

We construct a progressive obliteration of a generalized Yao circuit by
stepping through the pseudorandom table row by row, replacing each string
in the table by a uniformly random string. With respect to a particular
input assignment, 
%$\inkeyind,$ 
a set $S$ of voided components, and an
additional parameter $T \subseteq [n],$ the strings that are actually used
in the percolation and evaluation of the circuit, or that are voided or
otherwise given special exception, are not replaced.  This generates a
sequence of hidden circuits that are indistinguishable.  

For a given set of inputs and a given circuit for $F,$ the
values $\wireval[i,j]$ on each wire are determined.
The indices $\perc[i,j]$
of the keys that are percolated during evaluation are determined
by the key translation bits $\keytrans$ and the wire values:
\[
\perc[i,j] = \keytrans[i,j] \oplus \wireval[i,j].
\]

For a given $T,$ $S \subseteq T,$ and $M$ ($0 \leq M \leq 2dwn$), 
the obliterated table is as follows.
Let $\randtab$ be a string of $2dwnk$ bits, let $L(\mu)=(i,j,l,I),$
and define the obliteration of entry $m:$
\begin{eqnarray*}
\oblitgentabrow(\wires,\randtab,S,T,m) & = & \left\{
\begin{tabular}{ll}
$0^{3k}$ & 
if $I \in S$ 
\\
$\randtab[L(m)]$ &
if $I \not\in T,$ $l \not= \perc[i,j]$ 
\\
$\gen(S,\wires)[L(m)]$ & 
otherwise
\end{tabular}
\right.
\end{eqnarray*}
Now, row $m$ of the $M^{th}$ obliterated table is:
\begin{eqnarray*}
\oblitgentab(\wires,\randtab,S,T,M)[m] & = & \left\{
\begin{tabular}{ll}
$\oblitgentabrow(\wires,\randtab,S,T,m)$ &
if $m \leq M$
\\
$\gen(S,\wires)[L(m)]$ &
otherwise
\end{tabular}
\right.
\end{eqnarray*}

The obliterated circuit is obtained by using the partly obliterated
pseudorandom table:
\[
\pyc(\wires,\randtab,\keytrans,S,T,M) =
\yaocircuit(\wires,\oblitgentab(\wires,\randtab,S,T,M),\keytrans,S)
\]

Finally, the progressively obliterated encrypted circuits are defined by:
\begin{eqnarray*}
& \oblhidecirc(\wires,\randtab,\keytrans,S,T,\vec{x},M) = & \\
& 
(\pyc(\wires,\randtab,\keytrans,S,T,M),
\inkeys(\wires,\keytrans,\vec{x}),B(\keytrans))
&
\end{eqnarray*}


Define ensembles $D(M)(z,k)$ for all $M$ as follows.
If $z$ is not of the form 
$n \circ m \circ d \circ w \circ S \circ T \circ \vec{x} \circ \vec{a}
\circ \keytrans$
or if $k < 2ndw,$
then all probability
weight is placed on the string $0.$ 
Otherwise, using the security parameter $k$ as the key length, 
set
\begin{eqnarray*}
D(M)(z,k) & = &
\{ \wires \leftarrow \{0,1\}^{2dwn}; \\
& &
\randtab \leftarrow \{0,1\}^{2dwn(1+2n)k}: \\
& &
\oblhidecirc(\wires,\randtab,\keytrans,S,T,\vec{x},M) 
\}
\end{eqnarray*}
Successive pairs $D(M-1)(z,k)$ and $D(M)(z,k)$ are indistinguishable 
because they
differ at most in the generation of a single pseudorandom sequence.  
Let us argue formally.

Suppose $D(M-1)(z,k)$ and $D(M)(z,k)$ are 
$(k^{-c-1})$-distinguishable.
In particular this means that 
$z=n \circ m \circ d \circ w \circ S \circ T \circ \vec{x} 
\circ \vec{a} \circ \keytrans$
and
\[
\oblitgentabrow(\wires,\randtab,S,T,M)  =  
\gen(\wires[L(M)]),
\]
for otherwise $D(M-1)(z,k)=D(M)(z,k).$
Then for any $c$ there exists a distinguisher $\scm$ such that
\[
\abs{ \scm_{D(m)(z,k)} - \scm_{D(m-1)(z,k)}} > k^{-c}
\]
for infinitely many $k.$

We overwrite the $(1+2n)k$-bit string in location $L(m)$ of $\randtab$
using the function
\begin{eqnarray*}
\overwrckt(\randtab,\sigma)[L(m')] & = & \left\{
\begin{tabular}{ll}
$\randtab[L(m')]$ &
if $m' \not= m$
\\
$\sigma$ &
if $m' = m$
\end{tabular}
\right.
\end{eqnarray*}
Consider the machine $\scm'$ that 
on input $\sigma,$ sets $k=\abs{\sigma}$ and selects $\wires$ and 
$\randtab$ uniformly at random,  It then sets
$\randtab' = \overwrckt(\randtab,\sigma),$ 
computes $\oblitgentab(\wires,\randtab',S,T,M),$ and constructs
hidden circuit $\hidecirc.$ Finally, it runs $\scm$ on $\hidecirc$ and returns
the output of $\scm.$

Define the ensembles
\begin{eqnarray*}
\scg(k) & = & \{X\leftarrow  \uniform(\{0,1\}^{k}): \gen(X)\} \\
\sch(k) & = & \uniform(\{0,1\}^{(1+2n)k}).
\end{eqnarray*}
Then
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabbing}  \standtabs
\>\>
$D(M-1)(z,k)=
\{\randtab \leftarrow \{0,1\}^{2dwn(1+2n)k};$ \\
\>\>\>\>\>
$\sigma \leftarrow \scg(k);$ \\
\>\>\>\>\>
$\randtab' = \overwrckt(\randtab,\sigma):$ \\
\>\>\>\>\>
$\oblhidecirc(\wires,\randtab',\keytrans,S,T,\vec{x},M) \}$ \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\>\>
$D(M)(z,k)=
\{\randtab \leftarrow \{0,1\}^{2dwn(1+2n)k};$ \\
\>\>\>\>\>
$\sigma \leftarrow \sch(k);$ \\
\>\>\>\>\>
$\randtab' = \overwrckt(\randtab,\sigma):$ \\
\>\>\>\>\>
$\oblhidecirc(\wires,\randtab',\keytrans,S,T,\vec{x},M) \}$
\end{tabbing}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
so that by the construction of $\scm',$
\[
\abs{ \scm'_{\scg(k)} - \scm'_{\sch(k)}} =
\abs{ \scm_{D(m)(z,k)} - \scm_{D(m-1)(z,k)}} > k^{-c}
\]
This holds for infinitely many $k,$ and certainly infinitely many
$k$ larger than $2dwn,$ so
$\scm'$ distinguishes $\scg$ from $\sch,$
contradicting the assumption that $\gen$ is a PRG.

Therefore, for all $M,$ $D(M-1) \indistEnC^{k^{-c-1}} D(M),$
so $D(0) \indistEnC^{k^c} D(2dwn)$ (recall $k \geq 2dwn$).

With this in mind, we argue that the task of an interface is
easy: 
obtain and return $x_i$ and $a_i$ for all players $i$ that
$A$ wishes to corrupt, by corrupting $i_{id}$ in 
$\idealname(F);$
use the input values shared by corrupted players $i$
to replace those of corrupted players $i_{id}$ in $\idealname(F),$
or have $i_{id}$ send $\Lambda$ if $i$ does not share a value;
determine the set $S$ of non-participating faulty players
from the interaction with $A$ ($S$ is the list
of players who are disqualified);
and return an {\em obliterated} circuit that is constructed
according to distribution $D(2dwn),$ namely according to the circuit for
$F$ and the output returned by the trusted host.

It is clear that distribution $D(2dwn)$ is easy to sample
given the list of gates in the circuit for $F,$ the value
returned by the trusted host, and the list
$S$ of voided components.  Now, in protocol 
$\anglebrack{A,\idealname(\hidecirc)},$
\[
\view_A^f = a_A \circ \vec{a}_T \circ \vec{x}_T \circ \EC
\]
where $T=T(q_A^f)$ and $\EC$ is returned by the host.
Note that the host samples 
\[
\EC \leftarrow 
D(0)(n \circ m \circ d \circ w \circ S \circ T
\circ \vec{x} \circ \vec{a},k).
\]
On the other hand, in protocol
$\anglebrack{A,\interface,\idf},$
\[
\view_A^f = a_A \circ \vec{a}_T \circ \vec{x}_T \circ \EC
\]
where $\EC$ is returned by $\interface.$
Note that $\interface$ samples 
\[
\EC \leftarrow 
D(2dwn)(n \circ m \circ d \circ w \circ S \circ T
\circ \vec{x} \circ \vec{a},k).
\]
We have already shown that the ensembles $D(0)$ and $D(2dwn)$ are
computationally indistinguishable, so the families of ensembles
satisfy 
$
[A,\idealname(\hidecirc)]^{Y_A} \indistFaC
[A,\interface,\idf]^{Y_A}.
$
Now, by the construction of $D(0)$ and $D(2dwn),$ the value of
$F$ that is percolated through an encrypted circuit is the same
regardless of which method is used to generate it, so
$
[A,\idealname(\hidecirc)]^{\vec{Y}} \indistFaC
[A,\interface,\idf]^{\vec{Y}}.
$
Hence $\idealname(\hidecirc) \resilasFaC \idf.$
\end{proof}


\subsection{Protocol \ccrproto Resiliently Computes $F$}
\label{sec-ccr-res-prf}

\begin{lemma}   \label{lem-ccr-yc}
Let the adversary class $\advclass$ be static and restricted
to nonuniform polynomial-time Turing machines, and let $t<n.$
Then:
\[
\ccrproto \resilasFaC_{\advclass} \idealname(\hidecirc)	
\]
\end{lemma}

\begin{proof}
The \ccrproto protocol is a composition of resilient computations.
The computation of random bits is a private function and
$t$-resilient.  The computation of each secret PRG output is $t$-resilient,
using Theorem~\ref{sec-zkmips}.  Revealing $S$ is private.
The \evalmin protocol evaluates
$\yaocircuit(\wires,G,\keytrans,S)$ in a constant number of rounds
since $\yaocircuit$ is of constant depth.  
In fact, the circuit construction requires an exclusive-or
of bit streams, some of which are voided according to $S.$  
Because $S$ is public, the indices of the appropriate pseudorandom
sequences to include are public and no secret
AND computations need be performed.  Therefore,
constructing the encrypted circuit secretly requires no interaction.
Secretly computing the input keys to reveal requires an execution of a
multiplication protocol (an AND must be secretly computed).
The encrypted circuit itself is a robust (all players learn it,
so a minority of alterations are not effective)
and private ({\em cf.} Lemma~\ref{lem-yc-ideal}) representation of
the result, $F(x_1,\ldots,x_n).$
The reconstruction stage is $t$-resilient.

By Theorem~\ref{thm-proto-concat}, the composition is as
resilient as the composition of the corresponding ideal
vacuous protocols with $\idealname(\hidecirc),$ the which composition
is in turn as resilient as $\idealname(\hidecirc).$
The adversary must be static in order that the subprotocols
be post-protocol corruptible and hence composable.
Each subprotocol of \ccrproto requires only a constant number
of rounds, so \ccrproto requires only a constant number of rounds.
\end{proof}


\section{Without Private Channels}

By an unpublished claim of Feldman \cite{fel88} 
(see \S\ref{sec-pub-priv}), private channels in a
protocol can be replaced by public channels over which encrypted messages
are broadcast.  Lemma~\ref{lem-feed-dist} along with a standard
probability walk as in \S\ref{sec-yao-pri-prf}
would provide a proof of this claim.

\begin{theorem}  \label{thm-ccr}
\index{constant rounds!cryptographic}
Assume there exists a one-way function.  Let $F$ be a polynomial-time
function family.  Consider a complete broadcast network of public channels,
where each player is a probabilistic polynomial-time Turing machine.  The
adversary class consists of polynomial-size circuit families and a fault
class allowing $2t<n.$ Then there is a $t$-resilient protocol for $F$ that
runs in {\em constant} rounds and has polynomial message complexity.
\end{theorem}





==> cns.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% con.tex                      Fast Oblivious Circuit Evaluation
%
%                            Copyright @1989  Donald Beaver.
%
% Presented at PODC 89, coauthored with Judit Bar-Ilan.  Primarily
% written by Donald Beaver, including matrix methods and proofs.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{=======}
\typeout{con.tex}
\typeout{=======}

\chapter{Efficient, Unconditionally Secure Multiparty Protocols}
\label{chap-con}

\chapquote{
%But the most dangerous effect of the exhaustion steadily gaining on 
%all engaged in the fight against the epidemic did not consist in their 
%relative indifference to outside events and the feelings of others, 
%but in the slackness and supineness that they allowed to invade their 
%personal lives.
They developed a tendency to shirk every movement that didn't seem 
absolutely necessary or called for efforts that seemed too 
great to be worthwhile.  
Thus these men were led to break, oftener and oftener, the rules of hygiene 
they 
themselves had instituted, to omit some of the numerous disinfections they 
should have practiced, and sometimes to visit the homes of people 
suffering from pneumonic plague without taking steps to safeguard themselves 
against infection, because they had been notified only at the last 
moment and could not be bothered with returning to a sanitary service station, 
sometimes a considerable distance away, to have the necessary injections.  
There lay the real danger; for the energy 
they devoted to fighting the disease made them all the more liable to it.  
%In short, they were gambling on their luck, and luck is not to be coerced.
}{
Albert Camus, {\em The Plague}}
% Vintage Books NY 1972 translated Stuart Gilbert
% pp 179-180
% La Peste



Ben-Or, Goldwasser, Wigderson, and Chaum, \crepeau, and \damgard\  
\cite{bgw88,ccd88} show how, given private communication channels and a
broadcast channel,%
\footnote{The requirement of a broadcast channel can be removed at the cost
of a constant factor increase in the number of rounds, using a Byzantine
Agreement protocol of Feldman and Micali \cite{fm88}; the communications
during the protocol are independent of all values except the broadcast
value, so that the protocol maintains privacy and resilience.}
a network can evaluate a circuit $C_F$ for a function
$F(x_1,\dots,x_n)$ in the presence of $t$ Byzantine faults, as long as $t <
\frac{n}{3}.$ No complexity-theoretic assumptions are necessary.  

Their construction requires a number of rounds of interaction proportional
to the depth of $C_F$ and messages which grow with its size.  In fact,
since most early protocols for securely computing a function $F$ were based
on evaluating a circuit for $F$ gate by gate, this led many researchers to
conjecture that the circuit depth of $F$ was a lower bound on the number of
rounds of interaction, and the circuit size a lower bound on the message
size.

We prove to the contrary that the communication complexity of securely
computing $F$ need not be related to the computational (circuit) complexity
of $F.$ First, we show that the number of rounds of interaction can be
reduced by a logarithmic factor while maintaining small message sizes.  The
number of rounds required for any function in the broad class $NC^1$ is
constant.  In fact, the number of rounds for {\em any} function is
reducible to a constant, though at the price of larger messages (see
\S\ref{sec-any-const}) or lower fault tolerance (see
Chapter~\ref{chap-mpp}).

Our protocols are simple to implement: they employ matrix multiplication,
polynomial evaluation, and polynomial interpolation as their most
complicated subroutines.  All of the local computations are fast.

The main result of this chapter is a protocol to evaluate a
function in a constant number of rounds using a technique
that avoids gate-by-gate simulation.
(see \S\ref{sec-tools}--\S\ref{sec-iter-mult})
Before presenting our results,
we must first describe the threshold schemes that underlie most of the
protocols in this dissertation.  By recombining values that have been
distributed according to the threshold scheme, new, robustly shared results
are constructed.  We give a method, similar to yet more efficient than that
of \cite{bgw88,ccd88}, for evaluating the AND, OR, and NOT gates of a
circuit, representing the results using the threshold scheme.  Because
proofs and formal specifications of the protocols in \cite{bgw88,ccd88}
have not appeared, we must provide proofs of the underlying methods as
well.  We present a general paradigm for modular protocol design and prove
it robust.

{\bf Assumptions made in this chapter.}  The network is complete,
with private lines, $n$ processors,
and at most $t < \frac{n}{3}$ Byzantine faults, chosen dynamically.
The protocols are information-theoretically secure,
or in other words, the results are perfectly resilient.

\section{Threshold Schemes}
\label{sec-threshold}

A particularly efficient and simple threshold scheme is presented by Shamir
\cite{sha79}; we refer to it as {\em secret sharing}.%
\index{secret sharing}%
\index{secret sharing!polynomial}%
\index{secret sharing!Shamir}
Fix a finite field
$E$ of size greater than $n,$ the number of players.  For example, the set
${\bf Z}_p$ of integers taken modulo $p$ will do, where $p$ is a prime
number in the range $n < p < 2n.$ Arithmetic over ${\bf Z}_p$ is extremely
easy to compute.  Another convenient field to use, though slightly less
intuitive to implement, is $\gf(2^n),$ which has the often useful property
that $x+x=0$ for any $x.$


\figstretch
\boxfig{
\noindent{\bf \share}$(s)$
\begin{itemize}
\item
Fix field $E,$ $\abs{E} > n,$ and elements $\alpha_1,\dots,\alpha_n \not=
0.$
\item
Dealer selects $a_t,\dots,a_1 \in E$ at random.
\item
Dealer sets $p(u) = a_t u^t + \cdots + a_1 u + s.$
\item
Dealer computes $\piece_i(s) \leftarrow p(\alpha_i).$
\item
Dealer sends $\piece_i(s)$ to player $i.$
\end{itemize}
\caption{\label{fig-share}
\index{\share}
Protocol for dealer to secretly share value $s \in E.$
}}
\figstretchend


In any case, the dealer {\em shares} $s \in E$ by the method displayed in
Figure~\ref{fig-share}.  The dealer chooses $t$ random coefficients
$a_t,\dots,a_1$ in $E$ and creates a polynomial $p(n)$ of degree $t$ using
these coefficients, with $p(0) = s.$ Then, for fixed, public,
nonzero evaluation
points $\alpha_1,\dots,\alpha_n,$ he constructs the ``piece'' $\piece_i(s)$
by evaluating $p(\alpha_i).$  Finally, he sends $\piece_i(s)$ to player $i,$
privately.  Distributions $\unifpolyn(t,s)$ and $\unifpieces(n,t,s),$
discussed in $\S\ref{sec-notation},$ describe the distributions
on polynomials and vectors of pieces so generated.

Any $t+1$ players can determine $s$ easily, since $t+1$ points determine a
polynomial of degree $t.$ By interpolating the polynomial of degree $t$
passing through their points, a sufficiently large collection of players
can recover $p(0)=s.$ As long as the number of omitted pieces, which is
bounded by $t,$ leaves $t+1$ valid pieces remaining, the reconstruction is
possible; hence $n-t \geq t+1$ must be satisfied, or equivalently $2t<n.$
Thus at the appropriate time specified by the protocol, it is easy to
reconstruct the secret from the information held by reliable players.

\figstretch
\boxfig{
\noindent{\bf \reconstruct}$(\piece_{i_1}(s),\dots,\piece_{i_{t+1}}(s))$
\begin{itemize}
\item
Each player $i$ sends $\piece_i(s)$ to player $j.$
\item
Player $j$ selects $t+1$ of the pieces he collects.
Player $j$ interpolates the polynomial $p(u)$ passing through
$(i_1,\piece_{i_1}(s)),\dots,(i_{t+1},\piece_{i_{t+1}}(s)).$
\item
Player $j$ computes $s=p(0).$
\end{itemize}
\caption{\label{fig-reconstruct}
\index{\reconstruct}
Protocol to reveal secret $s$ to player $j.$
}}
\figstretchend

Intuitively speaking, any $t$ or fewer evaluation points of a
$t^{th}$-degree polynomial do not determine that polynomial.  Thus, an
adversary who gains the information held by a coalition of $t$ or fewer
players learns nothing; it obtains a uniformly distributed vector of
values, regardless of the value of $s.$  

\begin{lemma}  \label{lem-ss}
(Shamir 1979)
Let $E$ be a field and let $1 \leq t < \abs{E}.$
Then for any $s \in E,$ for any $t' \leq t,$ 
and for any set 
$T=\{\alpha_1,\dots,\alpha_{t'}\} 
\subset E - \set{0}$ of size ${t'},$
\[
\set{ \vec{a} \leftarrow \uniform(E^t): (p_{s,\vec{a}}(i_1),
\ldots,p_{s,\vec{a}}(i_{t'})) }
=
\uniform(E^{t'})
\]
where $p_{s,\vec{a}}(u) = s + \sum_{j=1}^t a_j u^j.$
In particular, for any $n < \abs{E},$ 
$\alpha_1,\ldots,\alpha_n,s \in E,$
and $T \subseteq [n]$ with $\abs{T} \leq t,$
\[
\set{ \vec{p} \leftarrow \unifpieces(n,t,s) : \vec{p}_T }
=
\uniform(E^{\abs{T}})
\]
\end{lemma}

Given some pieces of a secret,
new pieces remain uniformly random, up to a total of $t:$
\begin{lemma}  \label{lem-ss-new}
Let $E$ be a field and let $1 \leq t < n < \abs{E}.$
Then for any $s \in E,$ for any disjoint $T,T' \subseteq [n]$ 
satisfying $\abs{T \cup T'} \leq t,$ and for any
$\vec{q} \in E^n,$ 
\[
\set{ \vec{p} \leftarrow \unifpieces(n,t,s) : \vec{p}_{T'} \mid 
\vec{p}_{T} = \vec{q}_{T} }
=
\uniform(E^{\abs{T'}})
\]
\end{lemma}

\begin{proof}
Elementary linear algebra.
\end{proof}


\begin{lemma}
\label{thm-share-private-pass}
For $3t < n,$ in a completely connected network of $n$ processors with
private channels, the method for secret sharing presented above is
$t$-resilient against dynamic, passive adversaries.
\end{lemma}

\begin{proof}
In the ideal protocol, the dealer sends $n$ pieces to the
trusted host, who then distributes them.  
Before the adversary corrupts the dealer, the interface need
only generate random field elements in response to corruption
requests, which it does according to Lemma~\ref{lem-ss-new}
by generating uniformly random field elements.  If the adversary
corrupts the dealer, then the interface first chooses 
$t-\abs{T}$ remaining pieces uniformly at random as directed
by Lemma~\ref{lem-ss-new}, and corrupts
the dealer in the ideal protocol, obtaining $s.$  Given $s$ and
$t$ pieces, the polynomial is uniquely determined and $\interface$
simply solvers for the remaining pieces.  It constructs a view of
the dealer consisting of $s,$ the coefficients, and the entire
list of pieces, and provides the list to the adversary.  Subsequent
requests for corruptions are computed by evaluating the polynomial. 
\end{proof}


Polynomial interpolation is extremely fast and efficient, especially at
fixed interpolation points.  One way to perform the interpolation of $p(x)$
from values $p(1),\dots,p(n)$ is through the LaGrange interpolation
formula:
\begin{eqnarray} \label{eqn-lagrange-interp}
p(x) & = & \sum_1^n L_i(x) p(i)
\end{eqnarray}
where the LaGrange polynomial $L_i(x)$ is defined by
\begin{eqnarray*}
L_i(x) & = & \prod_{j=1..n; j\not=i}  \frac{x-j}{i-j}.
\end{eqnarray*}
Each $p(i)$ is a constant in Equation~\ref{eqn-lagrange-interp}, so that
$p(x)$ is the weighted sum of polynomials $L_i(x).$ This sum is easily and
efficiently computable.  (Note that even if the degree of $p(x)$ is
$t<n-1,$ the polynomial thus interpolated will be identical to $p(x);$ the
terms will cancel properly to ensure the final polynomial is of degree
$t.$)

The coefficients of the polynomials $L_i(x)$ are easy to compute as well,
and need only be computed once.  An alternative means to compute them is to
compute the inverse of the Vandermonde matrix $M$ defined as $M_{ij} =
(\alpha_i)^{j-1}.$

A particularly suitable set of evaluation points is given by $\alpha_i =
\omega^{i-1},$ so that $M_{ij} = \omega^{(i-1)(j-1)},$ where $\omega$ is an
$n^{th}$ root of unity over the field $E$ used for secret sharing.  The
evaluation of the polynomial $p(u)$ becomes a {\em fast Fourier transform}:
\begin{eqnarray*}
M \vec{a} =
\left[
\begin{tabular}{ccccc}
1 & 1 & 1 & $\cdots$ & 1 \\
1 & $\omega$ & $\omega^2$ & $\cdots$ & $\omega^{n-1}$ \\
1 & $\omega^2$ & $\omega^4$ & $\cdots$ & $\omega^{2(n-1)}$ \\
\vdots &  & & & \vdots \\
1 & $\omega^{n-1}$ & $\omega^{(n-1)2}$ & $\cdots$ & $\omega^{(n-1)(n-1)}$
\end{tabular}
\right]
\cdot
\left[
\begin{tabular}{c}
$s$ \\
$a_1$ \\
$a_2$ \\
\vdots \\
$a_t$ \\
0 \\
\vdots \\
0
\end{tabular}
\right]
& = &
\left[
\begin{tabular}{c}
$p(\omega^0)$ \\
$p(\omega^1)$ \\
$p(\omega^2)$ \\
\vdots \\
$p(\omega^{t-1})$ \\
$p(\omega^t)$ \\
\vdots \\
$p(\omega^{n-1})$
\end{tabular}
\right]
= \vec{p}
\end{eqnarray*}
so that the inverse of M gives the desired weights:
\[
\vec{a} = M^{-1} \vec{p}.
\]
As observed crucially by Ben-Or {\em et al} \cite{bgw88}, the use of these
particular evaluation points supports the use of error-correcting codes,
which will be essential to defend against malicious errors.

Regardless of the choice of evaluation points, the weights can be
precomputed at the cost of a matrix inversion.  Using roots of unity as
evaluation points, evaluating $p$ and interpolating $p$ is even faster
($O(n \log n)$ time {\em vs.} $O(n^3)$) since the computations become
fast Fourier transforms.  Using the precomputed weights in the online
interpolation of $p(u)$ costs a matrix multiplication.

\subsection{Verifiability}

The astute reader will note that a single error in any of
the values will throw off the interpolation and produce an incorrect value
for $s.$  Certainly, $t+1$ reliable players will have sufficient
information to reconstruct $s$ at the appropriate time (the ``appropriate''
time is specified by their programs, which, since they are reliable, is
specified by the protocol designer), but they must be able to distinguish
correct pieces from incorrect ones.  Furthermore, they ought to be able to
tell if the dealer distributed a valid set of pieces in the first place.

This problem is known as {\em verifiable} secret sharing
\cite{cgma85,bgw88,br89}.%
\index{secret sharing!verifiable}
Cryptographic solutions often involve ideas such as
digitally signing the pieces to ensure that they aren't changed and
zero-knowledge proofs to ensure that they do interpolate to a proper
polynomial of degree $t.$ In this chapter, however, we are concerned with
unconditionally secure protocols: we make no complexity-theoretic
assumptions or restrictions, and cannot rely on such cryptographic
approaches.

For the range $t < \frac{n}{3},$ Ben-Or {\em et al} present a technique to
ensure verifiability with unconditional security.  In
Chapter~\ref{chap-min} we give a method for verifiable secret sharing for
$t < \frac{n}{2},$ which is unconditionally secure with high probability.

Ben-Or {\em et al} base their methods on BCH codes, using particular values
$\alpha_1 = \omega^0, \alpha_2 = \omega^1, \dots,
\alpha_n = \omega^{n-1}$ as the evaluation points for $p(u),$  where
$\omega$ is a primitive $n^{th}$ root of unity in the field $E$
used for secret
sharing.  We shall not list the details of error correction
here, instead referring the
interested reader to \cite{bgw88,pw72}.  The essential property to note is
that there is an error-correcting method to interpolate polynomials
evaluated at roots of unity that tolerates omissions and changes in up to a
third of the values.

For completeness and for the purposes of proving resilience (a proof has
not appeared), we describe their method for verifiability using BCH codes.
The dealer chooses a bivariate polynomial $p(u,v)$ of degree $t$ in $u$ and
$v,$ subject to $p(0,0)=s,$ and sends the polynomials
$p_i(u)=p(u,\omega^{i-1})$ and $q_i(v)=p(\omega^{i-1},v)$ to player $i.$
The original piece $\piece_i(s)$ corresponds simply to $p_i(0);$ the other
information is for verification.  Then each player $i$ sends
$p_i(\omega^{j-1})$ to player $j.$ Player $j$ can check for himself that
the values $p_1(\omega^{j-1}),\dots,p_n(\omega^{j-1})$ match his values for
$q_j(\omega^{0}),\dots,q_j(\omega^{n-1});$ if not, he requests that the
dealer broadcast the true values of $p(i,j)$ at the discrepancies.

Now, if any player detects more than $t$ errors or had to correct one of
his values, then he {\em impeaches} the dealer.  An impeachment is a
broadcast request by player $i$ to reveal $p_i(u)$ and $q_i(v).$  If a
player finds a contradiction with the polynomials broadcast by the dealer,
he too impeaches the dealer.  Finally, any player seeing $t+1$ or more
impeachments decides that the dealer is faulty, and otherwise accepts the
secret, since at least $n-t \geq t+1$ reliable players have accepted their
values and therefore determine a secret uniquely.  Figure~\ref{fig-vss-bgw}
lists the steps involved.  The following theorem is proved in 
\S\ref{sec-prove-vss}.




% PROTOCOL VSS WAS HERE!  MOVED TO END BECAUSE
% LATEX ALWAYS PUSHES IT THERE!


\begin{theorem}
\label{thm-share-private-byz}
[after Ben-Or, Goldwasser, Wigderson 1988]
 For $3t < n,$ in a completely
connected network of $n$ processors with private channels, protocol \VSS is
$t$-private and correct against Byzantine adversaries.
\end{theorem}

%A justification of this lemma has been presented; a more formal proof
%will be presented at the end of this chapter (see \S\ref{sec-con-formal}).

\section{Fundamentals: Computing With Secrets}
\label{sec-std-map}
\label{sec-fundamental}

Let $C_F$ be a boolean circuit for $F$ over the gates
$\set{\logand,\logor,\lognot},$ having inputs $x_1,\dots,x_n.$ Such a
circuit is represented as an {\em arithmetic} circuit over field $E$ using
the standard mapping $\phi$ taking $x_i^{\phi} \mapsto x_i, (x \logand
y)^{\phi} \mapsto xy, (x \logor y)^{\phi} \mapsto x+y-xy, (\lognot x)
\mapsto 1-x.$

The three-stage paradigm, ``Share Inputs; Compute New Secrets; Reconstruct
Results,'' forms the basis for constructing multiparty protocols to compute
a function $F(x_1,\dots,x_n).$ The intermediate stage is the backbone of
secure multiparty protocols: a collection of subprotocols to add and to
multiply secrets, creating new secrets from old, and thus to evaluate $C_F$
gate by gate, secretly.  In this section we review and improve techniques
of \cite{bgw88} for evaluating $F$ via $C_F.$ Formally speaking, for now we
consider computing $F$ directly without dividing it into several
intermediate functions $F^i.$ Our more general techniques will be
introduced in \S\ref{sec-tools} and \S\ref{sec-const-nc}.


\subsection{Linear Combinations}

Given secretly shared values $X_1$ and $X_2,$ a protocol to create a new
secretly shared $Y$ whose value is their sum is easy to construct (see
Figure~\ref{fig-proto-add}).  Each player computes his new piece as
$\piece_i(Y) = \piece_i(X_1+X_2) \leftarrow \piece_i(X_1) + \piece_i(X_2).$
Behind the scenes, if $X_1$ and $X_2$ are shared using polynomials
$p_{X_1}(u)$ and $p_{X_2}(u),$ then the polynomial defined by
$\piece_1(Y),\dots,\piece_n(Y)$ is $p_Y(u) = p_{X_1}(u)+p_{X_2}(u),$ a
polynomial of degree $t$ and with uniformly random coefficients subject to
$p_Y(0)=Y=X_1+X_2.$
This protocol requires no communication.  Noting that $(c \cdot p)(X) = c
\cdot p(X)$ is uniformly distributed and of degree $t$ with free term
$c\cdot p(0) = cX,$ it easily generalizes to multiplying secrets by fixed
constants and hence to linear combinations of secrets.  To effect a
constant multiplication, each player multiplies his piece by that constant,
since $(c \cdot p)(\alpha_i) = c \cdot p(\alpha_i).$



\figstretch
\boxfigwide{5.5in}{
\noindent{\bf \addone}
\begin{tabbing}  \standtabs
{\For $i=1..n$ \Dopar}  \\
\> Player $i$ sets \\ 
\>\>
%\begin{center}
$\piece_i(Y) 
%= \piece_i(c_0+c_1 X_1+\cdots+c_N X_N) 
\leftarrow
c_0 + c_1 \cdot \piece_i(X_1) + \cdots + c_N \cdot \piece_i(X_N).$
%\end{center} 
\end{tabbing}
\caption{\label{fig-proto-add}
\index{\add}
Protocol to create a new secret $Y= c_0+c_1 X_1+\cdots+c_N X_N,$ where
$c_0,\dots,c_N$ are fixed constants and $X_1,\dots,X_N$ are secret.
}}
\figstretchend


The protocol to compute several linear combinations simultaneously is
simple: repeat the single linear combination protocol in parallel.  No
interaction is needed.  Figure~\ref{fig-proto-add-many} describes the
extension.

\figstretch
\boxfigwide{5.5in}{
\noindent{\bf \add} ($\set{c_{jl}},\set{X_{jl}}$)
\begin{tabbing}  \standtabs
{\For $i=1..n$ \Dopar} \\
\>{\For $j=1..M$ \Do}  \\
\>\> Player $i$ sets  \\
\>\>
$ \piece_i(Y_j) 
\leftarrow
c_{j0} + c_{j1} \cdot \piece_i(X_{j1}) + \cdots + 
c_{jN} \cdot \piece_i(X_{jN}). $
\end{tabbing}
\caption{\label{fig-proto-add-many}
Protocol to create new secrets $Y_1,\ldots,Y_M$ whose values are
$Y_j= c_{j0}+c_{j1} X_{j1}+\cdots+c_{jN} X_{jN}.$  The $\set{c_{jl}}$
values are fixed (``public'') constants and the the $\set{X_{jl}}$ are secrets.
}}
\figstretchend

\begin{lemma}  \label{lem-add-bgw}
Protocol \add is a $t$-resilient protocol to compute a robust and private
representation $\robsec(G)$ where
\[
G(\set{c_{jl}},\set{X_{jl}}) = (c_{10}+\sum_1^N X_{1l},\ldots, 
c_{M0}+\sum_1^N X_{Ml} ).
\]
\end{lemma}

\begin{proof}
An interface for the protocol is trivial, since no messages
need be generated.  The interface need only request the inputs and
auxiliary inputs of the players that its black-box adversary $A$ requests
to corrupt, and supply the values to $A.$  
Post-protocol corruption is accomplished
by the same process.
It is easy to see that the results of the protocol are the correct secretly
shared values.  
\end{proof}

\subsection{Multiplying Secrets}
\label{sec-mult-bgw}
\label{sec-truncate}

The protocol for adding secrets does not immediately generalize to
multiplication, since the product $p_Y(u) = p_{X_1}(u) p_{X_2}(u)$ has
degree $2t.$  If the degree of the representation of the secrets is allowed
to grow, there will quickly by an insufficient number of pieces to
reconstruct the result.

Ben-Or {\em et al} and Chaum {\em et al} present the first methods to
reduce the degree of the polynomial represented by having each player
compute $\piece_i(X_1)\cdot\piece_i(X_2).$ They reduce the problem of
degree reduction to a linear combination of secrets using matrix
operations.  Before the degree reduction occurs, a random polynomial of
degree $2t$ (and zero free term) is added in order to ensure a uniform
distribution on the resulting coefficients.

We present an alternative and independently discovered approach to degree
reduction and a faster method for ensuring uniform randomness of the
resulting coefficients.  These minor optimizations are not the main thrust
of this chapter but are included because they also have certain conceptual
advantages.

We have seen in Equation~\ref{eqn-lagrange-interp} how a polynomial can be
interpolated using a weighted sum of LaGrange polynomials.  Let
$\overline{p}(u)$ denote the result of truncating all terms of polynomial
$p(u)$ having degree higher than $t;$ that is, $\overline{p}(u) = p(u) \mod
x^{t+1}.$  Then we have
\begin{eqnarray} \label{eqn-interp-trunc}
\overline{p}(x) & = & \sum_1^n \overline{L}_i(x) p(i).
\end{eqnarray}
Clearly, then, we can express the value of $\overline{p}(u)$ at the point
$\alpha_j$ as a weighted sum of the values $p(1),\dots,p(n):$
\begin{eqnarray} \label{eqn-interp-trunc-i}
\overline{p}(\alpha_j) & = & \sum_1^n \overline{L}_i(\alpha_j) p(i).
\end{eqnarray}
The weights, $\overline{L}_1(\alpha_j), \dots, \overline{L}_n(\alpha_j),$
are easily precomputed.  Furthermore, $\overline{p}(0) = p(0).$

If the values $p(1),\dots,p(n)$ are themselves shared as secrets, 
then Equation~\ref{eqn-interp-trunc-i} indicates how to express each value
$\overline{p}(\alpha_j)$ as a linear combination of secrets.  
Thus, $\overline{p}(u)$ could be used as a secret-sharing polynomial to
represent the secret $p(u),$ since it has degree $t.$  Unfortunately, the
coefficients of $\overline{p}(u)$ are not uniformly random unless the
original coefficients of $p(u)$ are.

To randomize the coefficients, it suffices to add a random polynomial of
degree $t+1$ and free term 0 to $p(u)$ before truncation.  This observation
differs from \cite{bgw88}, who use $t$ different polynomials to
construct a polynomial of degree $2t$ in order to randomize {\em all}
high-order coefficients.  However, it is necessary only to randomize
coefficients of degree $t$ or less, since the others will be truncated.
Their protocol hence requires a $t$-fold increase in the expense of
this subprotocol.

If $r(u)$ is
completely random and of degree $t,$ then $u \cdot r(u)$ is of degree $t+1$
with free term 0 as desired.  To create a random polynomial $r(u)$ (whose
free term is random), each player $i$ shares a secret $R_i$ using a
polynomial $r_i(u).$  Their sum, $r(u)=\sum_i r(u),$ is what we need;
each player $j$ holds the value $r(j) = \sum_i r(j) = \sum_i
\piece_j(R_i).$  The truncation protocol is given in
Figure~\ref{fig-truncate}.

\figstretch
\boxfig{
\noindent{\bf \truncate} $p(u)$
\begin{itemize}
\item[(T1.1)]
Choose $R_i$ at random and share it.
\item[(T1.2)]
Receive $\piece_i(R_1),\dots,\piece_i(R_n).$
\item[(T2)]
Set $\piece_i(R) \leftarrow \piece_i(R_1) + \cdots + \piece_i(R_n).$
\item[(T2.1)]
Set $\gamma_i \leftarrow p(i) + i \cdot \piece_i(R).$
\item[(T2.2)]
Share $\gamma_i.$
\item[(T2.3)]
Receive $\piece_i(\gamma_1),\dots,\piece_i(\gamma_n).$
\item[(T3)]
Set $\piece_i(p(0)) \leftarrow \overline{L}_1(i) \piece_i(\gamma_1)
+ \cdots + \overline{L}_n(i) \piece_i(\gamma_n).$
\end{itemize}
\caption{\label{fig-truncate}
\index{\truncate}
Protocol to secretly share $p(0)$ when each player $i$ holds $p(i),$
and $p(u)$ is of degree $2t.$   (Code for player $i.$)
}}
\figstretchend

Given a protocol to truncate a high-degree polynomial secretly, the
protocol to compute the product of two secrets can be stated concisely
(see Figure~\ref{fig-multiply}).  Simply: each player computes the product
of his pieces and participates in a truncation protocol, which involves
secretly sharing $\piece_i(X_1) \piece_i(X_2)$ itself.



\figstretch
\boxfig{
\noindent{\bf \multone}
\begin{itemize}
\item[(MO1)]
Set $p(i) \leftarrow \piece_i(X_1) \piece_i(X_2).$
\item[(MO2)]
Run the {\sc Truncate} protocol on $p(u)$ to obtain 
$\piece_i(p(0)) = \piece_i(X_1 X_2).$
\end{itemize}
\caption{\label{fig-multiply-one}
\index{\multone}
Protocol to multiply secrets $X_1$ and $X_2.$
(Code for player $i.$)
}}
\figstretchend

\figstretch
\boxfig{
\noindent{\bf \mult}
\begin{tabbing}  \standtabs
{\For $j=1..M$ \Dopar} \\
\> Execute protocol \multone to compute $Y_j = X_{j1} \cdot X_{j2}.$
\end{tabbing}
\caption{\label{fig-multiply}
Protocol to create new secrets $Y_1,\ldots,Y_M$ whose values are
$Y_j = X_{j1} \cdot X_{j2}.$  The $\set{X_{j1},X_{j2}}_{j\in [M]}$ are
secrets.  (Code for player $i.$)
}}
\figstretchend



\subsubsection{Byzantine Faults}

As before, we must be careful to check for misbehavior.  The protocols as
listed are secure against a passive adversary but are not reliable in the
presence of Byzantine faults.

Since the error-correcting codes (polynomials evaluated at roots of unity)
are additive, the addition of verified secrets need not be checked.
Multiplication, however, requires the resharing of pieces; it must be
checked that player $i$ correctly shares $p(i) = \piece_i(X_1)
\piece_i(X_2).$  In this section we review the method of \cite{bgw88};
in Chapter~\ref{chap-min}, we present a new method to achieve this goal
that tolerates a much larger number of faults.

\bigskip

\noindent
{\bf The ABC problem.}\index{ABC problem}
Alice knows the values of secrets $a$ and $b.$
Alice must share a new secret $c$ and prove to the other
players that the secret value of $c$ is indeed $ab.$
If Alice is honest, no information about $a,$ $b,$ or $c$
should be revealed.

\bigskip

A solution to this problem is detailed in Figure~\ref{fig-abc-bgw}.
Notice that if $f(0)g(0)$ differs from $h(0),$ then it is impossible
for Alice to select polynomials of degree $t$ to make $h(x)$ of
degree $t.$  The use of random coefficients ensures that if Alice
is nonfaulty, then an interface can easily generate messages from
Alice to faulty players, because those messages will contain uniformly
random field elements, according to Lemma~\ref{lem-ss-new}.

The protocol specifies twice that Alice participate in a \VSS
protocol using particular polynomials or pieces, in order that
the system may verify that Alice uses polynomials of degree $t.$
In other words, the subprotocols correspond to executing
\VSS but requiring that Alice send out $(p_i(u),q_i(v))$ values
in the first round that match the given polynomials.  The recipients
of these messages check in the first round whether Alice has sent
them consistent values, and if not, they consider Alice to have
sent them nothing, and continue the \VSS protocol exactly as specified
from there.

\figstretch
\boxfig{
\noindent{\bf \abc-bgw}$(s)$
\begin{tabbing}  \standtabs
(A1)
\> Alice:
\>\> {\For {$i=1..t$}  \for {$j=0..t-1$} \Do } \\
\>\>\>\> $r[i,j] \leftarrow \uniform(E)$ \\
\>\>\> {\For {$i=1..t$} \Do } \\
\>\>\>\> $h_i(x) = \sum_{j=0}^{t-1} r[i,j] x^j + $ \\
\>\>\>\>\> $x^t \cdot ( c_{t+i} - \sum_{j=1}^{t-1} r[t+1-j,j])$ \\
\> Alice shares $c_t,\ldots,c_{2t}$ using these polynomials. \\
(A2)
\> $(1 \leq i \leq n)$
\>\> $h(\alpha_i)=f(\alpha_i)g(\alpha_i) - 
\sum_{i=1}^t (\alpha_i)^t h_i(\alpha_i).$ \\
(A3)
\>Alice secretly shares $ab$ using these as $p_i(0)$ values.
\end{tabbing}
\caption{\label{fig-abc-bgw}
Protocol for Alice to verifiably share secret $c=ab.$ 
}}
\figstretchend


\begin{lemma}  \label{lem-mult-bgw}
Protocol \mult is a $t$-resilient protocol to compute a robust and private
representation $\robsec(G)$ of the produce of $M$ secrets, where:
\[
G(X_{11},X_{21},\ldots,X_{M1};X_{12},X_{22},\ldots,X_{M2})
=
(X_{11} \cdot X_{12},\ldots,X_{M1} \cdot X_{M2}).
\]
\end{lemma}

\begin{proof}
Step (MO1) of \multone 
is noninteractive and hence trivially $t$-resilient.
The \truncate protocol is $t$-resilient because it is
the concatenation of $t$-resilient protocols (\VSS and
\add).
Protocol \mult is a concatenation of two $t$-resilient subprotocols,
namely step (MO1) and the \truncate protocol,
so by Theorem~\ref{thm-concat} it is itself $t$-resilient.
\end{proof}

\subsection{Disqualification and Fault Recovery}
\label{subsec-disqual}

Rather than burden the descriptions of the protocols to come, we implicitly
require that, following an impeachment, namely a broadcast message from one
player $i$ stating that some player $j$ is faulty, each player checks to
see if the impeached player should be disqualified.  We consider a
processor {\em disqualified} if $t+1$ or more players have broadcast
impeachments of it.  The meaning of ``checks to see'' is determined by the
specifications of the particular protocol.  If the player is disqualified,
a recovery procedure may be necessary.  In this chapter, when the number of
faults is less than a third, no recovery procedure is necessary (though of
course, misbehavior is eliminated by eliminating the messages of faulty
players identified by error-correction) except in the Input stage.


If a fault occurs during the Input stage, namely when a player ought to
share its input, the faulty player's secret is replaced by a default value
selected (for full generality) according to some samplable distribution: in
addition to sharing the input $x_i,$ each player $i$ shares a set of random
bits which are used to construct a default input for player $j$ should it
fail.  Let $T$ be the set of players disqualified when sharing the inputs.
Then it is easy to describe a set of circuits $\set{C_j}_{j \in T}$ which
take as inputs the random bits shared by players $i \not\in T,$ compute
their exclusive or, and output default values for each $x_j.$ Rather than
evaluating $C_F$ directly, the protocol calls for an evaluation of the
circuit $C_F'$ which is the circuit $C_F$ with its $i^{th}$ input set to
either the output of $C_i$ or to the value $x_i$ shared by player $i;$
the circuit $C_F'$ selects one or the other by considering the sum of extra
inputs from each player specifying whether the player impeaches player $i.$
If the sum is large enough, the circuit selects the default input, and
otherwise selects $x_i.$
%Note that the description of $C_F$ is simple.   

We shall normally consider these conditions implicitly in our descriptions
of the protocols, for otherwise they would be tremendously difficult to
read.

\subsection{Putting It Together}


Given subprotocols to add and to multiply secrets, the specification of a
protocol to evaluate an arbitrary arithmetic circuit $C_F$ is not hard to
describe.  Let $E$ be a fixed finite field. A basis for a circuit is a set
of functions which the gates may compute.  An arithmetic gate is an element
of the set $\set{\times} \cup \set{(+,a_0,a_1,\dots,a_m)}_{a_0,\ldots,a_m
\in E}$ where the latter sort of gate is a {\em linear combination,}
producing $a_0 + a_1x_1 + \cdots + a_mx_m$ on inputs $x_1,\dots,x_m.$

For ease of description, we shall consider circuits as arrays of gates;
this allows us to specify circuits with multiple outputs or to describe
straight-line programs (circuits of width 1) as we desire.  It also allows
us to specify in a natural way that the outputs of particular gates at the
final level are given to distinct players.  Specifically, a circuit is a
$(d+1) \times w$ array of elements of the form
$(g_{ij},\inputgates(g_{ij})),$ where $\inputgates(g_{ij})$ is a set of
pairs $(a,b)$ describing the indices of gates whose output leads to
$g_{ij}.$ We define $\inputgates_k(g_{ij})$ to be $(a,b)$ if $g_{ab}$ is
the $k^{th}$ earliest gate (in row-major order) leading into $g_{ij}.$ Each
input $g_{ab}$ to gate $g_{ij}$ must satisfy $a<i.$ The $0^{th}$ layer
represents the inputs $x_1,\dots,x_n$ to the circuit.  Let $\outgates(i)$
denote the set of gates $g_{dj}$ whose output represents the value $F_i$
that player $i$ should learn.

Without loss of generality we assume that even-numbered levels contain only
linear combination gates and odd-numbered levels contain only
multiplication gates.  The depth of the circuit is doubled at most.
Denote the coefficients of the additive gate $g_{ij}$ by
$a_{i,j,0},a_{i,j,1},\ldots,a_{i,j,\mid \inputgates{g_{ij}} \mid}.$

A circuit with {\em bounded fan-in} satisfies $\abs{\inputgates(g_{ij})} <
c$ for some constant $c$ and for all $i,j.$ A circuit with {\em bounded
multiplicative fan-in} satisfies $\abs{\inputgates(g_{ij})} < c$ for some
constant $c$ and for all $i,j$ such that $g_{ij}=\times.$  A
$\times$-fanin-2 circuit has multiplicative fan-in of 2.

The class $NC^1$ consists of functions with unbounded fan-in
polynomial-size logarithmic-depth circuit families, over the basis
$\set{{\rm AND, OR, NOT}}.$ The class $ANC^1$ is described by
polynomial-size logarithmic-depth circuit families, over the arithmetic
basis $\set{(+,a_0,a_1,\dots,a_m),\times}.$  We consider a circuit {\em
efficient} if it is of polynomial size and polynomial depth.

\begin{theorem} (After \cite{bgw88})
\label{thm-bgw}
Let $\set{F^{n,m}}$ be a family of functions described by a
$\times$-fanin-2 circuit family $C_{F^{n,m}}.$ Then for $3t<n,$ there
exists a {\bf $t$-resilient} protocol leaking $F^{n,m}.$  This protocol 
requires
a polynomial number of bits (in the size of $C_{F^{n,m}}$) and $O({\tt
depth}(C_{F^{n,m}}))$ rounds of interaction.
\end{theorem}

\begin{proof}
The protocol (see Figure~\ref{fig-eval}) consists of secretly sharing all
the inputs, then evaluating $C_{F^{n,m}}$ layer by layer, maintaining the
gate outputs as secrets.  At each layer, all gates are evaluated in
parallel.  Finally, for $1 \leq i \leq n,$ each output secret in
$\outgates(i)$ is reconstructed for player $i.$

\figstretch
\boxfig{
\noindent{\bf \eval}-$C_F$
\begin{tabbing} \standtabs
(E1) \>
Each player $i$ runs \VSS($x_i$).   \\
\>\> Denote these secrets at level 0 of the circuit by 
$z_{01},\dots,z_{0w}.$ \\
(E2) \> \ccomment{Evaluate addition and multiplication layers} \\
\> {\For $l=1..d/2$ \Do} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\>\> Run \add with coefficients $\set{c_{lv,j}},$ secrets 
$\set{z_{\inputgates_j{g_{lv}}}}$ to compute: \\
\>\>\>
$z_{2l,v}= c_{2l,v,0} + \sum c_{2l,v,j} z_{\inputgates_j(g_{2l,v})} $
\>\>\>\>\>
($v=1..w,$ $j=1..\abs{\inputgates(g_{lv})}$)
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\>\> Run \mult with secrets 
$\set{(z_{\inputgates_1(g_{lv})}, z_{\inputgates_2(g_{lv})} )}$
to compute: \\
\>\>\>
$z_{2l,v}= 
z_{\inputgates_1(g_{lv})} \cdot z_{\inputgates_2(g_{lv})}$ 
\>\>\>\>\>
($v=1..w$) \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
(E3) \> 
{\For $i=1..n$ \Dopar} \\
\>\>
{\for $j\in \outgates(i)$ \Dopar} \\
\>\>\>
  Reveal $z_{lj}$ to player $i.$
\end{tabbing}
\caption{\label{fig-eval}
\index{\eval$(F)$}
Protocol to evaluate a circuit $C_F$ for $F(x_1,\dots,x_n).$
}}
\figstretchend

By lemmas \ref{lem-add-bgw} and \ref{lem-mult-bgw} and Theorem
\ref{thm-concat}, the overall protocol is $t$-resilient, since it is a
concatenation of perfectly $t$-resilient protocols for robust and private
functions.
\end{proof}




\subsection{Some Applications}
\label{sec-ballots}

Protocols for problems such as taking a secret ballot are now relatively
easy to describe.  Chapter~\ref{chap-app} also describes some simple
protocols for useful problems, though those protocols have been optimized
for efficiency using various tricks not evident in the preceding analysis.
Let us examine how, at this stage, secure multiparty protocols may be
constructed from simple gate operations.

\begin{exampleenv}  \label{exa-ballot}
{\bf Secret Ballot.}

A {\em secret ballot} is a private and reliable distributed computation of
the sum of 0/1 inputs.  Let us give a protocol for taking a secret ballot
which is private, correct, ensures that the voters cast votes
independently, and reveals the result to everyone, even when up to a third
of the voters may be untrustworthy.

The protocol is straightforward, given the secret linear-combination and
multiplication protocols.  Each voter casts his vote $X_i$ by secretly
sharing it. To ensure that each voter cast at most one vote, they secretly
compute $Z_i=X_i(X_i-1)$ for each $i,$ and reconstruct the result for
everyone.  Any voter whose value is nonzero is disqualified.  Let $J$ be
the set of voters who are not disqualified.  Then, together, the voters run
the \add protocol to compute $Y=\sum_{i \in J} X_i.$ Finally, they
reconstruct the result $Y$ for everyone.

It is easy to see that revealing $Z_i$ gives no information about the vote
cast by reliable voter $i.$ That is, the result for reliable players is
{\em always} 0, and hence a private and robust function.  Furthermore, this
protocol is fast and efficient, requiring one multiplication and two
additions, which take a small constant number of rounds.
\end{exampleenv}

\begin{exampleenv}   \label{exa-unan-ballot}
{\bf Unanimous Vote.}

A slightly more complicated goal is to decide if an entire committee votes
unanimously or not, without revealing the tally if the committee is not in
agreement.  As in Example~\ref{exa-ballot}, the voters secretly compute
$Y,$ the tally of the valid 0/1 votes.  Next, they compute the function
$f(y) = 1-(n-y)^{p-1},$ where $p$ is the size of the field being used for
sharing.  Notice that $f(n)=1$ whereas $f(y)=0$ for $y \not= n.$
Finally they reveal $f(y)$ to everyone.

An algebraic circuit of depth $\log p$ suffices to compute $f(y),$ noting
that the multiplicative gates are restricted to fan-in 2.  If we take $p$
to be on the order of $n,$ then the depth is roughly $O(\log n).$ The
number of rounds required to perform the unanimous ballot is $O(\log n),$
and the number of bits is polynomial in $n.$ This is a prime example of a
protocol whose running time is made efficient through our methods for
constant-rounds protocols.



\figstretch
\boxfig{
\noindent{\bf \protostyle Unanimous-Vote}
\begin{itemize}
\item
Each voter $i$ shares $X_i.$
\item
Compute and reveal $Z_i=X_i(X_i-1)$ for $1\leq i \leq n.$  Let $J$ be the set
of $i$ for which the result is 0.
\item
Compute $Y = \sum_{i \in J} X_i.$
\item
Compute $V_1 = Y-n$ and $W_1 = Y-n.$
\item
{\For $j = 1 .. \lfloor \log p \rfloor$ \Do}
%
\begin{itemize}
\item
Compute $W_{i+1} = W_{i}^2.$
\item
If the $i^{th}$ bit of the binary expansion of $p-1$ is 1,
compute $V_{i+1} = V_i W_{i+1},$ else let $V_{i+1} = V_i.$
\end{itemize}
%
\item
Reconstruct $V_{\log p}.$  If 0, output ``unanimous,'' else output
``disagreed.''
\end{itemize}
\caption{\label{fig-unan-ballot}
Protocol to decide if secret ballot is unanimous without revealing the
tally. (Network protocol.)
}}
\figstretchend

\end{exampleenv}

\section{Tools for Efficient Protocols}
\label{sec-tools}

In this section we present a collection of useful and important
subprotocols.  The technique for unbounded fan-in multiplication presented
in \S\ref{sec-iter-mult} is the critical tool for developing protocols that
require a constant number of rounds as opposed to a number of rounds
proportional to the depth of a circuit for $F.$

\subsection{Random Secret Values}

We often have need of secretly shared random field elements whose value no
player knows.  That is, we desire a secret whose value is uniformly random
and independent of the information of any $t$ or fewer players.

\figstretch
\boxfig{
\noindent{\bf \randomsecret}$(R)$
\begin{itemize}
\item
Each player $i$ chooses $R_i$ uniformly at random from the field $E$ and
runs \VSS to share it.  The default value is 0 for misbehaving players.
\item
Run \add to compute $R = R_1 + \dots + R_n.$
\end{itemize}
\caption{\label{fig-randomsecret}
Protocol to create random secret field element $R.$  
}}
\figstretchend

Random secret bits are also useful.  They are generated simply by computing
the parity of 0/1-valued secrets shared by each player.  Over a field of
characteristic 2, one computes the parity by computing simply the sum,
requiring no interaction beyond the secret sharing.  Over other fields, a
logarithmic-depth circuit is needed (though \ref{thm-nc1} shows how to
perform this in constant rounds).  Before computing the parity, each shared
bit is verified to be 0 or 1 by computing $b_i(b_i-1),$ which is 0 iff
$b_i$ is 0 or 1, and which is a private function since its value is
independent of $b_i.$

\figstretch
\boxfig{
\noindent{\bf \randombit}$(b)$
\begin{itemize}
\item
Each player $i$ sets $b_i \leftarrow \uniform(\set{0,1})$ and shares it.
\item
Run \add and \mult to compute $c_i=b_i(b_i-1).$
\item
Run \add to compute $b = \sum_{c_i = 0}  b_i.$
\end{itemize}
\caption{\label{fig-randombit}
Protocol to create random secret field element $b$ in a field of
characteristic 2.
}}
\figstretchend


\subsection{Groups and Inverses}

The best known algebraic circuit to compute multiplicative inverses in a
field is fairly deep.  It turns out, surprisingly, that the number of
rounds required to secretly compute the multiplicative inverse of a secret
is the same as that needed to multiply two elements, despite the large
number of rounds that would be required by simulating an arithmetic circuit
directly.  The power of this result will be evident in the next section,
where we shall use it to construct a protocol to invert matrices, which in
turn will support a constant-round protocol for any $NC^1$ circuit.

\begin{theorem}   \label{thm-group-inv}
{\bf (Constant Rounds for Group Inverses)}
Let $G$ be a group, and let $X \in G$ be secretly shared.  Let $\Pi_M$ be a
protocol to multiply {\em two} elements in $G$ that runs in $T_M$ rounds
and uses $C_M$ bits; let $\Pi_R$ be a protocol to generate a random element
in $G$ that runs in $T_R$ rounds and uses $C_R$ bits.  Let
$T=$max$(T_M,T_R)$ and $C=$max$(C_M,C_R,C_{\mbox{\scriptsize share}}),$
where $C_{\mbox{\scriptsize share}}$ is the number of bits used to
secretly share a group element.  

Then there is a protocol to secretly compute $X^{-1}$ using $O(T)$ rounds
and $O(C)$ bits.  Specifically, if multiplication of two elements requires
constant rounds then inversion requires only constant rounds.
\end{theorem}

\begin{proof}
The protocol is exhibited in Figure~\ref{fig-group-inv}.  Its security
rests on the elementary observation that, for any $X,$ the distribution
induced by multiplying by a uniformly random field element is uniform over
the group.  In other words, the intermediate function $F^1(X)=(V,U)$ is
private and robust, since the public results ($V$) have the same
distribution regardless of $X,$ and the other results are secretly shared;
so the computation of $F^1$ is as easy to simulate as the ideal vacuous
protocol.  The function $F^2$ is such that $F^2(V,U)=V^{-1}U=X^{-1}$
and $F^2$ admits a resilient protocol $\Pi_M.$  Thus $F=F^2 \closedcomp
F^1$ and Theorem~\ref{thm-concat} applies.


\figstretch
\boxfig{
\noindent{\bf \invert}$(X)$
\begin{itemize}
\item
Run $\Pi_R$ to secretly generate a random secret element $U \in G.$
\item
Run $\Pi_M$ to secretly compute $V \leftarrow UX.$
\item
Reconstruct $V$ for every player.
\item
Each player $i$ computes $V^{-1}$ individually.  It can now be treated
as a fixed public constant.
\item
Secretly compute $Y \leftarrow V^{-1}U.$
\end{itemize}
\caption{\label{fig-group-inv}
Protocol to compute secret inverse of a secret group element. 
}}
\figstretchend
\end{proof}


\subsection{Secret Matrices and Matrix Inversion}
\label{sec-secret-matrices}

A {\em secret $n\times n$ matrix} is a collection of $n^2$ secrets, each
representing an element of the matrix.  Thus each player holds $n^2$
pieces, one of each entry.  Figure~\ref{fig-multmatrix} shows how to
multiply matrices secretly.

\figstretch
\boxfig{
\noindent{\bf \multmatrix}$(A,B,C)$
\begin{itemize}
\item
{\For $i=1..\alpha$ \Dopar}
{\for $j=1..\gamma$ \Dopar}
run \add to compute 
\[
C_{ij} = \sum_{k=1}^{\beta}  A_{ik} B_{kj}.
\]
\end{itemize}
\caption{\label{fig-multmatrix}
Protocol to secretly multiply secret matrices $A$ and $B$ of dimensions
$\alpha \times \beta$ and $\beta \times \gamma,$ respectively. 
}}
\figstretchend

Each entry of the inverse of a $3 \times 3$ matrix $M$ is easily expressed
as a small, constant-depth circuit applied to the nine entries of $M.$
By Theorem~\ref{thm-bgw}, we have the following:

\begin{corollary}   \label{cor-three-matrix-inv}
There exists a protocol to invert a full-rank secret $3 \times 3$ matrix
using a polynomial number of bits and a {\em fixed constant} number of
rounds.
\end{corollary}


Given a constant-rounds protocol $\Pi_R$ to generate a random $n \times n$
secret matrix of full rank, Theorem~\ref{thm-group-inv} implies the
following result:

\begin{corollary}   \label{cor-matrix-inv}
There exists a protocol to invert a full-rank secret $n \times n$ matrix
using a polynomial number of bits and a constant expected number of rounds.
\end{corollary}

\begin{proof}
Consider the group $G$ of full rank matrices under multiplication.  To
generate random $n \times n$ secret matrices having full rank, it suffices
to generate a pair $(R,S)$ of uniformly random secret matrices such that
$RS$ has full rank.  See Figure~\ref{fig-full-rank-matrix}.  Because $S$ is
therefore uniformly random of full rank, the distribution on $U=RS$ is
uniformly random over full-rank matrices regardless of the value of $R.$
Hence the desired function (generate a full rank random matrix) can be
written as the composition of two private and robust functions, the first
computing $U$ and the second computing the full rank matrix.  Because the
probability of generating a uniformly random matrix of full rank is
constant,
%(roughly $1/e$) 
the expected number of rounds is constant.  Clearly, a single repetition
suffices with high probability
%(roughly $1-1/e^k$) 
if several ($k$) of these pairs are generated and tested in parallel, and
the first qualifying pair is used.  Because the subprotocol to generate
random group elements uses expected constant rounds, the overall protocol
is {\em expected} constant rounds.  This differs from the {\em fixed}-size
matrix inverse problem, whose solution requires {\em fixed} constant
rounds.

\figstretch
\boxfig{
\noindent{\bf \randommatrix}$(X)$
\begin{itemize}
\item[(RM1)]
Generate uniformly random secret matrices $R,S,$
using the \randomsecret protocol to create each entry.
\item[(RM2)]
Secretly compute $U=RS$ and reveal the result.  If $U$ has full rank, use
$R.$  Otherwise go to step 1.
\end{itemize}
\caption{\label{fig-full-rank-matrix}
Protocol to generate random secret matrix of full rank.  
}}
\figstretchend
\end{proof}

\subsection{Random Inverse Pairs and Large Fields}

The following theorem describes another useful tool for a computation for
which no shallow circuit is known: inverting secret {\em field} elements.
In order to avoid revealing a 0-valued secret because of a failed attempt
to invert it, we extend the multiplicative inverse so that $0^{-1}=0.$

\begin{theorem}   \label{thm-large-inv}
{\bf (Constant Rounds for Multiplicative Field Inverses)}
Let $E$ be a {\em field}, and let $X \in E$ be secretly shared.  Let
$\Pi_M$ be a protocol to multiply or add {\em two} elements in $E$ that
runs in $T_M$ rounds and uses $C_M$ bits; let $\Pi_R$ be a protocol to
generate a random element in $E$ that runs in $T_R$ rounds and uses $C_R$
bits.  Let $T=$max$(T_M,T_R)$ and $C=$max$(C_M,C_R,C_{\mbox{\scriptsize
share}},\abs{E}^4),$ where $C_{\mbox{\scriptsize share}})$ is the number of
bits used to secretly share a group element.  

Then there is a protocol to secretly compute $X^{-1}$ using $O(T)$ rounds
and $O(C)$ bits.  Specifically, if multiplication of two elements requires
constant rounds then inversion requires only constant rounds.
\end{theorem}

\begin{proof}
The protocol is exhibited in Figure~\ref{fig-field-inv}.  The distribution
on $U_i$ and $V_i$ is clearly independent of $X.$ Notice that the
distribution on $R_i,$ given $U_i=V_i=0,$ is uniform over {\em all} field
elements, {\em including 0.} Hence $X-R_i$ is uniform over all field
elements regardless of $X,$ and the intermediate results have the same,
uniform distribution for any $X.$ It is not hard to see that pairs of
extended inverses are the only pairs to give zeros in both tests in step
(FI2).  Thus, the inverse function $F$ is written as the composition of
private and robust intermediate functions, and Theorem~\ref{thm-concat}
applies.  Choosing $\abs{E}^4$ random pairs ensures that with probability
at least $1-2^{-\abs{E}}$ all such pairs will appear and that step~(FI5)
will succeed.

\figstretch
\boxfig{
\noindent{\bf \fieldinvert}$(X)$
\comment{Invert a secret field element.}
\begin{enumerate}
\item[(FI1)]
Generate $\abs{E}^4$ random secret pairs $(R_i,S_i).$
\item[(FI2)]
For each $1 \leq i \leq \abs{E}^4,$ secretly compute
\begin{eqnarray*}
U_i & = & R_i( 1 -  R_i S_i ),\\
V_i & = & S_i( 1 -  R_i S_i ).
\end{eqnarray*}
\item[(FI3)]
Reveal all the $U_i$ and $V_i.$
\item[(FI4)]
For each $i$ such that $U_i=V_i=0,$
compute and reveal $X-R_i.$
%run {\em Test-for-Zero($X-R_i$)}.
\item[(FI5)]
Call $Y$ the first secret $S_i$ such that \\
$X-R_i=0.$ If none exists, go to step 1.
\end{enumerate}
\caption{\label{fig-field-inv}
\index{\fieldinvert}
Protocol to compute secret multiplicative inverse of a secret in a field
$E.$ 
}}
\figstretchend
\end{proof}


\subsection{Iterated Multiplication}
\label{sec-iter-mult}

The final set of tools provide the crucial support for reducing the number
of rounds of interaction.  We show the surprising result that large fan-in
multiplication of group elements can be performed in constant rounds.  A
naive approach would require $\log N$ rounds, where $N$ is the number of
elements to multiply.  Specifically, we show:

\begin{theorem}   \label{thm-iterated-mult}
{\bf (Constant Rounds for Iterated Multiplication)}
Let $G$ be a group, and let $X_1,\dots,X_N \in G$ be secretly shared.  Let
$\Pi_M$ be a protocol to multiply {\em two} elements in $G$ that runs in
$T_M$ rounds and uses $C_M$ bits; let $\Pi_R$ be a protocol to generate a
random element in $G$ that runs in $T_R$ rounds and uses $C_R$ bits.  Let
$T=$max$(T_M,T_R)$ and $C=N \cdot {\rm max}(C_M,C_R,C_{\mbox{\scriptsize
share}}),$ where $C_{\mbox{\scriptsize share}}$ is the number of bits used
to secretly share a group element.

Then there is a protocol to secretly compute $Y=X_1 \cdots X_N$ using
$O(T)$ rounds and $O(C)$ bits.  Specifically, if multiplication of two
elements requires constant rounds then multiplication of $N$ elements
requires only constant rounds.
\end{theorem}

\begin{proof}
Figure~\ref{fig-iter-mult} describes the protocol.
The following demonstrates that $Y$ is the desired product:
\begin{eqnarray*}
Y & = & R_0 S R_N^{-1} \\
  & = & R_0 R_0^{-1} X_1 R_1 R_1^{-1} X_2 \cdots X_j R_N R_N^{-1} \\
  & = & X_1 \cdots X_N
\end{eqnarray*}

\figstretch
\boxfig{
\noindent{\bf \itermult}$(X_1,\ldots,X_N)$
%\comment{Multiply many secrets.}
\begin{enumerate}
\item[(IM1)]
Generate $N+1$ secret uniformly random
group elements $R_0,\dots,R_N \in G.$
\item[(IM2)]
Secretly compute the inverses, 
$R_0^{-1},\dots,R_N^{-1}.$
\item[(IM3)]
For $j=1,\dots,N,$ simultaneously compute the following new secrets:
\[
S_j = R_{j-1}^{-1} X_j R_j.
\]
\item[(IM4)]
Reveal all the secret elements $S_j.$
\item[(IM5)]
Each player privately computes 
\[
S = S_1 \cdots S_N.
\]
\item[(IM6)]
Secretly compute $Y = R_0 S R_N^{-1}.$ 
\end{enumerate}
\caption{\label{fig-iter-mult}
\index{\itermult}
Protocol to compute the product of several elements in a field $E.$ 
}}
\figstretchend

Since each $R_j$ is generated uniformly at random,
and since each $R_j$ and each $X_j$ is invertible,
revealing $S_1,\dots,S_N$ gives no information about $X_1,\dots,X_N.$
That is, the list of elements $(S_1,\dots,S_N)$ is distributed uniformly
at random, given by the following easy lemma:

\begin{lemma}
\label{lem-secret-iter-mult}
Let $G$ be a group.  For any $X_1,\dots,X_N \in G,$ 
\begin{tabbing}  \standtabs
\> $\uniform( G^N ) =$
\>\>\>
$\{(R_0,\ldots,R_N) \leftarrow \uniform(G^{N+1}));$ \\
\>\>\>\>
$
S_1 \leftarrow R_0 X_1 R_1^{-1};
\ldots;
S_N \leftarrow R_{N-1} X_N R_N^{-1}:
(S_1,S_2,\ldots,S_N) \}
$ 
\end{tabbing}
\end{lemma}

Formally speaking, protocol \itermult computes a four robust and private
intermediate functions.  The first function $F^1$ supplies each player with
pieces of random group elements; the second, $F^2,$ provides pieces of
their inverses; the third, $F^3,$ generates a public (hence robust)
uniformly distributed (hence private) vector of values $(S_1,\ldots,S_N);$
and the fourth provides pieces of $Y.$ Theorem~\ref{thm-concat}
implies the resilience of \itermult.

Applying Theorem~\ref{thm-group-inv}, we need only $O(C)$ rounds to invert
each secret $R$ in (IM2).  Steps (IM3) and (IM6) use constant depth
circuits and are easily performed with a constant number of rounds of
interaction.  Step (IM4) requires a round of interaction and step (IM5)
requires none.
\end{proof}


\section{The Power of Iterated Multiplication}
\label{sec-const-nc}


In this section we prove the crucial and surprising result that is the
focus of this chapter.  The result depends critically on the ability to
perform iterated multiplication of secret $3 \times 3$ matrices;
Theorem~\ref{thm-iterated-mult} of the previous section is key.
Let $ANC^1$ denote the class of functions which can be written
as polynomial size algebraic formulas, or logarithmic depth circuits,
over a fixed finite field $E.$
(The abbreviation derives from ``Algebraic NC.'')
The standard approach of simulating a circuit suggests that the number
of rounds required to evaluate $F \in ANC^1$ grows unboundedly, and
it was conjectured that a logarithmic lower bound on the number of
rounds would hold.  We prove to the contrary that a fixed number 
of rounds suffice.

\begin{theorem}      \label{thm-nc1}
\index{constant rounds!NC1}
For $3t<n$ and any function $F \in ANC^1$ (or $F \in NC^1$),
there exists a $t$-resilient protocol to compute $F$ 
in a {\em constant} number of rounds, with polynomial message sizes.
\end{theorem}

\begin{proof}
In \cite{bar86} Barrington showed that $NC^1$ is equivalent
to multiplying polynomially-many permutations of 5 elements.
Ben-Or and Cleve \cite{bc88} generalized this to show that computing 
polynomial-size algebraic formulas (complete for $ANC^1$) 
over a field $E$ is equivalent
to multiplying polynomially-many $3 \times 3$ matrices over that field.
Our method for computing $ANC^1$ was facilitated by a table-chaining technique 
suggested by M. Rabin \cite{rab88-pc}.  %personal communication

Let $F$ be representable by an algebraic formula $\scf$ of depth $d$ having
variables $X_1,\dots,X_n.$ By \cite{bc88}, there is a sequence of $3 \times
3$ matrices $M_1,\dots,M_{p(d)}$ whose product $M[\scf]$ contains
$F(X_1,\dots,X_n)$ in the upper right entry $(1,3).$ Here, $p(d)=O(4^d).$

For completeness we describe the sequence of matrices corresponding to
$\scf.$  Let
\[
\begin{tabular}{rclrcl}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$J_1$ & = & 
$\left[
\begin{tabular}{rrr}
 0 &  1 &  0 \\
-1 &  0 &  0 \\
 0 &  0 &  1 \\
\end{tabular}
\right]$
&
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$J_2$ & = & 
$\left[
\begin{tabular}{rrr}
 0 &  0 & -1 \\
 1 &  0 &  0 \\
 0 &  1 &  0 \\
\end{tabular}
\right]$
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$J_3$ & = & 
$\left[
\begin{tabular}{rrr}
 0 &  1 &  0 \\
 0 &  0 &  1 \\
 1 &  0 &  0 \\
\end{tabular}
\right]$
&
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$J_4$ & = & 
$\left[
\begin{tabular}{rrr}
 0 &  0 &  1 \\
-1 &  0 &  0 \\
 0 &  1 &  0 \\
\end{tabular}
\right]$
\end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}{lcr}
$J_5$ & = & 
$\left[
\begin{tabular}{rrr}
-1 &  0 &  0 \\
 0 &  0 &  1 \\
 0 &  1 &  0 \\
\end{tabular}
\right]$
\end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\]

Furthermore, let
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}{lcr}
$M[f]$ & = & 
$\left(
\begin{tabular}{rrr}
 1 &  0 &  $f$ \\
 0 &  1 &  0 \\
 0 &  0 &  1 \\
\end{tabular}
\right)$
\end{tabular}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Constants and variables are represented by $M[c]$ and $M[x_i].$ The product
$M[\scf]$ is derived from the following observations:
\begin{eqnarray*}
M[f+g] & = & M[f] \cdot M[g] \\
M[f \cdot g] & = & J_1 \cdot M[g] J_2 \cdot M[f] 
\cdot J_3 \cdot M[g] J_4 \cdot M[f] \cdot J_5. 
\end{eqnarray*}

The protocol is simple: each $M[x_i]$ is shared by player $i,$ and the
network multiplies all the matrices together.  Notice that the matrices are
all full-rank and therefore form a group under multiplication.  According
to Theorem~\ref{thm-iterated-mult} and
Corollary~\ref{cor-three-matrix-inv}, the secret product $M[\scf]$ takes a
constant number of rounds to compute.  The result is the secret $M[\scf](1,3)$
and is revealed or left secret for use in further protocols.  

Figure~\ref{fig-evalconst} gives more details.  For the sake of efficiency,
the constant matrices are collapsed at the start: 
let $H=\set{M_i \mid M_i
\mbox{\hspace{0.1in} contains a variable}},$ 
let $q = \abs{H},$ let $h(i)$ be the index of
the $i^{th}$ member of $H,$ let $G(i)=\set{M_j \mid h(i)<j<h(i+1)}$ be the
set of constant matrices to the right of $M_{h(i)},$ and let $G(0)$ be the
set of matrices to the left of $M_{h(1)}.$ Define $N_1 = [\prod G(0)] H(1)
[\prod G(1)]$ and $N_j = H(j)[\prod G(j)].$

\figstretch
\boxfig{
\noindent{\bf \evalconst}$(F)$
\begin{itemize}
\item
Each player $i$ shares $x_i.$
\item
Secretly compute each $N_1,\ldots,N_q$ using \add, noninteractively.
\item
Run \itermult($N_1,\ldots,N_q$) to obtain secret matrix $M[\scf].$
\item
The result is the top right secret of $M[\scf],$ {\em i.e.} $M[\scf](1,3).$
\end{itemize}
\caption{\label{fig-evalconst}
\index{\evalconst$(F)$}
Protocol to evaluate $NC^1$ or $ANC^1$ circuit in constant rounds and
polynomial message sizes.
}}
\figstretchend


\end{proof}


\subsection{Reducing Rounds for Polynomial Size Circuits}

The results of the previous section easily show how to reduce the number of
rounds for circuit-based protocols.

\begin{corollary}  \label{cor-reduce-rounds}
For $3t<n$ and any function family $F$ described by a polynomial-size
circuit family $C_F,$ there exists a $t$-resilient protocol to compute $F$
using $O({\tt depth}(C_F)/(\log nm))$ rounds, with messages of size
polynomial in $n$ and $m.$
\end{corollary}

\begin{proof}
Define the slice function $F^i$ to be the set of outputs at the $(i\cdot
\log nm)^{th}$ level of circuit $C_F.$ Clearly, $F$ can be written as the
product of ${\tt depth}C_F/(\log nm)$ of these functions, and each function
is in $NC^1.$ By Theorem~\ref{thm-nc1}, there is a set of protocols to
evaluate each slice function; by eliminating the final step
from each protocol, we obtain a protocol that produces secretly
shared values rather than revealing the outputs of that level.  By
Theorem~\ref{thm-concat}, the concatenation is $t$-resilient.  The number
of rounds required by the concatenated protocol is clearly $\log nm$ times
the number of rounds to compute a slice function, which is constant.
\end{proof}

\subsection{Determinants in Constant Rounds}

In fact, Theorem~\ref{thm-nc1} gives a stronger result using iterated
multiplication of $n \times n$ matrices.  By
Theorem~\ref{thm-iterated-mult} and Corollary~\ref{cor-matrix-inv}, there
is an {\em expected} constant-rounds protocol to compute the product of a
polynomial number of matrices.  Cook \cite{coo85} and Berkowitz
\cite{ber84} show that the iterated product of integer $n \times n$
matrices is complete for \mbox{DET$^*$}, the class of all problems that are
$NC^1$ reducible to DET, namely those that are $NC^1$ reducible to
computing the determinant of an $n \times n$ matrix.
\begin{corollary}      \label{cor-det}
For $3t<n$ and any function $F \in \mbox{DET$^*$},$ there exists a
$t$-resilient protocol to compute $F$ in a {\em constant expected} number
of rounds, with polynomial message sizes.
\end{corollary}


\section{Any Function In Constant Rounds}
\label{sec-any-const}

In fact, at the expense of a possible exponential blowup in message size,
it is certainly possible to achieve secure protocols in constant rounds for
$3t<n.$ The idea is based on representing a function $F(x_1,\ldots,x_n)$ as
a weighted sum whose addenda are computable in constant rounds.  The
message size depends on the number of addenda, which itself depends on $F.$
Ignoring the number of addenda, each of which can be computed in parallel
and then added non-interactively, the protocol requires constant rounds.

\begin{lemma}  \label{lem-can-f-delta}
Any function $F : E^n \rightarrow E$ has a canonical representation
as a function $c_F$ such that on $\set{0,1}^n,$ $c_F(x_1,\ldots,x_n) =
F(x_1,\ldots,x_n),$ in the following manner:
\[
c_F(x_1,\ldots,x_n) =
\sum_{(\epsilon_1,\ldots,\epsilon_n) \in \set{0,1}^n}
F(\epsilon_1,\ldots,\epsilon_n)  \cdot
\delta((\epsilon_1,\ldots,\epsilon_n),(x_1,\ldots,x_n))
\]
where $\delta((\epsilon_1,\ldots,\epsilon_n),(x_1,\ldots,x_n))=1$%
\index{Kronecker delta}%
\index{delta function}
iff each $\epsilon_i=x_i,$ and otherwise is 0.
\end{lemma}

\begin{theorem}  \label{thm-any-const-exp}
For $3t<n$ and any function $F,$
there exists a $t$-resilient protocol to compute $F$ 
in a {\em constant} number of rounds.  The message sizes may grow
exponentially, depending on the nature of $F.$
\end{theorem}

\begin{proof}
The protocol is trivial, given Lemma~\ref{lem-can-f-delta} and a means to
compute $\delta$\index{delta} in constant rounds: in parallel,
secretly compute $\delta$
for all $(\epsilon_1,\ldots,\epsilon_n)$ values such that
$F(\epsilon_1,\ldots,\epsilon_n)\not=0,$ and then compute the secret linear
combination of the results using the publicly-known weights
$F(\epsilon_1,\ldots,\epsilon_n)$ as specified.

Define the normalization of $x$ to be $\norm{x}=1$ iff $x \not= 0,$ and
$\norm{0}=0.$  Then we have
\[
\delta((\epsilon_1,\ldots,\epsilon_n),(x_1,\ldots,x_n)) =
1- \norm{ \sum_{i=1}^n  \norm{\epsilon_i-x_i} ~~~ }
\]
But Theorem~\ref{thm-large-inv} states that there is a constant-rounds
protocol for computing the extended multiplicative inverse of a secret.
Clearly, $\norm{x}=x \cdot x^{-1},$ for this extended inverse.  Then the
protocol to compute $\delta$ is simple: normalize each difference by
calling the \fieldinvert protocol on $\epsilon_i-x_i;$ sum the results
non-interactively; normalize the sum; and subtract the result from 1,
non-interactively.
\end{proof}

An alternative but equivalent formulation arises from the following
observation: 
\begin{lemma}  \label{lem-can-f-poly}
Any function $F : E^n \rightarrow E$ has a canonical representation as a
polynomial $c_F$ {\em of degree $n$} such that on $\set{0,1}^n,$
$c_F(x_1,\ldots,x_n) = F(x_1,\ldots,x_n).$  In particular, any function
$F : \set{0,1}^n \rightarrow \set{0,1}$ has such a representation as a
polynomial of degree $n$ over $E.$
\end{lemma}

\begin{proof}
Follows from simple algebra and the following definition:
\[
c_F(x_1,\dots,x_n) =
\sum_{(\epsilon_1,\ldots,\epsilon_n) \in \set{0,1}^n}
F(\epsilon_1,\ldots,\epsilon_n)  \cdot
\prod_{i=1}^n (1 - (x_i-\epsilon_i)(-1)^{\epsilon_i} )
\]
\end{proof}


\section{Formal Proofs}
\label{sec-con-formal}

Describing an interface is usually far more tedious and difficult than
giving a convincing argument that the information held by an adversary is
independent of the inputs of reliable players.  It should be remarked that
the protocol designer need not concern himself with the details of the
interface; given a protocol compiler and a list of subprotocols that can be
concatenated, the actual implementation of a protocol has nothing to do with
the specification of a interface for the protocol.  Thus the only purpose
of the following specifications are to prove the resilience of the protocol
and are irrelevant to the implementation.

\iffalse
\subsection{Step By Step Simulation}

In constructing messages from reliable players or reconstructing the state
of a newly corrupted player, it is essential to distinguish which portion
of the player's information is implicitly or explicitly determined by the
current view of the adversary, and which portion is completely unknown to
the adversary. In our protocols there are two extremes: either the
adversary already ``knows'' the value of a variable held by a reliable
player (as in the case of a piece distributed by a corrupted player), or it
``knows'' nothing, in the sense that the variable is uniformly distributed
({\em e.g.} over the set of field elements).  Thus the task of the
interface is easy, once it has determined which local variables have
already been fixed; it must simply choose the other local
variables according to the appropriate conditional distributions (fixed and
usually uniform).

There are many dependencies among the random variables describing the views
of the players and the adversary; therefore, we introduce a notation to
clarify the conditional distributions which the interface samples from when
interacting with the adversary.  The important point to note about each
variable is whether it is known ({\em i.e.} determined by a current view) or
hidden ({\em i.e.} unknown but distributed according to some known
distribution).
\begin{definition}
{\bf (Compromised Information)}
Let $T \subseteq [n] \cup \set{A},$ and let $\rho \leq r.$
A random variable $\rv(v_i,\rho)$
of player $i$ at round $\rho$ is
{\em compromised by $T$ at round $r$} 
if there exists a function $f$ such that $f(\view_T^r) = \psi(v_i,\rho).$
We write this as $\view_T^r \vdash \rv(v_i,\rho).$
\end{definition}
\fi

\subsection{Data Structures and Local Variables}
\label{sec-data-struct}

In order to examine the progressive states of each player and in order to
implement any of the protocols, we need to list explicitly the local
variables that make up each player's state.  The value of each variable is
a string representing a bit, a field element, or a message; if unassigned,
the value is $\Lambda.$  The local variables listed below are certainly
redundant to some degree:
\begin{itemize}
\item
$x_i,$ its input.
\item
$a_i,$ its auxiliary input.
\item
$y_i,$ its auxiliary input.
\item
$\randfield_i = (\rho_{i1},\rho_{i2},\ldots),$
an array of generic values, some of which may represent secretly shared
values ({\em e.g.} wire values), other public information ({\em e.g.}
publicly known constants and other information), and other information
necessary to the particular protocol ({\em e.g.} information used to verify
pieces). 
\item
$\randbits_i = (b_{i1},b_{i2},\ldots),$
an array of random bits.
\item
$\vec{s} = (s_1,s_2,\ldots),$
an array of known values, some of which may represent secrets and others of
which may represent information necessary to the protocol (such as
additional information used to verify pieces).
\item
$\pieces_i = (\piece_1(s_1),\ldots,\piece_n(s_1);
\piece_1(s_2),\ldots,\piece_n(s_2); \ldots),$
an array of the pieces of all the secrets.  Player $i$ will know either one
of the pieces or all of the pieces of each given secret.
\item
$\disqual_i = (d_1,d_2,\ldots,d_n),$
an array of disqualifications.  $\disqual_i[j]=1$ if player $i$ believes
player $j$ to be corrupt; otherwise it is 0.
\item
$\globdisqual_i = (g_1,g_2,\ldots,g_n),$
an array of global disqualifications.  $\globdisqual_i[j]=1$ if player $i$ 
believes all reliable players have disqualified player $j.$  (This should
have the same value among all reliable players.)
\item
$\mess([n],i,1..R),$ messages from other players.
\item
$\mess(i,[n],1..R),$ messages to other players.
\end{itemize}
A state $q_i$ is specified by the vector 
\begin{eqnarray*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& (x_i,a_i,\randfield_i,\randbits_i,\vec{s}_i,\pieces_i,\disqual_i,
\globdisqual_i, &  \\
& \mess([n],i,1..R),\mess(i,[n],1..R)). & 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{eqnarray*}
As in Chapter~\ref{chap-pre}, \S\ref{sec-exec-prot-adv}, we use these as
labels to parametrize distributions in more detail.  That is, instead of
considering simply the distribution $\rv(q_i,r)$ on the state of player $i$
at round $r,$ we consider the distribution $\rv(\piece_i(s_1),r)$ on the
value of player $i$'s local variable $\piece_i(s_1)$ at round $r,$ the
distribution $\rv(\piece_i(s_2),r)$ on the value of player $i$'s local
variable $\piece_i(s_2)$ at round $r,$ and so on. The collection of random
variables is parametrized by $r$ and the set $\rvnames'$ of variable names
obtained from $\rvnames$ by replacing each $q_i$ in $\rvnames$ by the
individual labels listed above.

Our goal is to specify the distributions $\rvAA$ describing variables for
$\VSS$ and the distributions $\rvASB$ describing variables for $\VSS$
induced by $\interface$ in the $\idealname(\share)$ protocol and to show
that they are equal.  Some are not sampled by $\interface,$ and we denote
unsampled variable values by $\rvASB(v,r)=\notsamp.$ 
Implicit in the operation of an interface is the specification that 
after each round of interaction with $A,$ $\interface$ sets
$\rvASB(v,r+1)=\rvASB(v,r)$ for each $v$ such that
$\rvASB(v,r) \not= \lambda.$

In each round we
describe corruptions and then rushed messages from $\tbar.$ After each
round of $\VSS,$ $\interface$ records messages from $A$ in
$\rvASB(\mess(T,\tbar,r),r)$ accordingly. 
We give arguments along the way that $\rvAA(v,r)=\rvASB(v,r)$ for
sampled variables.




\subsection{Proofs of Resilience}
\label{sec-prove-resil}

\subsubsection{Verifiable Secret Sharing}
\label{sec-prove-vss}

\begin{proofof}{Theorem~\ref{thm-bgw}}
We would like to show that $\VSS \resilasFa \idealname(\share) \resilasFa
\vacuous.$  First we construct an interface $\interface$ from $\VSS$ to
$\idealname(\share).$  For clarity we refer to player $i$ in $\VSS$ and
to player $i_{id}$ in $\idealname(\share).$

The $\idealname(\share)$ protocol allows the dealer, $D,$ to supply pieces
to the host, who distributes them if they are properly interpolatable, but
otherwise sends \cheating\  to all players.  The interface runs most of
$\VSS$ with $A$ before finishing the first round of $\idealname(\share).$

\medskip

\noindent{\bf Remark.}  The intuition that $A$ gains no information by
complaining and forcing $D$ to reveal pieces because $A$ knows them already
is formalized by $\interface$ having at a given stage in $\VSS$ set the
random variable $\rvASB(x,r)$ to some value that either has come from $A$
or has been generated by $S$ for $A$ in response to a corruption request.

\medskip

If $A$ corrupts $D$ before it supplies secret $s,$ $\interface$ requests
$D_{id}$ be corrupted and supplies $A$ with $s.$  If $A$ requests $i$ be
corrupted, $\interface$ corrupts $i_{id}$ and returns the auxiliary input.

(V1)  If $D$ is corrupt, $\interface$ does nothing but record the 
outgoing message of $A$ as $\rvASB(\mess(D,[n],1),1).$
Otherwise, 
$\interface$ chooses $\rvASB(\piece_i(s),1) \leftarrow \uniform(E)$ 
for all $i \in T,$ constructs 
\[
\{ p_i(u) \leftarrow \unifpolyn(n,t,\piece_i(s)) \}
\]
and 
\[
\{ q_i(v) \leftarrow \unifpolyn(n,t,0) \mid
(\forall j  \in T)  q_i(\omega^{j-1}) = p_j(\omega^{i-1}) \},
\]
and delivers these messages to $A.$  By Lemma~\ref{lem-ss-new},
the conditional distributions satisfy 
\[\rvASB(\mess(D,i,1;(p_i(u),q_i(v))),1) = 
\rvAA(\mess(D_{id},n+1,1;(p_i(u),q_i(v))),1).
\]


(V2)  If $A$ newly corrupts $D,$ $\interface$ corrupts $D_{id},$ sets
\[
\{ g(u) \leftarrow \unifpolyn(n,t,s) \mid
(\forall i \in T)  g(\omega^{i-1}) = \piece_i(s) \},
\]
%
sets for all $i \not\in T$
\[
\{ p_i(u) \leftarrow \unifpolyn(n,t,\piece_i(s)) \mid
(\forall j \in T)  p_i(\omega^{j-1}) = q_j(\omega^{i-1}) \},
\]
%
sets
\[
\{ h(v) \leftarrow \unifpolyn(n,t,s) \mid
(\forall i \in T)  h(\omega^{i-1}) = q_i(0) \},
\]
%
sets for all $i \not\in T$
\[
\{ q_i(v) \leftarrow \unifpolyn(n,t,h(\omega^{i-1}) \mid
(\forall j \in T)  p_i(\omega^{j-1}) = q_j(\omega^{i-1}) \},
\]
and sets $\rvASB(\mess(D,i,1),1) = (p_i(u),q_i(v))$ for all $i \in T.$
Interface $\interface$ sends $A$ the view of $D$ using $x_D,$ $a_D,$
$\rvASB(\mess(D,T,1),1).$  
%Interface $\interface$ corrupts $i_{id} \in T$ and
%returns their views, $x_i \circ a_i \circ \rvASB(\mu(D,i,1),1).$
By Lemma~\ref{lem-ss-new}
each of these distributions satisfies $\rvASB(x,1) = \rvAA(x,1)$
and is polynomial-time computable, being uniform over an easily computed set
of solutions determined by the conditions listed above.  This computation
in effect induces the variable $\rvASB(p(u,v),1) = \rvAA(p(u,v),1).$

If $A$ newly corrupts player $i$ we must consider whether $D$ is yet
corrupted.  If $D$ is corrupt, then all information held by $i$ is
known, in particular, $\rvASB(\mess(D,i,1),1).$
The interface corrupts $i_{id}$ to obtain $a_{id}$
(note that $x_{id}$ is nil)
and constructs $\view_i^1$ from these values.  
It then provides $A$ with the view.
If $D$ is not corrupt, then $\interface$ must construct the
$(p_i(u),q_i(v))$ message that $D$ sent to $i$ in round (V1).

To generate rushed messages from nonfaulty players, if $D$ is nonfaulty
then $\interface$ sets $\rvASB(\mess^{\broad}(i,[n],2),2) = 0$
for all $i \not\in T,$ since a nonfaulty player will accept the
proper (but private) message from a nonfaulty dealer.
If $D$ is faulty, then its messages to nonfaulty players are
determined by $\rvASB(\mess(D,[n],1),1),$ and $\interface$
sets $\rvASB(\mess^{\broad}(i,[n],2),2)$ to be $0$ if the
message to $i$ describes polynomials of degree $t,$ and $\interface$
sets the variable to $1$ otherwise.  Clearly this is the same
probabilistic computation $\delta_i$ that each nonfaulty player
applies in (V2).

(V3)
Now, if $A$ newly corrupts $i$ while $D$ is nonfaulty, $\interface$
generates $p_i(u)$ and $q_i(v)$ as in (V1), and returns them.  If $D$ is
already corrupt, $\interface$ uses $\rvASB(\mess(D,T,1),1)$ to determine
$p_i(u)$ and $q_i(u).$  

To generate messages from nonfaulty players, $\interface$ does the
following.  For each $i\not\in T$ and $j \in T,$  the $p_i(w^{j-1})$
values sent by nonfaulty players are determined already by the values
sent to corrupt players, so $\interface$
sets $\rvASB(\mess(i,j,2;p_i(\omega^{j-1})),2) =
\rvASB(\mess(D,j,1;p_i(\omega^{j-1})),1).$ 

(V4)  If $A$ newly corrupts $D,$ corrupt $D_{id}$ and construct
$\rvASB(\mess(D,T,1..2),1..2)$  as before.  If $A$ newly corrupts $i,$
$\interface$ creates an earlier view as in (V3) and must then construct
incoming messages about $p_k(\omega^{i-1})$ in round (V3).
For each $k \in T,$ check if $k$ sends $i$ a proper 
$p_k(\omega^{i-1})$ according to whether
$\rvASB(q_i(\omega^{k-1}),1) =
\rvASB(\mess(i,k,2;q_i(\omega^{k-1})),2).$
The former is fixed by previous computations of $\interface.$
Set $L(i,k)$ accordingly.
If $D$ is nonfaulty then set $L(i,k)=0$
for all $k \not in T,$ 
because all nonfaulty players send what $D$ sent them.
If $D$ is faulty but $k \not in T,$ use $\rvASB(\mess(D,k,1),1)$ and 
$\rvASB(\mess(D,i,1),1)$ to determine whether $i$ complains.  
This determines $\rvASB(L(i,k),2)$ for all $k,$ and $\interface$ supplies
it along with $a_i$ (obtained by corrupting $i_{id}$) to $A.$

To generate the broadcast messages from nonfaulty players, $\interface$
performs the same computation as the new corruption of $i$ just described.
It uses the vector $L(i,\cdot)$ as the broadcast value from $i\not\in T.$

(V5)
The view of a newly corrupt dealer includes that generated according to
(V4) along with the broadcast messages $\rvASB(\mess^{\broad}(T,[n],4),4)$
and $\rvASB(\mess^{\broad}(\tbar,[n],4),4)$ generated by $A$ and
$\interface$ in round (V4).  The view of a newly corrupted $i$ is generated
as in (V4), also attaching the list of broadcast messages.

If $D$ is nonfaulty, all disputes involve at least one faulty player $i,$
so $\interface$ has already specified in 
$\rvASB(\mu(D,i,1;p_i(\omega^{i-1}),1)$ the correct
value.  So $\interface$ sets $\rvASB(\mess(D,[n],4;p(i,j)),4)=
\rvASB(\mu(D,i,1;p_i(\omega^{i-1}),1).$   If $D$ is faulty, no messages
from nonfaulty players need be generated.

(V6)
New corruptions of $D$ or player $i$ are treated as in (V5), and
$\interface$ adds on the messages broadcast by $D$ in (V5), whether
generated by $\interface$ or by $A.$

If $D$ is nonfaulty, every player $i\not\in T$ does not impeach $D,$ so
$\rvASB(\mess^{\broad}(i,[n],6;M(i)),6) = 0.$  Otherwise it is easy for
$\interface$ to compute whether player $i\not\in T$ impeaches $D$
from the values of $\rvASB(\mu(D,i,1),1)$ and 
$\rvASB(\mu(D,[n],4),4),$ since these previous messages  from $D$ to $i$
have already been recorded (if not generated) by $\interface,$ and since
$\rvASB(\mu(D,i,1),1)=
\rvAA(\mu(D,i,1),1)$ and
$\rvASB(\mu(D,[n],4),4)=
\rvAA(\mu(D,[n],4),4).$

(V7)
New corruptions of $D$ or $i$ are treated as in (V6), adding the broadcast
impeachments from (V6) on the end of the views.

If $D$ is nonfaulty, impeachments come from faulty players only,
so $D$ will broadcast $(p_i(u),q_i(v))$ values that $\interface$
has already generated:
\begin{eqnarray*}
\rvASB(\mess^{\broad}(D,[n],7;M'(i)),7) & = &
\rvASB(\mess(D,i,1),7) \\
& = & \rvAA(\mess(D,i,1),7) \\
& = & \rvAA(\mess^{\broad}(D,[n],7;M'(i)),7) 
\end{eqnarray*}
For $i\not\in T,$ $D$ broadcasts $M'(i)=0,$ of course.  If $D$ is faulty,
$\interface$ simply records $\rvASB(\mess^{\broad}(D,[n],7),7)$
as generated by $A.$


(V8)
New corruptions are as in (V7), with the broadcast values 
$\rvASB(\mess^{\broad}(D,[n],7),7)$ concatenated at the end.

If player $i$ is nonfaulty, $\interface$ checks whether
$\rvASB(\mess^{\broad}(D,[n],6;M(i)),6)=0.$
If so, it sets $\rvASB(\mess^{\broad}(i,[n],8),8)=0.$
Otherwise, it checks whether, for all $j$ for which $D$
broadcasts $(p_j(u),q_j(v)),$ the values agree with $i$'s
value $p_j(\omega^{i-1})$ as derived accordingly from
$\rvASB(\mess(D,i,1),8)$ or 
$\rvASB(\mess^{\broad}(D,[n],5),8)$
or $\rvASB(\mess^{\broad}(D,[n],7),8),$
the choice depending on whether $i$ has complained before.
If so, $\interface$ sets $\rvASB(\mess^{\broad}(i,[n],8),8)=0,$
and otherwise sets it to $1.$

Finally, if $\rvASB(\globdisqual_i(D),8)=1$ for any $i\not\in T$
($\interface$ calculates this easily from 
$\rvASB^{\broad}(\tbar,[n],8),8)$), then $\interface$
requests that the corrupted dealer $D_{id}$ send
$\Lambda$ in the ideal protocol.
The trusted host will supply each player with the output,
$(0,\rej).$  Otherwise, if the dealer $D$ is corrupted,
$\interface$ requests that $D_{id}$ send the pieces
that were finally accepted by nonfaulty players, and fills out
the list with values for corrupted players $i_{id}$ that provide
a polynomial of degree $t.$  These corrupted players will receive
those values but their outputs are considered to be $\Lambda,$
as described in Chapter~\ref{chap-pre}.  The nonfaulty players
in $\idealname(\share)$ will output
$\rvAA(Y_i,8)=(\piece_i(s),\acc)=(p_i(0),\acc)=\rvASB(Y_i,8).$

This concludes the description of $\interface.$  We claim that for
every $r$ and every $v$ such that 
$\rvASB(v,r) \not= \lambda,$ 
$\rvASB(v,r) = \rvAA(v,r).$
At each step, $\interface$ samples new variables $\rvASB(v,r)$
as a probabilistic function (sometimes even deterministic,
as when reporting values already broadcast) $f$ of earlier samples.
Each time, $\interface$ uses either:
\begin{itemize}
\item
a previous output of $A;$
\item
uniform distributions based on Lemma~\ref{lem-ss-new};
\item
direct computation of a nonfaulty player on values already broadcast
or known by virtue of correct behavior of other nonfaulty players
({\em e.g.} nonfaulty players do not impeach other nonfaulty
players).
\end{itemize}

With the aid of Lemma~\ref{lem-ss-new} and broadcast channel properties,
it holds that
\[
\rvASB(v,r+1) = f(\rvASB(v_1,r),\ldots,\rvASB(v_K,r)) =
f(\rvAA(v_1,r),\ldots,\rvASB(v_K,r)) = \rvAA(v,r+1)
\]
for some $K.$  In particular, 
$\rvAA(\outfn(q_i),8) = \rvASB(\outfn(q_i),8)$ for all
$i$ and $\rvAA(q_A,8) = \rvASB(q_A,8),$ hence 
$\ensAAlpha\protoIn = 
\ensASBeta\protoIn.$
\end{proofof}

\iffalse
\subsubsection{Multiplication}
\label{sec-prove-mult}
\fi



\figstretch
\boxfig{
\noindent{\bf \VSS}$(s)$
\begin{tabbing}  
\hspace{0.3in} \= \hspace{0.7in} \= \hspace{0.4in} \= \hspace{0.4in}
\hspace{0.4in} \= \hspace{0.4in} \= \hspace{0.4in} \= \hspace{0.4in}
\kill
(V1)
\> Fix $E=E(m,n)$ and $\omega.$ \\
\> $(1 \leq i \leq n)$ \\
\> $D:$ 
\> $\{ p(u,v) \leftarrow \uniform( p \in E[u,v] \mid  p(0,0) = s,
p(u,v) = \sum_1^t \sum_1^t p_{ij} u^i v^j \}$ \\
\> $D \rightarrow i:$
\> $(p_i(u),q_i(v)) = (p(u,\omega^{i-1}), q(\omega^{i-1},v))$ \\
%%%%%%%%%%%
(V2)
\> $(1 \leq i \leq n)$ \\
\> $i \rightarrow [n]:$ 
\> \If degree $t$ \Then $0$ \Else $1.$ \\
%%%%%%%%%%%
(V3)
\> $(1 \leq i,j \leq n)$ \\
\> $i \rightarrow j:$ 
\> $p_i(\omega^{j-1})$ \\
%%%%%%%%%%%
(V4)
\> $(1 \leq i,j \leq n)$ \\
\> $i:$
\> $L(i,j) = \left\{
\begin{array}{ll}
0 & \mess(j,i,3;p_j(\omega^{i-1})) =  \mess(j,i,3;q_i(\omega^{j-1})) \\
1 & \mbox{ otherwise }
\end{array}
\right.$
\\
\> $i \rightarrow [n]:$ 
\> $(L(i,1),\ldots,L(i,n))$
\\
%%%%%%%%%%%
(V5)
\> $(1 \leq i \leq n)$ \\
\> $D:$ 
\> $L'(i) = \left\{
\begin{array}{ll}
0 & \mess(i,[n],4;L(i,j))=0 \\
p_i(\omega^{j-1}) & \mbox{ otherwise }
\end{array}
\right.$
\\
\> $D \rightarrow [n]:$ 
\> $(L'(1),\ldots,L'(n))$ \\
%%%%%%%%%%%
(V6)
\> $(1 \leq i \leq n)$ \\
\> $i:$ 
\> \If $(\exists j)$ $\mess^{\broad}(i,[n],4;L(i,j))=1$ \\
\>\> or  $\mess^{\broad}(j,[n],4;L(j,i))=1,$  \\
\>\> and $\mess^{\broad}(D,[n],5;p_i(\omega^{j-i})) \not= $ \\
\>\>\>\> $\mess(D,i,1; q_i(\omega^{i-1}))$ \\
\>\> \Then $M(i)=1$ \Else $M(i)=0.$ \\
\> $i \rightarrow [n]:$ 
\> $M(i)$
\\
%%%%%%%%%%%
(V7)
\> $(1 \leq i \leq n)$ \\
\> $D:$ 
\> $M'(i) = \left\{
\begin{array}{ll}
0 & \mess(i,[n],6;M(i))=0 \\
(p_i(u),q_i(v)) & \mbox{otherwise}
\end{array}
\right.$
\\
\> $D \rightarrow [n]:$
\> $(M'(1),\ldots,M'(n))$ \\
%%%%%%%%%%%
(V8)
\> $(1 \leq i \leq n)$ \\
\> $i:$ 
\> \If $\mess^{\broad}(i,[n],6];M(i)) = 0$ or \\
\>\>\> $\mess^{\broad}(D,[n],7];(p_i(u),q_i(v)))$ is consistent \\
\>\> \Then $\disqual_i(D)=0$  \Else $\disqual_i(D)=1.$ \\
\> $i \rightarrow [n]:$
\> $\disqual_i(D)$ \\
%%%%%%%%%%%
\> $(1 \leq i \leq n)$ \\
\> $i:$
\> \If $t+1$ players disqualified $D,$ \\
\>\> \Then set $\globdisqual_i(D)=1.$ \\
\>\>\If $\globdisqual_i(D)=1$ \\
\>\>\Then $Y_i=(0,\rej)$  \Else $Y_i=(p_i(0),\acc).$
%%%%%%%%%%%
\end{tabbing}
\caption{\label{fig-vss-bgw}
\index{\VSS}
Protocol for dealer to verifiably share secret $s.$  
See text for more details.  
}}
\figstretchend


==> def.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% def.tex                    Definitions for security and reliability.
%
%                            Copyright @1990  Donald Beaver.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{=======}
\typeout{def.tex}
\typeout{=======}

\chapter{Formal Definitions for Reliability and Security}
\label{chap-def}

\chapquote{
To think is to forget differences, generalize, make abstractions.  In
the teeming world of Funes, there were only details, almost immediate
in their presence.
}{
Jorges Luis Borges, {\em Funes the Memorious}}





The most striking problem with current definitions of security and
reliability, apart from their scarcity, is the {\em ad hoc} and
incremental nature in which they have developed.  Correctness and
privacy are naturally the most important goals of a reliable, secure
computation.  Their formal specifications, however, are more subtle than
their intuitive simplicity suggests.  Furthermore, even though protocols
for distributed system security have been designed with such intuitively
simple properties in mind, other equally desirable security properties
have since arisen, requiring each protocol to be reconsidered --- if not
redesigned --- in light of these new properties.  Definitions of
security have thus been clouded not only be unforeseen subtleties in the
precise formulation of very simple properties but by the confusing and
disharmonious set of overly detailed formalizations tailored differently
to each property.

We propose a new and concise definition of a property we call {\em
resilience} that captures at a single blow every desirable property of a
distributed protocol.  Not only is this new definition simple and broad
enough to avoid the pitfalls of previous approaches, it appears to
capture {\em a priori} all the natural properties one might imagine.
With such a unifying definition, we need design protocols and prove
their resilience only once; new and unforeseen properties are simply
new, previously unnoticed aspects of the single property of resilience.

In this chapter, we take a brief look at previous, {\em ad hoc}
approaches to formal definitions and discuss their difficulties and
insufficiencies.  We then introduce the most important tool of this
work: a means to compare the resilience --- namely the security and
reliability --- of two arbitrary protocols.  
By defining a specific, {\em ideal} protocol, we provide a
standard by which to measure the resilience of {\em any} protocol.  In
an ideal protocol, a trusted and incorruptible host receives all the
inputs and returns the correct outputs. Though such a situation cannot
be guaranteed in reality, its robustness is the absolute standard we
seek.  Our techniques and standards provide not only a concise way to
define and to understand security and reliability but also, as we shall
see in Chapter~\ref{chap-mod}, a concise and formal means to consider
protocol composition and modularity.

Our point is this: a protocol is not meant to compute $F$ while
satisfying a list of desirable properties; rather, {\em it must achieve
the same results, in a rigorous sense (see \S\ref{sec-resil}), as an 
{\em ideal} protocol in which a trusted host performs the computation.}
The ability to compare the results of two protocols is essential
to showing such a case is true.  This chapter addresses these two
new and crucial observations.

\section{Where {\em ad hoc} Definitions Fail}

Privacy and correctness are the most obvious properties required by
secure and reliable computations.  They are intuitively easy to
understand: a protocol reveals no unnecessary information if the view of
an adversary can be generated from the bounded information to which it
is entitled (inputs and auxiliary inputs of corrupted players).  A
protocol is correct if the output of each player is in fact the function
$F(x_1,\ldots,x_n)$ applied to the inputs.

At closer inspection, subtle problems appear.  Definitions of privacy
often concentrate too closely on the privacy of the inputs and make
little reference to other information that may be leaked.  (\cite{hab88}
is a notable exception; \cite{afk89} and \cite{bf90} introduce a
specific measure of information that is hidden or leaked for the related
problem of instance-hiding schemes.) It may not be the case that,
running one protocol after another, the second protocol preserves the
privacy of the information in the first.  Each protocol might hide its
own inputs but leak all the secret information of another protocol if
the definitions are not made carefully.  Since the protocols in the
literature usually happen to satisfy the stronger requirement that no
information except $F(x_1,\ldots,x_n)$ is leaked, this issue is
overlooked.  In order to compose protocols, however, a careful measure
of the information leaked by each subprotocol is necessary.

Even the definition of as obvious an idea as an {\em input} to a
protocol requires great care.  Defining inputs and outputs is a far more
sensitive task than the established study of single-processor
computations would suggest.  If a player is {\em supplied} with an
input, what happens if it behaves absolutely properly but as though it
received a different input? Does one define correctness with respect to
behavior or with respect to some ``actual'' input? What does ``actual''
mean in this case?

Often, rather than delve into the subtleties, researchers make particular
assumptions ({\em e.g.}, encryptions of every input are supplied to each
party, or every input is ``secretly shared'') in order to finesse the
issue.  The notion of {\em committal} to an input plays an important
part: after an initial stage (either all processors are supplied with
immutable encryptions of other processors' inputs, or the inputs are
validly shared), correctness can be defined with respect to the
committed inputs.  While such approaches are interesting as particular
methods to accomplish security goals, they are too specific to merit
approval as general definitions of security. 

Definitions for the related problem of Byzantine Agreement do not
suffice, since the goal of that problem is simply to agree on a common
value, a process that is fairly insensitive to individual variations in
a fraction of the input values, as opposed to determining a result that
may be extremely sensitive to individual inputs.  We must find a broader
means to understand and define correctness without resorting to such
specific aspects of the process as committal, which, although it turns
out to be a necessary implication of protocol resilience, is not the
primary focus.

Hindering us in our search for clean definitions is the problem of when
to stop looking for new properties.  Privacy and correctness were once
thought sufficient.  Other important properties have since become
evident.  For example, what if, in a secret ballot, one voter
were able to cast a vote opposite to that of another, through some
clever and malicious manipulation of messages in an intricate protocol,
even that corrupt player were not able to learn the vote that it
cast? A two-thirds majority could always be prevented by malicious
coalitions.  Or, for example, what if the system must generate a random
bit upon which some decision must be based? If malicious players can
choose their inputs depending on those of reliable players, then using
the parity of random bits supplied by each player will fail.  The
property of {\em independence of input selection} is immediately seen as
desirable, even though it is orthogonal to the properties of correctness
and privacy.  Beaver (\cite{bea88-n2}, see technical report)
gave a broad definition of
independence with respect to a broad ({\em i.e.} nonspecific and
general) committal function defined on transcripts of protocol
executions, but this early approach is unsatisfying for the reasons
noted above.  Notice that when players are computationally unbounded,
independence of inputs can be neatly formulated via independence of 
random variables describing inputs.  When players and adversaries are 
computationally bounded, however, subtle and difficult points arise: 
for example, a faulty player may use the {\em encrypted value} it sees
of another player's input as its own input, in which case the two inputs
are information-theoretically quite dependent, but formulating that they
are independent in some computational task is intricate and unclean.

Another example, occurring primarily in the domain of protocols
tolerating extremely high fault rates, is that of {\em fairness}.
Reliable players must not be prevented from learning their outputs of
the protocol if corrupted players are able to learn theirs.  That is,
even if an adversary is able to bring the whole computation to a halt
--- which, fortunately, is not an issue in protocols with a faulty
minority --- then it should not enjoy the fruits of the computation
while denying them to reliable participants.  In order to maintain
parity in the knowledge gained by adversary and by reliable players,
methods for gradual disclosure of the results are employed 
\cite{lmr83,cle86,yao86,ghy87}.
The two primary definitions for fairness are related to the algorithmic
solutions provided by their proponents.  Yao, and later Galil, Haber,
and Yung, allow the reliable players to run a recovery algorithm based
on the program used by the adversary, if a majority of players have
become faulty \cite{yao86,ghy87}.  Beaver and Goldwasser propose a
stronger definition in which the reliable players do not have access to
the program of the adversary, thereby allowing the adversary itself to
depend on the programs of the reliable players.  Further discussion can
be found in Chapter~\ref{chap-maj}, where protocols tolerating a faulty
majority are presented, and in \S\ref{sec-adhoc}, where we demonstrate
how our unified definition implies the current set of desired
properties.

Our definitions capture all of these properties in a concise and simple
manner by avoiding the {\em ad hoc}, divide-and-conquer approach.
The properties we have discussed are related to each other: they are
each aspects of an ideal protocol.  The ideal protocol and the notion
of relative resilience bind them together.

\section{Relative Resilience: Simulators and Interfaces}
\label{sec-rel-resil}

The key idea behind our approach is a means to compare one
protocol to another in terms of their security and reliability.  
We call the combination of security and reliability, {\em resilience.}
We measure not only the {\em information} gained by an
adversary during an execution of a protocol, but the {\em influence} it
has on the outputs.

This essential idea, unnoticed, was the source of many of the
inherent difficulties in previous approaches: even in an {\em ideal}
protocol, with a trusted host who computes results accurately, an
adversary has {\em some} influence over the outputs.  An adversary who
is not able to attack the trusted host is nevertheless able to choose
inputs that corrupted players will send to the host, thereby having some
limited but unavoidable effect on the computation.  Thus, we must
examine an attack not only with respect to what the adversary learns
(ideally, only the inputs and outputs of corrupted players), but with
respect to how the adversary affects the computation (ideally, only
through its choice of inputs for corrupted players).

Before delving into the nature of the {\em ideal} protocol that will
become our standard, we first investigate how to compare the resilience
of two arbitrary protocols.  The notion of privacy introduced by
Goldwasser, Micali, and Rivest \cite{gmr89} in the realm of
zero-knowledge proof systems and later applied to multiparty protocols
(\cf\  \cite{gmw87,hab88}) provides a springboard for the ultimate
definition of resilience. 

As described in \S\ref{sec-def-zk}, zero-knowledge proof systems make
use of a {\em simulator} to demonstrate that the conversation seen by a
corrupted verifier is in fact generable solely from the theorem, ``$x
\in L$.'' We phrase it in a more suggestive manner: the simulator
demonstrates that the conversation is generable solely from the
information (\ie\  ``$x \in L$'') that it would obtain in an ideal
situation (given a trusted oracle, \ie\   prover).  
In any general interactive protocol
execution, we would like to ensure that the adversary can simulate its
portion of the history of a protocol using only the information that it
is entitled to learn.  Galil, Haber, and Yung \cite{ghy89} utilize such a
generalization and make use of a {\em fault oracle} that supplies the
bounded information (inputs and outputs of corrupted players) to which
the adversary is entitled.  A simulator must, with that information,
generate an accurate view of the real protocol execution.  In
computationally bounded models, where the verifier has limited
resources, the simulator must also use such bounded resources, in order
to demonstrate not just that no extra {\em information} is leaked but
that no results that are {\em computationally infeasible} to generate
are leaked.

A related idea that avoids the computational orientation of simulation
says that the distribution on views seen by the adversary must be {\em
independent} of the reliable player's information, or more generally
that the distribution depends {\em only} on the final output and the
inputs of the corrupted players.  This sort of approach forms the basis
for the instance-hiding schemes of \cite{afk89,bf90}.  When the players
are not computationally bounded, defining privacy according to
independence of variables is often a cleaner approach (see Chapters
\ref{chap-pri},\ref{chap-ihs},\ref{chap-lrr}).  
In general, if a distribution is independent of certain
variables, then it can be simulated without the ``knowledge'' of the
values of those variables (though, of course, there is no {\em a priori}
guarantee that simulating the distribution is efficient).  With this in
mind, we shall adopt the simulation approach, since it also has the
advantage of covering computationally-bounded models.

But such definitions for privacy are not sufficient to analyze
the security and reliability of interactive
multiparty protocols.  
Simulation is essentially a passive approach: give the simulator
information, and let it create a view for the adversary.  
The {\em influence}
of an adversary on others is not taken into account. 

Let us consider two interactive multiparty protocols, $\protoa$ and
$\protob.$ Each has an associated class of allowable adversaries,
$\advclass_{\protoa}$ and $\advclass_{\protob}.$ To compare the
resilience of protocol $\protoa$ against an adversary $A \in
\advclass_{\protoa}$ to the resilience of protocol $\protob,$ we should
like to allow $A$ to wreak havoc on protocol $\protob.$ Unfortunately,
$\protoa$ and $\protob$ may be radically different protocols.  One might
have many more players than the other, one might disallow certain
players from being corrupted, one might be written in {\sc C}
while the other
is written in {\sc FORTRAN,} {\em etc}.  We cannot simply run protocol
$\protob$ with adversary $A.$

Instead, we surround $A$ by an {\em interface}, $\interface.$ 
The interface $\interface$
creates an environment for $A$ so that $A$ will believe it is
participating in protocol $\protoa.$ On the other hand, $\interface$ 
itself is
allowed to wreak havoc on protocol $\protob.$ In other words, the
combination $\interface(A,\cdot)$ with $A$ built into $\interface$ is
used itself as the
adversary to an execution of protocol $\protob.$ (The notation indicates
that $\interface$ has two communication lines, one of which is used to
communicate with $A,$ and the other of which is used as its adversarial
input/output line in a protocol execution.)  The combination 
$\interface(A,\cdot)$
must be a permissible adversary in $\advclass_{\protob}.$%
\footnote{Technically, there must be a machine in $\advclass_{\protob}$
with an identical input/output behavior as the single tape machine
$\interface(A,\cdot).$}

Consider, for example, the special case where protocol $\protob$ is the
particular and simple protocol in which an incorruptible host sends one
message (containing ``$x \in L$'') to the corruptible player.  An
adversary to protocol $\protob$ can obtain only this information (and
has no influence on the results, in this particular simple case).  An
interface $\interface$ receives this message and must present a proper
environment for $A.$ In this manner, the interaction corresponds to the
special case of zero-knowledge proof systems (see \S\ref{sec-zk-resil}),
and the interface is used only as a simulator.

In actuality, simulation is only half of its job.  We shall later
discuss how the interface covers all aspects of the definition of
zero-knowledge; first, let us examine how it captures all aspects
of multiparty security, including privacy and correctness.

\begin{definition}
\label{def-interface}
{\defstyle (Interface)} An {\defstyle interface}
$\interface(\cdot,\cdot)$ is a machine (interactive Turing machine
or general player)
with two communication lines; the first is
called an {\defstyle environment simulation}\index{environment
simulation line} line, and the second is called an {\defstyle
adversarial}\index{adversarial line} line.  
If $\protoa$ admits adversary class $\advclass_{\protoa}$ and
$\protob$ admits adversary class $\advclass_{\protob},$ we say
$\interface$ is an {\defstyle interface from} $\protoa$ 
{\defstyle to} $\protob$
if for every $A \in \advclass_{\protoa},$ 
$\interface(A,\cdot) \in \advclass_{\beta}.$
\end{definition}

We denote an interface by $\interface(\cdot,\cdot).$ When hooked up to an
adversary $A$ (with auxiliary input $a$) which itself is simply an
interactive machine having a single communication line, we consider the
combination $\interface(A(a),\cdot)$ as an adversary of its own right.  
As a unit, it has a single communication tape, namely the adversarial tape.
We treat $\interface(A(a),\cdot)$ as an adversary to $\beta$ 
simply by using the
corruption requests and corrupt messages 
$\interface$ writes on its adversarial line and by supplying $\interface$
with the requested messages and information held by corrupted players
in $\beta,$ as would normally happen in the execution of protocol $\beta$
with an adversary.

We should like to formalize the intuitive statement that adversary $A$
can wreak no more havoc on protocol $\protoa$ than it could on protocol
$\protob$ --- given an interface to translate its requests for
corruptions and specifications of corrupted messages.  If this is the
case, we shall say that $\protoa$ is {\em as resilient as} $\protob.$

In each protocol, every reliable player ends up in a state according to
some distribution.  We should like that the adversary's influence on the
state of reliable players is the same, whether it attacks $\protoa$ or
with help from an interface it attacks $\protob.$ The adversary itself
ends up in some state when it attacks protocol $\protoa;$ the
distribution on its final state should be the same whether it attacks
$\protoa$ or is fed the environment simulated by $\interface.$ (Recall
that an {\em attack} of an adversary is just a sequence of strings
including requests for states of newly corrupted players, messages to
replace those of corrupted players, the states of those players, and
messages sent by reliable players to corrupted players.  The states and
reliable messages are supplied either by the formal execution of
protocol $\protoa$ or by the computations of interface $\interface.$)
This says that the adversary gains no more information in $\protoa$ than
it would in protocol $\protob.$


Formally, let us consider the distributions $\ensAAlpha(n,m)\protoIn$
and $\ensASBeta(n,m)\protoIn.$ 
The former is induced by running protocol $\protoa$ with
adversary $A(a)$ and the given inputs and auxiliary inputs.  The latter
is induced by running protocol $\protob$ with adversary
$\interface(A(a),\cdot)$ and the same inputs and auxiliary inputs.
When $n,$ $m,$ $\vec{x},$ $\vec{a}$, and $a$ are allowed to vary,
we have two protocols that each induce an ensemble,
$\ensAAlpha$ and $\ensASBeta,$ respectively.
These two ensembles describe the final states of the players, reflecting
the {\em influence} of the adversary, and the final state of the
adversary, reflecting the {\em information} gained by the adversary. 

\begin{definition}
\label{def-rel-resil}
{\defstyle (Black-Box Auxiliary-Input Relative Resilience)}%
\index{resilience!relative}%
\index{resilience!relative!black-box auxiliary input}%
\index{$\resilasFa,$ relative resilience}
A protocol $\protoa$ is {\defstyle as
$(\advclass_{\protoa},\advclass_{\protob})$-resilient as} protocol
$\protob,$ written 
\[
\protoa
\resilasFa_{(\advclass_{\protoa},\advclass_{\protob})} 
\protob,
\]
if there exists an interface $\interface$ from $\protoa$ to $\protob$
such that for all adversaries $A \in \advclass_{\protoa},$
\[
\ensAAlpha
\indistFa
\ensASBeta
\]
\end{definition}
The subscript $(\advclass_{\protoa},\advclass_{\protob})$ is omitted
where clear from context.  We say the protocols are 
{\em exponentially}
($\resilasFaE$), {\em statistically} ($\resilasFaS$), or {\em
computationally} ($\resilasFaC$) relatively resilient according to how
indistinguishable the induced ensembles are.  It is clear that the use
of auxiliary inputs can be removed simply by omitting them from the
definitions, if one wishes to consider strictly uniform computations. 
To avoid potential confusion, we remark
that definition of indistinguishability already takes 
the inputs and auxiliary inputs into account:
for {\em every} $z,$ namely for every value of $n,$ $m,$ and $\protoInZ,$ 
the two sequences of
distributions induced by $\protoIn$ must approach each other
as $k$ gets large.  A trivial modification of the definitions
removes auxiliary inputs from consideration, which may be useful
if one wishes to consider strictly uniform computations with uniform
adversaries.  Auxiliary inputs, as mentioned, are useful for other
reasons, and we include them in our definition.

When $n$ and $m$ are fixed, we may compare two protocols in the same
manner: $\protoa(n,m)$ is as resilient as $\protob(n,m),$
written $\protoa(n,m) \resilas\index{$\resilas,$ relative resilience}
\protob(n,m),$
if there exists an interface $\interface$ such that
$\ensAAlpha(n,m) \indistEn \ensASBeta(n,m).$  The technical distinction
is that here we compare ensembles, whereas above we compare
families of ensembles.


The study of zero-knowledge often considers a weaker form of simulation
in which there need not be a universal simulator $\interface$ but rather
there need only be a specific simulator $\interface_A$ for each
adversary $A.$ The simulator can depend on the internal structure of the
adversary.  For completeness, we give the analogous definition for
resilience, considering an interface $\interface_A$ that acts as an
adversary to protocol $\protob$ in the same way $\interface(A,\cdot)$ did
previously.  We shall not consider this definition further.
%
\begin{definition}
\label{def-rel-resil-weak}
{\defstyle (Weak Auxiliary-Input Relative Resilience)}%
\index{resilience!relative!weak} 
A protocol $\protoa$ is
{\defstyle weakly as
$(\advclass_{\protoa},\advclass_{\protob})$-resilient as} protocol
$\protob,$ if for any adversary $A \in \advclass_{\protoa},$ there
exists an interface $\interface_A$ from $\protoa$ to $\protob$
such that
\[
\ensAAlpha
\indistFa
\ensASBeta
\]
\end{definition}
%

%These definitions, concise as they are, will be more concrete once we
%specify a particular protocol $\protob$ with respect to which we measure
%resilience on an absolute scale.  Figure~\ref{fig-scenario} gives a more
%explicit description for the case in which protocol $\protob$ has an
% incorruptible, trusted host; the details will be made clear in
%\S\ref{sec-resil}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Ideal Interaction With a Trusted Host}
\label{sec-trusted-host}

Given a means to compare the resilience of protocols, we come now to 
the other important half of the approach we propound:
{\em a secure and reliable protocol must achieve the same results as 
an {\em ideal} protocol 
in which a trusted host performs the computation.}  

Chapter~\ref{chap-pre} describes the mechanics of a general protocol,
whether generic or attacked by an adversary.  A {\em real} protocol is one
having a fault class consisting of arbitrary subsets of up to $t$ players,
and having some arbitrary set of communication channels.  For example, a real
protocol may provide broadcast channels and private channels between each
pair of players.  The essential point is that no player need be 
incorruptible.

An {\em ideal} protocol, on the other hand, provides an absolutely
reliable and secure trusted host, 
even though in the ``real'' world, it is neither prudent nor efficient to
rely upon such an immensely vulnerable, centralized situation.
Computation with a trusted host must nevertheless
take into account the presence of an adversary.  
In the ideal case, however, the limited powers of the adversary are
more clearly delineated than among the intricacies of a complex protocol,
giving a convincing justification for claims of absolute security and
reliability.

Figure~\ref{fig-exec-ideal} describes the {\em ideal protocol} for $F.$ The
participants are the usual $n$ players along with a central, trusted host,
player $(n+1).$ Each player has a private communication line to
player~$(n+1),$ so we need not consider information leaked implicitly
through interaction among the players.


\figstretch
\boxfig{
\noindent{\bf \protostyle Ideal-Protocol} $\protoId$%
\begin{tabbing} \standtabs
%%%%%%%%%%%%%%%%%%
(I1) \>
\parbox[t]{4.6in}{
Each player $i$ ($1 \leq i \leq n$) starts with input and auxiliary input
$(x_i,a_i).$  Player $(n+1),$ the trusted host, has no input.
Each player $i$ sends $x_i$ to player $(n+1),$ for $1 \leq i \leq n.$
}
\\
(I2) \>
\parbox[t]{4.6in}{
Player $(n+1)$ sets $x_i^{\star}=\Lambda$ for any messages not falling in the
domain $X_i$ and sets $x_i^{\star}$ to the message from player $i$ otherwise.
It computes the sample
$(y_1,\dots,y_n) \leftarrow F(x_1^{\star},\dots,x_n^{\star}).$
(Without loss of generality assume that $F$ is defined on input $\Lambda.$)
Player $(n+1)$ sends $y_i$ to player $i$ for $1 \leq i \leq n.$
}
\end{tabbing}
\caption{\label{fig-exec-ideal}
\index{ideal protocol}%
\index{protocol!ideal}%
\index{$<\idf>$!ideal protocol}
Ideal computation with a trusted host and reliable parties.
}}
\figstretchend

When an adversary is allowed to attack the ideal protocol, its powers are
strictly limited to learning and influencing the inputs of players in the
range $\set{1,\dots,n};$ player~$(n+1)$ is immune to corruption.  That is,
the {\em ideal-$t$-fault-class} $\idealfclass$ consists of all subsets of
$\set{1,\dots,n}$ of size $t$ or less.  The {\em ideal-$t$-adversary class}
$\idealaclass$ consists of all adversaries that only request coalitions in
the ideal $t$-fault class.  For the purposes of discussing
complexity-based security, in which adversaries and players are assumed to
perform probabilistic polynomial-time computations, we may restrict this
class to computationally-bounded adversaries.  In that case, the adversary
must not only request coalitions strictly in the specified fault class, but
it must be a polynomial time Turing machine as well.

The execution of the ideal protocol in the presence of a dynamic, Byzantine 
adversary is described informally
in Figure~\ref{fig-ex-ia}.  
The formal specifications of the distributions and histories obtained in this
interaction should be clear from the definitions given in 
Chapter~\ref{chap-pre}.  
The interactions in the presence of a weaker adversary,
such as a passive or static one, should also be clear.
Notice that a dynamic adversary may base its
choice of players to corrupt on information gained from previously
corrupted players in an adaptive fashion.  
It may also choose to corrupt more players after $F$ has been computed.  


The idea of committal to inputs corresponds to the end of round 1: each
player has sent its input to the host, and the computation of $F$ has not
yet begun.  A special protocol that is useful in formally capturing ideas
of commitment and privacy is the 
{\em ideal vacuous protocol}, $\vacuous,$%
\index{vacuous protocol}%
\index{protocol!ideal vacuous}%
\index{$\vacuous,$vacuous protocol}
which is the ideal protocol in which each player must supply a 0 input; the
trusted host returns a string of $n$ bits, each of which is 0 if the
corresponding player supplied a 0 and is 1 otherwise.  Essentially, no
information besides the identities of the cheating parties is returned.

\figstretch
\boxfig{
\noindent {\bf \protostyle Ideal-Protocol-With-Adversary} 
$\protoAId$
\begin{tabbing} \standtabs
%%%%%%%%%%%%%%%%%%
(IA1) \>
\parbox[t]{4.6in}{
\begin{itemize}
\item
Each player $i$ ($1 \leq i \leq n$) starts with input and auxiliary input
$(x_i,a_i).$  Player $(n+1),$ the trusted host, has no input.
\item
The adversary computes and chooses an allowable subset $T \subseteq
\set{1,\dots,n}$ of players to ``corrupt.''  (The trusted host 
is {\em not} included in the class of allowable faults.)  It obtains the
inputs $(\vec{x}_T,\vec{a}_T)$ of those players, and nothing else.  A
dynamic adversary may repeat this step as often as it pleases (modulo
resource bounds, and modulo the requirement that new coalitions contain old
ones).
\item
The adversary chooses an alternate set of effective inputs $x_i'$
for the members of coalition $T,$ and sends them to the trusted host.
\item
Every uncorrupted player sends its input $x_i$ to the trusted host.
\end{itemize}
} \\
%%%%%%%%%%%%%%%%%%
(IA2) \>
\parbox[t]{4.6in}{
\begin{itemize}
\item
The trusted host sets $x_i^{\star}$ to be $\Lambda$ for each $i$ from
which it received a message out of range, and otherwise sets $x_i^{\star}$
to be the message it received.
The trusted host samples 
$(y_1,\dots,y_n) \leftarrow F(x_1^{\star},\dots,x_n^{\star}),$
where $x_i^{\star}$ is either $x_i,$ $\Lambda,$ or a corrupted but possible
input choice.
\item
The trusted host sends $y_i$ to player $i$ for each $i.$  The adversary
thereby receives outputs $\vec{y}_T.$
\item
The adversary may choose more players to corrupt, obtaining their inputs
$(x_i,a_i)$ and their output values $y_i,$ with the same restrictions on
coalitions as before.
\end{itemize}
}
%%%%%%%%%%%%%%%%%%
\end{tabbing}
\caption{ \label{fig-ex-ia}
\index{ideal protocol!with adversary}%
\index{protocol!ideal!with adversary}%
\index{$<A,\interface,\idf>$!ideal protocol with adversary}
Ideal computation with 
a trusted host, dynamic malicious adversary, and reliable parties.  
This protocol requires two rounds.  %Compare Figure~\ref{fig-exec-byz}.
}}
\figstretchend


\section{Resilience: The Unified Theory}
\label{sec-resil}

The groundwork is laid for the concise and precise definition
of security and fault-tolerance for multiparty computations.
Using the concept of {\em relative resilience} and using the ideal
protocol as a standard:

\begin{definition}
\label{def-resil}
\index{resilience}
{\defstyle (Resilience)}
A protocol $\protoname$ with fault class $\faultclass$ is 
{\defstyle $\faultclass$-resilient leaking $F$} if
\[
\protoname 
\hspace{0.1in} 
\resilasFa_{(\faultclass,\idealaclass)}
\hspace{0.1in} 
\idealname(\computef).
\]
\end{definition}

We say {\em exponentially, statistically,} or {\em computationally}
if $\resilasFaE,$ $\resilasFaS,$ or $\resilasFaC$ holds, respectively.


\subsection{Three Scenarios: A Summary}

The diagram in Figure~\ref{fig-scenario} illustrates the three scenarios
of key importance.  The first represents the ideal world, in which a
trusted and reliable host is available and ensures that the adversary is
truly restricted to gaining only the inputs and outputs of players of
its choice.  The third represents the real world, in which no player can
be trusted but a protocol must be designed to perform the same
computations as in the ideal world, correctly and privately.  The second
and intermediate scenario joins the two, modelling the interaction
in an ideal protocol attacked by a real adversary that is assisted by an
interface.  Allowed to attack the ideal protocol as best
it may, the information and influence of the adversary is clearly
delineated in this central case.  It connects the clear measurements of
security and reliability in the ideal case to the less easily understood
powers of the adversary in the real world.


\begin{figure}
  \setlength{\unitlength}{1in}
    \begin{picture}(5.5,5.8)(1.3,2.8)
%    \special{psfile=three.ps}  % drb2020
        \includegraphics{three.pdf}  % drb2020
    \end{picture}
  \setlength{\unitlength}{0.0125in}
\caption{ \label{fig-scenario}
Three scenarios:  first, an ideal protocol with a trusted host, clearly
delineating the limited information and influence of an adversary;
second, an adversary attacking a trusted host by way of an interface
that creates a simulated environment for it; third, an adversary attacking
a real protocol with no trusted parties.
Squares and circles indicate players; squares within
the interface are simulated players.  
The {\bf X} marks indicate corrupted players.  
}
\end{figure}

\subsection{Zero-Knowledge at One Blow}
\label{sec-zk-resil}


Resilience captures all aspects of zero-knowledge proof systems, 
not just privacy, in a concise way.  Consider a zero-knowledge proof
system as a two-party protocol in which any number of players
may be corrupted.  The {\em ideal} protocol provides a trusted host.
The prover tells the trusted host, ``$x \in L,$'' for some $x \in L,$
or declines to participate by sending some other message.  The host
simply sends ``$x\in L$'' or ``\cheating'' to the verifier, accordingly.

It is clear that the most an adversary can do is to cause the prover
detectably to cheat without convincing the verifier, or to gain
at most the information that the verifier learns, which in this case
amounts only to ``$x\in L$.''  Separately, these possibilities
correspond to soundness and to privacy.  Resilience unifies them.

The ideal protocol, denoted
$\idealname(F_L)=\anglebrack{P_L,V_L},$ computes the function
$F_L$ defined by
\[
F_L(p, 0) = 
\left\{
\begin{tabular}{cl}
``$x \in L$'' &
if
$p = \mbox{ ``$x \in L$''}$ and 
$x \in L$ \\
``\cheating'' &
otherwise
\end{tabular}
\right.
\]

\begin{theorem}
\label{thm-zk-is-resil}
$\anglebrack{P,V}$ is a (statistical, computational) 
zero-knowledge proof system for $L$
if and only if it is a (statistically, computationally)
 $2$-resilient protocol for $F_L.$
\end{theorem}

\begin{proof}
If $\anglebrack{P,V}$ is a zero-knowledge proof system for L, then
there exists a black-box simulator $S_{PV}.$  
Construct an interface $\interface$
that does the following.  Do nothing until adversary $A$ requests a
corruption.  If $A$ corrupts $V,$ request corruption of $V_L$ in
protocol $\idealname(F_L),$ and obtain $V_L$'s output, ``$x \in L.$''
Adversary $A$ may have waited until some later round $r$ to request
a corruption, so, by internally simulating $V$ and running the
simulator $S_{PV}(x)$ to generate a transcript, create a history of
the protocol through round $r.$  Note that the output of the simulator
is accurate for a proof system with no cheating ({\em i.e.} only passive
corruption) and with $x\in L.$  Therefore the prefix is accurate.
Now, supply $A$ with the current state of internally simulated
$V,$ and run $S_{PV}(x)$ to the end, with access to $A$ as the corrupt
verifier.%
\footnote{Weak zero-knowledge, in which the simulator is not
restricted to unresettable, black-box use of $V,$ corresponds to
weak resilience.  The interface $\interface$ simply awaits the
output of such a simulator and then uses it as its own output.}

If $A$ corrupts $P,$ then $\interface$
corrupts $P_L.$  The interface $\int$ operates $V$ internally%
\footnote{$V$ is polynomial time and its tapes are public.}
carrying on a correspondence with $A$ as the prover.  At the
end of the process, the internal $V$ either accepts some $x\in L$
or rejects.  If $V$ accepts, $\interface$ requires the corrupt
$P_L$ to send ``$x \in L$'' in the ideal protocol;
the host will approve and $V_L$ will accept.
If $V$ rejects, $\interface$ requires the corrupt $P_L$ to
send $\Lambda$ in the ideal protocol; the host and $V_L$ reject.
In either case the final outputs of the uncorrupted players,
$V$ and $V_L,$ are identical.
The adversary $A$ receives a view of an interaction with an
honest verifier.

Finally, if at some point $A$ corrupts both $P$ and $V,$
$\interface$ stops interacting with $A,$
since there are no nonfaulty outputs and no more nonfaulty players to
corrupt or to receive messages from.

Now, if $\anglebrack{P,V}$ is statistically
2-resilient, then for some interface
$\interface,$
\[
[P,V] \indistFaS [\interface(A),P_L,V_L].
\]
Hence for any adversary that corrupts $V,$
\[
[P,V]^{Y_A} \indistFaS  [\interface(A),P_L,V_L]^{Y_A}
\]
so $\anglebrack{P,V}$ is statistically $t$-private,
and for any adversary that corrupts $P,$
\[
[P,V]^{Y_V} \indistFaS  [\interface(A),P_L,V_L]^{Y_V}
\]
so with asymptotically high probability, an honest $V$'s output
is 1 when $x \in L$ and 0 otherwise.
\end{proof}


\section{Fault Oracles}

An intermediate approach pursued by Beaver \cite{bea89-def} and
independently by Kilian, Micali, and Rogaway \cite{kmr90}
uses the idea of a fault-oracle that provides limited information
from which to construct a simulated view for an adversary.
Fault-oracles are a natural extension of zero-knowledge.  Galil,
Haber, and Yung \cite{ghy89} proposed a function-oracle for the
case of two-party minimum knowledge {\em decision} proof systems,
in which the prover proves either $x \in L$ or $x \not\in L.$
Because the verifier should receive the result of a {\em decision}
about membership in $L$ in addition to a proof, the simulator
that produces its view ought to receive exactly that much information.
Thus, the simulator is allowed a single query to an oracle that computes
the characteristic function for $L.$

To define multiparty {\em privacy}, Beaver \cite{bea89-def} and Rogaway
\cite{rog89} extended the function-oracle to a fault-oracle.
Some additional requirements are needed, since the powers of
an adversary in a protocol are more diverse.  
\todoMaybe
%Figure~\ref{fig-fault-oracle}
%describes the queries a $t$-fault-oracle $\foracle$ for $F$ permits.
\todoMaybeEnd
Essentially, the simulator having access to $\foracle$ is allowed
to request inputs of up to $t$ players and to substitute its own.
Then it receives from $\foracle$ a single computation of $F$ using
the unrevealed inputs of uncorrupted players.  In Beaver's model,
it is also allowed to request more corruptions (up to a total of
$t,$ and obtaining inputs and outputs) after the computation,
since a dynamic adversary does have the option of doing so
after a normal protocol.

As with zero-knowledge, leaked information is bounded by the amount
of information a simulator needs to construct an accurate view of
a real protocol execution.

A key step, noted independently by Beaver and by Kilian, Micali,
and Rogaway, is that the computation of $F$ 
{\em induces output values} $F_i(x_1,\ldots,x_n)$ {\em for nonfaulty
players,} even though these values are not returned.  Correctness can
thus be defined to hold when these induced outputs match those in 
the real protocol, for then, since the induced outputs are correct,
so must the real ones be.

The definition of security becomes one of matching simulated to real
adversarial views, and matching induced to real nonfaulty outputs.
It is remarkably more concise and comprehensible than earlier approaches.  
Unfortunately, the
definition is not overly flexible.  For example, the concatenation of
two secure protocols may correspond to two fault-oracle queries,
but to prove the concatenation secure, one either allows only one
query or must redefine security and the fault oracle.

The essential step that was not previously observed was that the oracle
is far better regarded as a trusted host actually participating in
a protocol.  This observation paves the way for developing a general
concept of protocol comparison.  It serves as the basis to our approach.
The definition of {\em relative resilience} is as
concise, if not more so, as the definition of a fault oracle
and of security with respect to a fault oracle.
The fault oracle, even though a key stage in the development of 
good definitions, is a very limited and inflexible
application of a very broad and powerful concept.




\section{Satisfying the {\em ad hoc} Properties}
\label{sec-adhoc}

The important properties of the trusted host are several.  First, the
trusted host ensures that the inputs are not revealed, apart from
information leaked solely from the output of the function itself.  Second,
it returns a correct set of values based on the inputs it has received.
Third, because it waits until all inputs are received (privately) before
evaluating the function, it ensures that faulty or maliciously chosen
inputs do not depend on the choices made by reliable players.  Finally,
every player is assured of receiving its respective output, and fairness is
achieved.

We claim that the ideal case captures {\em a priori} 
all desirable properties that are as yet unconsidered; that is,
it declares precisely what needs to be accomplished by a secure protocol
and it specifies how malicious influences must be limited.  New properties
that one might like to consider reflect a deeper understanding of the ideal
protocol as opposed to a change in the model and in the idea of security.


We can analyze the {\em ad hoc} list of individual properties as aspects
of our definition of resilience.  {\em Correctness} addresses the
accuracy of the results computed by reliable players; {\em privacy}
addresses what results the adversary can compute based on what he sees.
\begin{definition}
{\defstyle (Correctness and Privacy)}
\begin{itemize}
\item
A protocol $\protoa$ is {\defstyle $t$-correct leaking $F$} if 
there exists an interface $\interface$ such that
\[
\ensAPi^{\vec{Y}}
\indistFa
\ensASId^{\vec{Y}}.
\]
\item
Protocol $\realpf$ is {\defstyle $t$-private leaking $F$} if 
there exists an interface $\interface$ such that
\[
\ensAPi^{Y_A}
\indistFa
\ensASId^{Y_A}.
\]
\end{itemize}
\end{definition}

{\em Independence of inputs,} a more tricky property to define formally,
is also captured by the ideal case.  In the ideal case there is
absolutely no interaction among players; the choice of input by a faulty
player is completely independent of messages sent by reliable players to
the trusted host, since those messages are carried on private channels.
Since the adversary cannot capture a reliable player's input or be
influenced by it in the ideal case without deciding to corrupt that
player, its choice of inputs is the same regardless of the information
held by reliable players.  Resilience implies that the adversary's
behavior and hence its choice of inputs is the same in real and ideal
cases, so the faulty inputs are not influenced by the reliable ones.%
\footnote{One could certainly make a weaker statement that if the outputs
of nonfaulty players have the same distribution in the real and ideal
cases, then even if the adversary's choice of {\em inputs} depends on
nonfaulty player's inputs, the final effect amounts to nothing.  But
because the {\em adversary's} view, containing the choice of inputs,
must be identical in both cases, we need not weaken the claim.}

Our definition implies {\em fairness,} and in fact an even stronger
property: not only do all reliable players obtain their results whenever
the faulty players do, they obtain them regardless of the faulty players'
behavior.

Yao \cite{yao86} and Beaver and Goldwasser \cite{bg89} (presented in
Chapter~\ref{chap-maj}) examine protocols where $t \geq n/2.$ In this
scenario, it is impossible for reliable players to force a computation
to finish.  It is impossible to achieve resilience.  But it may be
possible to ensure correctness and privacy if a computation is not
halted.  The issue of {\em fairness} has more meaning here.  What if
some players should learn the results while others do not?

Whereas perfect fairness is impossible, \cite{bg89} use a weaker
property to attain an approximation to fairness.  The weaker property
states that, if any reliable player fails to obtain an output, then all
reliable players detect cheating.  With cryptographic assumptions or
given a network supporting oblivious transfer, \cite{bg89} showed that
misbehaving players can be identified.  While this doesn't prevent
other faulty players from changing their inputs if the protocol were to
be run a second time after detecting some faults, it is a useful outcome
(especially in a litigious society).  Hence we may extend the output to
be a vector of values or a value $(T,\cheating)$ which states that
coalition $T$ was agreed by all reliable players to be cheating.

An approximation to fairness based on the ability to detect cheating is
attainable \cite{bg89}.  If cheating does not occur, then all players
can progress slowly but equally toward knowing their output.
Nevertheless, defining this approximation is still tricky, since it is
not clear what an {\em ideal} protocol would achieve.  A rough sketch is
as follows.  A trusted party would accept inputs and compute the
function.  It would then take several rounds to reveal the results
gradually.  Intuitively, the odds of each player to know its result
$y_i$ after each round must advance in lock-step.  A more precise
treatment of this concept appears in Chapter~\ref{chap-maj}.



\section{Strong Security: Solving a Subtle Error}
\label{sec-strong-sec}

A simple yet subtle bug exists in all known multiparty protocols.
If the $t$ corrupted players send all their information to a single
reliable player $i,$ then that player now knows {\em every} input.
For example, protocols based on secret sharing ({\em cf.}
\cite{sha79,gmw87,bgw88,ccd88}) have the property that the information held
by any $t+1$ players determines all the inputs.  Therefore if $t$ players
give up their information to player $i,$ player $i$ knows everything.  One
way to circumvent this is to say that player $i$ is ``reliable'' and hence
``ignores'' improper messages.  What reliable person would believe what the
adversary says, anyway?  An honest-but-curious player (one who behaves in
terms of messages but may try to determine additional information) may be
tempted to gamble that the adversary is telling the truth in leaking
information, and may benefit from improper extra knowledge if the adversary
is indeed leaking information.

But this sort of philosophizing is far from formal.  If the information
arrives at a node, the bottom line is that it should not be there.
More formally, the set of messages given to the honest-but-curious player $i$
ought to be simulatable from the knowledge held by player $i$ and the
adversary; the inputs of other uncorrupted players should not be
compromised, and hence should not be needed to simulate the conversations
seen by player $i.$

We may consider this as an example of the following situation: in addition
to the malicious adversary $A,$ there are one or more passive adversaries
$B_1,B_2,\ldots$ A passive adversary $B,$ like the Byzantine adversary $A,$
is an automaton which requests states of players, but which does not
replace messages from those players.  Each reliable player is a fixed
passive adversary with access only to its own communications.  We would
like the protocol to be secure simultaneously against $A$ and at least
against such passive adversaries.

We address this {\em formally} in the following manner.  Denote 
the distribution on {\em all} output strings and views by
\begin{eqnarray*}
[A,B,\protoname]^{hist}
(n,m)
(\vec{x} \circ \vec{a} \circ a \circ a_B,k)
 & = & \\
(Y_A,Y_B,Y_1,\ldots,Y_n,
\view_A,\view_B,\view_1,\ldots,\view_n).
 & &
\end{eqnarray*}  
Here, $a_B$ is the auxiliary input of the passive adversary $B.$

We extend the interface $\interface$ to have a 
third communication tape, to
interact with a (black-box) passive adversary $B.$ As before, consider
an execution of the {\em ideal} protocol with $\interface$ acting as the
Byzantine adversary.  We also allow $\interface$ to corrupt
a second set of players passively, 
just as B would.  The number of additional players that $\interface$
can passively compromise is bounded by $t_B,$ the bound on the number of
players that $B$ could corrupt in a real protocol.  (We would at least
like to ensure security for $t_B=1,$ corresponding to a single
honest-but-curious player.)

Let 
$[A,B,\interface,\idealname]^{hist}(n,m)
(\vec{x} \circ \vec{a} \circ a \circ a_B,k)$
denote the distribution on outputs and views during an ideal
protocol execution with $\interface$ playing the part of the adversary,
allowing $\interface$ to request $(t+t_B)$ inputs.  

We define the ensemble families 
$[A,B,\protoname]$ and
$[A,B,\interface,\idealname]$ as subsets of
the random variables, namely just the $Y$ variables in 
$[A,B,\protoname]^{hist}$ and
$[A,B,\interface,\idealname]^{hist}$
as earlier.
Then the more careful notion of security is the following:
\begin{definition}  \label{def-resil-simult}
Protocol $\realpf$ is {\defstyle strongly $t$-resilient leaking $F$ }
if there exists an interface $\interface$
such that for any Byzantine $t$-adversary $A,$ 
for any passive $1$-adversary $B,$
%the ensembles
\[
[A,B,\protoname]
\indistFa
[A,B,\interface,\idealname]
\]
\end{definition}


We remark that similar modifications apply to the case of {\em relative}
resilience, though we shall not occupy additional space with them.
Auxiliary inputs can, as before, be excluded if so desired.



==> end.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% end.tex                    Conclusions, Final Chapter.
%
%                            Copyright @1989  Donald Beaver.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{=======}
\typeout{end.tex}
\typeout{=======}

\chapter{Conclusions}        \label{chap-end}

\chapquote{
Forsan et haec olim meminisse iuvabit.
\footnote{Perhaps this will be a pleasure to look back on one day.}
}{
Virgil, the {\em Aeneid}}

The issues of this dissertation are three-fold.  First, reliability and
security are best ensured by avoiding assumptions that particular
processors are reliable.  Second, proving the security and reliability of
distributed protocols requires clear and concise definitions.  Our
definition of resilience captures security and reliability simultaneously
and {\em a priori} captures all the intuitive properties one expects of a
robust system.  Third, theoretical protocols are interesting, but to be
practical a higher standard of efficiency must be met.  Protocols requiring
more than a dozen rounds of interaction are likely to be too complex or too
inefficient to be implementable; low communication complexity is of utmost
importance.

In general, we have made some strong simplifying assumptions, such as the
presence of a complete, synchronous network with private channels.  These
issues are of deep practical and theoretical significance, but we place
them aside in the hope that a modular approach provides a deeper
understanding of the fundamental nature of security and reliability in
interactive protocols.  Chapter~\ref{chap-app} (\S\ref{sec-strong-ass})
discusses the incorporation of solutions for underlying network problems.
The robustness of our protocols against message omissions and fail-stop
faults suggests a cautious optimism that, with appropriate formal proofs,
they can be provided with modular subroutines to withstand a weakening of
the simplifying assumptions.

The understanding of security and reliability has been hampered by a lack
of formal proofs and definitions.  Much current research develops
techniques that are intuitively secure but which have not been proven
secure.  We provide a definition for resilience that solidifies the
foundations of research into security.  
Precise definitions of standard properties such as correctness and privacy
fall out as an easy consequence.  We believe that all the desirable
properties of security and reliability are captured {\em a priori} by
considering the {\em ideal} protocol as our standard of computational
resilience.  Privacy, correctness, and other properties are aspects of the
same definition, tied together by the idea of an ideal, trusted party,
and measurable by the idea of relative resilience.

Our definition for resilience provides not just a means to rate the
security of a protocol with respect to an {\em ideal} situation but a means
to compare arbitrary protocols.  The ability to measure relative resilience
provides a greater flexibility and modularity in proof techniques and
protocol design.  Rather than directly prove a protocol is secure, one can
compare it to an intermediate protocol that is itself proven secure.
Relative resilience also provides a conceptually easier means to show when
protocol concatenation preserves the security of the protocols, a very
important issue that is often difficult to analyze.

It remains to be seen if unconditional security, high fault-tolerance,
highly complex function computation, and low communication complexity can
be achieved simultaneously.  For functions of arbitrarily high complexity,
the locally random reductions of Chapter~\ref{chap-mpp} provide low
communication complexity, but at a cost of lower ($O(\log n)$) fault
tolerance.  Chapter~\ref{chap-ccr} achieves low communication complexity
and high fault-tolerance, but the results are conditioned on the existence
of a one-way function.  If the computational complexity of the function is
restricted, Chapter~\ref{chap-con} demonstrates that
low communication complexity and low local computational
complexity are simultaneously achievable.

Locally random reductions with better parameters --- {\em i.e.} a higher
ratio of the independence-set size $k$ to the number $m$ of queries --- are
one path to achieving higher fault-tolerance for arbitrarily complex
functions while using a constant number of rounds.  A characterization of
the achievable parameters for locally random reductions would be of general
interest beyond serving simply to provide more secure protocols.

\medskip

We have separated the communication complexity of secure computation from
the computational complexity of the desired result.  This bodes well for
practical implementations, but is more striking from a theoretical
standpoint.  The crucial tool of {\em locally random reductions} vastly
reduces upper bounds on the number of rounds of communication for a
variety of cryptographic protocols.  In a deeper sense, it has triggered
other research leading to a result, $\ip=\pspace,$ which relates a
complexity class associated with interaction to a complexity class
associated with computational complexity.  The algebraic nature of the
locally random reductions we develop suggests not only wide
applications but a deeper understanding of the nature of interaction,
computational complexity, and reliable computation.



==> ihs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ihs.tex                    Instance Hiding Schemes.
%
%                            Copyright @1989  Donald Beaver.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{=======}
\typeout{ihs.tex}
\typeout{=======}

\chapter{Instance Hiding Schemes}    
\label{chap-ihs}


An {\em instance-hiding scheme} is a method by which a weak
(polynomial-time) processor can obtain the value $f(x)$ of a function it
cannot compute on its own, by querying more powerful processors, without
having to reveal the instance $x$ at which it would like to compute $f.$

Our research into instance-hiding schemes motivated the development of a
new tool, called a {\em locally random reduction,} which inspired a broad
range of results in cryptography and complexity theory, including a theory
of program testing \cite{lip89} and a recent line of research leading to
the proof that \mbox{IP = PSPACE}\index{interactive proof system!IP=PSPACE}
\cite{nis89-cosat,lfkn89,sha89}.  These applications are discussed in
Chapter~\ref{chap-lrr}, which investigates locally random reductions in
depth.  In this chapter we provide some of the motivations for our
development of locally random reductions and investigate the first of many
applications which locally random reductions solve, namely instance-hiding
schemes.

Abadi, Feigenbaum, and Kilian were the first to investigate the problem of
using a powerful, public resource to solve a problem without revealing the
instance of the problem \cite{afk89}.  They developed a formal model to
measure the information which is hidden or leaked during the interaction
between querier and oracle.  They were motivated by the practical question
of whether a weak, private computing device, such as a smart card or
terminal, can take advantage of a powerful, shared computing device while
keeping private some important aspects of its user's data.  They were also
motivated by the theoretical question of whether several well-studied yet
intractable number-theoretic functions, such as discrete logarithm and
quadratic residuosity, whose instances {\em can} be hidden significantly
when querying an oracle for the solution, are examples of a more general
phenomenon; that is, do other seemingly intractable problems, such as SAT,
also have instance-hiding schemes?

The main result of Abadi, Feigenbaum, and Kilian is negative: if $f$ is an
NP-hard function, a weak querier $A$ cannot query a single oracle $B$ while
hiding all but the size of the instance, assuming that the polynomial
hierarchy does not collapse.  Their proof draws on a connection between
single-oracle instance-hiding schemes and the nonuniform complexity classes
NP/poly and CoNP/poly, and it is related to other complexity-theoretic
notions, such as random-self-reducibility.  This negative result holds even
if $B$ is modelled as an oracle Turing Machine and is given access to an
arbitrary (non-r.e.) oracle set.  We refer the interested reader to
\cite{afk89} for full details.

\begin{theorem} \label{thm-afk}
[Abadi, Feigenbaum, Kilian 1989]
If language $L$ admits an instance-hiding scheme hiding all but $\abs{x},$
then $L \in \mbox{NP}/poly \cap \mbox{coNP}/poly.$
\end{theorem}

Following a question originally posed by Rivest \cite{riv86}, we generalize
instance-hiding schemes to handle several, physically separate oracles,
$B_1,\dots,B_m$ and show that, given sufficiently many oracles, any
function admits a multioracle instance-hiding scheme.  This contrasts with
the single oracle case, where not only is one oracle insufficient for some
functions \cite{afk89} but, as we shall see, one oracle is insufficient for
most functions.

We consider two models for $m$-oracle instance-hiding schemes:
\begin{itemize}
\item 
Oracles $B_1$ through $B_m$ may collude before the start of the protocol,
but they are kept physically separate during the protocol.  In this model,
$m = |x|$ oracles suffice for any function $f$.
\item 
Oracles $B_1$ through $B_m$ may not collude at all, either before or during
the protocol.  In this model, $m = 2$ oracles suffice for any function $f$.
Conversely, for most boolean functions $f,$ two oracles are necessary.
\end{itemize}

In the first model, our proof of sufficiency demonstrates an unintuitive
connection between instance-hiding schemes and secure multiparty protocols
\cite{bgw88,ccd88}.  The connection is unintuitive for many reasons, the most
obvious of which is that, in the first problem, we require explicitly that
the oracles not communicate at all and, in the second problem, we require
that they communicate extensively.  More fundamentally, the two problems
seem at first to exemplify two incompatible views of distributed
computations with secret data.  The instance-hiding problem first defined
in \cite{afk89} and generalized in Section \ref{sec-prelim} below
formalizes the following view.  A weak processor A requires interaction
with powerful processors $B_1$ through $B_m$, because A does {\em not} have
enough computational resources to compute $f;$ A does not want to reveal
more than necessary about its private input $x$ because the $B_i$'s are
public resources.  Secure multiparty protocols address an alternative view:
mutually untrusting, {\em equally powerful} processors $B_1$ through $B_m$
must interact in a computation because each of them has a private input
$x_i$ {\em without which} the computation cannot proceed.



\section{Preliminaries} \label{sec-prelim}

Following Abadi, Feigenbaum, and Kilian, we take A to be a probabilistic
polynomial-time Turing Machine transducer \cite{afk89}.  Let $f$ be a
boolean function on $\set{0,1}$ for which no probabilistic
polynomial-time algorithm is known.  In order to compute $f(x),$ A
consults players $B_1$, $\ldots$, $B_m$, where $m$ is (necessarily)
bounded by a polynomial in $\sizex.$  Each $B_i$ is an interactive
oracle Turing machine that can use an unbounded amount of time and
space.  It is convenient to think of the oracle tape of $B_i$ as a
random variable $O_i.$  Player $B_i$ is completely specified by its finite
control and the value of $O_i$.

An {\em m-oracle instance-hiding scheme} for $f$ is a $R$-round,
synchronous protocol executed by players $A,$ $B_1$, $\ldots$, $B_m.$
Player $A$ draws input $x$ according to a distribution $X.$ The
round-complexity $R$ is bounded by a polynomial in $\sizex.$ Let
$\view_A^{1..r}$ denote the sequence of messages sent and received by $A$
in rounds 1 through $r$, let $\delta_A$ denote its finite control, and let
$R_A$ denote its random tape.

At round $r+1$ of the protocol, $A$ performs a probabilistic
polynomial-time computation producing $m$ messages $y_{r,1},\ldots,y_{r,m}$
for $B_1,\ldots,B_m,$ based on $x, \view_A^{1..r}, \delta_A,$ and
$R_{A}.$ Each $B_i$ computes a response $z_{r+1,i}$ based on
$y_{1,i},\ldots,y_{r+1,i}$ and sends it to player $A.$

In the simple case, which corresponds to the motivating idea of a
collection of public servers supplying answers to queries, this response is
a function $g$ applied to $y_{r+1,i};$ player $B_i$ can perform an
unbounded amount of local computation, and replies with $z_{r+1,i} =
g(y_{r+1,i}).$ After round $R$ of the protocol, $A$ computes $f(x)$ based
on $x,$ $\view_A^{1..r},$ $\delta_A,$ and $R_A.$ Note that we do not allow
the output of $A$ to be incorrect.

Let $Y_i$ be the induced distribution on the sequence 
$\anglebrack{y_{1,i},\ldots,y_{R,i}}$ of messages $A$ sends
to player $B_i.$

We wish to make precise the statements that an instance-hiding scheme
``leaks at most'' some function $L(x)$ to player $B_i$ or that it
``hides at least'' some function $H(x)$ from player $B_i$.  Note that
$L(X)$ and $H(X)$ are also induced random variables.

We consider two generalizations of the definitions in \cite{afk89}.  In both
models, all players ``know'' the plaintext distribution $X$ and the
contents of the finite controls
$\delta_A,\delta_{B_1},\ldots,\delta_{B_m}.$ Furthermore, in both models,
each player $B_i$ ``does not know'' the content of the random tape $R_A$,
and, for $i\neq j$, player $B_i$ ``does not see'' the messages $y_{r,j}$
that A sends to $B_j$ or the responses that $B_j$ sends back.  The
difference between the two models lies in whether or not $B_i$ ``knows''
the content of oracle tape $O_j$ for $j\not=i.$

\smallskip

\noindent
{\bf Model 1:}
\begin{itemize}
\item
\index{leak}\index{instance-hiding scheme}
An instance-hiding scheme {\em leaks} at most $L$ to oracle $B_i$ if,
for all plaintext distributions $X,$ 
for all $u \in \mbox{ \em Range}(L),$
the random variables $X$ and 
$\anglebrack{Y_i,O_1,\ldots,O_m}$
are independent given $L(X)=u.$
\item
An instance-hiding scheme {\em hides} at least $H$ from oracle $B_i$ if,
for all plaintext distributions $X,$ 
the random variables $H(X)$ and
$\anglebrack{Y_i,O_1,\ldots,O_m}$ are independent.
\end{itemize}

Intuitively, a player ``knows'' nothing about the outcome of a random
variable $X$ if the observations of random variables to which it has
access are independent of $X.$ Thus, in Model~1, we allow $B_i$ to
``know'' the contents of every oracle tape by virtue of measuring its
knowledge with respect not only to the query sequence $Y_i$ and oracle
tape $O_i$ but to the entire set of oracle tapes.

Informally, this corresponds to the case in which the powerful players
can collude before, but not during, the execution of the protocol.
In Model~2, however, we allow no collusion at all, before or during the
execution of the protocol:

\smallskip

\noindent
{\bf Model 2:}
\begin{itemize}
\item
An instance-hiding scheme {\em leaks} at most $L$ to oracle $B_i$ if,
for all plaintext distributions $X,$ 
for all $u \in \mbox{ \em Range}(L),$
the random variables $X$ and 
$\anglebrack{Y_i,O_i}$
are independent given $L(X)=u.$
\item
An instance-hiding scheme {\em hides} at least $H$ from oracle $B_i$ if,
for all plaintext distributions $X,$ 
the random variables $H(X)$ and
$\anglebrack{Y_i,O_i}$ are independent.
\end{itemize}

Specifically, in Model~2, player $B_i$ has access only to $Y_i$ and
$O_i;$ it is possible that the additional knowledge of other oracle
tapes might lead to a dependence among random variables, revealing some
additional information.

In either model, we say that the scheme ``leaks $L$'' if it leaks at
most $L$ to each $B_i,$ and we say that it ``hides $H$'' if it hides at
least $H$ from each oracle $B_i.$ Throughout this paper, we are
primarily concerned with schemes that leak $\sizex$.  In either model,
we say that ``$f$ has an $m$-oracle instance-hiding scheme'' or that
``$m$ oracles suffice for $f$'' to mean that $f$ has an $m$-oracle
instance-hiding scheme that leaks $\sizex.$  As in \cite{afk89}, we 
define leaking and hiding in terms of independence of random variables.
Complexity-based cryptography is irrelevant, because A is time-bounded
and the $B_i$'s are time-unbounded.

\begin{observation} \label{obs-equiv}
Models 1 and 2 are equivalent if $m=1$. 
\end{observation}

We end this section with the proposition that if the querier A is
limited in space, but not in time or in number of rounds of interaction
with the $B_i$'s, then the instance-hiding problem is trivial.

\begin{theorem} \label{thm-space}
Every function has a 1-oracle instance-hiding scheme that leaks at most
$\sizex$ in which the querier A is limited to (deterministic) constant space.
\end{theorem}

The oracle simply sends every instance of size $\sizex$ along with its
answer, and the querier checks the instance against $x,$ copying the answer
to the output when the instance matches $x.$ We refer the interested reader
to \cite{c88,cle89,ds88,k88-2}, for example, for a discussion of the related
topic of (zero-knowledge) interactive proof systems with space-bounded
verifiers.

\section{Model 1: $\mid x \mid$  Oracles Suffice} 
\label{sec-model1}

Our main result on model-1 instance-hiding schemes uses Shamir's method for
secret sharing.
For notational convenience, we shall refer to a value $p(\alpha_i)$ of a
polynomial of degree $t$ with free term $s$ as a $t$-{\em point} of $s.$
The difference between a $t$-{\em point} and a {\em piece} of $s$ is that
the latter indicates that the polynomial has been selected uniformly at
random (subject to the constraints on degree and free term), whereas the
former concerns an arbitrary polynomial.  The randomness property will be
essential only for the initial queries of $A.$

The following lemma is an easy consequence of Lemma~\ref{lem-can-f-poly}.
\begin{lemma}  \label{lem-can-f-bool-poly}
Any boolean function $f(x)$ on inputs $x$ of length $n$ can be represented
as a polynomial $c_f(x_1,\ldots,x_n)$ over an arbitrary field $E,$
such that when the values $x_1,\ldots,x_n$ match the bits of $x,$
$f(x)=c_f(x_1,\ldots,x_n).$
\end{lemma}

With a few straightforward observations, we shall be able to construct
efficient instance-hiding schemes for arbitrary boolean functions.  First,
note that if elements $\gamma_1, \ldots, \gamma_k$ of $E$ are $t$-points of
$s_1, \ldots, s_k$, respectively, then $\gamma_1 + \cdots + \gamma_k$ is a
$t$-point of $s_1 + \cdots + s_k.$ In fact, any this holds for any linear
combination: if $\beta_1, \ldots, \beta_k$ are fixed constants in $E,$ then
$\beta_1 \gamma_1 + \cdots + \beta_k \gamma_k$ is a $t$-point of $\beta_1
s_1 + \cdots \beta_k s_k.$ Furthermore, $\gamma_1 \times \cdots \times
\gamma_k$ is a $kt$-point of $s_1 \times \cdots \times s_k$.  
(By comparison, recall that in the \mult protocol 
(Chapter~\ref{chap-con}), the product of two $t$-shares is a $2t$-point,
which later is converted to a $t$-share.)

Specifically, if $c_f(x_1,\ldots,x_n)$ has degree $n,$ and
$\gamma_1,\ldots,\gamma_k$ are $t$-points of $x_1,\ldots,x_n,$
then $c_f(\gamma_1,\ldots,\gamma_n)$ is a $nt$-point of $c_f(x_1,\ldots,x_n).$
A total of $(nt+1)$  $nt$-points suffice to determine $c_f(x_1,\ldots,x_n).$

\begin{theorem} \label{theorem-model1}
Let $f(x)$ be any function whose output $\abs{f(x)}$ is polynomially
bounded.  Then for any positive constant $c,$ $f(x)$ has a model-1 $(\sizex
- c \log \sizex)$-oracle instance-hiding scheme that leaks at most $\sizex.$
\end{theorem}

\begin{proof}
Assume WLOG that $f$ is boolean.  The result for general functions then
follows by regarding each output bit as a boolean function of the input.
We first show that $\sizex+1$ oracles suffice and then improve upon the
construction.

For concreteness, let $E$ be ${\bf Z}_p$ for the smallest prime exceeding
$n+2.$ By lemma~\ref{lem-can-f-poly}, there is a polynomial
$c_f(x_1,\dots,x_n)$ over $E$ which is equal to $f(x)$ at 0/1-valued
inputs.  Let each $B_i$ have access to an oracle for $c_f.$

The protocol begins with the querier secretly sharing $x_1,\ldots,x_n$
among $n+1$ oracles using $t=1$ as the bound on coalition sizes.  Each
oracle evaluates $c_f$ on the collection of $1$-points it receives, giving
a $n$-point of the final value.  Finally, $A$ interpolates the $(n+1)$
$n$-points to determine the $n^{th}$-degree polynomial $c_f.$
Figure~\ref{fig-ihs-n} lists the steps exactly.  The {\tt interpolate}
function outputs the coefficients of the minimal-degree polynomial running
through its arguments.

\figstretch
\boxfig{
\begin{tabular}{ll}
$A:$ &  $n\leftarrow \sizex,$ where $x=x_1x_2 \cdots x_n.$\\
$A:$ & select $p_1(u),\dots,p_n(u)$ randomly of degree 1 with $p_i(0)=x_i.$\\
$A:$ & $\piece_i(x_j) \leftarrow p_i(j).$
\hfill \hspace{0.4in} (for $1 \leq i \leq n+1.$) \\
$A:$ &  $y_i \leftarrow
\anglebrack{n, \piece_i(x_1),\ldots,\piece_i(x_n)}$
\hfill \hspace{0.4in} (for $1 \leq i \leq n+1.$) \\
$A \rightarrow B_i:$ &  $y_i$
\hfill \hspace{0.4in} (for $1 \leq i \leq n+1.$) \\
$B_i:$  &  $z_i \leftarrow c_f(\piece_i(x_1),\ldots,\piece_i(x_n))$ 
\hfill \hspace{0.4in} (for $1 \leq i \leq n+1.$) \\
$B_i \rightarrow A:$ &  $z_i$ 
\hfill \hspace{0.4in} (for $1 \leq i \leq n+1.$) \\
$A:$ & $p(u) \leftarrow \mbox{\tt interpolate}(z_1,z_2,\dots,z_{n+1})$ \\
$A:$ & $f(x) \leftarrow p(0).$
\end{tabular}
\caption{\label{fig-ihs-n}
\index{instance-hiding scheme!$n$ oracle}
Instance-hiding scheme for $f(x)$ with $n+1$ oracles.
Each $B_i$ has an oracle $O_i$ for $c_f.$
}}
\figstretchend

Intuitively, basing the protocol on ideas from secret-sharing ensures that
each $B_i$ learns nothing about $x.$ Even though $B_i$ can use its
unbounded resources to attempt to recover $x,$ it cannot communicate with
any of the other $B_j,$ so the only physically possible coalitions are
trivial ones of size~1.  Because player $B_i$ sees only the $1$-{\em
shares} of $x_1,\ldots,x_n$ and does not see the later collection of
$n$-points, he receives no information about $x.$

To prove that each $B_i$ learns nothing but $n,$ we use a simple lemma,
akin to the statement that secret sharing is $1$-private:
\begin{lemma}    \label{lem-lin-share}
For any $x_1, \ldots, x_n \in E$ and for any $i \not = 0,$ the
following distribution is the same as $\uniform(E^n):$
\[
\set{ (a_1,\ldots,a_n) \leftarrow \uniform(E^n): 
(a_1 i + x_1, \ldots, a_n i + x_n)}
\]
\end{lemma}

\begin{proof}
Clearly, for fixed $x_1,\dots,x_n$ and $i\not= 0,$ the mapping
$(a_1,\ldots,a_n) \mapsto (a_1 i + x_1, \ldots, a_n i + x_n)$ is
a bijection, so if $(a_1,\ldots,a_n)$ is uniform over $E^n,$
so is $ (a_1 i + x_1, \ldots, a_n i + x_n).$
\end{proof}

Thus, the distribution on messages $y_i$ seen by $B_i$ is the same for any
$x:$ uniform over $\set{n} \times E^n.$ Therefore the random variables $X$
and $\anglebrack{Y_i,O_i}$ are independent.  In fact, since each $B_j$ ($j
\not= i$) computes the same polynomial $c_f(x_1,\ldots,x_n),$ each oracle
tape is the same, and hence the random variables $X$ and
$\anglebrack{Y_i,O_1,\dots,O_{n+1}}$ are independent.  

To reduce the number of oracles queried in the protocol from $n+1$ to $n,$
we can ``instantiate'' the input bit $x_1$ and treat $f$ as though it were
a function of $n-1$ inputs.  The querier $A$ first executes the basic
protocol on input $0x_2\cdots x_n$, then executes it on input $1x_2\cdots
x_n$, and uses the result that corresponds to the original input $x_1 x_2
\cdots x_n$.  More generally, by instantiating $O(\log n)$ input bits (thus
generating $n^{O(1)}$ queries) the number of $B_i$'s queried can be reduced
to $n - O(\log n)$.
\end{proof}


\section{Model 2: Two Oracles Suffice} \label{sec-model2}

In this section, it is convenient to regard a boolean function $f$ as the
characteristic function $\chi_S$ of a set $S\subseteq \{0,1\}^*$ or as a
language $L_f = \set{x \mid f(x) = 1}.$ By {\it a random set} $S$, we mean
one in which $\chi_S(x)$ is the outcome of a fair coin toss, for each $x\in
\{0,1\}^*$.  The expression $S_1 \bigtriangleup S_2$ denotes the symmetric
difference of sets $S_1$ and $S_2$; that is, 
\[
\chi_{S_1 \bigtriangleup S_2}(x) \equiv \chi_{S_1}(x) \oplus \chi_{S_2}(x).
\]
If $s_1$ and $s_2$ are both $n$-bit strings, then $s_1 \oplus s_2$ is the
$n$-bit string whose $i^{\rm th}$ bit is the exclusive-or of the $i^{th}$
bits of $s_1$ and $s_2$.

We also use the following nonstandard terminology and notation.  A {\it
singleton sequence} is a subset of $\{0,1\}^*$ that contains exactly one
string of each length.  A {\em random singleton sequence} is one in which
the length-$n$ string is chosen u.a.r.~from $\{0,1\}^n$.  If $S$ is an
arbitrary set and $V = \{v_1, v_2, \ldots\}$ is an arbitrary singleton
sequence, then $S\circ V$ denotes the set with characteristic function
$$\chi_{S\circ V}(x) \equiv \chi_S(x\oplus v_{\sizex}).$$ Note that each
$v_n$ in $V$ effects a permutation of the bits in the characteristic vector
of $S \cap \set{0,1}^n.$

%\vfil\eject
\begin{theorem}\label{theorem-model2}
Every function%
\footnote{As before, we assume the size of the output, $\abs{f(x)},$
is polynomially bounded.}
has a model-2 2-oracle instance-hiding scheme that leaks at most $\sizex$.
Conversely, two oracles are necessary for most boolean functions.
\end{theorem}

\begin{proof}
Necessity follows from Observation~\ref{obs-equiv} and
Lemma~\ref{lem-kolm}, which is proved in the next section.  We show
sufficiency by demonstrating the existence of a model-2 2-oracle
instance-hiding scheme for an arbitrary function $\chi_S$ that leaks at
most $\sizex$.  As in the proof of Theorem \ref{theorem-model1}, we assume
WLOG that $f$ is boolean.

Let us illustrate the basic idea of the proof through the following simpler
argument.  Assume first that the conditional plaintext distribution $P(X
\mid \abs{X})$ is uniform.  Under this simplifying assumption, we can see that
the characteristic function of a random set $S$ has a model-2 2-oracle
instance-hiding scheme that, with probability 1, leaks at most $\sizex$ to
$B_1$ and at most $\chi_S(x)$ to $B_2$: Let $B_1$ have an oracle for a
random singleton sequence $V= \{v_n\}_{n=1}^\infty,$ and let $B_2$ have an
oracle for $S \circ V.$ On cleartext input $x,$ A first sends $\sizex$ to
$B_1$, who sends back $v_{\sizex}$.  A then sends $x \oplus v_{\sizex}$ to
$B_2$, who sends back $\chi_{S\circ V}(x \oplus v_{\sizex}) = \chi_S(x)$.
Clearly, $B_1$ learns only $\sizex$.  Intuitively, $B_2$ learns only
$\chi_S(x)$ because, for random $S$ and $V,$ $S\circ V$ is also random, and
the encrypted input $x \oplus v_{\sizex}$ is a uniformly distributed
$n$-bit string.  To make this idea work for the theorem as stated, we must
make an arbitrary $S$ ``look random,'' and we must show how to avoid
leaking $\chi_S(x)$ to $B_2$.  We accomplish this by using the symmetric
difference of $S$ with a random set and by ``splitting'' the singleton
sequence $V$ into two halves, one of which is given to each of $B_1$ and
$B_2$.

Suppose that $\chi_S$ is the (arbitrary) boolean function for which we seek
an instance-hiding scheme.  Let $R$ be a random set,
$V=\{v_n\}_{n=1}^\infty$ and $U = \{b_{1,n}\}_{n=1}^\infty$ be random
singleton sequences, and let $T = \{b_{2,n}\}_{n=1}^\infty$ be such that
$b_{2,n} = v_n \oplus b_{1,n}$.  Let the oracle $O_1$ for $B_1$ encode both
$R \circ V$ and $U$ in a standard way, and let the oracle $O_2$ for $B_2$
encode both $(S \bigtriangleup R)\circ V$ and $T.$ The instance-hiding
scheme is described in Figure~\ref{fig-ihs-two}.

\figstretch
\boxfig{
\begin{tabular}{ll}
A: &  $n\leftarrow \sizex$.\\
A $\rightarrow$ $B_1$, $B_2$: &  $n$. \\
$B_1$ $\rightarrow$ A: &  $b_{1,n}$. \\
$B_2$ $\rightarrow$ A: &  $b_{2,n}$. \\
A: &  $y\leftarrow x\oplus b_{1,n} \oplus b_{2,n}$.\\
A $\rightarrow$ $B_1$, $B_2$: &  $y$.\\
$B_1$ $\rightarrow$ A: &  $\chi_{R\circ V}(y)$.\\
$B_2$ $\rightarrow$ A: &  $\chi_{(S\bigtriangleup R)\circ V} (y)$.\\
A: &  $\chi_S(x)\leftarrow \chi_{R\circ V}(y) \oplus 
\chi_{(S \bigtriangleup R)\circ V}(y)$.
\end{tabular}
\caption{\label{fig-ihs-two}
\index{instance-hiding scheme!two oracle}
Instance-hiding scheme for $f(x)$ with two oracles.
Oracle $O_1$ encodes $(R \circ V,U);$ $O_2$ encodes
$((S \bigtriangleup R)\circ V,T).$
}}
\figstretchend


The querier obtains the result:
\begin{eqnarray*}
\chi_{R\circ V}(y) \oplus \chi_{(S \bigtriangleup R)\circ V}(y)
& = &
\chi_R(x \oplus b_{1,n} \oplus b_{2,n} \oplus v_n) \oplus
\chi_{S \bigtriangleup R}
(x \oplus b_{1,n} \oplus b_{2,n} \oplus v_n)
\\ & = & \chi_R(x) \oplus \chi_{S \bigtriangleup R}(x)
\\ & = & \chi_S (x).
\end{eqnarray*}

The messages seen by $B_1$ are $y_{1,1} = n$ and $y_{2,1} = x \oplus
b_{1,n} \oplus b_{2,n}.$ First let us show that for every $x$ of size $n,$
the distribution on $((y_{1,1},y_{2,1}),(R \circ V, U))$ is the same.

The distribution on $(R,V,U)$ given $n$ is uniform over the $2^{2^n} 2^n
2^n$ choices for $(R,V,U).$ For any particular $x$ of size $n,$ the
protocol induces a bijection with $(y_{2,1},R \circ V,U).$ Thus, for any
particular $x$ of size $n,$ the distribution on $(y_{2,1},R \circ V,U)$ is
uniform over all possibilities.  Since $y_{1,1}$ is always $n,$ the
distribution on $((y_{1,1},y_{2,1}),(R\circ V, U))$ is uniform over all
possible values, for each $x$ of size $n.$ Hence the random variable
$\anglebrack{Y_1,O_1}$ is independent of $x,$ given $n.$

Now consider $B_2.$ Any fixed $S$ induces a bijection on the set of
possible $R.$ Hence there is a bijection between $(R,V,U)$ and $(S
\bigtriangleup R,V,U).$ By definition, there is a bijection between the
latter set and $(S \bigtriangleup R,V,T).$ Using the argument of the
previous paragraph, there is a bijection between $(S \bigtriangleup R,V,T)$
and $(n,y_{2,2}, (S \bigtriangleup R) \circ V, T).$ Hence the distribution
on $((y_{2,1},y_{2,2}), ((S \bigtriangleup R) \circ V, T))$ is uniform, for
any $x$ of size $n.$  Thus $\anglebrack{Y_2,O_2}$ is independent of $x,$
given $n.$  
\end{proof}


\section{Other Results}
\label{sec-other}

\subsection{Unconditional Negative Results}

The main theorem of \cite{afk89} is that NP-hard functions have no 1-oracle
instance-hiding schemes that leak $\sizex$, unless the polynomial hierarchy
collapses at the third level.  This is a conditional negative result.  No
unconditional negative results about instance-hiding schemes that leak
$\sizex$ are provided in \cite{afk89}.  We give one here.

\begin{lemma} \label{lem-kolm}
Measure one of boolean functions do not have 1-oracle instance-hiding
schemes that leak at most $\sizex.$
\end{lemma}

\begin{proof}
Let $\vec{c}_n(f)$ denote the characteristic vector of $f$ for inputs
of $n$ bits 
(e.g., $\vec{c}_2(f)$ is the concatentation of $f(00)$,
$f(01)$, $f(10)$, and $f(11)$).  
Let $C(f)$ denote the set of characteristic vectors for $f,$ 
$\set{\vec{c}_n(f) \mid n \in {\bf N}}.$  We refer to a set
containing exactly one string of length $2^n$ for each $n$
as a characteristic set.

If $L_f,$ the set of $x$ such that $f(x)=1,$ is a language in NP/$poly,$
then it is not hard to see that for some constant $d,$ the Kolmogorov
complexity of $\vec{c}_n(f)$ is at most $n^d$ for all $n.$
We shall show that for any $d,$ the class of characteristic sets
consisting of strings with Kolmogorov complexity $n^d$ is contained
in a class having measure zero, using a natural measure.  

The measure we use is the natural one defined on the class of boolean
functions: any boolean function $f$ is equivalent to a real number $R_f$
between 0 and 1, where the $i^{th}$ bit of the number is $f(i).$ The
measure of a set of boolean functions is the Lebesgue measure on the
corresponding set of reals.  Since the representations of $f$ as a boolean
function, real number, language, or characteristic set are equivalent, we
loosely apply ``measure'' to classes of all of them, without loss of
generality.

For any $n,$ a straightforward counting argument shows that at least
$2^{2^n}/2$ strings of length $2^n$ have Kolmogorov complexity at least
$2^n-1.$ Let $K_n$ be the set of the lexicographically first $2^{2^n}/2$ of
these strings, and let $K = \cup_n K_n.$ If ${\cal C}$ is the class of
characteristic sets, then let $J = \set{ C \in {\cal C} \mid (\forall n)
\abs{K_n \cap C} < \infty};$ each characteristic set in $J$ contains at
most a finite number of vectors appearing in $K.$ The class $J$ is composed
of a countable number of subclasses ($J_l^m,$ the class of sets having $l$
vectors in common with $K$ but each of length at most $2^{2^m}$), each
similar to the Cantor set and having measure 0 by the standard argument.
The measure of $J$ is thus 0.

Let us argue that the characteristic set for any language in NP/$poly$ is a
member of $J.$ Let $L_f \in \mbox{NP}/poly,$ and let $L_f$ be recognized by
a nondeterministic Turing machine with a program of length $l$ and with
advice of length $n^e.$ For some $d,$ $l + n^e \leq n^d,$ and the
Kolmogorov complexity of any characteristic vector $\vec{c}_n(f)$ is
therefore at most $n^d.$ Now, for some constant $n_d,$ $n \geq n_d
\Rightarrow n^d < 2^n-1,$ and therefore $n \geq n_d \Rightarrow \vec{c}_n(f)
\not\in K_n.$ Hence a finite number of characteristic vectors are in $K,$
and $C(f) \in J.$

The class of characteristic sets for languages in NP/$poly$ is thus contained
in $J$ and has measure 0.   For every function $f$ having a 1-oracle
instance-hiding scheme, $L_f \in \mbox{NP}/poly,$ so the measure of
functions having 1-oracle instance-hiding schemes is 0.
\end{proof}


\subsection{Random-Self-Reducing Circuits}\label{sec-rsrc}

Intuitively, a random-self-reduction of a set $S$ is an
expected-polynomial-time, randomized algorithm that maps $S$ to $S$, maps
${\overline S}$ to ${\overline S}$, and, on each input $x$ in $S$, outputs,
with equal probability, each $y$ in $S \cap \{0,1\}^{\sizex}$.  Abadi,
Feigenbaum, and Kilian defined random-self-reducing algorithms rigorously
and related them to 1-oracle instance-hiding schemes \cite{afk89}.  In this
section, we consider random-self-reducing {\em circuits} in the same
context.

A {\em randomized {\sc psize} circuit family} is a set
$\{C_n\}_{n=1}^\infty$ of circuits in which the number of gates in $C_n$ is
at most $p(n)$ for some polynomial $p$, and $C_n$ has $n$ inputs
$x_1,\ldots,x_n,$ random inputs $r_1,\ldots,r_{q(n)},$ and outputs
$y_1,\ldots,y_{m(n)},$ for polynomials $q(n)$ and $m(n).$ We say that
$\set{C_n}$ {\em generates} a collection of distributions
$\set{D_n(x)}_{n\in\natsmall, x \in \{0,1\}^{*}}$ if for all $x,$
$C_{\abs{x}}$ outputs a sample point from $D_n(x)$ with probability at
least $1/2,$ and otherwise outputs a distinguished string $\Lambda.$

\begin{definition} \label{def-rsrc}
A set $S$ {\rm has random-self-reducing circuits} if there is a randomized
{\sc psize} circuit family $\set{C_n}$ that generates the distribution
$D_n(x)$ defined as the uniform distribution on $S \cap
\set{0,1}^n$ for $x \in S,$ or an arbitrary distribution on 
$\overline{S} \cap \set{0,1}^n$ for $x \in \overline{S}.$ The family
$\set{C_n}$ is called a {\rm random-self-reducing circuit family for} $S$.
\end{definition}

\begin{definition} \label{def-2srsrc}
A set $S$ {\rm has two-sided random-self-reducing circuits} if there is a
randomized {\sc psize} circuit family $\set{C_n}$ that generates the
distribution $D_n(x)$ defined as the uniform distribution on $S \cap
\set{0,1}^n$ for $x \in S,$ or the {\em uniform} distribution on 
$\overline{S} \cap \set{0,1}^n$ for $x \in \overline{S}.$ The family
$\set{C_n}$ is called a {\rm two-sided random-self-reducing circuit family
for} $S$.
\end{definition}
  
\begin{lemma} \label{lem-encnrsr}
If $S$ has two-sided random-self-reducing circuits, then $\chi_S$ has a
1-oracle instance-hiding scheme that leaks at most $\sizex$ and
$\chi_S(x)$.
\end{lemma}


Lemma \ref{lem-encnrsr} provides a way of showing that certain boolean
functions have model-1 instance-hiding schemes that use many fewer oracles
than the schemes given by Theorem \ref{theorem-model1}.  Unfortunately, as
the following theorem indicates, neither SAT nor ${\overline {\rm SAT}}$ is
likely to have random-self-reducing circuits.  (It is even less likely that
SAT has two-sided random-self-reducing circuits, as it would need for Lemma
\ref{lem-encnrsr} to apply.)

\begin{theorem} \label{thm-rsrc-collapse}
~\\
\begin{itemize}
\item[a.]
If ${\overline {\rm SAT}}$ has random-self-reducing circuits, then the
polynomial hierarchy collapses at the third level.
\item[b.]
If {\rm SAT} has random-self-reducing circuits, then the
polynomial hierarchy collapses at the third level.
\end{itemize}
\end{theorem}

\begin{proof}
By a proof of Nisan \cite{nis88-pc} that, if SAT had a random-self-reducing
algorithm, then ${\overline {\rm SAT}}$ would be in IP$[2]$.  Then, we use
the facts that ${\rm IP}[2] \subseteq {\rm AM}[4] \subseteq {\rm AM}[2]
\subseteq {\rm NP}/poly$ (see \cite{bm88,gmr89,gs86}) and that ${\overline {\rm
SAT}}\subseteq {\rm NP}/poly \Rightarrow {\rm PH} \subseteq \Sigma_3^p$
(see \cite{yap83}).  These results extend {\em mutatis mutandis} to the
case of random-self-reducing circuits for SAT and proof-systems with
circuit-verifiers.
\end{proof}

\subsection{Multiple Queries}

The instance-hiding schemes we give are easily extended to allow the
querier to ask an unlimited number of questions.  The scheme for Model~1
given in the proof of Theorem~\ref{theorem-model1} can be repeated
directly.  The scheme for Model~2 can be used only once, but by generating
an exponential number of (non-reusable) schemes for each $n$ and encoding
them in a direct way into the two oracles, the scheme can be modified to
support many queries.


\subsection{Nontrivial One-Oracle Schemes}
\label{sec-rsr-dlog}

Abadi, Feigenbaum, and Kilian show that certain well-known number-theoretic
functions, such as discrete logarithm and quadratic residuosity, have
one-oracle instance-hiding schemes that hide some significant information
about the input \cite{afk89}.  However, those schemes {\em do} leak more than
the size of the input $x$, and \cite{afk89} provides no nontrivial examples
of functions with instance-hiding schemes that leak at most
$\sizex$.\footnote{Examples of trivial instance-hiding schemes that leak at
most $\sizex$ are the obvious schemes for $\chi_S$, where $S$ is a set in
P/$poly$; the oracle simply sends the polynomial advice string, and the
querier computes on his own.}  Let us present a nontrivial example of a
presumably intractable function with a one-oracle instance-hiding scheme.

\begin{definition}  \label{def-dlog}
The {\em discrete logarithm} to the base $g$ modulo $p$ of a number $x,$
$\mbox{DLOG}_{g,p}(x),$ is the exponent $e$ such that $g^e \equiv x \mod
p.$  Here, $p$ is prime, and $g$ is a generator of the nonzero integers
$\mod p.$  No efficient method for computing DLOG is known.  
\end{definition}

\begin{exampleenv}
The instance-hiding scheme for DLOG given in \cite{afk89} is as follows.
On input $g\#p\#x,$ choose $r\in \set{1,\dots,p-1}$ uniformly at random,
and let $y=x g^r \mod p$ (if $x=0,$ pretend $x=1$ and note that the answer
is $\Lambda.$).  Clearly, $y$ is distributed uniformly over ${\bf
Z}_{p}^{*}$ for any $g\#p\#x$ of size $n,$ given $g$ and $p.$ On receiving
the answer $z =
\mbox{DLOG}_{g,p}(y),$ return $z-r.$ The reduction is correct:
\[
\mbox{DLOG}_{g,p}(y)- r =
\mbox{DLOG}_{g,p}(x g^r)- r =
\mbox{DLOG}_{g,p}(x) +r- r =
\mbox{DLOG}_{g,p}(x).
\]
Thus this scheme leaks $\abs{g\#p\#x}, g,$ and $p.$  We now define a
function that has a scheme which leaks only $\abs{g\#p\#x}.$

Let $p_n$\index{$p_n$!smallest prime exceeding $2^n$}
% 
denote the smallest prime exceeding $2^n,$ and $g_n$ the smallest generator
of ${\bf Z}_{p_n}.$ Define the function $f(x) =
\mbox{DLOG}_{g_{|x|},p_{|x|}}(x).$ (If $x\equiv 0 \mod p_{|x|},$ then say
$f(x)=\Lambda.$) As in the general case of the discrete logarithm, no
efficient method for computing $f(x)$ is known.

On the other hand, given $g_n$ and $p_n,$ the reduction described above is
easy to perform.  Thus, an instance-hiding scheme for $f(x)$ can be
constructed as follows.  First, the querier sends $n=\abs{x},$ and receives
$g_n$ and $p_n$ in return.  Then the querier performs the
random-self-reduction described above, and obtains the result as described
above.  The scheme hides everything but $\sizex.$
\end{exampleenv}



==> int.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% int.tex                      Introduction
%
%                            Copyright @1989  Donald Beaver.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{=======}
\typeout{int.tex}
\typeout{=======}

\chapter{Introduction}                            \label{chap-intro}


\chapquote{
It is true that you can fool all the people some of the time; \\
you can even fool some of the people all the time; \\
but you can't fool all of the people all the time.
}{
Abraham Lincoln}

In an ideal world, a single, reliable, and trusted computer would take care
of every computational need without delay.  In practice, however, no single
computer could be powerful enough, reliable enough, or even sufficiently
accessible to satisfy such an ideal.  For reasons of efficiency, reliability,
security, and for the immense benefits of interaction, distributed
computing is the only solution, and indeed it is rapidly being realized.
The tremendous increase in dependence on large, interconnected computer
systems makes a thorough analysis of their reliability of paramount
importance.  The issues of fault-tolerance and security are essential to
capitalizing on the advantages of scale and interaction.

At the same time, the need for practical methods to ensure reliability and
security can be satisfied only by efficient techniques.  Unwieldy and
inefficient methods are difficult to implement correctly and, even worse,
are likely to be ignored altogether.

The protection of {\em communications} among various parties has a long and
rich history, by no means restricted to the age of computers.
Cryptographers have long concerned themselves with developing codes to
encipher and decipher messages.  Similarly, limiting and authorizing access
to important resources (whether they are the headquarters of a military
command or the files in a centralized computer) has also been the focus of
centuries of analysis.  Often, the methods developed for one problem are
applicable to the other; for instance, the $\mbox{\sc
Unix}^{tm}\index{UNIX}$ operating system implements password schemes to
authorize logins by using encryption functions originally designed to
protect communications.

Security for {\em distributed computations,} however, is a more recent 
concern.
The direct approach is to use classical methods for security that treat a
collection of interacting computers as a group of individuals, protecting
each computer individually and then protecting the communications between
each pair of computers.  Often, methods for security and reliability depend
on the invulnerability of some central host which takes care of
authorization, exclusive access to files, and so on.


Research into distributed system reliability (without regard to security)
addresses the problems of failures in individual processors, and develops
methods such as transaction processing and process migration to recover
from individual failures.  Together, the collection of processors can carry
on computations despite local problems.  Like the methods developed to
protect communications, though, these methods still rely on one or a few
central hosts, such as name-servers, for essential operations.

The very presence of a large number of somewhat independent processors
affords a much greater degree of reliability and security than that
provided by a single, central host.  A large, distributed network of
computers is in some ways very much like a community of people.  Some
elements are reliable, some are not; some are prone to accidental mishaps,
others behave maliciously.  On the whole, most are reliable most of the
time, but there are few whom one would trust or depend upon completely.
Yet with the proper ``laws,'' individuals function together despite an
imperfect world, and societies prosper despite individual flaws.


In this work, we take advantage of the synergy provided by the interaction
among many processors in order to ensure that useful computations continue
despite failures in sizable and {\em arbitrary} portions of a network.
Interestingly and importantly, our methods apply to ensure both reliability
and security.  In retrospect this is not surprising: reliability and
security are two sides of the same coin.  A reliable system should be
resilient against the worst-case failure, which is best regarded as a
malicious attack.  On the other hand, ensuring that an adversary cannot
obtain information means that the nature of its attack is independent of
that information.  This has the advantage that, in an intuitive sense, the
attack can be treated more like a random or accidental failure.

In addition to these intuitive connections between reliability and
security, it turns out that the two have interesting and deeper connections
when defined formally.  Essentially, the two goals are unified by the
single purpose of simulating a trusted and reliable central host, even
though none is available and it would be imprudent even with assurances to
depend on a single, supposedly reliable party.  

A standard formal method to
ensure that unspecified information is not leaked during an interaction is
to demonstrate that the course of the interaction can be simulated, in a
certain formal sense, based only on the information that is supposed to be
leaked.  This information is measured with respect to an ideal setting in
which a trusted host is available; the trusted host leaks only specified
facts, by definition.

We examine interaction in a deeper sense, investigating not simply the {\em
information} flow from one processor to another but the {\em influence}
that one processor may have over the computation.  We develop broad
definitions that compare the information and the influence that a
participant or adversary has in one protocol to that which it would have in
another protocol.  The meaning of {\em correctness} in distributed
computation is closely tied to the measure of {\em influence} over outputs,
in the same way that {\em privacy} is tied to the measure of {\em
information.}  This observation forms the basis of a fundamentally new
and unified approach to distributed security.


\medskip

The focus of this dissertation is a collection of {\em efficient}
methods whereby
a collection of individuals can achieve reliable computations in a 
{\em provably}
secure manner, despite the failure or corruption of some minority of the
individuals.

Consider the following example.  The board of trustees of a company would
like to take a vote\index{secret ballot} on a pressing issue, yet none has
time to meet in a particular location.  At the same time, because of the
sensitivity of the issue, each trustee would prefer to keep his vote
private.  The everyday solution of writing a vote on a piece of paper and
shuffling the sheets before counting the votes is physically impossible in
this setting; the trustees can only communicate over telephone lines,
perhaps using their workstations as well.  An electronic analog of the
paper-solution will not work: there may be no trusted party to count the
votes; electronic messages may be easily traced or duplicated.  We shall
see how to take a secret ballot, and how to conduct more general
distributed computations, in a simple, efficient, reliable, and secure
manner.

The unusual and key aspect to our methods is that we do not assume the
reliability of any particular processor or the availability of a central,
trusted host.  A cynical and paradoxical synopsis\index{thesis} of our
approach might be, ``Trust everyone, but trust no-one.''  In less ambiguous
terms, the community as a whole is reliable, but there is no particular
individual whose reliability is guaranteed.  Through ``democratic'' means,
we ensure that the majority rules, and as long as the majority is reliable,
the particular individuals who fail do not matter.  In fact, reliable
operations are ensured even without the need to identify faulty elements in
advance, or to restart entire computations when failures occur (malicious
or otherwise) and the offending components are cast out.

\medskip

We treat a distributed computation in a general manner as follows.  Say
that each of $n$ processors in a network holds a private input value $x_i.$
Together, they must compute\index{secret computation} some function
$F(x_1,\dots,x_n),$ without revealing anything about the inputs other than
what could be deduced from learning $F(x_1,\dots,x_n)$ alone.  In the
secret ballot example, a unanimous vote clearly reveals all the individual
votes, but this is allowable since it is leaked by the {\em result}, not as
a side effect of a protocol used to compute the result.  In other words,
the network must simulate a trusted external party who receives
$x_1,\dots,x_n,$ computes $F(x_1,\dots,x_n),$ and returns only the result.

Since some {\em arbitrary} collection of $t$ of the processors may be
faulty\index{fault tolerance}, a centralized solution will not suffice.
Our goal is to develop multiparty protocols to compute the result even
though some of the processors or communication lines may be unreliable in a
random or malicious manner.

Research into secure multiparty computations can be divided roughly along
the same lines as the rest of cryptographic research: classical,
information-theoretic security\index{information-theoretic security} {\em
vs.} the modern approach of complexity-based
cryptography\index{complexity-based cryptography}.  The classical approaches
to security examine secure communications under conditions where an
eavesdropper has unlimited computational resources at his disposal.  Few
methods withstand such strong requirements for security.  Fortunately,
requiring perfect, information-theoretic security may be unnecessary in
practical situations, if one is assured of some limitation on an
eavesdropper's or adversary's resources.  Diffie and Hellman
pioneered the modern approach of computational
complexity-based cryptography, in which the processors, reliable or
otherwise, are assumed to have bounded amounts of time and memory to
achieve their purposes, honest or otherwise
\cite{dh76}.

Each approach has its own appeal and its own disadvantages.
Information-theoretic cryptography guarantees protection of the
information against any adversary (random or malicious in the worst
possible way), but it may require unreasonable amounts of
communication or computation.  Complexity-based cryptography broadens
the range of secure information processing since it permits only weaker
adversaries, but most complexity-based results are based on unproven
assumptions about the intractability of problems like factoring large
numbers.

Based on unproven complexity-theoretic assumptions, inefficient methods for
performing a variety of multiparty computations have been developed
\cite{yao82,yao86,gmw86,gmw87,ghy87,hab88,bg89}.  Yao introduced the
idea of private function computation by presenting a method for two
cooperating individuals to compute a function $F(x,y)$ without having to
reveal $x$ and $y,$ given that the individuals are restricted to
polynomial-time computations \cite{yao86}.  Goldreich, Micali, and
Wigderson showed that any function $F$ described by a Boolean circuit $C_F$
can be computed reliably and securely as long as a majority of the
processors are reliable
\cite{gmw87}.  Galil, Haber, and Yung improved the efficiency and
implemented other desirable aspects
\cite{ghy87,hab88}.  
Figure~\ref{fig-crypto-history} describes some of the cryptographic
results, and some of the ``non-cryptographic'' ones, about multiparty
computations.


\figstretch
\begin{figure}[htb]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}   \hline
%%%%%%%%%%%%%%%%%%%%%%
Reference & Fault-Tol. & Crypto & 
Rounds & Message Size & Local Time \\ \hline \hline
%%%%%%%%%%%%%%%%%%%%%%
\cite{yao86} &
$t=1,n=2$ & yes & const & poly & poly \\ \hline
%%%%%%%%%%%%%%%%%%%%%%
\cite{gmw87} &
$t<n/2$ & yes & $Dn^2$ & poly & poly \\ \hline
%%%%%%%%%%%%%%%%%%%%%%
\cite{ghy87} &
$t<n/2$ & yes & $D$ & poly & poly \\ \hline
%%%%%%%%%%%%%%%%%%%%%%
\cite{bgw88,ccd88} &
$t< n/3$ & no & $D$ & poly & poly \\ \hline
%%%%%%%%%%%%%%%%%%%%%%
\cite{bb88} &
$t<n/3$ & no & $D/\log n$ & poly & poly \\ \hline
%%%%%%%%%%%%%%%%%%%%%%
\cite{bb88} &
$t<n/3$ & no & const & poss exp & poss exp \\ \hline
%%%%%%%%%%%%%%%%%%%%%%
\cite{br89,bea88-n2} & 
$t<n/2$ & no & $D$ & poly & poly \\ \hline
%%%%%%%%%%%%%%%%%%%%%%
\cite{bfkr89} &
$t < \log n$ & no & const & poly & poss exp \\ \hline
%%%%%%%%%%%%%%%%%%%%%%
\cite{bmr90} &
$t<n/2$ & yes & const & poly & poly \\ \hline
%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\end{center}
\caption{ \label{fig-crypto-history}
Various protocols for 2-party and $n$-party secure computations.
``Crypto'' indicates unproven complexity assumptions;
$D$ is the depth of a circuit $C_F$ for the function $F$ to be
computed; $n$ represents the number of players and the sizes of the inputs
(for clarity of presentation); ``poly'' means polynomially-bounded;
``poss exp'' means possibly exponential (depending on the complexity
of $F$).  The cost measures include 
fault-tolerance,
number of rounds of interaction, 
message size,
and local computation time.
Some of these results appear here.
}
\end{figure}
\figstretchend


%% \figstretch
%% \boxfig{
%% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}   \hline
%% %%%%%%%%%%%%%%%%%%%%%%
%% Reference &  \cite{yao82} & \cite{gmw87} & \cite{ghy87} &
%% \cite{bgw88,ccd88} & \multicolumn{2}{c}{\cite{bb88}}
%% & \cite{br89,complexity bea88-n2} & \cite{bfkr89} & \cite{bmr90} \\   \hline \hline
%% %%%%%%%%%%%%%%%%%%%%%%
%% Fault-Tol. & $t=1,n=2$ & $t<n/2$ & $t<n/2$ &
%% $t<n/3$ & $t<n/3$ &  $t<n/3$ & 
%% $t<n/2$ & $t < \log n$ & $t<n/2$ \\ \hline
%% %%%%%%%%%%%%%%%%%%%%%%
%% Unproven Assump. & yes & yes & yes &
%% no & no & no & 
%% no & no & yes \\ \hline
%% %%%%%%%%%%%%%%%%%%%%%%
%% Rounds & const & $Dn^2$ & $D$ &
%% $D$ & $D/\log~n$ & const & $D$ & 
%% const & const \\   \hline
%% %%%%%%%%%%%%%%%%%%%%%%
%% Message Size & poly & poly & poly & 
%% poly  & poly & poss exp & poly &
%% poly & poly \\  \hline
%% %%%%%%%%%%%%%%%%%%%%%%
%% Local Time &  poly & poly & poly & 
%% poly & poly & poss exp & poly &
%% poss exp & poly \\   \hline
%% %%%%%%%%%%%%%%%%%%%%%%
%% \end{tabular}
%% \caption{ \label{fig-history-crypto}
%% Various protocols for 2-party and $n$-party secure computations.
%% Here, $D$ is the depth of a circuit $C_F$ for the function $F$ to be
%% computed, $n$ represents the number of players and the sizes of the inputs
%% (for clarity of presentation), ``poly'' means polynomially-bounded,
%% ``poss exp'' means possibly exponential (depending on the complexity
%% of $F$).  The cost measures include 
%% fault-tolerance,
%% number of rounds of interaction, 
%% message size,
%% and local computation time.
%% Some of these results appear within.
%% }}
%% \figstretchend

The disadvantages to the early, cryptographic solutions are twofold.
First, because these methods are based on evaluating a circuit $C_F$
representing the function $F$ gate by gate, the amount of interaction may
become prohibitive.  We shall say more about this issue momentarily.

The second disadvantage lies in the set of assumptions\index{assumptions}
on which these solutions are founded.  Many assume that factoring large
numbers is difficult, or determining the discrete logarithm of a number
modulo some prime is hard; others rely on the general assumption that
one-way trapdoor functions exist, {\em i.e.} functions which are easy to
compute but hard to invert (one-way), but which are easy to invert given
additional, trapdoor information.  Though these protocols are apparently
secure given the current lack of efficient methods for factoring or
computing discrete logarithms and the like, an advance in the techniques
for solving these apparently intractable problems could destroy the
foundations on which the protocols are based.

Ben-Or, Goldwasser, Wigderson, Chaum, \crepeau, and \damgard have recently
introduced a new, ``non-cryptographic'' approach which circumvents the use
of unproven assumptions, replacing them with certain reasonable assumptions
about the network \cite{bgw88,ccd88}.  Namely, they assume that at most a
third of the processors between the processors are faulty, and that secure
pairwise communication lines are available.  In other words, let $t$ be a
bound on the number of faulty processors (for simplicity, regard a
processor as faulty if its communication lines are faulty).  As long as
$3t<n,$ any function $F(x_1,\dots,x_n)$ described by a Boolean circuit
$C_F$ can be computed reliably and securely in a complete network of $n$
processors with private communication lines.  Because the protocols are
based on circuit simulation using threshold schemes, the number of rounds
of interaction and the sizes of the messages involved are related to the
depth and size of $C_F.$

Since threshold schemes\index{threshold scheme} form the basis for many of
these protocols, let us digress for a moment to describe them.  Say that
one processor holds a private item of information, $s.$ It distributes this
secret among the network, sending values (known as ``pieces'') to each
processor $i,$ so that provided that at most $t$ processors fail, the
secret can be put together later.  The secret, however, must remain a
secret until then; no group of $t$ or fewer processors, even colluding and
malicious ones, can glean any information about $s$ from their pieces.
Shamir gave an elegant solution, known as secret sharing,%
\index{secret sharing}%
\index{secret sharing!polynomial}%
\index{secret sharing!Shamir}
based on
properties of random polynomials
\cite{sha79}.

The recent methods for secret computation are based on combining secretly
shared values to create new secretly shared values.  Say $x$ and $y$ have
been secretly shared among the system.  Using a protocol for addition or
multiplication, new secrets $u$ and $v$ can be constructed such that their
hidden values are $u=x+y$ and $v=xy.$ The new secrets have the same
reliability and secrecy properties as secrets which have been distributed
by some dealer, but there no longer need be a dealer who knows the hidden
values of $u$ and $v.$

By evaluating the Boolean circuit $C_F,$ a new secret $w$ whose hidden
value is $F(x_1,\dots,x_n)$ is constructed.  The use of secret sharing is
essential to hiding the intermediate values, which could reflect
information about the inputs which should not be revealed.  Most multiparty
protocols, cryptographic or not, revolve around interactively simulating a
circuit gate by gate, following a procedure introduced in \cite{gmw87}.
Thus, the communication complexity of most protocols is directly related to
the computational (circuit) complexity of $F.$ In concrete programming
terms, the number of rounds of interaction is proportional to the time that
a centrally-run program would take to compute $F.$

Even for useful functions having reasonable circuit depth, the number of
rounds of interaction becomes prohibitive in a practical sense.  Because
communication is a bottleneck in distributed computations, protocols with
high communication complexity are at a great disadvantage.  The overhead of
ensuring security by using these methods counteracts the advantages of
computing distributively, even to the point of making simple computations
too expensive to perform.

\section{The Communication Complexity of Secure Computation}

We examine a new measure of communication complexity:\index{communication
complexity} the {\em communication complexity of secure computation}, which
measures the number of rounds of interaction and the number of bits sent
during a protocol which computes a function {\em reliably} and {\em
securely}.  Developing secure and practical protocols with small
communication complexity is the primary focus of this dissertation.

We may contrast the communication complexity of secure computation with the
standard measure of communication complexity as follows.  If we relax the
demand for security, any function has a ``small'' communication complexity:
each processor simply broadcasts its input $x_i,$ and then individually
computes $F(x_1,\dots,x_n)$ from the messages it received.  (Technically,
we have ignored an important issue, namely how to achieve broadcast
reliably using private communications, but this problem, known as Byzantine
Agreement, has efficient solutions.)  Thus, few rounds and small messages
would suffice.

It is reasonable to expect that more and longer messages may be required to
hide information otherwise leaked by a direct approach.  This expectation
holds for the particular protocols mentioned earlier, and even led some
authors to conjecture that the circuit depth of a function is a lower
bound on the number of rounds needed for secret computation.

We disprove that conjecture with our first result \cite{bb88}, which is the
first to address the issue of communication complexity in secure
computation: any circuit of depth $D$ can be evaluated in $O(D/ \log n)$
rounds using small messages.  For all functions in $NC^1$ (or more
generally for any function admitting a circuit of polynomial size and
logarithmic depth), this result gives protocols which operate in a small,
constant number of rounds.  

For example, consider a secret ballot over a legal measure which will pass
only if there is a two-thirds majority.  There is a simple and efficient
protocol which operates in constant rounds regardless of the number of
voters, to determine if the law is passed, without revealing the individual
votes or even the exact tally.  A variety of useful functions becomes
efficiently computable using our techniques.

An even stronger and more surprising statement can be made if one is
willing to permit fewer than $O(\log n)$ faults in the network, as opposed
to the most general bound of $n/2$ or $n/3:$
\begin{quote}
\begin{singlespace}
{\em Any\/} function, {\em regardless\/} of its circuit depth or size, can
be computed in a {\em constant\/} number of rounds of interaction and using
small messages.
\end{singlespace}
\end{quote}
This is a very surprising result: the communication complexity of secure
computation need not be related to the computational complexity of the
function being computed.  It lends great hope to the practical
implementation of methods for distributed security, since communication is
an expensive resource.

At the risk of basing protocols on unproven complexity-theoretic
assumptions, we show also that the goal of achieving constant-round
protocols to compute functions of arbitrary circuit depth can be achieved
at the higher levels of fault-tolerance ($2t < n$).

The common idea underlying many of our protocols is the following: to
compute a function in a distributed manner, convert it to several problems
that can be computed locally and then combined to give the solution,
despite errors in some of the local computations.  The key, however, is to
ensure that each locally computed problem is independent of the original to
a certain degree, which hides information about the original problem and
its answer and simultaneously provides a degree of resilience against local
errors.  The brunt of the computation is placed on local computations
rather than communications.

These are important tools for practical methods for distributed security
and reliability.  With ample levels of fault-tolerance, and using small
messages, the number of rounds of interaction is reduced greatly.

\section{Fault Tolerance}

The non-cryptographic protocols of \cite{bgw88,ccd88} tolerate faults in a
third of the network, namely $3t<n.$ It is not difficult to show that a
majority of faults is intolerable ({\em e.g.} the AND function cannot be
computed by a half-faulty network \cite{bgw88}).  This left a gap between
the achievable $3t<n$ bound and the $2t \leq n$ impossibility result.

We close the gap, showing that as long as the number of faults satisfies
$2t<n,$ any circuit can be evaluated securely and reliably.  The crucial
discovery that supports the tight bound on fault-tolerance relies on a
simple problem which we call the {\em ABC Problem}: one processor must share
three secrets, $a,$ $b,$ and $c,$ and then prove that $ab=c$ without
revealing any other information.

Our solution is simple and efficient, and supports secret computations
based on arithmetic over exponentially large ($n$-bit) fields (such as the
set of integers modulo $m,$ where $m$ is an $n$-bit prime).  A similar but
less efficient result was obtained independently by Ben-Or \cite{br89}; in
contrast, that solution uses bitwise operations which would require $O(n
\log n)$ times as many rounds for the same arithmetic.  Both methods rely
on a recent technique by Rabin \cite{tr88} for verifiable secret sharing
without using cryptographic assumptions.  ({\em Verifiable} secret sharing
has the added property that all nonfaulty processors are assured that the
secret is well-defined and reconstructable even when the dealer of the
secret may be faulty.)

\paragraph{Zero-Knowledge Proof Systems}

Our solution to the ABC problem also provides a fast and efficient way for
one processor to prove that a general property holds on a string of bits, 
without having to reveal the proof.

Goldwasser, Micali, and Rackoff \cite{gmr89} and Babai \cite{bm88} pioneered
the concept of zero-knowledge proof systems, in which one party, the
prover, attempts to convince another party, the verifier, that a string
$x$ is in a particular language $L.$ The verifier learns whether $x \in L,$
but as in the multiparty protocols discussed above, he learns nothing more
than that result.  Presumably the prover has far greater power to
prove language membership, while the verifier is limited to
polynomial time computations.

A similar but distinct kind of proof system involves committed strings,
and is similar to the ABC problem described above.
Say that the prover can place bits in envelopes and seal them, so that the
verifier cannot read the bits but the prover cannot change them before
opening the envelopes at some future time.  In this case, the prover
commits to a string of bits $x,$ and then proves to the verifier that $x
\in L,$ without revealing the bits in $x.$  

We give a formulation of both types of zero-knowledge proofs for a network
of processors.  Assuming that a majority of individuals are reliable, we
show that a prover can prove membership in {\em any} language in
$\ip$\index{interactive proof system!IP} 
(the class of languages with polynomial-time 2-player proof
systems) without having to know which processors are reliable.  Our result
applies to both flavors of proof systems, proving statements about known
strings and proving statements about hidden but committed strings.

Thus, if the prover, the verifier, and a third party are present, the
prover is assured that his proof leaks no additional information, as long
as {\em either} the verifier {\em or} the third party is reliable.

Multiparty zero-knowledge proof systems are distinct from the related idea
of Goldwasser {\em et al} \cite{bgkw88}, who examine two-{\em prover} proof
systems in which provers are kept physically separate.  Here, we allow
communication between all processors, where just one of them is a prover.

\section{Locally Random Reductions}

We develop a powerful new tool called a {\em locally random reduction}%
\index{locally random reduction}
to achieve many of the results mentioned above, along with other results we
shall describe in a moment.  A {\em random reduction} from the problem of
computing some function $f(x)$ to the problem of computing another function
$g(y)$ is a pair of probabilistic, polynomial-time algorithms $P$ and $Q.$
By computing $P(x),$ one obtains a list of values $(y_1,\dots,y_m)$ at
which to evaluate $g.$ The results are interpolated to determine $f(x)$ by
evaluating $Q(g(y_1),\dots,g(y_m)).$ The reduction is {\em $(k,m)$-locally
random} if for any subset $S$ of the $y$'s such that $\abs{S} \leq k,$ the
distribution on $\set{y_i \mid i \in S}$ induced by $P$ is the same,
regardless of $x.$

This new tool has widespread applications.  It forms the basis of a theory
for program testing\index{program testing} developed by Lipton
\cite{lip89}, who also observed that, using our general technique for
LRR's, the {\sc Permanent} function has a locally random reduction.  Blum,
Levin, and Luby \cite{bll89} used it to show that if the {\sc Permanent}
function is computable on average in polynomial time with a uniform
distribution, then ${\#}P \subseteq \mbox{ZPP}.$ Nisan \cite{nis89-cosat}
showed that any language in the polynomial time hierarchy admits a
two-prover interactive proof system; subsequently, Fortnow, Lund, Karloff,
and Nisan \cite{lfkn89} showed that 
$\mbox{PH} \subseteq \ip.$\index{interactive proof system!IP}
Previously, it was not known whether even coSAT admitted interactive
proofs.  Finally, Shamir \cite{sha89} solved a fundamental open question,
showing $\mbox{IP} = \mbox{PSPACE}.$%
\index{interactive proof system!IP}%
\index{interactive proof system!IP=PSPACE}
The algebraic approach of locally random reductions has sparked quite a bit
of interesting results in cryptography and complexity theory.

We apply locally random reductions to several problems in cryptography
including the secure multiparty computations and zero-knowledge proof
systems described above.  As mentioned, the communication complexity of
secure computation can be made independent of the computational complexity
of the function.  Locally random reductions serve this purpose by allowing
us to move the computational effort needed to compute the function from the
communication lines to the local processors, thus removing a serious burden
of secure protocols.

Locally random reductions were inspired by the problem of {\em
instance-hiding schemes}\index{instance-hiding scheme} \cite{afk89,bf90}: a
weak processor, $A,$ wishes to utilize the computational resources of
powerful oracles $B_1,\dots,B_m,$ in order to compute an intractable
function $f(x).$ The weak processor does not, however, want to reveal
anything about $x.$ We show that, using a $(1,m)$-LRR (defined in
Chapter~\ref{chap-lrr}), any function of $m$ bits has an instance-hiding
scheme.

\section{Extreme Fault-Tolerance}

\paragraph{Privacy Without Cryptographic Assumptions}

We have mentioned that general computations are impossible when fault
levels constitute a majority of the network.  To understand better the
nature of privacy in distributed computations, we examine protocols
tolerating greater numbers but strictly weaker types of faults.  In fact,
let us assume that no processor fails at all, but that some number $t$ of
them may pool their information to attempt to glean information that should
remain private.  What sorts of functions can be computed {\em privately}
when $2t \geq n,$ without making unproven assumptions?

We take a first step in this direction by completely characterizing the
functions $f$ which can be computed privately by $n=2$ parties, any $t=1$
of which may ``collude.''  That is, for general functions of two arguments,
we give a straightforward method to determine if $F$ is privately
computable.  This result was obtained independently (with an incorrect
proof) by Kushilevitz \cite{k89}.  For the case of $n \geq 2,$ Chor and
Kushilevitz \cite{ck89} showed that a very limited subset of the class of
Boolean valued functions are privately computable\index{private function}
for $2t \geq n.$ The generalization to general-valued functions of several
arguments remains open.

\paragraph{Privacy and Reliability With Cryptographic Assumptions}

Not only are most functions impossible to compute with perfect security
when $2t \geq n,$ but an issue of fairness arises.  In general, if a
majority of participants halt, the whole computation must come to a halt.
A faulty majority can therefore halt just after learning the result of the
computation, and just before the nonfaulty participants learn the result.

By restricting the processors and the adversarial processors to
polynomial-time computations, we give new protocols which solve both of
these problems, making the weakest possible unproven cryptographic
assumption in this case, that a protocol for two-player Oblivious Transfer
exists.  A processor with unbounded resources
could break encryption schemes; thus we do not violate the impossibility of
perfect secrecy.

The important aspect of computations with a faulty majority is the issue of
fairness.  Yao \cite{yao86} and Galil, Haber, and Yung \cite{ghy87} proposed a
definition which did not allow the adversary to have access to the programs
of the nonfaulty processors, and gave cryptographic solutions under these
circumstances.  We formulate a stronger definition, allowing the adversary
access to the programs of the reliable processors, and which we believe
best captures the notion of fairness in a quantitative and intuitive sense.
Furthermore, we are able to achieve this stronger property of fairness.

In addition to developing extremal protocols based on cryptographic
assumptions, we consider instead a network equipped with ``noisy''
channels, namely channels which allow messages to pass with a 50-50 chance.
We give alternative protocols which utilize these channels instead of
depending on unproven assumptions, showing that fairness, privacy, and
correctness are achievable even when faults abound.

\section{Definitions and Formal Proofs}

In order to prove that protocols are correct and private, a formal model
for distributed protocols and the adversaries that represent the faulty
behavior of the participants is needed.

While the current literature contains many new techniques, it often omits
any mention of an underlying formal model for security, often giving only
intuitive arguments for the claimed results.  While intuitive arguments are
satisfactory to the cursory reader, and ideal for the fast dissemination of
results, the lack of formal proofs undermines any assurance that the
methods do provide security and fault-tolerance.  Furthermore, with the
variety of assumptions and network characteristics used by the various
solutions, it is difficult to compare the advantages of one over another.

The formulation of a rigorous and coherent model is a primary contribution
of this dissertation.  The computational power of the participants and the
adversaries, the available communication channels, the assumptions made to
ensure secrecy, the nature of the adversaries, the definitions of
correctness, privacy, and fairness, all require a formal and explicit
treatment.  We give a framework to define and prove various properties of
the networks and the protocols, enabling one to compare what is achievable
across the range of network characteristics and assumptions made.
In keeping with the historical trend of cryptography, we provide a model
which supports an analysis of perfect, information-theoretic security, yet
is adaptable to the modern approach of computational complexity-based
cryptography.

But our work goes far beyond the mere clarification of mechanical
specifications of interactions --- which, though necessary for formal
proofs of resilience, are less than stimulating.  We address the difficult
and often subtle problem of giving formal definitions for properties such
as correctness and privacy, issues that seem so intuitively easy that
common sense often leads down the wrong path.  The research literature is
filled with {\em ad hoc} properties and with attempts to formalize each of
them.  Few definitions are satisfactory, and because of their {\em ad hoc}
nature, few attempts to actually prove claims to security and reliability
appear.

We give a surprisingly simple and coherent definition of {\em resilience}
(see \ref{def-resil} in \S\ref{sec-resil}), a combination of security
and reliability that unifies the various properties that one desires in a
multiparty computation.  The subtle and key aspect of our approach is to
avoid analyzing each desired property of a protocol separately, instead
giving a single definition from which all properties arise.  In a nutshell:
a real multiparty protocol is intended to achieve the results that an {\em
ideal} protocol having a trusted host would achieve, and the information
and influence of an adversary must be no greater than that in the ideal
case.  We define rigorously what it means to ``achieve the same results,''
giving a general and powerful tool for measuring the accomplishments of one
protocol against those of another.


\section{Applications}

The protocols we provide achieve secure and reliable distributed
computations of arbitrary functions $F(x_1,\dots,x_n).$  We demonstrate how
this abstraction can fit in with practical goals.

We develop some efficient applications to practically-motivated problems.
For example, we give a fast method for a processor to authenticate itself
and to authorize its transactions.  We provide a quick protocol to deliver
mail anonymously, protecting the identity of the sender and even of the
receiver.  We describe a reliability mechanism which resists traffic
analysis, by hiding not just the results of its computations but the nature
of the computations themselves ({\em e.g.} whether it is idle or processing
a request for a file, etc.).

\section{Summary}

We develop a host of communication-efficient protocols to achieve optimally
fault-tolerant and secure distributed computations.  
%Let $F(x_1,\dots,x_n)$ be a function described by a circuit $C_F.$
Figure~\ref{fig-our-results} describes the various combinations and
trade-offs in rounds, message sizes, and the computational complexity of
the desired computations.


\begin{figure}
\begin{tabular}{|c|c|c|c|c|} \hline
Faults & Rounds & Bits & Local Time & Function Class \\ \hline
$t < n/2$ & $\mbox{depth}(C_F)/\log n$ & poly & poly & 
P (or poly-size circuits) \\ \cline{2-5}
& constant & poly & poly & $NC^1$ (or log-depth circuits) \\ \cline{3-5}
& & exp & size($C_F$) & any $C_F$ \\ \cline{1-5} 
$t = O(\log n)$ & constant & poly & exp & any $C_F$ \\ \hline
\end{tabular}
\caption{\label{fig-our-results}
Various tradeoffs in communication complexity, fault-tolerance, 
and function-complexity for the results developed here.
}
\end{figure}

We give the first protocol to achieve a secure multiparty computation using
a number of rounds less than the circuit depth of the function to be
computed.  In fact, we give the first protocols that use only a constant
number of rounds.

Our protocols are proven secure and reliable using a concise and precise
set of formal definitions.  The formulation of these definitions is a major
contribution of this dissertation and provides a clear and general basis
for proving the resilience of other protocols in the literature.

We investigate fault tolerance when faults constitute a majority of the
network.
We characterize the class of functions which are privately computable
against a passive adversary.
We give a strong formal definition for fairness when the faults are
Byzantine, and show how to achieve it using additional assumptions.

We develop a powerful new tool, the {\em locally random reduction}, which
has broad applications.  It reduces the communication complexity of many
secure protocols drastically, regardless of the computational complexity of
the computation the protocol attempts to achieve.  It provides a solution
to the problem of utilizing powerful public resources without compromising
privacy.  It has inspired applications to program testing and interactive
proof systems and led to several fundamental new results.


%% \paragraph{Organization of the Dissertation}
%% 
%% Each chapter begins with a verbal description of the problems and their
%% solutions, along with pseudo-code specifications of the protocols, and a
%% readable justification of correctness and privacy.  The necessary but less
%% palatable formal proofs follow.
%% 


==> lrr.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% lrr.tex                    Locally Random Reductions.
%
%                            Copyright @1989  Donald Beaver.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{=======}
\typeout{lrr.tex}
\typeout{=======}

\chapter{Locally Random Reductions}
\label{chap-lrr}

\chapquote{
However, this bottle was {\em not} marked ``poison,'' so Alice
ventured to taste it, and finding it very nice (it had, in fact, a
sort of mixed flavour, of cherry-tart, custard, pine-apple, roast
turkey, toffee, and hot buttered toast), she very soon finished it
off.

``What a curious feeling!'' said Alice.  ``I must be shutting up like
a telescope.''

And so it was indeed: she was now only ten inches high, and her face
brightened up at the thought that she was now the right size for going
through the little door into that lovely garden.
}{
Lewis Carroll, {\em Alice's Adventures in Wonderland}}

Locally random reductions are a new class of reductions from one
computational problem to another.  Inspired by the problem of {\em
instance-hiding schemes} (presented in Chapter~\ref{chap-ihs}), locally
random reductions have found a broad variety of applications since their
introduction by Beaver and Feigenbaum.  These results include methods for
program testing \cite{lip89,blr89} and the surprising result that
$\ip=\pspace$\index{interactive proof system!IP=PSPACE} 
\cite{sha89}.  We describe some of these
important subsequent developments in \S\ref{sec-lrr-subsequent}, and show
how LRR's drastically reduce the communication complexity of zero-knowledge
proof systems and secure multiparty protocols in Chapters
\ref{chap-zkp} and \ref{chap-mpp}.

Reductions from one language to another are fundamental to complexity
theory.  One can reduce the problem ``is $x \in L_1?$'' to solving the problem
``is $y \in L_2?$'' if there is an efficiently computable function $P$ such
that $x \in L_1 \Leftrightarrow P(x) \in L_2.$ A reduction from a {\em
function} $f(x)$ to another function $g(y)$ similarly maps an instance $x$
in the domain of $f$ to an instance $y=P(x)$ in the domain of $g.$  It also
requires that the value of $g(y)$ be {\em interpolated} to obtain the
answer: $f(x) = Q(g(y)).$

In general, a reduction from $f$ to $g$ can produce several
instances $y_1,\dots,y_m$ at which to evaluate $g,$ and need not
generate these instances deterministically.  Let $X$ be the domain of
$f$ and $Y$ be the domain of $g.$

\begin{definition}
A {\em random reduction} from $f(x)$ to $g(y)$ is a pair of
probabilistic, polynomial time algorithms $(P,Q)$ satisfying the
following properties:
\begin{description}
\item[(Reduction)]
$P : X \rightarrow \dist(Y^m \times \sigstar),$ that is, the querying
algorithm $P$ produces a sample $(y_1,\dots,y_m,\sigma)$ according to
distribution $P(x),$ where each $y_i$ is in the domain of $g,$ and $\sigma$
is a string.
\item[(Interpolation)]
If $(y_1,\dots,y_m,\sigma)$ has nonzero weight in the distribution $P(x),$
then the interpolation algorithm gives $Q(g(y_1),\dots,g(y_m),\sigma) =
f(x).$
\end{description}
\end{definition}

The term {\em locally random} refers to the distributions on subsets of the
queries $y_1,\dots,y_m$ produced by $P(x).$ In a certain sense, it
generalizes the idea of secret-sharing, in that secret-sharing ensures a
uniform distribution on sufficiently small subsets of pieces, regardless of
the secret.  Here, we should like that the distributions on subsets of the
pieces must be the same for any $x$ of a given size $n,$ even though it
need not be {\em uniform,} as it is in the case of secret sharing.

\begin{definition}
Let $B \subseteq \set{1,\dots,n}.$  Then $D_x^B$ denotes the distribution on 
$\set{y_i \mid i \in B}$ induced by $P(x).$
\end{definition}

\begin{definition}
A {\em $(k(n),m(n))$-locally random reduction} (LRR) from $f(x)$ to $g(y)$
is a random reduction $(P,Q)$ satisfying:
\begin{itemize}
\item
$P(x)$ produces $m(n)$ queries on inputs of size $n;$
\item
For all $n,$ for all subsets $B\subseteq \set{1,\dots,n}$ of size
$\leq k(n),$ the distribution $D_x^B$ is the same for all $x$ of size
$n.$
\end{itemize}
\end{definition}

\begin{exampleenv}
The {\em discrete logarithm} function, $\mbox{DLOG}_{g,p}(x),$ was defined
in Definition~\ref{def-dlog}.  No efficient algorithm for computing DLOG is
known.  The random-self-reduction given for $DLOG$ is in fact a
$(1,1)$-locally random reduction: it produces one query $y=xg^r,$ and the
distribution on query sets of size $\leq 1$ is the same for every $x.$
\end{exampleenv}

\begin{exampleenv}
For illustration, let us demonstrate a $(10,21)$-locally random reduction
from the multiplication function to itself.  Let $f(x_1,x_2) = x_1 x_2,$
over ${\bf Z}_{p_n}$ for concreteness.  Let $g(x_1,x_2) = x_1 x_2.$
We reduce $f$ to $g$ via $(P,Q)$ as follows.

The querying algorithm $P(x_1,x_2)$ chooses
$a_1,\dots,a_{10},b_1,\dots,b_{10} \in {\bf Z}_{p_n}$ uniformly at random,
and sets $p_1(u)=a_{10}u^{10}+\cdots+a_1 u+x_1$ and
$p_2(u)=b_{10}u^{10}+\cdots+b_1 u+x_2.$ It computes $y_i = (p_1(i),p_2(i))$
for each $1 \leq i \leq 21.$ 
%It also outputs a string $\sigma$ containing
%all the coefficients $a_1,\dots,a_{10},b_1,\dots,b_{10}.$

The interpolation algorithm $Q(z_1,\dots,z_{21},\sigma)$ does just that: it
interpolates the polynomial $q(u)$ of maximal degree 20 passing through the
points $(i,z_i)$ for $1\leq i \leq 21.$  It returns the value $q(0).$

To see that the reduction is correct, observe that $g(p_1(i),p_2(i)) =
p_1(i)p_2(i) = q(i)$ for $1 \leq i \leq 21,$ and both $g(p_1(u),p_2(u))$
and $q(u)$ are polynomials of maximal degree $20.$  By elementary algebra,
$g(p_1(u),p_2(u))=q(u),$ hence $g(p_1(0),p_2(0))=q(0).$

To see that the reduction is (10,21)-locally random, note that because the
coefficients of $p_1(u)$ and $p_2(u)$ are chosen uniformly at random, the
distribution on any $10$-set of values of $p_1(u)$ or $p_2(u)$ is uniform
over $({\bf Z}_{p_n})^{10}$ regardless of $x_1$ and $x_2.$ Thus for any
subset $B$ of $10$ or fewer queries, $D_{x_1,x_2}^B$ is the same for any
$(x_1,x_2).$
\end{exampleenv}

\bigskip

The main results of this chapter are twofold: the first shows the existence
of locally random reductions for polynomials $f(x_1,\dots,x_m)$ and the
second for arbitrary boolean functions.  These reductions inspire a variety
of applications from program testing to interactive proofs to secure
distributed protocols.

\begin{theorem} \label{thm-lrr}
~
\begin{itemize}
\item[a.]
For any {\em polynomial} $f(x_1,\dots,x_n)$ of degree at most $n$ over some
field $E,$ there is a $(1,n+1)$ locally random reduction from $f$ to
itself.
\item[b.]
For any {\em boolean} function $f(x),$ there exists a $(1,n+1)$ locally
random reduction from $f(x)$ to some function $g(y).$ In particular, for
any field of size exceeding $n+1,$ $g(y)$ can be taken to be a polynomial
$c_f(x_1,\ldots,x_m)$ of degree $n$ over that field.
\end{itemize}
\end{theorem}

\begin{proof}
See Lemmas \ref{lem-lrr-poly-basic} and \ref{lem-lrr-boole-basic},
proved below in \S\ref{sec-lrr-poly-basic} and
\S\ref{sec-lrr-boolean-basic}.
\end{proof}

In fact, a stronger statement is achievable:

\begin{theorem} \label{thm-lrr-improve}
~
\begin{itemize}
\item[a.]
For any {\em polynomial} $f(x_1,\dots,x_n)$ of degree at most $n$ over some
field $E,$ for any $d(n),$ and for any constant $c>0,$ there is a $(d,dn/(c
\log n))$ locally random reduction from $f$ to a polynomial 
$h_f(w_1,\ldots,w_{n^{c+1}/(c \log n)})$ of degree $n/(c\log~n)$ 
over that field.
\item[b.]
For any {\em boolean} function $f(x),$ for any $d(n),$ and for any constant
$c>0,$ there exists a $(d,dn/(c \log n))$ locally random reduction from
$f(x)$ to some function $g(y).$ In particular, for any field of size
exceeding $(dn/(c \log n)),$ $g(y)$ can be taken to be a polynomial
$h_f(w_1,\ldots,w_{n^{c+1}/(c \log n)})$ of degree $n/(c\log~n)$ over that
field, where each $w_i$ itself is a product of at most $O(\log~n)$ variables
$x_i.$
\end{itemize}
\end{theorem}

\begin{proof}
See Lemmas \ref{lem-lrr-poly-more} and \ref{lem-lrr-boole-more}.
\end{proof}



\section{LRR's for Multivariate Polynomials}
\label{sec-lrr-poly-basic}

\begin{lemma} \label{lem-lrr-poly-basic}
For any {\em polynomial} $f(x_1,\dots,x_n)$ of degree at most $n$ over some
field $E,$ there is a $(1,n+1)$ locally random reduction from $f$ to
itself.
\end{lemma}

\begin{proof}
We assume without loss of generality that $\abs{E} > n+1$ (otherwise, we
may use an extension field).  The query function $P(x_1,\dots,x_n)$ is
described in Figure~\ref{fig-query-poly}, and the interpolation function
$Q(z_1,\dots,z_{n+1})$ is described in Figure~\ref{fig-interp-poly}.  
By Lemma~\ref{lem-lin-share}, the
distribution $D_{x_1,..,x_n}^{i}$ is 
uniform on $E^n$ for all assignments to $x_1,\ldots,x_n.$

\figstretch
\boxfig{  
\noindent{\bf \lrrPbasic}
\begin{itemize}
\item
Choose $a_1,\dots,a_n \in E$ uniformly at random, and set
$p_1(u)=a_1 u +x_1, 
p_2(u)=a_2 u +x_2, 
\dots, p_n(u)=a_n u +x_n.$
\item
Set $y_i \leftarrow (p_1(i),\dots,p_n(i))$ for $1 \leq i \leq n+1.$
\end{itemize}
\caption{\label{fig-query-poly}
Query function $P(x_1,\dots,x_n)$ for self-reducing the multivariate
polynomial $f(x_1,\dots,x_n).$ 
}}
\figstretchend

The interpolation function $Q$ is easy to specify: given $n+1$ values
$z_1,\dots,z_n,$ interpolate the polynomial $q(u)$ of degree $n$ running
through the $n+1$ points.  Return $q(0).$ That this reduction is correct
can be verified by simple algebra: $f(p_1(u),\ldots,p_n(u))$ and $q(u)$ are
both polynomials in $u$ of degree $n.$ They agree at $n+1$ points
($q(i)=f(p_1(i),\ldots,p_n(i)),$ $1\leq i \leq n+1$).  They must therefore
be identical, so $q(0)= f(p_1(0),\ldots,p_n(0)) = f(x_1,\ldots,x_n).$

\figstretch
\boxfig{  
\noindent{\bf \lrrQbasic}
\begin{itemize}
\item
Interpolate the polynomial $q(u)$ passing through $(i,z_i)$ for $1\leq i
\leq n+1.$
\item
Return $q(0).$
\end{itemize}
\caption{\label{fig-interp-poly}
Interpolation function $Q(z_1,\dots,z_{n+1})$
for self-reducing the multivariate polynomial $f(x_1,\dots,x_n).$
}}
\figstretchend
\end{proof}

\section{LRR's for Boolean Functions}
\label{sec-lrr-boolean-basic}

\begin{lemma} \label{lem-lrr-boole-basic}
\index{locally random reduction!boolean}
For any boolean function $f(x),$ there exists a $(1,n+1)$ locally random
reduction on inputs of size $n$ from $f(x)$ to some function $g(y).$ In
particular, for any field of size exceeding $n+1,$ $g(y)$ can be taken to
be a polynomial $c_f(x_1,\ldots,x_n)$ of degree $n$ over that field.
\end{lemma}

\begin{proof}
By Lemma~\ref{lem-can-f-bool-poly},
every function $f$ on inputs of length $n$
can be expressed as a polynomial $c_f$ of degree $n$ over an arbitrary
field $E,$ such that when the variables $x_1,\ldots,x_n$ are assigned
values in $\set{0,1}$ that match $x,$ $c_f(x_1,\ldots,x_n) = f(x).$

By Lemma~\ref{lem-lrr-poly-basic}, then, $c_f$ is $(1,n+1)$-locally-random
reducible to itself, which implies that $f$ is $(1,n+1)$-locally-random
reducible to $c_f.$
\end{proof}


\section{Reducing the Number of Queries}
\label{sec-lrr-more}

By an appropriate change of variables, we can decrease the number of
queries needed to reduce a polynomial to itself by a logarithmic factor
(and, correspondingly, to reduce a boolean function to a polynomial).

\begin{lemma}    \label{lem-change-vars}
\index{locally random reduction!fewer queries}
Every polynomial $f(x_1,\dots,x_n)$ of degree $n$ is expressible as a
polynomial $h_f(w_1,\dots,w_N)$ of degree $\frac{n}{\log n}$ over new
variables $w_1,\dots,w_N,$ where $N = n^2/\log~n,$ and each variable $w_i$
is a product of at most $\log n$ of the $x$-variables.
\end{lemma}

\begin{proof}
Express $f$ as a weighted sum of its monomials:
\[
f(x_1,\dots,x_n) = 
\sum_{\epsilon} c_{\epsilon} \prod_{i=1}^n x_i^{\epsilon(i)}
\]
where $\epsilon : \set{1,\dots,n} \rightarrow \set{0,1}$ indicates whether
variable $x_i$ is in a given monomial of $f,$ and $c_{\epsilon}$ is 0 or 1
according to whether the monomial represented by $\epsilon$ appears in $f.$
The sum is taken over all possible $\epsilon.$ We group the $x$'s into
blocks of size $\log n$ and assign a variable $w$ to every product of a
combination of $x$'s taken from a single block.  For example, if
$n=16,$ then we take blocks $\set{x_1,x_2,x_3,x_4},
\set{x_5,x_6,x_7,x_8},
\set{x_9,x_{10},x_{11},x_{12}},
\set{x_{13},x_{14},x_{15},x_{16}},$
and we take $w_1=1, w_2=x_1, w_3=x_2, w_4=x_2x_1,w_5=x_3,\ldots,
w_{256}=x_{13}x_{14}x_{15}x_{16}.$
Defining
\[
\psi(b,\epsilon)  = 
bn + \sum_{i=1}^{\log n} 2^{i-1} \epsilon(i + (b-1) \log n),
\]
for block number $b$ in the range $\set{1,\dots,\frac{n}{\log n}},$ 
we have the correspondence
\[
w_{\psi(b,\epsilon)}   = 
\prod_{i=(b \log n)+1}^{(b+1)\log n}  x_i^{\epsilon(i)}.
\]
Then $f$ is expressed in terms of the new variables as
\[
f(x_1,\dots,x_n) =
h_f(w_1,\dots,w_N) \equiv
\sum_{\epsilon} c_{\epsilon} 
\prod_{b=1}^{n/\log~n}  w_{\psi(b,\epsilon)}
\]
It is not hard to see that $h$ has degree $\frac{n}{\log n}$ over
$N=n^2/\log~n$ variables.
\end{proof}


\begin{lemma} \label{lem-lrr-poly-more}
\index{locally random reduction!polynomial}
For any {\em polynomial} $f(x_1,\dots,x_n)$ of degree at most $n$ over some
field $E,$ for any $d(n),$ and for any constant $c>0,$ there is a $(d,dn/(c
\log n))$ locally random reduction from $f$ to a polynomial 
$h_f(w_1,\ldots,w_{n^{c+1}/(c \log n)})$ of degree $n/(c\log~n)$ 
over that field.
In particular, a polynomial $h_f(w_1,\dots,w_N)$
of degree $n/(c\log~n)$ suffices, where $N=\frac{n^{c+1}}{c\log~n}.$
\end{lemma}

\begin{proof}
The idea behind the reduction is to decrease the degree of $f$ to
$n/(c\log~n),$ and then to use random polynomials of degree $d$ to hide the
variables. Assume WLOG that $c\log~n$ divides $n.$

By an easy extension of Lemma~\ref{lem-change-vars}, there exists a
polynomial $h_f(w_1,\dots,w_N)$ of degree $n/(c\log~n)$ in
$N=n^{c+1}/(c\log~n)$ variables.  Given $x_1,\dots,x_n,$ computing
$w_1,\dots,w_N$ is an easy $NC^1$ computation: simply multiply together all
the $x_j$ appearing in the monomial corresponding to $w_i,$ for each $w_i.$

Instead of choosing linear polynomials as in the proof of
Lemma~\ref{lem-lrr-poly-basic}, the query algorithm \lrrPlogn selects
uniformly random polynomials $p_1(u),\dots,p_n(u)$ of degree $d$ subject to
$p_1(0)=w_0,\dots,p_N(0)=w_N.$ It then generates
$y_i=(p_1(i),\dots,p_N(i))$ for $1 \leq i \leq dn/(c\log~n).$

On input $z_1,\dots,z_{1+dn/(c\log~n)},$ \lrrQlogn interpolates the points
$(i,z_i)$ to a polynomial $q(u)$ of degree $dn/(c\log~n)$ and returns
$q(0).$

Correctness is satisfied through straightforward algebra:  $q(u)$ and
$h_f(p_1(u),\dots,p_N(u))$ have degree $dn/(c\log~n)$ and agree at
$1+dn/(c\log~n)$ points, so they are identical;
\[
q(0) = h_f(p_1(0),\dots,p_N(0))
= h_f(w_0,\dots,w_N) = f(x_1,\dots,x_N).
\]

Any $d$-subset of the $y_i$'s contains $d$ values on each polynomial
$p_1(u),\dots,p_N(u).$ By Lemma~\ref{lem-ss} these values are distributed
uniformly over $E^d$ for any $w_1,\dots,w_N;$ that is, for any
$x_1,\dots,x_n.$

The extra ``+1'' in the number of queries is removed by
instantiating $w_0$ to 0 and then to 1 (see the proof of
Theorem~\ref{theorem-model1} in Chapter~\ref{chap-ihs}), generating queries
that are twice as long.
\end{proof}


\begin{lemma} \label{lem-lrr-boole-more}
For any {\em boolean} function $f(x),$ for any $d(n),$ and for any constant
$c>0,$ there exists a $(d,dn/(c \log n))$ locally random reduction from
$f(x)$ to some function $g(y).$ In particular, for any field of size
exceeding $(dn/(c \log n)),$ $g(y)$ can be taken to be a polynomial
$h_f(w_1,\ldots,w_{n^{c+1}/(c \log n)})$ of degree $n/(c\log~n)$ over that
field, where each $w_i$ itself is a product of at most $O(\log~n)$ variables
$x_i.$
\end{lemma}

\begin{proof}
The proof of Lemma~\ref{lem-lrr-boole-more} is virtually the same as that
of Lemma~\ref{lem-lrr-boole-basic}: $f(x)$ is equivalent to a polynomial
$g(x_1,\dots,x_n)$ of degree $n$ over an arbitrary field $E.$  The only new
observation we must make is that $g$ is $(d,dn/(c\log~n))$ locally random
reducible to some polynomial $h_f,$ by virtue of Lemma~\ref{lem-lrr-poly-more}.
\end{proof}


\section{Instance Hiding Schemes}
\label{sec-ihs}

The construction of the scheme given in the proof of
Theorem~\ref{theorem-model1} used secret-sharing with maximal coalition
size $t=1$ to generate a a $(1,n+1)$-locally-random reduction, which gave
rise to a $(n+1)$-oracle instance hiding schemes.  

In fact, it is not hard to show that any function $f(x)$ admitting a
$(1,m)$-locally random reduction to some function $g(y)$ also has an
$m$-oracle instance hiding scheme.  This gives a direct way to generate
instance hiding schemes for arbitrary functions.

\begin{theorem}
\label{thm-lrr-ihs}
\index{locally random reduction!instance-hiding scheme}
\index{instance-hiding scheme!locally random reduction}
If there exists a $(1,m(n))$-locally random reduction from $f(x)$ to $g(y),$
then there exists an $m(n)$-oracle instance hiding scheme for $f(x).$
\end{theorem}

\begin{proof}
The protocol is similar to the one given in the proof of
Theorem~\ref{theorem-model1}, except that instead of computing $y_i$
as a list of $1$-shares of $x_1,\ldots,x_n,$ we let $y_i$ be the result of
computing the reduction $P(x).$  In other words, the querier computes
$(y_1,\dots,y_m) \leftarrow P(x),$ and sends $y_i$ to $B_i,$ who computes
$g(y_i).$  Then $A$ determines $f(x)$ by computing
$Q(g(y_1),\ldots,g(y_m)).$   Since $(P,Q)$ is a $(1,m)$ locally-random
reduction, the distribution $D_n^{\set{y_i}}$ on query $y_i$ is the same
for any $x$ of size $n,$ so the random variables
$\anglebrack{Y_i,O_1,\ldots,O_m}$ and $X$ are independent given
$\abs{x}=n.$   (Note that the oracles are identical, as before, and each
computes $g(y)$.)
\end{proof}


\section{IP$=$PSPACE and Other Subsequent Work}
\label{sec-lrr-subsequent}

\subsection{Program Testing and the Permanent}

Lipton \cite{lip89} has designed a theory of program testing based on
locally-random self reductions.  Given a program which is presumed to work
with reasonably high probability on most inputs, he investigates means to
check the answer of the program on a particular input by calling the
program on several random but related inputs.  Based on
Theorem~\ref{thm-lrr}, which gives a $(1,n+1)$ locally-random self
reduction for any polynomial of degree $n$ in $n$ variables, his main
theorem states that any program for a function expressible as a polynomial
of degree $n$ is testable using $n+1$ calls to the program.  (See
\cite{bk89,blr89} for a related, earlier approach to program checking and
correcting.)

In particular, Lipton observes the following:
\begin{observation}   \label{obs-perm}
[Lipton 1989]  The {\sc Permanent} function is
testable of order $n+1,$ {\em i.e.} it has a $(1,n+1)$-locally random
reduction.
\end{observation}
\index{permanent}
The {\sc Permanent} of a $n \times n$ matrix $A$ is given by the following
expression, similar to the determinant:
\[
\mbox{\sc Perm\   } A \equiv \sum_{\sigma} \prod_1^n A_{i,\sigma(i)},
\]
where the sum is over all permutations of $\set{1,\ldots,n}.$  

The interesting and important property to note is that the {\sc Permanent}
is not known to be efficiently computable.  In fact, it is complete for the
class $\#P$ of counting problems \cite{val79}, presumed to be
extremely intractable.  The polynomial hierarchy (PH), which contains NP
and coNP, is contained in $P^{\#P}$ by a result of Toda \cite{tod89};
the {\sc Permanent} function is certainly as hard and presumably harder
than any problem in NP or coNP.

\subsection{Interactive Proofs: IP$=$PSPACE}

Beaver, Feigenbaum, Kilian, and Rogaway \cite{bfkr89} applied locally random
reductions to show that zero-knowledge proofs of properties about bits
which are committed but remain secret require only a constant number of
rounds of interaction and a small polynomial message size.  In other words,
one processor places several bits in envelopes and seals them, and then
claims and proves to another processor that a certain property holds on the
bits in the envelopes.  The bits are not revealed.  Previous methods
required a message complexity proportional to the size and depth of a
circuit describing the property to be shown.  Chapter~\ref{chap-zkp}
describes and proves this result in more detail.

Nisan \cite{nis89-cosat} used Observation~\ref{obs-perm} to show that there
is a multiprover interactive proof system for $\#P.$ That is, two
physically separate provers can convince a polynomial-time verifier of the
value of the permanent of some matrix, despite the difficulty of computing
the permanent.  Based on Nisan's solution, Fortnow, Lund, Karloff, and
Nisan \cite{lfkn89} showed that there is a {\em single}-prover proof system
for ${\#P},$ namely that one prover can convince a verifier of the value of
a permanent.  Since the polynomial hierarchy is contained in $P^{\#P}$ by
\cite{tod89}, this implies interactive proof systems for languages in
coNP, which was a large open question.

Shamir showed that in fact 
$\ip=\pspace,$\index{interactive proof system!IP=PSPACE} namely that the
class of languages that are interactively provable is the same as the class
of languages computable by a Turing machine using a polynomial amount of
memory \cite{sha89}.  His proof, based on the line of research inspired by
locally random reductions, uses simple algebraic techniques.

Interestingly, the proof that $\ip=\pspace$ connects a class based on
interaction and communication with a class based on computational
complexity.  The line of research sparked by the algebraic methods of
locally random reductions joins communication complexity with computational
complexity.  On the other hand, the results of \cite{bfkr89}, described in
Chapters \ref{chap-zkp} and \ref{chap-mpp}, show how to make
communication complexity and computational complexity {\em independent} in
protocols for security and reliability.

Thus, locally random reductions elucidate the connection between
communication complexity and computational complexity.  Their
straightforward, algebraic nature and the concise and simple solutions they
provide and inspire suggest that more applications are waiting to be found.



==> min.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% min.tex                      Tolerating a Minority of Faulty Processors.
%
%                            Copyright @1989  Donald Beaver.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{=======}
\typeout{min.tex}
\typeout{=======}

\chapter{Tolerating a Minority of Faulty Processors}   \label{chap-min}

\chapquote{
Democracy is the recurrent suspicion that more than half of the people
are right more than half of the time.
}{
E. B. White, {\em The Wild Flag}}


The methods of \cite{bgw88,ccd88} and even the far more efficient methods
we have presented in Chapter~\ref{chap-con} allow faults in at most a third
of the network ($3t<n$).  Perfect privacy is not achievable with higher fault
tolerance for even some simple functions like AND \cite{bgw88} (but see
Chapter~\ref{chap-pri} for a characterization of functions computable with
perfect privacy at high, passive fault-tolerance levels).

The natural question to ask, though, is whether higher fault tolerance is
possible if the assurances of security and reliability need not be
absolute.  We show that, allowing for a negligible chance of error, $2t<n$
can be achieved.  That is, as long as only a minority of the processors are
faulty, we can construct protocols to compute any function reliably and
securely.  For larger numbers of faults, it becomes impossible for the
players even to share a secret, which does not immediately imply a negative
result but gives a strong intuition as to why higher fault-tolerance is
generally impossible without making other assumptions about the network
model.

Notice that the major problems with extending the methods of 
\cite{bgw88,ccd88} to $2t<n$ are that verifiable secret sharing fails
and that the specific techniques for the ABC Problem fail.

Rabin \cite{tr88} made initial and significant
progress in the direction of improving
the fault bounds from $3t<n$ to $2t<n$ by demonstrating a method for
verifiable secret sharing for $2t<n,$ using a broadcast network.
Earlier methods for verifiable secret sharing with a faulty minority
required cryptographic assumptions \cite{cgma85}.
The extension to performing {\em computations} for $2t<n,$ however,
remained open until this work.

We give a new and efficient method to solve the ABC problem when
secret addition is possible, for $2t<n.$
Our techniques utilize verifiable secret sharing for $2t<n,$ and
allow the field used for secret sharing to be of exponential size.  
Ben-Or \cite{br89} and Kilian \cite{kil-n2} have
independently developed methods to
tolerate a faulty minority, based on standard ideas of boolean circuit
simulation.  Their methods require that the field used for secret sharing 
be of
polynomial size, which restricts the efficiency of their solutions.

\begin{theorem}   \label{thm-min}
There exists a protocol \evalmin \ \  that is $t$-resilient against
against dynamic Byzantine adversaries for $2t \leq n.$
\end{theorem}


Because we can simulate large-field arithmetic operations quickly and
directly while alternative methods use bit-simulations or small-field
arithmetic, our protocols have the practical advantage of using far fewer
rounds of communication for many natural functions.  Joined with the
techniques of Chapter~\ref{chap-con}, our techniques use tremendously fewer
rounds of interaction.  The bit-simulation techniques of
\cite{br89,kil-n2}, on the other hand, are incompatible with reducing
rounds through the arithmetic circuit reductions of Chapter~\ref{chap-con}
since they require the added cost of simulating arithmetic operations by
bitwise Boolean operations.

As before, our methods are secure against adversaries with unbounded
resources, while at the same time requiring only polynomial time to
execute.

We shall first describe a modification of the solution in \cite{tr88}
for verifiable secret sharing, show how to add secrets, and then give
our solution to the ABC problem when $2t<n.$  The framework of
\cite{bgw88,ccd88} can then be applied, using these more resilient
subprotocols to support the share-secrets-create-secrets paradigm.

\medskip 

{\bf Assumptions made in this chapter.}  The network is complete,
with private lines, broadcast lines, $n$ processors,
and at most $t < \frac{n}{2}$ Byzantine faults, chosen dynamically.
The protocols are information-theoretically secure with high probability,
or in other words, the results are statistically resilient.  No unproven
complexity-theoretic assumptions are made.


\section{Verifiable Time-Release Messages}

There is a long history of solutions for VSS under various 
unproven assumptions.  We
wish to avoid unproven cryptographic assumptions and to tolerate $2t<n.$ We
shall utilize a method for VSS for $2t<n$ very similar to that given by
\cite{tr88}, but somewhat more convenient and efficient.  Briefly, it uses
Shamir's method for sharing a secret, and requires that each piece be
reshared using a weak form of sharing.  The weaker form of sharing includes
information called ``check vectors,'' which allow verification of the
pieces.  Our modification of the protocol is a new method for constructing
check vectors.  For completeness, because formal proofs of
\cite{tr88,br89} have not appeared, and
because we use different subroutines,
we shall present the essential details of \cite{tr88,br89} but
we refer the reader to that work for a deeper discussion.

The verification property of Rabin's scheme relies on a subprotocol for
what we call Verifiable Time-Release Messages.

We consider three players, a sender S, a receiver R, and an intermediary I.
The sender would like to give a secret bit to the intermediary, who will
pass it on at a later time to the receiver.  The receiver must be able to
detect any tampering on the part of the intermediary.  At the same time,
the intermediary should know whether the information given him will in fact
satisfy the receiver at the appropriate time.  He must therefore be able to
check the behavior of the sender during the initial part of the protocol.

Rabin \cite{tr88} provides an elegant way to satisfy these properties
in a manner similar to secret sharing with threshold 1.  Her
idea involves generating nonzero random numbers $u$ and $v$ $\mod p$ and
setting $w=b+uv.$ The receiver gets $(v,w)$ while $I$ gets $(b,u).$ When
$I$ passes the value on to R later, he sends $(b,u),$ and R checks that
$w=b+uv.$ In order to convince R of an incorrect value, the intermediary
must change $u$ correctly, which he cannot do with non-negligible
probability.  Checking that the sender is correct uses a cut-and-choose
idea, which we shall use below.

We present a simple alternative with the nice property that 
no multiplications are necessary.  In terms of polynomial-time
algorithms, this makes no difference, but in terms of actual 
implementations, multiplications over a finite field are 
considerably more expensive than additions.
Our approach is derived from work on a
different problem with Feigenbaum and Shoup \cite{bfs90}.

If S and R were to share a one-time pad (a private sequence of random
bits), then how may S send a secret bit to R via another player I?  Player
I might change some of the bits.  Our simple solution uses $3k$ bits of the
one-time pad and ensures that tampering is detected with probability
$1-2^{-k}.$  See Figure~\ref{fig-ver-onetime}.  Intuitively, for I to
change the bit $b$ without detection, it must guess the exact sequence of
bits $\alpha(1),\ldots,\alpha(k),$ which it can do with probability at most
$2^{-k}.$ 

\figstretch
\boxfig{
\noindent{\bf \vermsg} $(b)$
\begin{tabbing}  \standtabs
Phase I.\\
(VM1)
\>S reads $\set{(\alpha(i),\beta_0(i),\beta_1(i))}_{i=1..k}$
from the one-time pad. \\
\> $(1\leq i \leq k)$  S: \\
\>\>\>\> $\gamma_0(i) \leftarrow \beta_0(i) + b \cdot \overline{\alpha}(i)$ \\
\>\>\>\> $\gamma_1(i) \leftarrow \beta_1(i) + b \cdot          {\alpha}(i)$ \\
\>S: 
\>\>\> $M_b \leftarrow \set{(\gamma_0(i),\gamma_1(i))}_{i=1..k}.$ \\
\>$S \rightarrow I:$
\>\>\> $M_b$ \\
Phase II.\\
(VM2)
\>$I \rightarrow R:$
\>\>\> $M_b$ \\
\end{tabbing}
\caption{\label{fig-ver-onetime}
Protocol for S to send a bit $b$ to R via player I.  
Note that addition may be either modulo two, if the $\alpha$ and
$\beta$ values on the pad are bits, or it may be addition over
a finite field, if the $\beta$ values are field elements.
}}
\figstretchend

We use this verifiable one-time pad to construct a {\em verifiable
time-release scheme}%
\index{time-release scheme!verifiable}
as follows.  Roughly speaking, the sender sends the
one-time pad privately to R, and sends the message $M_b$ to I, who holds
onto it until the time it should be released.  The one-time pad serves
as a {\em check vector}\index{check vector}, \ie\  a sequence
of bits used to check the accuracy of the secret held by I.
The property that the
intermediary is convinced that R will accept the message later on must also
be satisfied, and we now turn our attention to that problem.

As in \cite{tr88}, we use a cut-and-choose method.  Instead of generating
$k$ $(\alpha,\beta_0,\beta_1)$ triples, generate $2k$ of them.  Half of
these will be revealed to I by R so that I can check for misbehavior.  In
order for S to cheat undetected, it must misbehave on exactly that half of
the triples that R does {\em not} immediately send to I.  Notice that $I$
learns $b$ upon receiving a single $(\alpha,\beta_0,\beta_1)$ triple.  To
keep $b$ secret from $I,$ the sender simply splits $b$ into two random bits
as $b=b_I \oplus b_R,$ and gives $b_I$ to $I$ and $b_R$ to $R.$  

The protocol is detailed in Figure~\ref{fig-time-release}.  If $M$ is a message
that one party is supposed to send to another, we denote by $M'$ the
message it actually sends.  

Intuitively, if S attempts to cheat, it must guess in advance the exact
set of indices $i(1),\ldots,i(k)$ that R selects at random, and it must
behave properly on that list but must cheat on every other row of the
table.  The chances of this are certainly at most $2^{-k}.$



\figstretch
\boxfig{
\noindent{\bf \vertimerel} $(b)$
\begin{tabbing} \hspace{0.8in} \= \hspace{0.5in} \=
\hspace{0.5in} \= \hspace{0.7in} \= 
\hspace{0.5in} \= \hspace{0.5in} \=
\hspace{0.5in} \= \hspace{0.5in} \= \kill
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Phase I. \\
(VTR1) \>
$S$ computes:  
\>\>\>
$b_I \leftarrow \uniform(\set{0,1});$  $b_R \leftarrow b \oplus b_I.$ \\
\>$S$ computes $(i=1..2k):$ 
\>\>\>$\{(\alpha(i),\beta_0(i),\beta_1(i))\} \leftarrow \set{0,1}^{3}$ \\
\>\>\>\>$\gamma_0(i) = \beta_0(i) \oplus b_I \cdot \overline{\alpha}(i)$ \\
\>\>\>\>$\gamma_1(i) = \beta_1(i) \oplus b_I \cdot          {\alpha}(i)$ \\
\>
$S \rightarrow R:$ 
\>\>\>
$b_R; \set{(\alpha(i),\beta_0(i),\beta_1(i))}_{i=1..2k}.$
\\
\>
$S \rightarrow I:$ 
\>\>\>
$b_I; \set{(\gamma_0(i),\gamma_1(i))}_{i=1..2k}.$
\\
\\
(VTR2) \>
$I$ generates: 
\>\>\> $i(1)..i(k) \in_R \set{1,\dots,2k}$ such that\\
\>\>\>\>$i(j) \not= i(j')$ for $j \not= j'.$
%%\\
\>
$I \rightarrow R:$ 
\>\>\>
 $i(1)..i(k).$
\\
\\
(VTR3) \>
$R \rightarrow I:$
\>\>\>
$\set{(\alpha'(i(j)),\beta'_0(i(j)),\beta'_1(i(j)))}_{j=1..k}.$
\\
\\
(VTR4) \>
\If there exists $j$ such that\\
\>\>\>\>$\gamma'_0(i(j)) = \beta''_0(i(j)) \oplus b_I 
\cdot \overline{\alpha''}(i(j))$ 
or \\
\>\>\>\>$\gamma'_1(i(j)) = \beta''_1(i(j)) \oplus b_I
\cdot          {\alpha''}(i(j))$ \\
%\> \Then let $I'={\rm\em reject}$ \Else let $I'={\rm\em accept}.$ \\  %drb2020
\> \Then let $I'=\rej$ \Else let $I'=\acc.$ \\
\> $I \rightarrow S,R:$
\>\>\>  $I'.$ \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\
Phase II. \\
(VTR5) \>
$I \rightarrow R:$
\>\>\>
$b_I, \set{(\gamma'_0(i),\gamma'_1(i))}_{i=1..2k}.$
\\
\>
If there exists $i$ such that\\
\>\>\>\>$\gamma'_0(i) = \beta''_0(i) + b_I \cdot \overline{\alpha''}(i)$ 
or \\
\>\>\>\>$\gamma'_1(i) = \beta''_1(i) + b_I \cdot          {\alpha''}(i)$ \\
%\> then let $R={\rm\em reject}$ else let $R={\rm\em accept}.$ \\  %drb2020
\> then let $R=\rej$ else let $R=\acc.$ \\
\end{tabbing}
\caption{\label{fig-time-release}
\index{\vertimerel}
Protocol for S to send a bit $b$ to R via player I, who holds on to the bit
before passing it on.  If $M$ is a message that the protocol specifies to
send, then $M'$ denotes the message actually sent.  
Note that $\oplus$ may denote field addition instead of exclusive or,
in which case the $\beta$ values
are instead selected uniformly at random from the field.
Using field addition is conducive to adding the unreleased 
values together without revealing them.
}}
\figstretchend



\todoMaybe
\iffalse

\subsection{Simulating the Time-Release Scheme}

No formal proof of the techniques used in \cite{tr88} has appeared to
date, so we must include a proof for completeness.

\fi
\todoMaybeEnd

\begin{theorem}   \label{thm-time-release}
Protocol $\vertimerel$ is exponentially
$2$-resilient against Byzantine adversaries.
\end{theorem}

\todoMaybe
\iffalse

\begin{proof}

\fi
\todoMaybeEnd


The ideal protocol $\idVTR$ is as follows.  In Phase I,
the sender $S$ sends two bits, $b_I$ and $b_R,$ to the host.
The host sends $b_i$ to $I$ and $b_R$ to $R$ if it indeed received
two bits; otherwise it sends \cheating.  Then, $I$ and $R$ send
a 0 to the host to indicate they wish to participate, and the host
passes on either $0$ or \cheating\  to $I$ and $R$ to indicate whether
they chose to participate.  In Phase II, $I$ again sends 0 to indicate
it wishes to reveal the value, and the host sends $b_i$ to $R,$ or
it sends \cheating\  if $I$ supplied a nonzero value.

\todoMaybe
\iffalse

The simulator does the following.  For corruptions before round
(VTR1), it corrupts the corresponding player in $\idealname(VTR)$
and returns the inputs to $A.$  To generate the message from honest
$S$ to corrupt $R,$ the interface generates $6k$ random field elements
and sets $b_R$ by corrupting $R_{id}$ in $\idealname(VTR)$ after it receives
$b_R.$  To generate the message from honest $S$ to corrupt
$I,$ the interface generates $2k$ random field elements 
and sets $b_I$ by corrupting $I_{id}$ in $\idealname(VTR)$ after it receives
$b_I.$  
If both $R$ and $I$ are corrupt, then the interface corrupts them
in $\idealname(VTR)$ to obtain $b_I$ and $b_R,$ calculates 
$b=b_I\oplus b_R,$ and performs the computation of $S$ to generate
the $\alpha, \beta, \gamma$ tables.  If $S$ is corrupt, the interface
obtains its two messages, checks to see if they are possible
(by solving for $\gamma_0,\gamma_1$), and if not, causes $S_{id}$ to
output $\Lambda.$  Notice that whereas 
$\rvAA(\mess(S,\{I,R\},1) = \rvASB(\mess(S,\{I,R\},1),$
the resulting distribution on final player outputs in $\idealname(VTR)$
will be only exponentially indistinguishable from those in
$\vertimerel,$ because  with probability at most
$2^{-k},$ $S$ will cheat undetected in $\anglebrack{A,\vertimerel}.$
In that case, because the players in $\idealproto(VTR)$ reject $S,$
their outputs are different.  But by Lemma~\ref{lem-feed-dist}, we
may use a probabilistic function that differs exponentially little
from the ``proper'' one, and the net result is exponentially close.

(VTR2)  
New corruptions are easy to specify by solving the equations
$\gamma_0(i)=\beta_0(i) + b \cdot \overline{\alpha}(i)$ and
$\gamma_1(i)=\beta_1(i) + b \cdot {\alpha}(i)$ using information
from corrupting a player in the ideal protocol or from the variables
sampled already in (VTR1).  

If $I$ is nonfaulty whereas $R$ is faulty, then the interface simply generates
$i(1),\ldots,i(k)$ randomly as specified and supplies them to $A.$
If $I$ is faulty and sends an improper list, then the interface specifies
that $I_{id}$ send $\Lambda$ to the trusted host to indicate
lack of participation.  The distributions on outputs of 
$R$ and $R_{id}$ will be identical, namely both will indicate \cheating.

(VTR3)
If $R$ is nonfaulty whereas $I$ is faulty, then the interface does one
of two things.  If $S$ is already corrupted, it uses the values
of $\alpha,\beta_0,\beta_1$ already sent by $A.$  If $S$ is not corrupt,
the interface nevertheless knows $b_I$ and
the values of $\gamma_0$ and $\gamma_1$
held by $I,$ so it generates the $k$ values of $(\alpha,\beta_1,\beta_2)$
by selecting $\alpha$ uniformly at random and solving for $\beta_0$
and $\beta_1.$  It is not hard to see that this is the correct
conditional distribution given the values of $\gamma_0$ and $\gamma_1,$
if $S$ and $R$ are not corrupt.

(VTR4)
If $I$ is faulty, the interface does nothing.  Otherwise, 
if $I$ is nonfaulty, and $S$ is faulty,
the interface can calculate from the current history
whether $I$ detects if $S$ has cheated, and it sets 
$\rvASB(\mu(I,\{S,R\},4),4)$ accordingly.  If $I$ does detect
cheating then the interface requests that $S_{id}$ send $\Lambda$
to the trusted host, in which case the output of nonfaulty players
in $\idealname(VTR)$
will have a distribution exponentially indistinguishable from those
in $\rvAA.$

If $I$ is nonfaulty and $R$ is faulty, then the interface has
a record of what $S$ sent to $R$

(VTR5)



In order to demonstrate the resilience of the time-release scheme, we must
demonstrate a simulator.  The task is not difficult but requires
case-by-case analysis.  We consider 8 possibilities corresponding to
whether or not S, I, and R are corrupted (bad or good) respectively.
First let us assume the adversary is static, and later we examine how to
extend our simulator to handle a dynamic adversary.

\todoMaybePrint{todo: fill in cases -- easy}

\noindent{\bf Case GGG.}
Nothing to simulate.

\noindent{\bf Case GGB.}

\noindent{\bf Case GBG.}

\noindent{\bf Case GBB.}

\noindent{\bf Case BGG.}

\noindent{\bf Case BGB.}

\noindent{\bf Case BBG.}

\noindent{\bf Case BBB.}

\fi
\todoMaybeEnd



In the VSS%
\index{secret sharing!verifiable}
method of \cite{tr88}, all players act both as intermediaries
and recipients for pieces of the secret $u.$ Each piece $\piece_i(u)$ of
$u$ is given to an intermediary $i,$ and check vectors $s_j(\piece_i(u))$
are sent out to every other processor $j.$ At reconstruction time, the
intermediaries $i$ broadcast their check vectors $\vec{s}(\piece_i(u)),$
which include $\piece_i(u).$ Each player, acting as a recipient,
reconstructs $u$ using the pieces he concludes are accurate.

\begin{theorem} (after T. Rabin \cite{tr88})
There exists a VSS protocol for $2t<n$ that is $t$-resilient.
\end{theorem}

\todoMaybePrint{expand, list, prove}


\section{Addition of Secrets}       \label{sec-add}


%% \begin{lemma}      \label{lemma-add}
%% Let $u$ and $v$ be secretly shared values, and let $a,b$ and $c$ be
%% publicly known field elements.
%% Then for $2t<n,$ there exists a $t$-resilient protocol 
%% $w \leftarrow au+bv+c$
%% to provide each player with a piece of a new secret $w$ whose value is
%% $au+bv+c.$ 
%% Protocol \add  is such a protocol.
%% %without revealing any information about $u,v,$ or $w.$
%% \end{lemma}
%% 

It is possible though not trivial to extend the VSS method given above
to a method for linearly combining secrets.  
%\todoMaybe
%We shall first give an overview of the addition protocol
%\add (see Figure~\ref{fig-add}),
%and show it is correct with high probability;
%a discussion of its privacy appears in \S\ref{sec-proof-privacy}.
%and then prove it is valid and private in \S\ref{sec-prove-add}.
%
%\todoMaybeEnd
Say that $u$ and $v$ were shared using polynomials $f(x)$ and
$g(x),$ respectively.
Let $h(x)=af(x)+bg(x)+c;$ then $h(0)=af(0)+bg(0)+c =w.$
Sums of the pieces are pieces of the sum;
Each player $i$ uses 
\[
\piece_i(w) = a \cdot \piece_i(u) + b \cdot \piece_i(v) + c
\]
as his piece of $w.$

In order that $w$ be a verifiable secret according to the VSS protocol,
each $\piece_j(w)$ must be reshared in a weak fashion.  This involves
the use of check vectors for the pieces of $h(j).$
Each player $i$ holds pieces of every other
player's pieces, $\piece_i(\piece_j(u))$  and
$\piece_i(\piece_j(v)).$
He sets
\[
\piece_i(\piece_j(w)) = 
a \cdot \piece_i(\piece_j(u)) + b \cdot \piece_i(\piece_j(v)) + c.
\]

The only remaining part of the VSS structure is the set of
check vectors for the pieces $\piece_j(\piece_i(w)).$
Since player $i$ knows $\piece_i(w),$ he creates and distributes new
check vectors for the pieces of this value.  The other players check the
correctness of his vectors using the protocol specified in
the VSS scheme \cite{tr88}.


\figstretch
\boxfig{
\noindent{\bf \add(a,b,c,u,v,w).}\\
Compute $w = au+bv+c.$
\begin{itemize}
\item Set
\[ \piece_i(w) = a \cdot \piece_i(u) + b \cdot \piece_i(v) + c. \]
\item For each $j,$ compute pieces of the pieces:
\[
\piece_i(\piece_j(w)) = 
a \cdot \piece_i(\piece_j(u)) + b \cdot \piece_i(\piece_j(v)) + c.
\]
\item Choose new check vectors 
for $\piece_j(\piece_i(w))$ for all players $j\not = i,$
and participate in their verification,
as per the VSS protocol.
\item Receive check vectors for other pieces $\piece_i(\piece_j(w))$
and participate in their verification, as per the VSS protocol.
\end{itemize}
\caption{\label{fig-add}
Protocol for linear combinations of secrets.
(Code for processor $i.$)  
}}
\figstretchend

%% \subsection{Proving the Privacy of Addition}
%% \label{sec-prove-add}
%% 

The \add protocol is resilient
because each of its steps is either a non-interactive computation
of a robust and private representation of some secret value,
or an application of a subprotocol for VSS that is itself resilient.
It is clear that players who deviate from the protocol cannot create
convincingly false check vectors with probability
exceeding some $\frac{1}{2^{k_1}},$ as determined by
the security parameter $k_1$ of the VSS protocol.
In this case, an interface would fail to be able to provide a 
correct argument, since the adversary would learn information 
to which it is not entitled, and the interface would need to 
corrupt additional players to obtain that information.
The net weight of these events is exponentially small, however.
In fact, the only undetectable misbehavior is the possible
choice of acceptable check vectors
% \todoMaybe
% (see Equation~(\ref{eqn-check}))
% \todoMaybeEnd
according to an inappropriate
distribution.  
This is, however, easily dealt with by an interface, which
needs merely record what the {\em adversary} specifies;
the interface need not itself generate these distributions.
Note that nonfaulty players' behavior is independent
of how the faulty players generate check vectors, even
{\em acceptable} ones.




\section{Multiplication of Secrets}       
\label{sec-mult}

The protocol for multiplication of secrets is more complicated;
the key new idea is a method for giving a proof that the
product of two secrets is a third.  In fact, the ability to
prove products of secrets is the basis for achieving high
fault-tolerance in all of the results of this paper.

The protocol we shall present relies on a protocol for addition
of secrets.  
%In \S\ref{sec-proof-privacy} we shall show that
%the multiplication protocol is $t$-resilient, demonstrating
%that Theorem~\ref{thm-addthenmult}, which states that
%a protocol for addition gives a protocol for multiplication,
%is true.

%% \begin{thm}      \label{thm-mult}
%% Let $u$ and $v$ be secretly shared values.
%% Then for $2t<n,$ there exists a $t$-resilient protocol 
%% %$W \leftarrow U \cdot V$
%% to provide each player with a piece of a new secret $w$ whose value is
%% $uv.$
%% % without revealing any information about $u,v,$ or $uv.$
%% \end{thm}
%% 
%% By Lemma~\ref{lemma-add}
%% it suffices to show Theorem~\ref{thm-addthenmult},
%% which states that an addition protocol implies a multiplication
%% protocol.
%% %We prove Theorem~\ref{thm-addthenmult} by describing the protocol.
%% 

Our solution follows a few brief steps (cf. \cite{bgw88}).
As before,
let $u$ and $v$ be shared using $f(x)$and $g(x).$  
Each player $i$ secretly shares the value $f(i)g(i)$ and
``proves'' that he has in fact shared this value 
(see \S\ref{subsec-vermult}).
If his proof fails, he is disqualified (see \S\ref{subsec-disqual}).
From the collection of secret products determines
the polynomial $h(x)=f(x)g(x),$
of degree $2t$ and free term $uv.$
Using a protocol to add a random polynomial
of degree $t+1$ and free term 0
and then to truncate the polynomial to degree $t$
(see \S\ref{sec-truncate}),
each player $i$ is supplied with 
the value $h(i)$ for the resulting polynomial
$h(x)$ of degree $t$ and free term $uv.$  
Figure~\ref{fig-mult} describes the \mult protocol.

\figstretch
\boxfig{
\noindent{\bf \mult(u,v,w).}\\
\begin{itemize}
\item Secretly share $h(i)=\piece_i(u) \piece_i(v).$
\item Run the \abc protocol to prove that player $i$ shared this
value.
\item Receive pieces $\piece_i(h(j))$ from each player $j \not= i.$
\item Participate in the \abc protocol for $2t<n$ to verify that
player $j$ shared the correct value.
\item Run the \truncate protocol using $h(i)$ to obtain a 
piece $\piece_i(w)$ of a random, degree $t$ polynomial
whose free term is $w.$
\end{itemize}
\caption{\label{fig-mult}
Protocol to multiply two secrets.
(Code for processor $i.$)
}}
\figstretchend



\subsection{Verifiable Multiplication}        
\label{subsec-vermult}

In order to accomplish the resilient verifiable sharing of $f(i)g(i),$
we must provide a solution to the ABC problem when $2t<n.$
In fact, we describe a new method that shows that, if secret addition
is possible, then multiplication is possible, for $2t<n.$

\bigskip

Given a protocol for the ABC problem, Alice will be able to
prove to the network that the new secret which she shares
is indeed $f(i)g(i).$

\begin{lemma}    \label{lem-abc}
(ABC Lemma.)\index{ABC Lemma}
If there exists a $t$-resilient protocol for linear combinations
of secrets, then
there exists a $t$-resilient protocol to solve the ABC problem.
\end{lemma}


The protocol is exhibited in Figure~\ref{fig-abc}.
First, an overview:
In the first phase,
Alice shares several triples of secrets $({\cal R},{\cal S},{\cal D})$
satisfying a simple equation
(of the form ${\cal D}=(a+{\cal R})(b+{\cal S})$),
which will be used to ensure that Alice does not misbehave.
In the second phase,
the players select and reveal combinations of some of these triples in order
to confirm that every triple satisfies the simple equation.
Finally, each unrevealed triple of secrets gives rise to
a simple linear combination
of secrets that should equal the desired product $ab.$
The third phase checks that the linear combinations are consistent.

Let ${k_0}$ denote a security parameter; the chance of incorrectness
will be bounded by $\frac{1}{2^{k_0}}.$
For simplicity we take ${k_0}>n$ and ${k_0}$ a power of two.

\figstretch
\boxfig{
\noindent{\bf \abc.}\\
\begin{itemize}
\item  Let $a$ and $b$ be verifiably shared.
\item  Alice verifiably shares $c = ab.$
\item  Alice shares secrets $r_1,\dots,r_{2{k_0}}$ and $s_1,\dots,s_{2{k_0}}$
chosen uniformly at random over the field $E.$
\item  For $j = 1,\dots,2{k_0},$ Alice computes $d_j = (a+r_j)(b+s_j),$
and shares $d_j.$
\item  The network confirms with high probability that each
$d_j = (a+r_j)(b+s_j):$
  \begin{itemize}
  \item  For $i = 1,\dots,{k_0},$ the network selects a random index
  $j_i$ by having each player select a random secret $\mod (2{k_0}+1-i),$
  sharing it (over fields of characteristic $p$ such that 
  $p \mid 2{k_0}+1-i,$ so that the distribution is uniform), and
  then computing the sum.
  \item  Let $Y = \set{j_1,\dots,j_{k_0}}.$
  \item  For all $j \in Y,$ run the \add protocol on $(a,r_j)$ 
  to obtain the sum $a+r_j.$
  \item  For all $j \in Y,$ run the \add protocol on $(b,s_j)$ 
  to obtain the sum $b+s_j.$
  \item  For all $j \in Y,$ reconstruct $a+r_j,$ $b+s_j,$ and $d_j.$
  Disqualify Alice if any of the $d_j$ are not equal to
  $(a+r_j)(b+s_j).$
  \end{itemize}
\item  The network confirms that $c$ matches the product $ab.$
  \begin{itemize}
  \item  For all $j \not \in Y,$ reconstruct the values $r_j, s_j.$
  \item  For all $j \not \in Y,$ compute 
  \[  c_j  =  c - d_j + as_j + br_j + rs  \]
  \item  For all $j \not \in Y,$ reconstruct $c_j.$
  \item  If any $c_j \not= 0,$ disqualify Alice.
  \end{itemize}
\end{itemize}
\caption{\label{fig-abc}
\index{\abc}
\index{ABC problem}
Protocol to prove that the product of two secrets is a third secret.
(Code for Alice and network.)
}}
\figstretchend

%Consider the protocol \abc described in Figure~\ref{fig-abc}.
Now let us consider the \abc protocol in more depth.
If Alice is honest, 
all of the sums $(a+r_j)$ and $(b+s_j)$ are independent of
$a$ and $b,$ since $r_j$ and $s_j$ are uniformly
random field elements.  The products $d_j$ are also independent
of $a$ and $b.$  The choice of ${k_0}$ indices $j_1,\dots,j_{k_0}$ to check
is independent of $a$ and $b,$ given that any one player in the
system is honest and shares uniformly random numbers.
The partial views obtained by faulty players during the addition protocols
are independent of the good players' inputs.
%by Lemma~\ref{lemma-add}.
Finally, since Alice is honest, $d_j = (a+r_j)(b+s_j) = c + as_j+br_j+rs,$
so $c_j=0$ always.
Therefore, the set of messages are $t$-wise
independent of $a$ and $b,$
and messages from nonfaulty to faulty players are easily generated
accurately by an interface.

We would like to show that the chance that $c \not = ab$ without
Alice's being detected is smaller than $\frac{1}{k_0}.$ 
We shall show that she must behave properly on exactly the indices
in $Y$ and she must misbehave on all the others.
Let $X$ be the set of indices $j$ for which Alice shares $d_j$ correctly,
that is, for which Alice shares $d_j$ having the value $(a+r_j)(b+s_j).$
The set $Y$ of indices chosen by the system must be
a subset of $X,$ or else Alice's misbehavior is detected
for some $j \in Y \backslash X.$
The remaining indices $j \not \in Y$ must all satisfy 
$c_j = c - d_j + as_j + br_j + rs = 0$
or else Alice is caught.
If $c \not= ab$ (Alice is cheating), 
none of the indices $j \not \in Y$ is in $X.$
Hence $X=Y,$ and
since $Y$ is chosen randomly after Alice has shared all her secrets,
the probability that Alice can cheat without being detected
is no more than $\frac{1}{2^{k_0}}.$  An interface fails to 
produce a correct output
an exponentially small amount of the time, hence the overall
distributions are exponentially indistinguishable.




\section{The Protocol Compiler for Faulty Minority}
\label{sec-mainthm}

At this point we have described all the tools necessary to
create a multiparty protocol to evaluate any circuit $C_F$ for
$F(x_1,\dots,x_n)$ privately, tolerating $t< \frac{n}{2}$ faults.
The protocol is the same as that of protocol \eval
(Figure~\S\ref{fig-eval}), with the new \add and \mult protocols of this
chapter substituted for the ones called by that specification.  The
disqualification procedure is different, as well: after each cycle of
evaluating gates, a recovery procedure is initiated if faults have been
detected.  

Let $\tau$ be the number of faults.  The $(n-\tau,t-\tau)$ recovery
protocol uses a stripped-down version of the \truncate protocol to reduce
the degrees of each polynomial being used by $\tau.$ The remaining players
in fact reconstruct each {\em piece} of the various secrets held by the
$\tau$ faulty players, using straightforward linear combinations of
existing pieces, as seen by the following argument.  Without loss of
generality take the set of reliable players to be $1,\ldots,t+1.$ Then the
LaGrange interpolation gives
\[
p(j) = \sum_1^{t+1} L_i(j) p(i),
\]
so that the piece $\piece_j(s) = p(j)$ is easily computed as a weighted sum
of secrets.  That is, each player verifiably reshares his pieces and then
the system computes the given linear combinations.  If more faults occur
then the process is restarted.  Notice that the players {\em do not}
reconstruct all the information held by the faulty players; instead, they
reconstruct {\em pieces} of secrets held by the faulty processor.  This
bears no relation to the value of that faulty player's input; such
information is not revealed.

Now, each reliable player has learned the pieces held by disqualified
players.  It now adjusts the value of its own pieces through a simple
computation in order to obtain pieces of the original secrets, but shared
with polynomials of degree $t-\tau.$ For concreteness, assume only one
player has been disqualified.  Say that secret $s$ is shared via polynomial
$p(u)=\sum_0^t a_t u^t.$ Player $i$ has $\piece_i(s)=p(\alpha_i).$ The
newly publicized piece of the disqualified player is $p(\alpha_j)=\beta.$
Let $m_1(u)=\prod_{i\not=j} (u-\alpha_i),$ $m_2(u)=(u-\alpha_j),$ and
$M(u)=m_1(u) m_2(u).$ Define $g(u) = f(u) \mod m_1(u);$ then by the Chinese
Remainder Theorem,
\begin{eqnarray*}
M_1(u) & = & [m_2(u)^{-1} (\mod m_1(u))] \cdot m_2(u) \\
M_2(u) & = & [m_1(u)^{-1} (\mod m_2(u))] \cdot m_1(u) \\
f(u) & = & M_1(u) g(u) + M_2(u) \beta   \hspace{0.3in} (\mod M(u))
\end{eqnarray*}
Then player $i$ computes its new piece of $s$ as:
\[
g(\alpha_i) = [f(\alpha_i) - M_2(\alpha_i) \cdot \beta ] / M_1(\alpha_i).
\]
When using or revealing this value, the verification information is easily
adjusted since it verifies the $f(\alpha_i)$ value, which is itself easy
to recover from the $g(\alpha_i)$ value since $M_1,$ $M_2,$ $\alpha_i,$ and
$\beta$ are publicly known.

\todoMaybe
\iffalse

\section{Proof of Resilience}
\label{sec-proof-privacy}

\fi
\todoMaybeEnd



==> mod.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% mod.tex                    Modular Protocol Design.
%
%                            Copyright @1989  Donald Beaver.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{=======}
\typeout{mod.tex}
\typeout{=======}

\chapter{Modular Protocol Design}
\label{chap-mod}

Secure multiparty protocols are often based on a paradigm introduced by
Goldreich {\em et al} \cite{gmw86,gmw87}: ``Share Inputs; Compute New
Secrets; Reconstruct Results.''  The value of reducing a function
computation to a circuit evaluation is clear: by constructing
subprotocols to add and multiply secretly shared values, one provides the
modules for a simple and modular protocol to compute the overall function.

Though the direct application of this approach to circuit evaluation
results in inefficient protocols, we shall follow it and modify it to
provide a more general and far more efficient modular approach.  Rather
than decomposing a function into subprotocols centered around each gate of
a circuit, we focus on constructing a sequence of intermediate functions
whose results can be revealed, unlike the outputs of intermediate gates 
in a circuit, 
without compromising security.  We propose a more general modular
approach.

To support a modular approach, however, the concatenation of
protocols and the composition of functions require particular attention in
terms of security and reliability.  In this chapter we address the
particular intuitive and formal issues arising from the pursuit of a
modular approach.  We prove some intuitive lemmas regarding composition and
concatenation, some of which are intuitive results --- such as the validity
of composing polynomially many protocols --- whose statements as
folk-theorems are sufficiently imprecise that they do not hold.  
We give the formal requirements under which they do hold.
In the next chapter we present particular protocols; this chapter
focuses on technical lemmas and methodology.


\section{Robust and Private Representations}
\label{sec-threshold-def}

A threshold scheme allows one player, the {\em dealer,} to distribute a
secret value $s$ among the network in such a way that only certain
coalitions of players have sufficient information to determine $s.$
When a bound $t$ on the number of faulty or curious participants
is given, the power to reconstruct $s$ is given to groups of size $t+1$ or
more, but not to any group of size $t$ or less.  

There are two properties we should like to satisfy.  The first states that
there is a means to reconstruct a shared value despite errors.  Given a
vector $\vec{y}$ of $n$ values, a 
$t$-{\em modification}\index{modification}
of $\vec{y}$ is a
vector differing in at most $t$ places from $\vec{y},$ namely a vector of
Hamming distance $t$ or less from $\vec{y}.$  
\begin{definition}  \label{def-robust-rep}
A function $\sha:S \rightarrow (\sigstar)^n$ is a {\defstyle $t$-robust
representation}\index{representation!robust}\index{robust} if there exists
a function $\recons$ such that,
for all $s \in S,$
for all $t$-modifications $\vec{y}\prime$
of $\vec{y}=\sha(s),$ we have $\recons(\vec{y}\prime)=s.$
\end{definition}

Broadcast channels are useful to maintain robustness,
in which case the value is not kept private.  
Secret sharing, which does achieve privacy at the same time,
is also useful.

The second property states that the information distributed to the players
preserves the privacy of $s.$ Recall that the vacuous
protocol\index{vacuous protocol} reveals no information
(\S\ref{sec-trusted-host}).

\begin{definition}  \label{def-private-rep}
A function $\sha$ is a {\defstyle $t$-private function}%
\index{private function}
if there exists a protocol $\share$ to compute $\sha$ that is as
$t$-resilient as the ideal vacuous protocol.
\end{definition}

Any function that produces the same results regardless of its inputs is
certainly private, though not necessarily robust.  Though such a function
is apparently useless at first glance, we shall find important uses.
Robustness and privacy together define secret sharing:

\begin{definition}  \label{def-threshold}
A {\defstyle threshold scheme}\index{threshold scheme} with threshold $t$
is a pair of protocols $\gensha$ and $\genrec,$ where $\gensha$ computes a
$t$-robust and $t$-private representation $\sha,$ and $\genrec$ computes
the function $\recons.$
\end{definition}


\section{Composing Functions}
\label{sec-compose-fn}

In order to develop modular protocols, let us consider protocols intended
to compute some sequence of intermediate functions.  For clarity of
exposition, first consider only two functions, $F(x_1(1),\dots,x_n(1))$ and
$G(x_1(2),\dots,x_n(2)),$ in sequence.  To be precise, the inputs to $G$
may include or be influenced by the inputs and outputs of $F.$  We
consider $x_1(2)$ to be a function of $y_1(1)$ (which
itself specifies $x_1(1),$ without loss of generality) 
and of $x_1^{new}(2),$ a new portion
of the input.  The desired application may certainly specify that
$x_1^{new}(2)$ is ignored; our protocols do not actually take advantage of
new inputs, and we shall soon omit any mention of them for
the sake of readability.

There are a few different ways to combine functions that are useful
({\em cf.} \S\ref{sec-function}):
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item $(F,G):$ the computation of the function
$H(x_1,\ldots,x_n)$ that concatenates the outputs of $F$ and $G:$
namely $H_i(x_1,\ldots,x_n)=(F_i(x_1,\ldots,x_n),G_i(x_1,\ldots,x_n)).$ 
The inputs to $G$ do not depend on the outputs of $F.$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item 
$(F;G):$ the {\em sequential} computation of 
$G$ with $F.$
The inputs to $G$ do not necessarily depend on the outputs of $F.$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item  \label{ite-open-comp}
$\opencomp \set{F,G}$ or $(F; G\circ F):$ 
the {\em open composition} of $F$ then $G,$ 
using the outputs of $F$ in the computation of $G.$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item  \label{ite-hide-comp}
$\closedcomp \set{F,G}$ or $(G \closedcomp F):$ 
the {\em hidden composition} of $G$ with $F,$ 
revealing the results of function $G \circ F$ 
without revealing the results of $F.$
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The two of greatest interest are (\ref{ite-open-comp}) 
{\em open composition}
and (\ref{ite-hide-comp}) {\em hidden composition}.
The idea of computing on hidden values, using the results of $F$ to compute
$G$ without revealing them in the interim, is extremely useful.  

A {\em collection} of function families is denoted
$\scf=\set{F^1,F^2,\ldots}$ where each $F^i$ is a family $F^i =
\set{F^{i,n,m}}.$ Let $f(n,m,k)$ be some function from integers to integers.

\begin{definition}  \label{def-closedcomp}
The {\defstyle closed composition}%
\index{composition!closed}
of $f(n,m,k)$ functions from $\scf$, written $\closedcomp \scf$ or informally
$F^{f(n,m,k)}\closedcomp \cdots \closedcomp F^1,$ is defined as the function
family $F=\set{F^{n,m}},$ where each $F^{n,m}$ is: 
\[
F^{n,m} = F^{f(n,m,k),n,m} \circ F^{f(n,m,k)-1,n,m} \circ \cdots \circ F^{1,n,m}.
\]
\end{definition}
%% The function family $G=\set{G^{n,m}}$ where
%% \[
%% G^{n,m} = F^{f(n,m,k),n,m}
%% \]
%% is called the {\em final} function (as opposed to the final result),
%% representing the last function applied in the composition.

\begin{definition}  \label{def-opencomp}
The {\defstyle open composition}%
\index{composition!open}
of $f(n,m,k)$ functions from $\scf$, written
$\opencomp \scf,$ includes the progressive results in the composition of
the $f(n,m,k)$ functions:
\[
F^{n,m\cdot f(n,m,k)} = (F^{1,n,m},F^{2,n,m}\circ F^{1,n,m},\ldots,
F^{f(n,m,k),n,m} \circ \cdots \circ F^{1,n,m}).
\]
Note the use of $m\cdot f(n,m,k)$ in the indexing; the function has an
output that is $f(n,m,k)$ times as large.  (We define the functions
$F^{n,m\cdot f(n,m,k) + a}$ for $0<a<f(n,m,k)$ to be identically 0.)
\end{definition}


\section{Concatenating Protocols}
\label{sec-compose}

We shall speak of protocols, protocol families, and collections
of protocol families; to make the presentation more clear, 
Figure~\ref{fig-proto-hier} outlines the various levels on which 
we group together and discuss protocols and the events they induce.  
Recall that a protocol execution on a particular set of inputs 
$\vec{x},$ $\vec{a},$ and $a,$ with particular values of $n,$
$m,$ and $k,$ induces a {\em distribution} on histories.  By 
varying these parameters, we consider larger and larger 
conglomerations of protocols ({\em e.g.} protocols, families 
of protocols, {\em etc.}) which induce larger and larger 
probabilistic conglomerations ({\em e.g.}, distributions, 
ensembles, families of ensembles, {\em etc.}).  

%\unboxfig{
{\begin{figure}[htb]
\mbox{
	\small
	\hbox{\quad
	\begin{minipage}{5.2in}   % was 4.8
\begin{tabular}{|l|l|l|}      \hline
Fixed & Protocol Group & History Group \\ 
Parameters  &          &               \\
\hline \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$i,n,m,$    &  
protocol on particular inputs &   
distribution \\
$k,\vec{x},\vec{a},a$ &
$\protosa(i)(n,m)\protoIn$ &
$[A,\protosa(i)](n,m)\protoIn$ \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$i,n,m$    &   
protocol  &
ensemble \\
&
$\protosa(i)(n,m)$ &
$[A,\protosa(i)](n,m)$ \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$i$    &   
family of protocols &
family of ensembles\\
&
$\protosa(i)=\{\protosa(i)(n,m)\}_{n,m \in\natsmall}$ &
$[A,\protosa(i)]=\{[A,\protosa(i)(n,m)]\}_{n,m \in\natsmall}$ \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&   
collection of families  &
collection of families \\
&
of protocols &
of ensembles \\
&
$\protosa=\{\protosa(i)\}_{i\in\natsmall}$ &
$[A,\protosa]=\{[A,\protosa(i)]\}_{i\in\natsmall}$ \\ \hline
\end{tabular}
\caption{\label{fig-proto-hier}
Hierarchy of protocols and associated probability spaces.  
After the first row, inputs $\protoIn$ are taken to vary
over all possible values.
}
	\end{minipage}
	\quad}
	}
\end{figure}
}
%}

\subsection{Concatenating General Protocols}
\label{sec-concat-prot}

Let $\protosa=\set{\protoa(1),\protoa(2),\dots}$ be a collection of
protocol families, and let $f(n,m,k)$ be some function from $\nat$ to 
$\nat.$
Let $\set{x_i^{new}(r)}_{i,r \in \natsmall}$ be a collection of
inputs that are to be supplied as the execution of the protocol progresses.
Let $\set{a_i^{new}(r)}_{i,r \in \natsmall}$ be a collection of
auxiliary inputs that are to be supplied as the execution of the protocol
progresses.  Let $x_i(1)=x_i^{new}(1)$ and $a_i(1)=a_i^{new}(1)$ for all
$i.$ Let $\set{\chi^{n,i,r}}_{n,i,r \in \natsmall}$ be a
collection of probabilistic functions mapping an output and auxiliary input
to a new input.

The {\em sequential concatenation}\index{concatenation} of protocols in
$\protosa$ is the protocol described in Figure~\ref{fig-concat} and is written
$\circ \protosa,$ or $\protoconc_{i=1}^{f(n,m,k)} \protoa(i),$ or
$(\protoa(1);\protoa(2);\ldots;\protoa(f(n,m,k))).$ For each $n,$
$f(n,m,k)$ protocols are executed in turn.  The input of player $i$ to the
$r^{th}$ protocol is denoted $x_i(r).$ Before the $r^{th}$ protocol is
executed, each player $i$ obtains an external auxiliary input,
$a_i^{new}(r),$ which is combined with its view of previous executions to
provide the auxiliary input $a_i(r)$ for the $r^{th}$ protocol.  Player $i$
chooses an input $x_i(r)$ for the $r^{th}$ protocol based on the output of
the previous protocol $y_i(r-1)$ and its new input $x_i^{new}(r),$
according to the function $\chi^{n,i,r}.$ This allows the player to base its
next input on the results of previous protocols as well as other
information it may have.  The functions $\chi^{n,i,r}$ are part of the
protocol and players are required to use them; the protocol designer is
free to specify that players ignore previous outputs or that they use them
in some particular way.  Note that players corrupted by a Byzantine
adversary are certainly allowed to specify inputs chosen differently.

We must include one restriction on the adversary: the set of players it
corrupts throughout the entire concatenated protocol must be a subset of
some allowable coalition in the fault class.  Formally, if the adversary
classes are $\sca_1,\sca_2,\ldots,$ then the adversary class for the
concatenation of protocols is $\sca= \cap \sca_r.$ In each successive
execution, the adversary may be treated as a new adversary receiving the
view of the previous execution as its auxiliary input.


\figstretch
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Figure:  Concatenating Protocols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\boxfig{
\noindent{\bf \protostyle Concat-Protocol}($\protosa,f(n,m,k)$)%
\index{concatenation!protocol}
\begin{tabbing} \standtabs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
(CP1) \> Run protocol $\protoa(1):$ \\
\>\>\>
$\view(1) \leftarrow \ensAAlphao(n,m)\protoIn$ \\
\>\>\>
$y_i(1) \leftarrow Y_i(\view_i(1))$ 
\>\>\>\>\> $(1 \leq i \leq n)$ \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\
(CP(r)) \> {\For $r=2..f(n,m,k)$ \Do} \\
\>\>\>
$a_i(r) \leftarrow (\view_i(r-1),a_i^{new}(r))$ 
\>\>\>\>\> $(1 \leq i \leq n)$ \\
\>\>\>
$a(r) \leftarrow (\view_A(r-1),a^{new}(r))$ \\
\>\>\>
$x_i(r) \leftarrow \chi^{n,i,r}(y_i^{r-1},x_i^{new}(r))$ 
\>\>\>\>\> $(1 \leq i \leq n)$ \\
\>\>\>
$\view(r) \leftarrow \ensAAlphar(n,m)\protoInr$
\\
%\>\>\>\>\> \ccomment{Run subprotocol} \\
\>\>\>
$y_i(r) \leftarrow Y_i(\view_i(r))$ 
\>\>\>\>\> $(1 \leq i \leq n)$
\end{tabbing}
\caption{\label{fig-concat}
Concatenation of $f(n,m,k)$ protocols from the collection of protocol families 
$\protosa=\set{\protoa(1),\protoa(2),\ldots}.$
}}
\figstretchend





\subsection{Concatenating Ideal Protocols}
\label{sec-concat-ideal}

Though the definitions of \S\ref{sec-concat-prot} demonstrate how ideal
protocols are concatenated, the direct concatenation of ideal protocols
will not provide quite the level of security and reliability we desire.
Operating two protocols $\idealname(F)$ and $\idealname(G)$ in sequence
does not ensure that the inputs to the second protocol are in any way
related to the inputs or outputs of the first.  That is, a corrupt player
might obtain $y_i(1)$ as its output of $F$ but instead supply
$(y_i(1)+1,x_i^{new}(2))$ as its input $x_i(2)$ to $G.$

In many circumstances this is quite undesirable.  For example, the
employees of a company might wish to calculate their average overall salary
and the average salary of management.  First, they compute the overall
average.  For the second computation, however, the management may report
lower salaries to obtain an advantage in salary negotiations.

As defined in \S\ref{sec-function}, let $\scf=\set{F^i}_{i \in
\natsmall}$ be a possibly infinite collection of families
$F^i=\set{F^{i,n,m}}$ of finite functions, and let $f : \nat^3 \rightarrow
\nat.$  (We normally take $f(n,m,k)$ to be polynomial.)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}   \label{def-open-concat-ideal}
The {\defstyle open concatenation of $f$ ideal protocols}% 
\index{concatenation!ideal}
using $\set{\chi^{n,i,r}}_{n,i,r \in \natsmall}$
%according to \S\ref{sec-concat-prot}, 
is the following protocol, denoted by
$\ocip= \circ_i \idealname(F^i).$  Consider $n+f(n,m,k)$ players.
A $t$-fault class is, as usual, the collection of subsets of $[n];$ players
$i > n$ are incorruptible.  The protocol requires $2f(n,m,k)$ rounds;
let $r$ range from $1$ to $f(n,m,k):$ 
\begin{description}
\item[(Round $1$)]
Each player $i \in [n]$ sends $x_i(1)=x_i$ to trusted player $(n+1).$
\item[(Round $2$)]
Player $(n+1)$ computes the value $F^1(x_1,\ldots,x_n)$ and returns the
results.
\item[(Round $2r-1$)]
Each player $i\in [n]$ chooses an input $x_i(r) \leftarrow
\chi^{n,i,r}(y_i(r-1),x_i^{new}(r-1))$ and sends it to trusted player $(n+r).$
\item[(Round $2r$)]
Player $(n+r)$ computes the value $F^r(x_1,\ldots,x_n)$ and returns
$y_i(r)$ to each player $i\in [n].$
\end{description}
\end{definition}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Technically, the objection to simply concatenating protocols directly is
the following.  Operating ideal protocols in sequence invokes {\em
different} trusted parties, one to compute $F^1,$ one to compute $F^2,$ and
so on.  None of the trusted parties share any information or communicate at
all.

The ideal {\em composite} protocol%
\index{composite protocol!ideal}
should have {\em one} trusted party.  The protocol is slightly longer:
first the trusted host requests $x_1(1),\ldots,x_n(1),$ and returns
$F^1(x_1(1),\ldots,x_n(1)).$ The host retains the values of the outputs.
Since the inputs to the next computation are each some function of the
previous output and a new input, the players themselves need only supply
the new input, and the host can compute the next round's inputs using
$x_i(r) \leftarrow \chi^{n,i,r}(y_i(r-1),x_i^{new}(r)).$ This prevents
changing the output of previous protocols, while permitting a protocol
designer to include new information during the protocol if desired.  More
specifically:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}   \label{def-idoc}
The {\defstyle ideal open composite protocol}%
\index{composite protocol!ideal open}
for $p$ functions from $\scf,$
using $\set{\chi^{n,i,r}}_{n,i,r \in \natsmall},$ is the following
protocol, denoted $\idoc.$ For each $n,$ consider $n+1$ players.  Player
$(n+1)$ is incorruptible; the $t$-fault class is the collection of subsets
of $[n].$ The protocol requires $2f(n,m,k)$ rounds:
\begin{description}
\item[(Round $1$)] 
Each player $i\in [n]$ sends $x_i(1)$ to trusted player $(n+1).$
\item[(Round $2$)]
Player $(n+1)$ computes the value $F^1(x_1,\ldots,x_n)$ and returns
$y_i(1)=F^1_i(x_1,\ldots,x_n)$ to each player $i \in [n].$
\item[(Round $2r-1$)]
Each player $i \in [n]$ sends $x_i^{new}(r)$ to the trusted host.
\item[(Round $2r$)]
In round $2r,$ player $(n+1)$ ({\em not} player $i$) computes $x_i(r)
\leftarrow \chi^{n,i,r}(y_i(r-1),x_i^{new}(r)),$ the next ``input'' for player
$i.$ Player $(n+1)$ then computes the value $F^r(x_1(r),\ldots,x_n(r))$ and
returns $y_i(r)$ to each player $i \in [n].$
\end{description}
\end{definition}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}   \label{def-idhc}
The {\defstyle ideal hidden composite protocol},%
\index{composite protocol!ideal hidden}
$\idhc,$ is the same as $\idoc$ except that in intermediate rounds the
trusted host always returns the same results as the vacuous protocol ({\em
i.e.} a vector describing honest and cheating players) instead of $y_i^r.$
In the final round, the trusted host does return the final result.
\end{definition}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Our ultimate goal is to achieve the two protocols $\idoc$ and $\idhc,$
since they ensure that information is consistent from one function
evaluation to the next.  Section~\ref{sec-compose-proof} presents a method
to ensure that the concatenation of ideal protocols does in fact achieve
the same results as an ideal composite protocol with a single trusted
host.  Verifiable secret sharing is essential, both for maintaining
consistency and for hiding progressive results.  For clarity, we shall omit
mention of the new inputs $x_i^{new}$ and of the functions $\chi^{n,i,r}.$


\section{The Modular Approach}
\label{sec-compose-proof}

The key to achieving efficiency is to avoid evaluating a circuit for $F$
directly, and instead to break the computation of $F$ into the computation
of several functions $F^1,\ldots,F^{f(n,m,k)},$ each of which reveals nothing
about the inputs.  Each of these computations is itself broken up into a
composition of fundamental operations $G,$ such as addition and
multiplication, according to the established paradigm.  Each input is
shared as a secret using a robust representation.  Instead of using the
fundamental computations, which would reveal information, {\em robust} and
{\em private} representations $\robsec(G)$ are used to compute pieces of
new secrets from the old ones.  For example, secrets are added or
multiplied, but the inputs and outputs are maintained in shared form.  The
use of a robust and private representation (secret sharing) allows us to
compute {\em open} compositions of functions, which allows us simply to
concatenate subprotocols.  It also provides the glue to ensure that the
computations are insensitive to faulty players who fail to supply the
output of one subprotocol as the input to the next.

The supporting machinery \cite{bgw88,ccd88} establishes how to compute each
intermediate function $F^i$ by reducing it to simple operations on secrets.
We shall use the protocols of Ben-Or {\em et al} (see
\S\ref{sec-fundamental}) for these simple operations.  We achieve vast
improvements in efficiency through careful choice of the intermediate
functions (see \S\ref{sec-const-nc}).  In the remainder of this chapter we
give formal arguments for the validity of our methods.

Using more formal notation, the general technique is as follows.  Function
family $F$ is first represented as the open composition $\opencomp \scf$ of
some collection of function families, each of which is private.  In other
words, $F$ is decomposed into a sequence of intermediate functions whose
results can be revealed openly without compromising essential information.
Then, each family $F^i$ in the collection is itself written as a {\em
hidden} composition of a collection $\scg^i$ containing more fundamental
functions (such as addition and multiplication).  In other words, we should
like that each $F^i$ is computed as a composition of fundamental functions
$\set{G^{ij}},$ even though the intermediate results of these computations
{\em cannot} be revealed.  Finally, to facilitate the hidden composition of
these fundamental functions, each fundamental function $G^{ij}$ must have a
private and robust representation $\robsec(G^{ij}).$ In other words,
$\robsec(G^{ij})$ is essentially a function that operates on secret pieces
of the inputs to $G^{ij}$ and produces secret pieces of the results of
$G^{ij},$ rather than producing the results themselves.  Diagrammatically:
\begin{eqnarray*}
F & \rightarrow & \opencomp_i \set{F^i} \\
F^i &  \rightarrow  & \closedcomp_j \set{G^{ij}} \\
G^{ij} & \rightarrow & \robsec(G^{ij})
\end{eqnarray*}

%% We remark that the following observations may be sensitive to the choice of
%% {\em perfect} relative resilience ($\resilas$).  Similar statements can be
%% made for weaker versions of indistinguishability, but a technical
%% requirement called {\em post-protocol corruptibility} (the ability of the
%% simulator to generate views of reliable players after the protocol has
%% finished) will be essential.


\section{Indistinguishability}
\label{sec-indisting-more}

In \S\ref{sec-def-indist} we defined how two ensembles are
indistinguishable, and we defined how two families of ensembles
(parametrized by $n$ and $m$) are indistinguishable.  In order to examine
concatenations of many protocols and in order to facilitate proofs of
resilience, we define indistinguishability for {\em collections} of ensemble
families and collections of protocol families.

\subsection{Collections of Families of Ensembles}
\label{sec-coll-fam-ens}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  ENSEMBLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let $\enssa=\set{\ensa(i)}_{i \in \natsmall}$ be a collection of families
of ensembles.  For concreteness, note that $\ensa(i)$ is a family of
ensembles, $\ensa(i)(n,m)$ is an ensemble, and $\ensa(i)(n,m)(z,k)$ is a
distribution on strings.  Let $\enssb=\set{\ensb(i)}_{i \in \natsmall}$
also be a collection of families of ensembles.  In the spirit of
mathematical analysis we define uniform indistinguishability, where
``uniform'' indicates not Turing machines but the flavor of uniform {\em
vs.} pointwise convergence.  We require that for any $n$ and $m,$ there is
a bound $\delta(i,k)$ on the closeness of corresponding ensembles
$\ensa(i)(n,m)$ and $\ensb(i)(n,m),$ and that the bound is approached
uniformly for all $i:$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   PAIRWISE  ENSEMBLE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}
Two collections of ensemble families $\enssa=\set{\ensa(i)}$ and
$\enssb=\set{\ensb(i)}$ are 
\begin{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
{\defstyle pairwise $O(\delta(i,k))$-indistinguishable}%
\index{indistinguishable!pairwise}%
%\index{$\indistCo$}
if for all $i,$ $\ensa(i) \indistFa^{O(\delta(i,k))} \ensb(i).$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
{\defstyle uniformly pairwise $O(\delta(i,k))$-indistinguishable}%
\index{indistinguishable!pairwise uniform}
if
\[
(\exists \Delta: \nat \rightarrow \nat) 
\mbox{\hspace{0.2in}}
(\forall i)
\mbox{\hspace{0.1in}}
\ensa(i) \indistEn^{\Delta(i,k)} \ensb(i)
\mbox{\hspace{0.3in} \rm and }
\Delta(k) = O(\delta(k)).
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% computational
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
{\defstyle pairwise $O(\delta(i,k))$-computationally indistinguishable}%
\index{indistinguishable!pairwise!computationally}
if for all $i,$ $\ensa(i) \indistFaC^{O(\delta(i,k))} \ensb(i).$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
{\defstyle uniformly pairwise $O(\delta(i,k))$-computationally
indistinguishable}%
\index{indistinguishable!pairwise uniform!computational}
if
\[
(\forall n,m)
(\forall A \in \mbox{\sc PPC})
(\exists c, k_0)
(\forall k \geq k_0)
(\forall z)
(\forall i)
\]
\[
\abs{A_{\ensa(i)(n,m)(z,k)}-A_{\ensb(i)(n,m)(z,k)}} \leq 
c \cdot \delta(i,k).	
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{itemize}
We write 
$\enssa \indistCo^{O(\delta(k))}%
\index{$\indistCo,$ uniformly indistinguishable collection}
\enssb$ 
for the uniform case
and 
$\enssa \indistCoC^{O(\delta(k))}%
\index{$\indistCoC,$ uniformly computationally indistinguishable collection}
\enssb$ for the uniform computational case.
\end{definition}
The essential point is that for {\em uniform} indistinguishability, the
same convergence parameter $k_0$\index{convergence parameter} applies to
all the families simultaneously.  That is, the closeness of the
corresponding pairs converges for sufficiently large $k,$ but the rate of
convergence ({\em i.e.} the point at which the families are thereafter
close) is the same for all pairs at once.  Clearly, any two equally-sized
{\em finite} collections of ensemble families are {\em uniformly} pairwise
$O(\delta(i,k))$-indistinguishable if they are
$O(\delta(i,k))$-indistinguishable.


We also examine a {\em single} collection of ensemble families with the
property that each ensemble is indistinguishable from its successor.
Before, there need be no relationship among families in the same
collection, whereas now we require one.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   SEQUENTIAL  ENSEMBLE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}    \label{def-seq-unif-indis}
A collection $\enssa=\set{\ensa(i)}$ of families of ensembles is
\begin{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
{\defstyle sequentially $O(\delta(k))$-indistinguishable}%
\index{indistinguishable!sequential} 
if for all $i,$ $\ensa(i) \indistFa^{O(\delta(k))} \ensa(i+1).$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
{\defstyle uniformly sequentially $O(\delta(k))$-indistinguishable}%
\index{indistinguishable!sequential uniform}
if
\[
(\exists \Delta: \nat \rightarrow \nat) 
\mbox{\hspace{0.2in}}
(\forall i)
\mbox{\hspace{0.1in}}
\ensa(i) \indistFa^{\Delta(k)} \ensa(i+1)
\mbox{\hspace{0.3in} \rm and }
\Delta(k) = O(\delta(k)).
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% computational
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
{\defstyle sequentially $O(\delta(k))$-computationally indistinguishable}%
\index{indistinguishable!sequential!computational}
if for all $i,$ $\ensa(i) \indistFaC^{O(\delta(k))} \ensa(i+1).$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
{\defstyle uniformly sequentially $O(\delta(k))$-computationally
indistinguishable}%
\index{indistinguishable!sequential uniform!computational}
if
\[
(\forall n,m)
(\forall A \in \mbox{\sc PPC})
(\exists c,k_0)
(\forall k \geq k_0)
(\forall z)
(\forall i)
\]
\[
\abs{A_{\ensa(i)(n,m)(z,k)}-A_{\ensa(i+1)(n,m)(z,k)}} \leq c \cdot \delta(k).
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{itemize}
\end{definition}
Clearly, any {\em finite} collection of ensemble families is {\em uniformly}
$O(\delta(k))$-indistinguishable if each successive pair of families is
$O(\delta(k))$-indistinguishable.




\subsection{Collections of Families of Protocols}
\label{sec-coll-fam-pro}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  PROTOCOLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The relative resilience of two collections of {\em protocol} families is
defined in a similar fashion as ensemble families: according to the
relative resilience of each corresponding pair of protocols.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   PAIRWISE  PROTOCOL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}  \label{def-rel-res-coll-prot}
Let $\protosa=\set{\protoa(i)}$ and $\protosb=\set{\protob(i)}$ be
collections of protocol families.  Then $\protosa$ is 
\begin{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
{\defstyle pairwise $O(\delta(i,k))$-resilient}%
\index{resilience!pairwise}
{\defstyle as} $\protosb$ if for all $i,$ 
$\protoa(i) \resilasFa^{O(\delta(i,k))} \protob(i).$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
{\defstyle uniformly pairwise $O(\delta(i,k))$-resilient}%
\index{resilient!pairwise uniform}
{\defstyle as} $\protosb$ if 
\[
(\exists \Delta: \nat^2 \rightarrow \nat) 
\mbox{\hspace{0.2in}}
(\forall i)
\mbox{\hspace{0.1in}}
\protoa(i) \resilasFa^{\Delta(i,k)} \protob(i)
\mbox{\hspace{0.3in} \rm and }
\Delta(i,k) = O(\delta(i,k)).
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{itemize}
We write $\enssa \resilasCo^{O(\delta(i,k))}\index{$\resilasCo,$ uniformly
resilient collection} \enssb$ for the uniform case.
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   SEQUENTIAL  PROTOCOL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}    \label{def-seq-unif-resil}
A collection $\protosa=\set{\protoa(i)}$ of protocol families
\begin{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
{\defstyle sequentially $O(\delta(k))$-resilient}%
\index{resilience!sequential}
if for all $i,$ $\protoa(i) \resilasFa^{O(\delta(k))} \protoa(i+1).$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item
{\defstyle uniformly sequentially $O(\delta(k))$-resilient}%
\index{resilience!sequential uniform}
if
\[
(\exists \Delta: \nat \rightarrow \nat) 
\mbox{\hspace{0.2in}}
(\forall i)
\mbox{\hspace{0.1in}}
\protosa(i) \resilasFa^{\Delta(k)} \protosa(i+1)
\mbox{\hspace{0.3in} \rm and }
\Delta(k) = O(\delta(k)).
\]
\end{itemize}
\end{definition}

The adjectives {\em perfect, exponential, statistical,} and {\em
computational} apply respectively, as in \S\ref{sec-def-indist} and
\S\ref{sec-coll-fam-ens}, {\em mutatis mutandis.}


\section{Indistinguishable Ensembles: Technical Lemmas}

%%%%%%%%%%%%%%%%%%%%% LEMMATA lemmata %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LEMMA   substring indistinguishability
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Two indistinguishable ensembles remain indistinguishable
when restricted to simple subranges of the samples.  
\begin{lemma}  \label{lem-ind-subrange}
(Indistinguishable Substrings) 
Let $\scg=\set{G(z,k)}$ and $\sch=\set{H(z,k)}$ be
ensembles where each $G(z,k)$ and $H(z,k)$ is a distribution on $\Sigma^{f(\abs{z},k)}.$  
Let $a(z,k)$ and $b(z,k)$ be
polynomial-time computable indices in the range $1,\ldots,f(\abs{z},k)),$ with
$a(z,k) \leq b(z,k).$  
Let $G[a,b](z,k)$ be the distribution
\[
\set{ \sigma \leftarrow G(z,k); \tau \leftarrow \sigma[a(z,k)..b(z,k)]:
\tau}
\]
and define $H[a,b](z,k)$ similarly.
Then subranges are indistinguishable:
\begin{eqnarray}
\scg \indistEn \sch & \Rightarrow & \scg[a,b] \indistEn \sch[a,b] 
\label{eqn-subone} \\
\scg \indistEnE \sch & \Rightarrow & \scg[a,b] \indistEnE \sch[a,b] 
\label{eqn-subtwo} \\
\scg \indistEnS \sch & \Rightarrow & \scg[a,b] \indistEnS \sch[a,b] 
\label{eqn-subthree} \\
\scg \indistEnC\sch & \Rightarrow & \scg[a,b] \indistEnC \sch[a,b]
\label{eqn-subfour} 
\end{eqnarray}
\end{lemma}

\begin{proof}
Statements (\ref{eqn-subone})-(\ref{eqn-subthree}) follow by observing that
$\scg \indistEn^{\delta(k)} \sch \Rightarrow \scg[a,b] \indistEn^{\delta(k)}
\sch[a,b],$ as shown by:
\begin{eqnarray*}
\abs{\probb{\scg[a,b]}{\tau}-\probb{\sch[a,b]}{\tau}}
& = &
\abs{\sum \probb{\scg}{\sigma \mid \tau}-\probb{\sch}{\sigma \mid \tau}}
\\
& = &
\abs{\sum_{\sigma \mid \sigma[a..b]=\tau} \probb{\scg}{\sigma} -
\sum_{\sigma \mid \sigma[a..b]=\tau} \probb{\sch}{\sigma}}
\\
& \leq & \delta(k),
\end{eqnarray*}
which holds for for sufficiently large $k,$ by the indistinguishability of
$\scg$ and $\sch.$

To verify (\ref{eqn-subfour}), which describes computational
indistinguishability, let us assume it fails.  Then there exists a machine
$M$ that distinguishes $G[a,b]$ from $H[a,b].$ Construct machine $M'$ which
does the following: on input $\sigma$ of length $n^c,$ set
$\tau=\sigma[a(n)..b(n)],$ run $M$ on $\tau,$ and use its output.  Now, for
any $c,$ the distinguisher $M$ outputs 0 with different probabilities:
%
$\abs{M_{G[a,b]}[\tau] - M_{H[a,b]}[\tau]} \geq n^{-c}$ 
%
infinitely often.  Clearly, 
%
$M'_{G}[\sigma] = M'_{G[a,b]}[\tau]$ and 
$M'_{H}[\sigma] = M'_{H[a,b]}[\tau].$ 
%
Therefore for any $c,$ 
%
$\abs{M'_{G}[\sigma] - M'_{H}[\sigma]} \geq n^{-c}$
%
infinitely often, contradicting the indistinguishability of $\scg$ and
$\sch.$
\end{proof}


Observe that replacing one ensemble in a series by an indistinguishable
ensemble gives rise to an indistinguishable entire series:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LEMMA   feed distributions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}  \label{lem-feed-dist}
Let $\scp_1, \scp_2^{\alpha}, \scp_2^{\beta},$ and $\scp_3$ be ensembles.
Define the ensembles
\begin{eqnarray*}
\scq^{\alpha}(z,k) & = & 
\{
z_1 \leftarrow \scp_1(z,k);
z_2^{\alpha} \leftarrow \scp_2^{\alpha}(z_1,k);
z_3^{\alpha} \leftarrow \scp_3(z_2^{\alpha},k):
z_3^{\alpha}
\} \\
\scq^{\beta}(z,k) & = & 
\{
z_1 \leftarrow \scp_1(z,k);
z_2^{\beta} \leftarrow \scp_2^{\beta}(z_1,k);
z_3^{\beta} \leftarrow \scp_3(z_2^{\beta},k):
z_3^{\beta}
\}
\end{eqnarray*}
If $\scp_2^{\alpha} \indistEn^{O(\delta(k))} \scp_2^{\beta},$
then $\scq^{\alpha} \indistEn^{O(\delta(k))} \scq^{\beta}.$  
The convergence parameters are identical.
\end{lemma}

\begin{proof}
Let $k_0$ be the convergence parameter for $\scp_2^{\alpha}$ and
$\scp_2^{\beta},$ 
with associated constant $c_0.$
Assume by way of contradiction that $\scq^{\alpha}
{\notindistEn}^{O(\delta(k))}
\scq^{\beta}.$  Then there is a $k \geq k_0$ and a $z$ such that
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{eqnarray*}
\sum_{z_1,z_2,z_3} \mid
\probb{\scp_3(z_2,k)}{z_3}
\probb{\scp_2^{\alpha}(z_1,k)}{z_2}
\probb{\scp_1(z,k)}{z_1} & & \\
-
\probb{\scp_3(z_2,k)}{z_3}
\probb{\scp_2^{\beta}(z_1,k)}{z_2}
\probb{\scp_1(z,k)}{z_1} \mid 
& > &
c_0 \cdot \delta(k)
\end{eqnarray*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Thus there exists a $z_1$ such that
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{eqnarray*}
\sum_{z_2,z_3} 
\mid (
\probb{\scp_3(z_2,k)}{z_3}
\probb{\scp_2^{\alpha}(z_1,k)}{z_2} & & \\
-
\probb{\scp_3(z_2,k)}{z_3}
\probb{\scp_2^{\beta}(z_1,k)}{z_2}
) \mid
& > &
c_0 \cdot \delta(k)
\end{eqnarray*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
It follows that
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{eqnarray*}
\sum_{z_2} 
\abs{
\probb{\scp_2^{\alpha}(z_1,k)}{z_2}
- \probb{\scp_2^{\beta}(z_1,k)}{z_2} 
} 
& = & \\
\sum_{z_2}
\left(
\sum_{z_3} \probb{\scp_3(z_2,k)}{z_3} \cdot
\abs{
\probb{\scp_2^{\alpha}(z_1,k)}{z_2}
-
\probb{\scp_2^{\beta}(z_1,k)}{z_2}
}
\right)
& > &
c_0 \cdot \delta(k).
\end{eqnarray*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Since $k \geq k_0,$ this contradicts $\scp_2^{\alpha}
\indistEn^{O(\delta(k))} \scp_2^{\beta}.$
\end{proof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LEMMA   feed distributions, computational
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}  \label{lem-feed-dist-compose}
Let $\scp_1, \scp_2^{\alpha}, \scp_2^{\beta},$ and $\scp_3$ be polynomially
generable and let $\scq^{\alpha}$ and $\scq^{\beta}$ be as in
Lemma~\ref{lem-feed-dist}.  
If $\scp_2^{\alpha} \indistEnC^{\delta(k)} \scp_2^{\beta}$ then
$\scq^{\alpha} \indistEnC^{\delta(k)} \scq^{\beta}.$
\end{lemma}

\begin{proof}
Let $k_0$ be the convergence parameter for $\scp_2^{\alpha}$ and
$\scp_2^{\beta}.$ 
Assume by way of contradiction that $\scq^{\alpha}
{\notindistEnC}^{\delta(k)} \scq^{\beta}.$
Then there exists a probabilistic polynomial size distinguisher $A$ such
that for some $z$ and infinitely many $k,$
\[
\abs{A_{\scq^{\alpha}(z,k)} - A_{\scq^{\beta}(z,k)}} > \delta(k).
\]
Now, $A_{\scq^{\alpha}(z,k)}$ is just
\[
\sum_{z_1,z_2,z_3}
\probb{A(z_3)}{1}
\probb{\scp_3(z_2,k)}{z_3}
\probb{\scp_2^{\alpha}(z_1,k)}{z_2}
\probb{\scp_1(z,k)}{z_1}
\]
so there exists a $z_1$ such that
\begin{eqnarray*}
\sum_{z_2,z_3}
\mid (
\probb{A(z_3)}{1}
\probb{\scp_3(z_2,k)}{z_3}
\probb{\scp_2^{\alpha}(z_1,k)}{z_2} & & \\
-
\probb{A(z_3)}{1}
\probb{\scp_3(z_2,k)}{z_3}
\probb{\scp_2^{\beta}(z_1,k)}{z_2}
) \mid & & \\
& > & \delta(k).
\end{eqnarray*}
Let $A'$ be the distinguisher that does the following.  On input $\sigma,$ 
sample $z_3 \leftarrow \scp_3(\sigma,k),$ and run $A(z_3).$  Return the
result of $A.$  It follows that
\begin{eqnarray*}
& & 
\mid
A'_{\scp_2^{\alpha}(z_1,k)} - A'_{\scp_2^{\beta}(z_1,k)}
\mid
\\
& = & 
\mid
\probb{A(z_3)}{1}
\probb{\scp_3(z_2,k)}{z_3}
\probb{\scp_2^{\alpha}(z_1,k)}{z_2}
\\ & & 
-
\probb{A(z_3)}{1}
\probb{\scp_3(z_2,k)}{z_3}
\probb{\scp_2^{\beta}(z_1,k)}{z_2}
\mid
\\
& > & \delta(k).
\end{eqnarray*}
Since this holds for some $z$ and $z_1,$ and for
infinitely many $k,$ $A'$ actually distinguishes
$\scp_2^{\alpha}$ from $\scp_2^{\beta},$ so $\scp_2^{\alpha}
{\notindistEnC}^{\delta(k)} \scp_2^{\beta}.$
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LEMMA   one sequence
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Given a collection of ensemble families and a function $f(n,m,k),$ we may
define a particular ensemble family using the $k^{th}$ distribution from
the $f(n,m,k)^{th}$ family.  
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}       \label{def-diagonal}
The {\defstyle diagonal ensemble family}%
\index{diagonal!ensemble}
$\ensa^f$ of a collection of ensemble families
$\enssa=\set{\ensa(0),\ensa(1),\ldots}$ is, for a given function $f: \nat^3
\rightarrow \nat,$ defined by the following:
\[
\ensa^f(n,m)(z,k) = \ensa(f(n,m,k))(n,m)(z,k).
\]
The {\defstyle diagonal protocol family}%
\index{diagonal!protocol}
$\protoa^f$ for a collection of protocol families
$\protosa=\set{\protoa(1),\protoa(2),\ldots}$ is the protocol defined by:
\[
\protoa^f(n,m)\protoIn  =
\protoa(f(n,m))(n,m)\protoIn.
\]
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%

The first ensemble family in a sequentially indistinguishable collection is
indistinguishable from the diagonal family to a certain degree:
\begin{lemma}  \label{lem-seq-ens}
Let $\enssa=\{\ensa(0),\ensa(1),\ldots \}$ be a uniformly sequentially
$O(\delta(k))$-indistinguishable collection of families of ensembles, and let
$f : \nat^3 \rightarrow \nat.$
Then $\ensa(0) \indistFa^{O(\delta(k) \cdot f(n,m,k))} \ensa^f.$
\end{lemma}

\begin{proof}
Let $k_0$ be the convergence parameter for $\enssa.$ Assume by way of
contradiction that $\ensa(0) {\notindistFa}^{\delta(k) \cdot f(n,m,k)}
\ensa^f.$ Then there are $n$ and $m$ such that $\ensa(0)(n,m)
{\notindistEn}^{\delta(k) \cdot f(n,m,k)} \ensa^f(n,m).$ Let $c$ be
arbitrary; there exists a $k \geq k_0$ and a $z$ such that
\[
\abs{\ensa(0)(n,m)(z,k) - \ensa(f(n,m,k))(n,m)(z,k)} > 
c \cdot \delta(k)f(n,m,k).
\]
That is,
\[
\abs{
\sum_{i=0}^{f(n,m,k)-1}
\ensa(i)(n,m)(z,k) - \ensa(i+1)(n,m)(z,k)
} > c \cdot \delta(k)f(n,m,k).
\]
So for some $i_0,$ we have $k \geq k_0$ and
\[
\abs{
\ensa(i_0)(n,m)(z,k) - \ensa(i_0+1)(n,m)(z,k)
} > \frac{c \cdot \delta(k)f(n,m,k)}{f(n,m,k)} = c \cdot \delta(k),
\]
contradicting the uniform $\delta(k)$-indistinguishability of $\enssa.$
\end{proof}

Adapting this proof to computational indistinguishability in a fashion
similar to the proofs of of Lemmas \ref{lem-feed-dist} and
\ref{lem-feed-dist-compose}, a similar result holds for {\em computational}
indistinguishability.
that 
\begin{lemma}  \label{lem-seq-ens-compose}
Let $\enssa$ be a uniformly sequentially $O(\delta(k))$-computationally
indistinguishable collection of families of ensembles.  Let each ensemble
be polynomially generable. Let $f(n,m,k)$ be a polynomial.
Then $\ensa(0) \indistFaC^{O(\delta(k) \cdot f(n,m,k))} \ensa^f.$
\end{lemma}

The following lemma summarizes direct consequences of Lemmas
\ref{lem-seq-ens} and \ref{lem-seq-ens-compose}:
\begin{lemma}  \label{lem-seq-ens-summary}
Let $\enssa$ be a uniformly sequentially $O(\delta(k))$-indistinguishable
collection of families of ensembles.  Let $f(n,m,k)$ be a polynomial. Then the
following hold according to the indistinguishability of $\enssa:$
\[
\begin{tabular}{lcrllcrcl}
perfect  &   $[(\forall i)$ &
$\ensa(i)$ & $\indistFa$ & $\ensa(i+1)]$
$\Rightarrow$ &  $\ensa(0)$ & $\indistFa$ & $\ensa^f$ \\
exponential & $[(\forall i)$ &
$\ensa(i)$ & $\indistFa^{O(c^{-k})}$ & $\ensa(i+1)]$
$\Rightarrow$ &  $\ensa(0)$ & $ \indistFaE$ & $\ensa^f$ \\
statistical & $[(\forall i)$ &
$\ensa(i)$ & $\indistFa^{O(k^{-c})}$ & $\ensa(i+1)]$
$\Rightarrow$ &  $\ensa(0)$ & $\indistFaE$ & $\ensa^f$ \\
computational & $[(\forall i)$ &
$\ensa(i)$ & $\indistFaC^{O(k^{-c})}$ & $\ensa(i+1)]$
$\Rightarrow$ &  $\ensa(0)$ & $\indistFaC$ & $\ensa^f$
\end{tabular}
\]
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LEMMA   pairwise
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We also consider the indistinguishability of two diagonal ensemble families
taken from two pairwise uniformly indistinguishable collections.

\begin{lemma}  \label{lem-pair-ens}
Let $\enssa=\{\ensa(i)\}$ and $\enssb=\{\ensb(i)\}$ be uniformly
$O(\delta(i,k))$ pairwise indistinguishable collections of families of
ensembles, and let $f : \nat^3 \rightarrow \nat.$ Then $\hat{\ensa}^f
\indistFa^{O(\delta(f(n,m,k),k))} \hat{\ensb}^f.$
\end{lemma}

\begin{proof}
Let $k_0$ be the convergence parameter for $\enssa.$ Assume by way of
contradiction that $\hat{\ensa}^f 
{\notindistFa}^{O(\delta(i,k) \cdot f(n,m,k))}
\hat{\ensb}^f.$ Then there are $n$ and $m$ such that $\ensa(f(n,m,k))(n,m)
{\notindistEn}^{O(\delta(i,k) \cdot f(n,m,k))} \ensb(f(n,m,k))(n,m).$ 
Hence for an arbitrary $c,$ there is a $k \geq k_0$ and a $z$ such that
\[
\abs{\ensa(f(n,m,k))(n,m)(z,k) - 
\ensb(f(n,m,k))(n,m)(z,k)} > c \cdot \delta(f(n,m,k),k)
\]
contradicting the {\em uniform} pairwise $O(\delta(i,k))$ indistinguishability
of $\enssa$ and $\enssb.$
\end{proof}

As before, the proof is adaptable to {\em computational}
indistinguishability, giving:
\begin{lemma}  \label{lem-pair-ens-compose}
Let $\enssa=\{\ensa(i)\}$ and $\enssb=\{\ensb(i)\}$ be uniformly
$O(\delta(i,k))$ pairwise computationally indistinguishable collections of
families of ensembles, and let $f$ be a polynomial.  Then $\hat{\ensa}^f
\indistFaC^{O(\delta(f(n,m,k),k))} \hat{\ensb}^f.$
\end{lemma}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{Formal Proofs}
\label{sec-mod-formal}

Generally, an interface creates a {\em simulated environment} for the
adversary.  Consider the collection of random variables describing the
views of all the players generated during a run of a given protocol:
\[
\set{\view_1^1,\ldots,\view_n^1,\view_A^1;
\view_1^2,\ldots,\view_n^2,\view_A^2;\ldots;
\view_1^R,\ldots,\view_n^R,\view_A^R}.
\]
With static adversaries, the interface need only keep track of a fixed
subset of these views.  Interfacing becomes more difficult when dynamic
adversaries are considered: even though the variables are dependent on one
another, the interface will not be able to specify in advance all of the
necessary views.  The interface must be able to answer two types of queries
from an adversary: requests for rushed messages, and requests for the view
of a newly corrupted player.  It computes these incrementally; as the
interaction between $\interface$ and $A$ progresses, $\interface$ 
fills in some of the views
(corresponding to newly corrupted players) as necessary.  For instance, if
player $i$ is corrupted at round $r,$ the interface must sample the values
of the variables $\view_i^1,\view_i^2,\ldots,\view_i^r,$ even though it had
not previously ``filled in'' these values.  To do
this, it must use appropriately chosen conditional distributions.

When a protocol is a composition of several subprotocols, the interface
$\interface$
actually runs sub-simulations $\interface_j$ for each of the intermediate
executions.  The simulation is not quite as simple as running
sub-simulations, however: the view an adversary gains when corrupting a new
player $i$ in the third subprotocol, say, includes not only the original
auxiliary input $a_i$ --- which is all that $\interface$ 
would obtain if it requests
the corruption of player player $i$ in the ideal protocol --- but also the
view $\view_i(1) \circ \view_i(2)$ of player $i$ in the earlier two
subprotocols.  In particular, in order to be able to run interface
$\interface_{j+1},$ $\interface$ must be able to generate auxiliary input 
$a_i(j),$ the
auxiliary input of player $i$ {\em in the $j^{th}$ subprotocol, when
$\interface_{j+1}$ requests it.}

Thus, before we are able to discuss the resilience of concatenating
resilient protocols, we must first consider (1) how to obtain an accurate
final set of views by sampling a subset of the random variables in some
order, and (2) how to ensure that a sub-simulation is not just resilient
but resilient enough to provide views even after the sub-simulation has
completed.

\subsection{Random Variables and Tableaus}

The description of a general protocol execution in the presence of an
adversary (Chapter~\ref{chap-pre}, \S\ref{sec-exec-prot-adv}) and the
particular specification of the protocol describe how to sample the
collection of random variables parametrized by $\rvnames \times [R]$ by
sampling some of them and later applying probabilistic functions to the
results in a specified order.  We are concerned on the one hand with the
distributions $\rv(y_1,R),\rv(y_2,R),\ldots,\rv(y_n,R),\rv(y_A,R),$ which
make up the ensemble $\realy(\vec{x} \circ \vec{a} \circ a,k)$ generated by
running protocol $\realpf(n,m,k)(\vec{x},\vec{a},A(a)).$ On the other hand
are the distributions
$\rv_{ideal}(y_1,R),\rv_{ideal}(y_2,R),\ldots,\rv_{ideal}(y_n,R),
\rv_{ideal}(y_A,R),$ which make up the ensemble $\idealy(\vec{x} \circ
\vec{a} \circ a,k)$ generated by running protocol
$\idealpf(n,m,k)(\vec{x},\vec{a},S(A(a),\cdot)).$ We must eventually show
that the interaction of interface with black-box adversary and ideal
protocol produces the same ensembles, even though the process of sampling
various distributions ($\set{\rvnames_{ideal}(v,r)}$) leading up to these
final ones is different than in the real protocol ({\em i.e.}, local
variables of reliable players are {\em never} assigned, and distributions
are sampled in a different order).

%% We consider two sets of random variables.  The first is $\set{\rv(v,r)},$
%% the set induced by the distribution $\realpf(\vec{x} \circ \vec{a} \circ
%% a)$ arising from an execution of the real protocol,
%% $\realpf(n,m,k)(\vec{x},\vec{a},A(a)).$ The second is
%% $\set{\rv_{ideal}(v,r)},$ induced by the ideal distribution
%% $\idealpf(\vec{x} \circ \vec{a} \circ a,k)$ induced by running
%% $\idealpf(n,m,k)(\vec{x},\vec{a},S(A(a),\cdot)).$
%% 
\iffalse
\begin{definition}
Let $\set{X_v}_{v \in V},$ be a collection of (joint) distributions on some
set X parametrized by $V \times {\bf N}.$ An {\em assignment tableau}
$\psi$ on $V$ is a function
\[
\psi : V \times {\bf N}  \rightarrow \set{\bot} \cup X
\]
satisfying 
\[
(\forall v \in V)(\forall r) \psi(v,r) \not= \bot \Rightarrow
\psi(v,r+1) = \psi(v,r).
\]
The meaning of $\psi(v,r)$ is the following.  If $\psi(v,r)=x,$ then
distribution $\rv(v,r)$ has been sampled with result $x.$ If $\psi(v,r) =
\bot$ then distribution $X_v$ has not been sampled.
\end{definition}

\newcommand{\tableau}{\psi}

Then a real protocol $\realpf$ induces a tableau $\tableau$ on $\rvnames$
such that $(\forall v \in \rvnames) \tableau(v,R) \not=
\bot.$  
That is, all distributions are sampled.  The specification of protocol
execution in the presence of an adversary (Chapter~\ref{chap-pre},
\S\ref{sec-exec-prot-adv}) describes exactly the particular sequence the
particular sequence of experiments and random variables that are analogous
to the distribution $P$ described above.  On the other hand, the tableau
$\psi_{ideal}$ on $\rvnames$ computed by a interface is not completely
instantiated, but it should be the case that the output distributions {\em
are} sampled: $(\forall i) \tableau(y_i,R) \not= \bot$ and $\tableau(y_A,R)
\not= \bot.$ 
\fi

To illustrate the principle behind our arguments, let us consider two
experiments.  Let $X_0$ be a distribution on some set $S,$ and let $\chi_1$
and $\chi_2$ be functions on $S$ such that  $x_0 = (\chi_1(x_0),\chi_2(x_0))$ 
for all $x_0 \in S.$ Let $f_3$ and $f_4$ be probabilistic functions.

The first experiment generates the following distribution:
\[
P = \set{ x_0 \leftarrow X_0; x_1 \leftarrow \chi_1(x_0);
x_2 \leftarrow \chi_1(x_0); x_3 \leftarrow f_3(x_2);
x_4 \leftarrow f_4(x_1,x_3) : x_4}.
\]
At the point at which $x_3$ is computed, the value of $x_1$ does not
matter; in a sense, though it has been specified, it is a hidden variable.
It comes into play later, when $x_4$ is computed.  Intuitively, this
experiment is analogous to the following sequence in a real protocol: a
reliable player computes its transition function, specifying hidden
information (new state and messages to reliable players) and compromised
information (messages known to the adversary).  Later, the adversary
decides to corrupt the player, and obtains the values of the hidden
variables, which it uses in later computations.

Now define the following distributions:
\[
X_1 = \set{ x_0 \leftarrow X_0: \chi_1(x_0) }
\]
\[
X_2 = \set{ x_0 \leftarrow X_0: \chi_2(x_0) }
\]
\[
(X_1 \mid x_2) = \set{ x_0 \leftarrow X_0: \chi_1(x_0) \mid \chi_2(x_0)=x_2 }
\]
The second experiment is the following:
\[
Q = \set{ x_2 \leftarrow X_2; x_3 \leftarrow f_3(x_2);
x_1 \leftarrow (X_1 \mid x_2); x_4 \leftarrow f_4(x_1,x_3) : x_4 }.
\]
In a sense, $x_1$ is not computed until after $x_3$ has been computed.
This is analogous to the operation of an interface: first the interface
computes the variable $X_2$ that is initially ``known'' to the adversary,
and it does not attempt to specify the variable $X_1.$ Later, the adversary
corrupts a new player, and requests the value of $x_0$ (that is, of $x_1$
and $x_2$).  The interface must now sample $X_1$ given the information it
has already committed to the adversary, namely given $x_2.$

It is not hard to see that distributions $P$ and $Q$ are identical.  
The essential principle to note is that the {\em order} of sampling the
distributions is irrelevant as long as the appropriate conditional
distributions are used.  

The task of proving privacy reduces to showing that the interface can
gradually fill in the necessary portions of a simulated tableau by sampling
the appropriate conditional distributions $(X_1 \mid x_2)$ {\em given} the
random variables ($x_2$) which it has already sampled and committed to $A,$
{\em by using} the information it has at hand (inputs obtained by
corruptions in the {\em ideal} protocol).



\subsection{Post-Protocol Corruption}

For proofs involving dynamic adversaries, simulating the view of a newly
corrupted player is essential.  Certainly, during the run of a protocol, an
interface must be able to compute such a view accurately.  In the case of
the sequential concatenation of protocols, however, the view of a reliable
player includes its view during previous protocols.  The task becomes more
difficult; despite the fact that the simulation of the earlier subprotocol
has already occurred, the earlier view must be generated so that it can be
included in the overall view of the newly corrupted player.  We therefore
consider an additional requirement on the interface, to facilitate proofs of
resilience.  This requirement is necessarily satisfied in the case of {\em
perfect} and {\em exponential} resilience, in the case of {\em static}
adversaries, or trivially in {\em memoryless} protocols.

Consider an execution of a protocol $\protob$ with $\interface(A,\cdot),$
giving distribution $\idealy\protoIn.$  At the
conclusion of the protocol, $\interface(A(a),\cdot)$ has corrupted 
some coalition
$T.$  It may be the case that $\abs{T} < t,$ in which case 
$\interface(A(a),\cdot)$
would have been permitted $(t-\abs{T})$ more corruptions.  The interface
$\interface$ can continue to run, since it simply receives requests for new
corruptions.  There is, in general, no guarantee that if it is supplied
with {\em additional} requests after $A(a)$ has halted, the views 
$\interface$
returns are accurate in any fashion.  Post-protocol corruptibility 
ensures that
the interface does have this power, namely that even after $A(a)$ has
halted, producing its output $Y_A,$ the interface can accurately output
$\view_i$ for other players.

Let $T'$ be a set of players.  When $\interface$ continues to run after 
$A(a)$ has
halted and is supplied in turn with each $i \in T'$ written to its input
tape as a request for a new corruption, it returns the views
$\set{\view_i \mid i \in T'},$ inducing the ensemble of distributions
\[
\protob^{\view_{T'}}\protoIn.
\]

\begin{definition}  \label{def-back-compose}
An interface $\interface(\cdot,\cdot)$ is 
{\defstyle post-protocol compatible}%
\index{compatible!post-protocol}\index{post-protocol compatible}
with respect to protocols $\protoa$ and $\protob$
if for any adversary $A,$ for any execution of
$\protoASBeta,$
for any $(\abs{T}-t)$-coalition 
$T' \subseteq [n]-T$ 
where $T$ is the final coalition selected by adversary
$A(a),$ the following ensembles are indistinguishable:
\begin{eqnarray*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\protoa\protoIn
& \indistEn &
\protob\protoIn
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\protoa^{\view_{T'}}\protoIn
& \indistEn &
\protob^{\view_{T'}}\protoIn
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{eqnarray*}
\end{definition}

\begin{definition}  \label{def-back-sim}
A protocol $\protoa$ is {\defstyle post-protocol corruptible}%
\index{post-protocol corruptible}
with respect to $\protob$
if it admits a post-protocol compatible interface $\interface.$
\end{definition}

Memoryless protocols are trivially post-protocol corruptible, since the views
are erased.  Protocols secure against static adversaries are also 
post-protocol corruptible, because the set of corrupted players is 
initially maximal so
that $T'=\emptyset$ always.

A protocol $\protoa$ that is perfectly as resilient as protocol $\protob$
({\em e.g.} a real protocol $\realpf$ that is perfectly resilient) against
dynamic adversaries is of necessity post-protocol corruptible by the following
argument.  For any adversary $A,$ let $A'$ be the adversary that operates
$A$ until the final round and then does the following.  If the coalition
$T$ has size less than $t,$ then $A'$ chooses
$T'=\set{\sigma_1,\dots,\sigma_{\tau}}$ uniformly at random from all
subsets of $[n]-T$ of size $(t-\abs{T})$ or less.  Then $A'$ requests the
corruption of the players in $T'.$  If follows that for all $T',$
$\view_{\sigma_1},\dots,\view_{\sigma_{\tau}},$ and $\view_A,$ the
resilience of $\protoa$ against $A'$ implies that
\begin{eqnarray*}
\probover{\protoa}{T',\view_{T'},\view_A}
& = &
\probover{\protob}{T',\view_{T'},\view_A}
\\
\probover{\protoa}{T'}
\probover{\protoa}{\view_{T'}\mid\view_A}
\probover{\protoa}{\view_A}
& = &
\probover{\protob}{T'}
\probover{\protob}{\view_{T'}\mid\view_A}
\probover{\protob}{\view_A}
\end{eqnarray*}
Summing over all possible views of $A,$
\begin{eqnarray*}
\sum_{\view_A}
\probover{\protoa}{\view_{T'}\mid\view_A}
\probover{\protoa}{\view_A}
& = &
\sum_{\view_A}
\probover{\protob}{\view_{T'}\mid\view_A}
\probover{\protob}{\view_A}
\\
\probover{\protoa}{\view_{T'}}
& = &
\probover{\protob}{\view_{T'}}
\end{eqnarray*}
Similar arguments show that any protocol that is exponentially or
statistically resilient against a dynamic adversary also must be 
post-protocol corruptible.  If we require that the 
convergence parameter is bounded by a
polynomial in $n$ and $m,$ {\em i.e.} that security is achieved when $k$ is
of size polynomial in $n$ and $m,$ then any protocol that is exponentially
resilient must be post-protocol corruptible.


\section{Relatively Resilient Protocols and Concatenation}

We observe that in a sequence of protocols, each as resilient as its
successor (to within $\delta(k)$), the first protocol is as resilient (to
within $\delta(k)\cdot f(n,m,k)$) as the particular protocol $\protoa^f$
constructed by using the $f(n,m,k)^{th}$ protocol from each family.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LEMMA   one sequence, protocols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}  \label{lem-seq-proto-resil}
Let $\protosa=\set{\protoa(0),\protoa(1),\ldots}$ be a uniformly
sequentially $O(\delta(k))$-relatively resilient collection of protocol
families.  Let $f:\nat^3 \rightarrow \nat.$ Then $\protoa(0)
\resilasFa^{O(\delta(k)f(n,m,k))} \protoa^f.$
\end{lemma}

\begin{proof}
Let $A$ be an adversary for protocol $\protoa(0)$ and let 
$\interface_0,\interface_1,\ldots$
be the interfaces postulated by the sequential resilience of the
collections.  Let $\interface^j(A,a)$ denote the nested interface
$\interface_j(\cdot,\interface_{j-1}
(\cdot,\cdots(\cdot,\interface_0(A,\cdot)))).$ 
Let
$\ensa(j)(n,m)(\vec{x} \circ \vec{a} \circ a,k)$ be the ensemble generated
by running $\protoa(j)(n,m,k)(\vec{x},\vec{a},A(a)).$ Because $\protosa$ is
uniformly sequentially $O(\delta(k))$ resilient, the collection
$\enssa=\set{\ensa(0),\ensa(1),\ldots}$ is uniformly sequentially
$O(\delta(k))$ indistinguishable.  Construct an interface
 $\interface$ that runs
$\interface^k$ when given security parameter $k,$ and note that
$\ensa^f(n,m)(\vec{x} \circ \vec{a} \circ a,k)$ is the ensemble generated
by running protocol $\protoa^f(n,m,k)(\vec{x},\vec{a},\interface^j(A,a)).$
Lemma~\ref{lem-seq-ens} implies:
\[
\ensa(0) \indistFa^{\delta(k)\cdot f(n,m,k)} \ensa^f.
\]
\end{proof}


The corresponding result holds for computational resilience:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LEMMA   one sequence, protocols, computational
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}  \label{lem-seq-proto-resil-compose}
Let $\protosa=\set{\protoa(0),\protoa(1),\ldots}$ be a uniformly
sequentially $O(\delta(k))$ computationally relatively resilient collection of
protocol families.  Let $f(n,m,k)$ be a polynomial.  Then, computationally,
$\protoa(0) \resilasFa^{O(\delta(k)f(n,m,k))} \protoa^f.$
\end{lemma}

The transitivity\index{relative resilience!transitive}
 of $\resilasFa$ falls out as an immediate corollary,
recalling that a {\em finite} sequentially resilient collection of 
protocol families is {\em uniformly} sequentially resilient.
\begin{lemma}  \label{lem-resil-trans}
(Transitivity)
Let $P_1, P_2,$ and $P_3$ be protocol families.
If $P_1 \resilasFa P_2$ and $P_2 \resilasFa P_3,$
then $P_1 \resilasFa P_3.$
Furthermore, 
if $P_1 \resilasFa^{O(\delta(k))} P_2$ and $P_2 \resilasFa^{O(\delta(k))} P_3,$
then $P_1 \resilasFa^{O(\delta(k))} P_3.$
\end{lemma}



Let $\protosa=\set{\protoa(i)}$ and $\protosb=\set{\protob(i)}$ be two
collections of protocol families.  Consider the $j$-fold concatenation of
protocols from each: $\hat{\protoa}(j) = \protoconc_{i=1}^j \protoa(i)$
and $\hat{\protob}(j) = \protoconc_{i=1}^j \protob(i).$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LEMMA   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}  \label{lem-proto-concat-fixed}
(Protocol Concatenation) Fix $j.$  If $\protosa \resilasCo^{O(\delta(k))}
\protosb$ with post-protocol compatible interfaces and with convergence
parameter $k_0,$ then $\hat{\protoa}(j) \resilasFa^{O(j \cdot \delta(k))}
\hat{\protob}(j)$ with convergence parameter $k_0.$
\end{lemma}

\begin{proof}
We gradually replace $\protoa$'s by $\protob$'s.  Define the hybrid
protocol family $\hybrids=\set{\hybrid(0),\hybrid(1),\ldots}$ by:
\begin{eqnarray*}
\hybunit(i,l)(n,m) 
& = &
\left\{
\begin{tabular}{ll}
$\beta(i)(n,m)$   &  $i<l$ \\
$\alpha(i)(n,m)$  &  $i \geq l$
\end{tabular}
\right.
%}
\\
\hybrid(l)(n,m)
& = &
\protoconc_{i=1}^l 
\hybunit(i,l)(n,m) \\
& = &
\hybunit(l,l)(n,m) \protoconc 
\hybunit(l-1,l)(n,m) \protoconc
\cdots \protoconc
\hybunit(1,l)(n,m)
\end{eqnarray*}

It suffices to show that $\hybrids$ is uniformly sequentially
$O(\delta(k))$ relatively resilient with convergence parameter $k_0,$ since
Lemma~\ref{lem-seq-proto-resil} with $f(n,m,k)=j$ implies that
\[
\hat{\protoa}(j) = \hybrid(0) \resilasFa^{O(\delta(k)\cdot f(n,m,k))} 
\hybrid^f =  \hat{\protob}(j).
\]
Assume otherwise; then for some $n,m,$ and $l,$
\[
\hybrid(l)(n,m) {\notresilas}^{O(\delta(k))}
\hybrid(l+1)(n,m).
\]
In particular, for all $c$ there are $\vec{x},\vec{a},A,a,$ and $k \geq
k_0$ such that
\begin{eqnarray}   \label{eqn-big-diff}
\abs{
\hybrid(l)(n,m)\protoIn -
\hybrid(l+1)(n,m)\protoIn}
> c \cdot \delta(k)
\end{eqnarray}
Let $\interface_1,\ldots,\interface_j$ be the 
post-protocol compatible 
interfaces for the $j$
subprotocols.  Because the interfaces are post-protocol corruptible, we may
treat the sequential execution of the subprotocols in $\hybrid(l)$ or in
$\hybrid(l+1)$ as a sequence of three probabilistic experiments, 
$(\scp_1,\scp_2^{\alpha},\scp_3),$ or 
$(\scp_1,\scp_2^{\beta},\scp_3),$
where:
\begin{eqnarray*}
\scp_1
& = & 
\protoa(l-1)(n,m)(\vec{x}(l-1) \circ \vec{a}(l-1) \circ a(l-1),k) 
\circ \cdots 
\\
& & 
\circ 
\protoa(1)(n,m)(\vec{x} \circ \vec{a} \circ a,k)
\\
\scp_2^{\alpha}
& = & 
\protoa(l)(n,m)(\vec{x}(2) \circ \vec{a}(2) \circ a(2),k) 
\\
\scp_2^{\beta}
& = & 
\protob(l)(n,m)(\vec{x}(l) \circ \vec{a}(l) \circ a(l),k) 
\\
\scp_3 
& = & 
\protoa(j)(n,m)(\vec{x}(j) \circ \vec{a}(j) \circ a(j),k) 
\circ \cdots 
\\
& & 
\circ 
\protoa(l+1)(n,m)(\vec{x}(l+1) \circ \vec{a}(l+1) \circ a(l+1),k)
\end{eqnarray*}
%% Recall that $x_i(2)=x_i \circ y_i(1),$ 
%% $a_i(2)=a_i \circ \view_i(1),$ $a(2)=a\circ \view_A(1),$ and so on.

By assumption, $\scp_2^{\alpha} \indistEn^{O(\delta(k))} \scp_2^{\beta}$
with convergence parameter $k_0.$ By Lemma~\ref{lem-feed-dist},
$\scq^{\alpha} \indistEn^{O(\delta(k))} \scq^{\beta}$ with parameter $k_0.$ But
$\scq^{\alpha} = \hybrid(l)(n,m)(\vec{x}\circ \vec{a} \circ a,k)$ and
$\scq^{\beta} = \hybrid(l+1)(n,m)(\vec{x}\circ \vec{a} \circ a,k).$ This
contradicts (\ref{eqn-big-diff}).
\end{proof}

We are now ready to measure the resilience achieved by concatenating 
a growing number of subprotocols.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREM
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}  \label{thm-proto-concat}
(Protocol Concatenation) 
Let $f: \nat^3 \rightarrow \nat.$
If $\protosa \resilasCo^{\delta(i,k)}
\protosb$ with post-protocol compatible interfaces and with convergence
parameter $k_0,$ then concatenating $f(n,m,k)$ protocols from each
satisfies: 
\[
\protoconc_{i=1}^f \protoa(i)
\resilasFa^{O(\delta(f(n,m,k),k) \cdot f(n,m,k))}
\protoconc_{i=1}^f \protob(i).
\]
In particular,
\[
\begin{tabular}{rllcrlllr}
$\protosa$ & $\resilasCo$  & $\protosb$ &
$\Rightarrow$ & 
$\protoconc \protosa$ & $\resilasFa$ & $\protoconc \protosb$ & 
 &
\hspace{0.2in}(1)
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$\protosa$ & $\resilasCoE$  & $\protosb$ &
$\Rightarrow$ & 
$\protoconc \protosa$ & $\resilasFaE$ & $\protoconc \protosb$ & 
(if $f(n,m,k)=O(k^c))$ &
\hspace{0.2in}(2)
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$\protosa$ & $\resilasCoS$  & $\protosb$ &
$\Rightarrow$ & 
$\protoconc \protosa$ & $\resilasFaS$ & $\protoconc \protosb$ & 
(if $f(n,m,k)=O(k^c))$ &
\hspace{0.2in}(3)
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$\protosa$ & $\resilasCoC$  & $\protosb$ &
$\Rightarrow$ & 
$\protoconc \protosa$ & $\resilasFaC$ & $\protoconc \protosb$ & 
(if $f(n,m,k)=O(k^c))$ &
\hspace{0.2in}(4)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\]
\end{theorem}

\begin{proof}
We define two collections of protocol families as follows.  The first is
$\linconcsa=\set{\linconca(1),\linconca(2),\ldots},$ the concatenation of
linearly many protocols from $\protosa:$
\[
\linconca(j)(n,m,k) = \protoconc_{i=1}^j \protoa(i)(n,m).
\]
The second is defined similarly: 
$\linconcsb=\set{\linconcb(1),\linconcb(2),\ldots},$ 
where
\[
\linconcb(j)(n,m,k) = \protoconc_{i=1}^j \protob(i)(n,m).
\]

Assume $\protosa \resilasCo^{O(\delta(i,k))} \protosb$ pairwise uniformly with
convergence parameter $k_0.$ By Lemma~\ref{lem-proto-concat-fixed}, $\protosa
\resilasCo^{\delta(i,k)} \protosb$ implies that, for each $i,$ $\linconcsa(i)
\resilasCo^{i \delta(i,k)} \linconcsb(i)$ with convergence parameter $k_0.$
It follows that $\linconcsa \resilasCo^{i\delta(i,k)} \linconcsb,$ pairwise
uniformly with convergence parameter $k_0.$ By
Lemma~\ref{lem-pair-ens}, the diagonal protocol families
% used to refer to lem-pair-proto-resil
$\hat{\linconca}^f$
and $\hat{\linconcb}^f$ satisfy
\[
\hat{\linconca}^f 
\resilasFa^{O(f(n,m,k) \cdot \delta(f(n,m,k),k))} 
\hat{\linconcb}^f.
\]
But
\begin{eqnarray*}
\hat{\linconca}^f & = & \protoconc_{i=1}^{f(n,m,k)} \protosa(i) \\
\hat{\linconcb}^f & = & \protoconc_{i=1}^{f(n,m,k)} \protosb(i) 
\end{eqnarray*}
It follows that
\[
\protoconc_{i=1}^{f(n,m,k)} \protosa(i)
\resilasFa^{O(f(n,m,k)\cdot\delta(f(n,m,k),k))}
\protoconc_{i=1}^{f(n,m,k)} \protosa(i)
\]

Implication (1) follows directly; implications (2), (3), and (4) are
straightforward.  For the proof of (4), we invoke the computational
versions of the corresponding supporting lemmas.
\end{proof}




If intermediate functions are private, then computing their open
composition is as secure as computing their closed composition:
\begin{lemma}   \label{lem-c-open-close}
(Open Function Composition)
Let $f:\nat^3\rightarrow\nat.$
Let $\scf = \set{F^i}$ be a collection of function families
where $F^{1,n,m},\ldots,F^{f(n,m,k)-1,n,m}$ are {\em private.}
Let $F=\circ \scf.$  
Then the ideal open composite protocol $\idoc$ for $\scf$
is as resilient as the ideal protocol $\idealy$ for $F:$
\[
\idoc \resilasFa \idhc \resilasFa \idealy.
\]
If $f(n,m,k)$ is polynomial, then this holds for exponential, statistical,
and computational relative resilience.
\end{lemma}

\begin{proof}
Since each $F^{1,n,m},\ldots,F^{f(n,m,k)-1,n,m}$ is {\em private,} each is
as resilient as the vacuous protocol.  So for each intermediate function
there exists a protocol $\idealpf(F^j)$ and an interface 
$\interface_j$ showing
$\idealpf(F^j)$ is as resilient as the ideal vacuous protocol.  Recall that
the ideal open composite protocol runs for $f(n,m,k)$ rounds, accepting an
initial set of inputs $x_1^1,\ldots,x_n^1,$ returning the value of
$F^r\circ \cdots \circ F^1(x_1^1,\ldots,x_n^1)$ at each round $r.$ The
ideal hidden composite protocol returns only the vectors of identities of
``cheating'' players (players not supplying a valid input) and returns the
final result.

The interface $\interface$ uses each $\interface_j$ to create the needed 
intermediate
function values $F_j\circ\cdots\circ F_1$ that are supplied to corrupted
players.  That is, at the first round, $\interface$ collects requests for
corruptions from $A,$ supplies them to $\interface_1,$ collects requests for
corruptions from $\interface_1,$ requests those corruptions itself, 
and returns the
results along the same paths.  When $A$ and $\interface_1$ are done 
requesting
corruptions, $\interface_1$ supplies messages from corrupted players 
(either 0 or 1
depending on if the player decides to cheat detectably), $\interface$ sends 
them in
the hidden protocol, and $\interface$ obtains the vacuous output from the 
trusted
host in round 1 of the hidden protocol.  Interface $\interface$ then 
supplies the
vacuous output to $\interface_1,$ who may request more corruptions but 
eventually
computes the values of $F_1$ to be sent to corrupted players.  When 
$\interface_1$
is finished, $\interface$ runs $\interface_2$ as before; if $\interface_2$ 
corrupts a player, $\interface$ must make a post-protocol corruption 
request to $\interface_1$ to produce the view of that player 
during round 1.
When $\interface_2$ is finished corrupting players, $\interface$ requests 
the vacuous output
of round $2$ of the hidden protocol and supplies it to $\interface_2.$ 

This continues for $f(n,m,k)-1$ steps.  At the last step, $\interface$ 
collects
requests for corruptions directly from $A$ and supplies responses as before.
When $A$ requests the $f(n,m,k)^{th}$ output from the open protocol, namely
the value of $F^{f(n,m,k)} \circ\cdots\circ F^1,$ $\interface$ requests it 
in the
hidden protocol and returns the result.

The second statement, $\idhc \resilasFa \idealy,$ is easy to see by noting
that an interface itself can compute the vacuous messages returned to $A$
for each round up to the penultimate one, based on the messages sent to 
$\interface$
by $A;$ its only interaction in protocol $\idealy$ is to request original
inputs of corrupted players.  In the final round, $\interface$ 
obtains the results
for corrupted players in $\idealy$ and returns them to $A.$
\end{proof}

Concatenating ideal protocols for robust functions is as resilient as a single
ideal composite protocol that computes their open composition --- this is
the motivation for robustness:
\begin{lemma}   \label{lem-comp-ideal-pro}
(Ideal Protocol Concatenation)
Let $f(n,m,k)$ be a polynomial.
Let $\scf = \set{F^i}$ be a collection of function families
where $F^{1,n,m},\ldots,F^{f(n,m,k)-1,n,m}$ are {\em robust.}
Then the concatenation of ideal protocols for $\scf$ 
is as resilient as the ideal open composite protocol for $\scf:$
\[
\ocip \resilasFa \idoc
\]
\end{lemma}

\begin{proof}
Protocol $\idealpf(\opencomp \scf)$ lasts $f(n,m,k)$ rounds.  For the first
$f(n,m,k)-1$ rounds, whenever adversary $A$ requests the corruption of
player $i,$ interface $\interface$ corrupts player $i$ in protocol
$\idealpf(\closedcomp \scf)$ and returns the original input, along with the
list of outputs generated thus far.  The output of each round is, as in the
vacuous protocol, a list of $n$ bits which are 0 for every uncorrupted
player and are 0 or 1 for corrupted players depending on whether the
adversary forced them to send a 0 message or not.  (Note that the vacuous
output is the same for all players; $\interface$ simply records what it has
generated at each round of the simulation in order to include it in the
information of later corruptions.)  

At round $f(n,m,k),$ however, when the adversary generates its last set of
messages for players in the $\idealpf(\opencomp \scf)$ protocol, the
interface $\interface$ sends the vector of messages it received for corrupted
players in the first round of the $\idealpf(\opencomp \scf)$ protocol:
these are the inputs upon which the computation of $F^{f(n,m,k)}$ is based.
Interface $\interface$ receives a message from the trusted host in protocol
$\idealpf(\closedcomp \scf)$ that contains the outputs for corrupted
players, and it relays this message to $A.$  That the final messages are
identically distributed in $\idealpf(\opencomp \scf)$ and
$\idealpf(\closedcomp \scf)$ is ensured by the robustness of each
intermediate result.
\end{proof}

Let $\gensha$ be a protocol that implements a robust and private
representation $\sha,$ and let $\genrec$ be a protocol that reconstructs the
represented value according to the $\rec$ function.  The robust and secret
version of an arbitrary function $H$ is the function:
\[
\robsec(H) = \sha \opencomp H \opencomp \rec
\]
We have,
\[
\rec \opencomp \robsec(H) \opencomp \sha = H
\]
or more generally, for a collection of families $\set{H^j},$
\begin{eqnarray}
\label{eqn-compose-hide}
\rec \circ ( \circ_j \robsec(H^j) ) \circ \sha = \circ_j H^j
\end{eqnarray}

The protocols in \cite{gmw87,bgw88,ccd88}, for example, are of the form
\[
\genrec \circ (\circ_j \Pi(\robsec(G^j))) \circ \gensha,
\]
where each $G^j$ is an arithmetic or Boolean function (a set of gates on
one level of a circuit).  In particular, the players share the inputs,
evaluate functions $G^1,\ldots,G^{f(n,m,k)}$ on them, and reveal only the final
result.  Our protocols will be of a somewhat more general form, computing
{\em several} intermediate functions whose values {\em are} revealed on the
path to computing $F:$
\[
\circ_i (\genrec \circ (\circ_j \Pi(\robsec(G^{ij}))) \circ \gensha).
\]
The following theorem demonstrates the resilience of our modular approach:
\begin{theorem}  
\label{thm-concat}
(Modular Protocol Construction) Let $p(n,m,k)=O((nmk)^c)$ and 
$q(n,m,k)=O((nmk)^c)$  for some $c.$ 
Let $\set{\scg^i}$ be a set of collections of function
families, where $\scg^i=\set{G^{i,j}},$ and $G^{i,j}=\set{G^{i,j,n,m}}.$
Let $F^i = \circ \scg^i$ be the composition of $p(n,m,k)$ functions from
$\scg^i.$ Let $\scf = \set{F^i},$ and let $F=\circ \scf$ be the composition
of $q(n,m,k)$ functions from $\scf.$

If each $F^{1,n,m},\ldots,F^{q(n,m,k)-1,n,m}$ is private and robust, and if
there exist $t$-resilient protocols $\Pi(\robsec(G^{ij}))$ for each $i,j,$
then:
\[
\protoconc_{i=1}^q (\genrec \protoconc 
   (\protoconc_{j=1}^p \Pi(\robsec(G^{ij}))) \protoconc \gensha)
\resilasFa
\idealpf
\]
In other words, the concatenation of the $t$-resilient protocols as
described above is a $t$-resilient protocol for $F.$ This is also true of
exponential, statistical, and computational resilience.
\end{theorem}

\begin{proof}
First let us examine the resilience of computing each $F^i$ by
concatenating the ideal protocols for the $G^{ij}$ functions:
\begin{center}
\begin{tabular}{rcll}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$\genrec \circ [ \circ_j \idealname(\robsec(G^{ij})) ] \circ \gensha$ &
$\resilasFa$ & 
$\genrec \circ \idealname( \opencomp_j \robsec(G^{ij})) \circ \gensha$ &
\mbox{(\ref{lem-comp-ideal-pro},\ref{lem-proto-concat-fixed})} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&
$\resilasFa$ & 
$\genrec \circ \idealname( \closedcomp_j \robsec(G^{ij})) \circ \gensha$ &
\mbox{(\ref{lem-c-open-close},\ref{lem-proto-concat-fixed})} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&
$\resilasFa$ & 
$\idealname( \recons \closedcomp [ \closedcomp_j \robsec(G^{ij}) ]
 \closedcomp \sha) $ &
\mbox{(\ref{lem-c-open-close},\ref{lem-comp-ideal-pro},
\ref{lem-proto-concat-fixed})}
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& $\resilasFa$ & $\idealname( \closedcomp_j G^{ij} ) $ &
\mbox{(\ref{eqn-compose-hide}) } \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&
$\resilasFa$ &
$\idealname( F^i )$ &
\mbox{(\ref{lem-c-open-close})} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\end{center}

At this stage, we have demonstrated enough to support the methods of
\cite{bgw88,ccd88}.  We wish to concatenate protocols that {\em do} reveal
(restricted) intermediate values:

\begin{center}
\begin{tabular}{rcll}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$\circ_i
(\genrec \circ [ \circ_j \idealname(\robsec(G^{ij})) ] \circ \gensha)$ &
$\resilasFa$ & 
$\circ_i \idealname( F^i )$ &
\mbox{(\ref{thm-concat})} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&
$\resilasFa$ & 
$\idealname( \closedcomp_i F^i )$ &
\mbox{(\ref{lem-comp-ideal-pro},\ref{lem-c-open-close}) } \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&
$\resilasFa$ &
$\idealpf$ &
\mbox{(\ref{lem-c-open-close})} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\end{center}

The theorem stipulates the existence of resilient protocols
$\Pi(\robsec(G^{ij}))$ for each $i,j.$  That is,
\[
\Pi(\robsec(G^{ij}))
\resilasFa
\idealname(\robsec(G^{ij}))
\]

Hence 
\begin{center}
\begin{tabular}{rcll}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$\circ_i
(\genrec \circ [ \circ_j \Pi(\robsec(G^{ij})) ] \circ \gensha)$ &
$\resilasFa$ & 
$\circ_i
(\genrec \circ [ \circ_j \idealname(\robsec(G^{ij})) ] \circ \gensha)$ &
\mbox{ } \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&
$\resilasFa$ & 
$\idealpf$
\mbox{ } \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\end{center}
\end{proof}




==> mpp.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% mpp.tex                    Multiparty Protocols for any function.
%
%                            Copyright @1989  Donald Beaver.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{=======}
\typeout{mpp.tex}
\typeout{=======}

\chapter{Efficient Multiparty Protocols for Any Function}
\label{chap-mpp}


\chapquote{
She was pale when she talked with the chaplain.
She said that the war instead of ennobling soldiers made beasts of them.
Downstairs the patients had stuck their tongues out at her and told
her she was a scarecrow and a frightful skinny old frump.
``Oh, how dreadful, chaplain,'' she said in German.
``The people have been corrupted.''
%
%And she described how she saw the religious education of a soldier.
%Only when he believes in God and has religious feelings can a soldier
%fight bravely for His Imperial Majesty and not fear death, because
%then he knows that paradise awaits him.
%
%She babbled on and said a few more stupid things like this, and it
%was clear that she was resolved not to let the chaplain go.  But he
%excused himself in a rather ungallant way.
}{Jaroslav Ha\v{s}ek, {\em The Good Soldier \v{S}vejk}}
% translation from Czech by Cecil Parrott; Penguin Books Middlesex England
% 1973
% p 154

Chapter~\ref{chap-con} gives secure and reliable protocols for any function
in $NC^1$ using a constant number of rounds and tolerating faults in a
third of the network.  The construction also gives constant round protocols
for any function but at a potential exponential blowup in message sizes.
Here we present secure and reliable protocols to compute {\em arbitrary}
functions\index{constant rounds!arbitrary functions} in {\em constant}
rounds, using small, polynomial-size messages, and tolerating $t=O(\log n)$
faults.  Thus, instead of incurring a price in message size in order to be
able to compute any function, we tolerate a smaller yet still reasonable
number of faults.

Locally random reductions\index{locally random reduction} appear twice in
our protocol.  First, they serve to to reduce a highly interactive network
computation of $F$ to an $n$-fold {\em local} computation of a polynomial
for $F.$ Second, they ensure that Byzantine faults are detected and
corrected.

The power of locally random reductions is evident in the results: {\em any}
function admits an unconditionally $t$-resilient protocol having {\em
constant} round complexity and {\em small} message complexity, {\em
regardless} of its computational complexity.  Through simple algebraic
approaches, we separate the {\em communication complexity of secure
computing} from the {\em computational complexity} of the function to be
computed.

Let us now consider the inputs as a single sequence of bits instead of a
set of $n$ different inputs each having length $m.$ That is, for $a=bm+c,$
define $\xhat_a$ to be the $c^{th}$ bit of input $x_b.$ Each player shares
each bit of its input separately.  Since we do have a bound on the number
of input bits in terms of the number of players, we shall consider the
number of output bits, $N(n),$ as a separate parameter.

\begin{theorem}   \label{thm-const-logn}
Let $t(n)$ and $m(n)$ satisfy $t(n)m(n)=O(\log n).$
Let $F$ be a family of functions $\set{F^n}$ mapping $(\Sigma^{m(n)})^n
\rightarrow \Sigma^{N(n)},$ where $N(n)$ is polynomial in $n.$ 
Then there exists a $t$-resilient protocol \evallog for
$F$ that runs in a {\em constant} number of rounds and uses a small
polynomial number of message bits.
\end{theorem}

%
%   n     number of players
%   m     number of bits
%   d=t   degree of sharing polynomials in LRR, also number of faults
%   m/q   degree of reduced function h_f
%   (d,dm/q)  LRR
%   q     such that there are 2^q m/q  new vars; need q logarithmic in m,n
%   r     number of vars,   r=2^q m/q
%
\begin{proof}
Let $\alpha_1,\dots,\alpha_n$ be fixed nonzero field elements over a field
$E$ of size exceeding $n.$ Let $q=\lceil \log n \rceil$ and let $M$ be the
least multiple of $q$ exceeding $nm.$ Let $r=(2^q) \frac{M}{q},$ which is
clearly polynomially bounded in $n.$ The function $F^n$ maps
$\xhat_1,\ldots,\xhat_{nm}$ to an $N$-bit string; let
$F^{nb}(\xhat_1,\ldots,\xhat_{nm})$ be the $b^{th}$ bit of
$F^{n}(\xhat_1,\ldots,\xhat_{nm}).$ Without loss of generality, consider
$F^{nb}$ to be an $M$-variate function that is insensitive to the extra
$M-nm$ variables.  By Theorem~\ref{thm-lrr-improve}, there is a polynomial
$h_F^{nb}(w_1,\dots,w_r)$ of degree $(m/q)$ for $F^{nb},$ such that each
$w_i$ is a product of at most $2^q$ variables $\xhat_j.$

Figure~\ref{fig-mpp-eval} describes the protocol.  We have expanded on the
locally-random reduction so that the steps of this protocol are more
concrete; note that any locally-random reduction computable in $NC^1,$ not
simply the one based on polynomial evaluation that sufficed for the proof
of Theorem~\ref{thm-lrr-improve}, will do.  The particular locally-random
reduction of Theorem~\ref{thm-lrr-improve} is easy to implement and very
efficient, so we use it directly.

Because the locally random reduction is in $NC^1$ (each $w_i$ is the
product of at most it can be secretly evaluated in constant rounds using
Theorem~\ref{thm-nc1}.  The system generates $N(n)$ sets of $n$ queries,
one set for each output bit.  The queries from each set are given to the
players individually.  The crux of the solution is that, though computing
the reduced functions $h^{nb}$ may be complicated, it is a local
computation requiring no interaction.

\figstretch
\boxfig{
\noindent{\bf \evallog($F$)}
\index{constant rounds!arbitrary functions}
\index{\evallog($F$)}
\begin{enumerate}
\item
\label{enu-share}
{\bf (Share $\hat{x}_1,\dots,\hat{x}_m.$)}
Each player $i$ shares its input as 
$\hat{x}_{m(i-1)+1},\dots,\hat{x}_{mi}.$
Variables $\hat{x}_{mn+1},\ldots,\hat{x}_{m}$ are taken to be 0.
\item
\label{enu-expand}
{\bf (Expand variables.)}
Compute new secrets $w_1,\dots,w_{r}$ by running protocol
\evalconst to evaluate $w_i(\hat{x}_1,\dots,\hat{x}_m).$
\item
\label{enu-lrr}
{\bf (Select LRR.)}
Select $rt$ random secrets $p_1^1,\dots,p_1^t;\ldots;p_r^1,\dots,p_r^t,$
using protocol \randomsecret.  These denote the higher coefficients of
polynomials $p_i(u)=w_i + \sum_j p_i^j u^j.$
\item
\label{enu-apply}
{\bf (Apply LRR.)}
Using protocol \evalconst, compute new secrets 
$w^i_j = p_j(\alpha_i)$ for $i=1..n,$ $j=1..r,$ in parallel.
Reveal $(w^i_1,\dots,w^i_r)$ to player $i.$
\item
\label{enu-local}
{\bf (Compute reduced problem locally.)}
Each player $i$ computes 
\[
v_i^b=h_F^{nb}(w^i_1,\dots,w^i_r)  \hspace{0.3in}  1 \leq b \leq N(n)
\]
and secretly shares $(v_i^1,\ldots,v_i^{N(n)})$ among the network.
\item
\label{enu-proof}
{\bf (Protect against Byzantine failures.)}
Run Protocol~\behave($i,j$) for each $1\leq i,j \leq n;$
thus each player $i$ proves to the network in zero-knowledge that 
\[
(v_i^1,\ldots,v_i^{N(n)})=
(F^{n1}(w^i_1,\dots,w^i_r),\ldots, F^{n,N(n)}(w^i_1,\dots,w^i_r))
\]
\item
Each player $j$ broadcasts a vote as to whether each player $i$ gave him a
satisfactory proof in step~\ref{enu-proof}.  Disqualify each player $i$ who
is impeached by a majority; reveal its query
$(w^i_1,\dots,w^i_r);$ 
and use
\[
v_i^b=h_F^{nb}(w^i_1,\dots,w^i_r)  \hspace{0.3in}  1 \leq b \leq N(n)
\]
as publicly known constants for the remainder of the protocol.
\item
\label{enu-inter}
{\bf (Reconstruct $f.$)} Run protocol \evalconst to secretly interpolate
each set $(v_1^b,v_2^b,\ldots,v_n^b),$ for $b=1..N(n)$ in parallel.
For each set, obtain the free term $y^b$ of the polynomial of degree $rt$
passing through the points.
\end{enumerate}
\caption{\label{fig-mpp-eval}
Protocol to evaluate any $F$ in constant rounds and low fault-tolerance.
}}
\figstretchend

Locally random reductions, however, are not necessarily robust against
errors in the reduced computations.  Reducing the overall computation to
locally independent computations suffices for privacy but not for
robustness.  Thus we need to verify that the results of
step~\ref{enu-local} are accurate before using them to interpolate the
final answer.

Let us expand upon step~\ref{enu-proof}.  Each player $i$ gives a ZKMIPS
proof (\S\ref{sec-zkmips}) to each player $j$ that the secret value of
$v_i^b$ it shared satisfies $v_i^b=h_F^{nb}(w^i_1,\dots,w^i_r),$ using the
methods of Chapter~\ref{chap-zkp}.  This is not quite sufficient {\em per
se}, since a faulty player may cause some good players to believe the proof
while others find fault.  Thus, after the proving phase, every player $j$
broadcasts a vote $V_{ji}$ as to whether it believes the proof of player
$i.$ If a majority vote to accept $i,$ then player $i$ is accepted.  A
majority vote in favor of player $i$'s honesty implies that at least one
reliable player found player $i$ correct, which means that player $i$ was
able to prove its correctness to someone, and its results are therefore
correct. If player $i$ is rejected by the vote, it failed to satisfy any
reliable player of its behavior, and the query $(w^i_1,\dots,w^i_r)$ with
which it is supposed to compute is revealed so that the reliable players
may incorporate it properly.

Thus, we have specified eight function families corresponding to the eight
modules of the protocol.  Each of these computes a robust and private
representation of its results (small lists of questions from the reductions
are independent of the inputs and hence private; the $v$ values are robust
given that the zero-knowledge proofs succeed, or else they are broadcast
implicitly through the revelation of $w^i_1,\ldots,w^i_r$; pieces of the
various secrets are robust and private representations).  By
Theorem~\ref{thm-concat}, the composition is $t$-resilient.

The number of rounds is constant, by the following observations.
Step~\ref{enu-expand} is an evaluation of several polynomials $w_i$ of
degree $2^q,$ which is an $NC^1$ computation.  By Theorem~\ref{thm-nc1},
this takes constant rounds and polynomial message sizes.

Step~\ref{enu-lrr}, the selection of $n$ random polynomials of degree $t$
with free terms $p_1^1,\dots,p_1^t;\ldots;p_r^1,\dots,p_r^t,$ requires the
secret choice of $rt$ coefficients.  The selection of these random secret
values is performed in parallel and requires constant rounds.
Applying polynomials $p_1,\dots,p_r$ to the known, fixed values
$\alpha_1,\dots,\alpha_n$ is a linear combination and hence requires no
interaction.  

Each player $i$ computes $h_F^{nb}$ locally and non-interactively,
and its resharing requires polynomial bits and constant rounds.
The zero-knowledge proofs of step~\ref{enu-proof} are slightly
more complicated yet still require constant rounds and polynomial
message sizes.
The interpolation of $y^b$ from $v_1^b,\dots,v_{n}^b,$
step~\ref{enu-inter}, uses an $NC^1$ circuit.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> mzk.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% mzk.tex                    Multiparty Zero Knowledge.
%
%                            Copyright @1989  Donald Beaver.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{=======}
\typeout{mzk.tex}
\typeout{=======}

\chapter{Multiparty Zero-Knowledge Proof Systems}
\label{chap-mzk}





In this chapter, we generalize the concept of a zero-knowledge proof
system\index{zero-knowledge proof} in two ways.  First, we consider
proofs that some condition holds on secretly shared values.  One player,
the prover \prover, knows the values of a collection of secrets, 
and through an
interaction with the rest of the network, it proves that a given predicate
$\scp$ holds on those secrets.  Second, we consider efficient interactive
proofs of general theorems, where secrecy is not the goal.  Rather, the
prover must prove a given theorem ({\em i.e.} prove membership in a
language) to one or more verifiers.  Instead of making unproven
cryptographic assumptions to guarantee zero-knowledge, we utilize the
presence of a majority of trusted players.  No single player need be
trusted.

{\bf Assumptions made in this chapter.} The network is complete, with
private lines, $n$ processors, and at most $t < \frac{n}{2}$ Byzantine
faults, chosen dynamically.  The protocols are unconditionally secure with
high probability; the results are statistical zero-knowledge (with high
probability {\em no} extra information is revealed).  There are two
distinguished parties, a {\em prover}, which is either polynomial-time or
polynomial-space bounded, and a {\em verifier}, which is either unbounded
or polynomial-time bounded.

\section{Zero-Knowledge Proofs About Secrets}
\label{sec-zkmips}

In Chapter~\ref{chap-min} we considered the ABC Problem: Alice, the prover,
must prove that $c=ab,$ where $a,b,$ and $c$ are secrets.  Here, we extend
Lemma~\ref{lem-abc} to demonstrate that a player may prove that a given
predicate $\predicate$ holds on $m$ shared secrets $v_1,\dots,v_m,$
revealing no additional information.  In a sense, this is analogous to the
two-player problem of giving zero-knowledge proofs that a predicate holds
on committed bits \cite{kil88-ot}. Here, we consider values shared among a
network instead of committed bits, which have slightly different
properties.  For example, though committed bits are secret and
unchangeable, they cannot be added together directly.  Since most secure
multiparty protocols are based on threshold schemes like secret sharing,
proofs about shared values are an important tool.

Let $\predicate$ be a function on $m$ variables over the field $E$ and let
$C_{\predicate}$ be an algebraic circuit over $E$ which computes
$\predicate;$ note that any boolean predicate on boolean inputs is easily
modelled using arithmetic over $E.$

Let $\prover$ and $\verifier$ be distinguished parties in the network.  We
consider $\prover$ or $\verifier$ to be ``cheating'' if they are corrupted
by an adversary $A.$

Let the prover's input be $x_{\prover}=(v_1,\dots,v_m,w)$
and let all other $x_i=0.$  
We define a function whose output is known only to the verifier:
$F_i(x_1,\dots,x_n) = 0$ if $i \not= \verifier,$ and
\[
F_{\verifier}(x_1,\dots,x_n)  =
\left\{
%}
\begin{array}{rl}
1 & \mbox{ if } x_{\prover}=(v_1,\dots,v_m,w) \mbox{ and }
w = \predicate(v_1,\dots,v_m) \\
0 & \mbox{ otherwise. } \\
\end{array} 
\right.
\]

Without regard to zero-knowledge, a simple proof system is trivial: 
simply reconstruct all the secrets and check if
$w=\predicate(v_1,\ldots,v_m).$  

\begin{definition}   \label{def-zkmips}
%{\bf (Multiparty Zero-Knowledge Interactive Proof System on Secrets 
%(\mzkipss))} 
A protocol $\Pi$ is a {\defstyle $(n,t)$ multiparty zero-knowledge
interactive proof system%
\index{\mzkipss!multiparty zero-knowledge
interactive proof system on secrets}%
\index{zero-knowledge proof}%
\index{multiparty zero-knowledge}%
\index{interactive proof system!on secrets}
on secrets for $\predicate$} if it
is a $t$-resilient $n$-player protocol for the function $F_{\predicate}$
defined above.
\end{definition}
The terms {\em statistical} and {\em computational} apply according
to whether the protocol is statistically or computationally resilient.
We call such a protocol a \mzkipss, for short.

\smallskip

Theorem~\ref{thm-bgw}
tells us that there exists a \mzkipss\  for any function $\predicate:$ 
simply compute $F_{\predicate}$ using the \eval protocol.

The purpose of this section, aside from defining the concept of proof
systems with many parties, is to introduce a protocol which allows a direct
proof system which is far more efficient than simulating $C_{\predicate}.$
Simulating a circuit level by level (or even $(\log n)$-slice by slice) is
an expensive undertaking.  We can take advantage here, however, of the fact
that the prover already knows the results of all of the gates.  The prover
shares the results of each and every gate, reducing the task of the
verifier to checking that each shared result is correct.  In other words,
the system does not need to evaluate the circuit layer by layer, but rather
only to verify that the collection of secrets representing the output
values of each gate is correct.  This verification requires only a local
examination of the secret inputs and secret output of each gate, an
operation which can be performed simultaneously for all the gates.
Figure~\ref{fig-provepred} details the protocol.

\figstretch
\boxfig{
\noindent{\provepred}$(\prover,\verifier;\predicate;v_1,\dots,v_m;w)$.\\
%\comment{Prove $w = \predicate(v_1,\dots,v_m).$}
\begin{tabbing}  \standtabs
\> 
{\For $0 \leq l \leq {\tt depth}(C_{\predicate})$}
{\for $1 \leq j \leq {\tt width}(C_{\predicate})$} \Dopar: \\
\>\>
\prover shares the output of each gate $g_{lj}$ as a secret, $w_{lj}.$ \\
\> 
{\For $0 \leq l \leq {\tt depth}(C_{\predicate})$}
{\for $1 \leq j \leq {\tt width}(C_{\predicate})$} \Dopar: \\
\>\>
the network secretly computes $u_{lj}$ as follows: \\
\>\>\> 
\If $g_{lj}=(\times)$ \Then run \mult to compute \\
\>\>\>\>
$u_{lj} = g_{\inputgates_1(g_{lj})} \cdot g_{\inputgates_2(g_{lj})}.$ \\
\>\>\> 
\If $g_{lj}=(+,a_0,\ldots,a_m)$ \Then run \add to compute \\
\>\>\>\>
$u_{lj} = a_0 + \sum_{j=1}^m g_{\inputgates_m(g_{lj})}.$ \\
\>
{\For $0 \leq l \leq {\tt depth}(C_{\predicate})$}
{\for $1 \leq j \leq {\tt width}(C_{\predicate})$} \Dopar: \\
\>\>
reveal $u_{lj}$ to \verifier. \\
\> If all $u_{lj}=0,$ \verifier outputs {\em accept}, else it outputs {\em
reject}. 
\end{tabbing}
\caption{\label{fig-provepred}
Protocol to prove $w = \predicate(v_1,\dots,v_m).$
\index{predicate!proof of}
\index{\provepred}
}}
\figstretchend

The results of Chapter~\ref{chap-min} give the following:
\begin{theorem}
\label{thm-zkp-pred-stat}
Let $\predicate$ be a family of predicates and let $F_{\predicate}$ and
$C_{\predicate}$ be as described above.  For $2t<n,$ protocol \provepred is
a statistical $(n,t)$-\mzkipss\  for $\predicate.$ It runs in constant rounds
and has message complexity polynomial in $(n,m,k,C_{\predicate}).$ of
$\predicate.$
\end{theorem}

When $3t<n,$ the results of $\cite{bgw88}$ ensure that the
gatewise verification of $C_{\predicate}$ occurs without error,
so that the simulation is perfect:
\begin{theorem}
\label{thm-zkp-pred-perf}
Let $\predicate$ be a family of predicates and let $F_{\predicate}$ and
$C_{\predicate}$ be as described above.  For $3t<n,$ protocol \provepred is
a perfect $(n,t)$-\mzkipss\  for $\predicate.$ It runs in constant rounds and
has messages complexity polynomial in $(n,m,k,C_{\predicate}).$
\end{theorem}

Protocols whose message complexity is polynomial in $n,$ {\em
independently} of the circuit complexity of $F_{\predicate},$ are presented
in Chapter~\ref{chap-zkp}.  They require the machinery of {\em locally
random reductions}, and may require the players to compute time-consuming
functions locally.  Though the results of this section require polynomial
local time if the circuit is of polynomial size, verifying huge circuits
requires very little local time per gate but great cumulative local time.
When the goal is to prove predicates regardless of their computational
complexity, then the cost must be paid somewhere; better it be on the local
computation than on the communication lines.  The next section, however,
describes a particular class of intractable functions for which only the
prover itself need perform more than polynomial time computations.



\section{Zero-Knowledge Proofs for IP}
\label{sec-zkp-ip}


Any language $L \in \ip$\index{interactive proof system!IP} 
certainly has a circuit $C_L$ which
describes its characteristic function $\chi_L;$ Theorems
\ref{thm-zkp-pred-stat} and \ref{thm-zkp-pred-perf} imply there is a
\mzkipss\  for $L$ in the presence of a partly trusted network.  The size of
$C_L,$ however, may be inordinately large, especially because
$\ip=\pspace$\index{interactive proof system!IP=PSPACE} 
\cite{sha89}.  Protocol \provepred would
therefore require a great deal of time and very large messages to compute,
and is unsuitable for proving intractable predicates in a network of
polynomial time machines.

We present a protocol which achieves a zero-knowledge proof system for any
language $L \in \ip,$%
\index{interactive proof system!zero-knowledge}%
\index{zero-knowledge proof!for IP} yet uses
only a polynomial number of rounds and polynomial message complexity.  In
particular, zero-knowledge proofs for any language in $\ip$ can be made
without complexity theoretic assumptions, if a partly trusted network of
probabilistic polynomial time Turing machines is available.  In contrast,
when there are only a prover and a verifier, perfect zero-knowledge proofs
for NP-complete languages (which are in IP) are impossible unless the
polynomial hierarchy collapses
\cite{for87}.

The task at hand is distinguished from \mzkipss\  in a few ways.  First of
all, there are no secretly shared values {\em a priori.}  Second, the
string $x$ and the language $L$ that must be proven to contain it are both
public knowledge, or at least known to both prover and verifier.
Third, the purpose of the network is not to act as a repository for secrets
and committed values but to minimize the information leaked by the proof
system while ensuring that the prover behaves.

We distinguish two members of the network as before, the prover $\prover$
and the verifier $\verifier.$ In a two-party interactive proof system
(\cite{gmr89,bm88}, and \S\ref{sec-def-ips}), the prover is a $\pspace$
machine and the verifier is a polynomial-time machine.  The protocol is
such that, if $x \in L$ and the prover is not corrupted, then an
uncorrupted verifier will output {\em accept} with high probability.
Otherwise, an uncorrupted verifier will output {\em reject}.  Any language
in $\pspace$ admits an interactive proof \cite{sha89}; the presence of a
network of processors is irrelevant.

For the purpose of restricting information, however, a network of
processors is invaluable.  Zero-knowledge proof systems are often based on
unproven complexity assumptions \cite{gmr89}; perfect zero-knowledge proofs
even for languages in $\np$ cannot be achieved, unless the polynomial
hierarchy collapses \cite{for87}.  Perfect zero-knowledge proof systems can
be obtained given {\em two} provers that are not allowed to communicate
\cite{bgkw88,bgg88}.  Here, we allow only one prover, and that prover is
allowed to communicate with all of the participants and to collaborate with
a constant fraction.

The idea of zero-knowledge proofs again corresponds to secure multiparty
protocols.  The protocol must provide the verifier with one of two outputs,
{\em accept} and {\em reject}.  If the prover and verifier are not
corrupted, then the verifier accepts with high probability if $x \in L,$
and otherwise rejects.  If the verifier is not corrupted and $x \not \in
L,$ then the verifier rejects with high probability.  As in the definition
of two-party zero-knowledge, a cheating verifier must be able to simulate
the conversation.  The definition of multiparty protocol resilience
suffices to provide privacy not only with respect to the verifier but with
respect to the prover as well.

We define a particular function $F_L$ that states whether a string $x$
agreed upon by two players is in a given language $L:$ $F_i(x_1,\dots,x_n)
= 0$ if $i \not= \verifier,$ and
\[
F_{\verifier}(x_1,\dots,x_n)  =
\left\{
%}
\begin{array}{rl}
1 & \mbox{ if } x_{\prover}=x_{\verifier}= x \not= \Lambda \mbox{ and }
x \in L \\
0 & \mbox{ otherwise. } \\
\end{array} 
\right.
\]
Note that either player can refuse to participate by failing to supply a
proper input ($x=\Lambda$).  The only way for an honest verifier to be
convinced that $x \in L$ is if the prover decides to participate and $x\in
L.$ 

\begin{definition}  \label{def-zk-network}
Let $L$ be a language.  
A $(t,n)$ {\defstyle zero-knowledge network proof
system} (ZKNPS) for $L$ is a $t$-resilient $n$-player protocol for $F_L.$
\end{definition}
As usual, the adjectives {\em perfect, statistical, computational} apply.

\begin{theorem}  \label{thm-zk-network}
For $2t<n$ and any $L \in \pspace,$ \provenzk is a statistical ZKNPS
for $L.$
For $3t<n,$ \provenzk is a perfect ZKNPS for $L.$
\end{theorem}

\begin{proof}
By a result of \cite{gs86}, $L$ admits an interactive proof if and only if
there is an Arthur-Merlin\index{Arthur-Merlin} protocol \cite{bm88} for
$L,$ in which the verifier takes the position of Arthur, and simply sends
random coins to Merlin.  Arthur accepts the proof based on a polynomial
time computation using the set of messages sent by Merlin.

Without loss of generality, assume that for some polynomial $p_1(m,k),$ the
AM protocol runs in $p_1(m,k)$ steps, and that at each step, the messages
are of length $p_2(m,k).$ The program of Arthur is simple to specify: at
round $r,$ generate $p_2(m,k)$ random bits, send them to Merlin, receive a
message $M_r$ from Merlin, and repeat $p_1(m,k)$ times; afterwards, compute
a polynomial-time function $V$ on the messages $M_1,\dots,M_{p_1(m,k)}$
from Merlin, and output the result.  Merlin, however, must compute some
presumably complicated function $P_r$ to generate the correct response
$M_r$ at each round.

Thus we may take the interactive proof system to be the hidden composition
of the functions
\[
V \closedcomp P_{p_1(m,k)} \closedcomp V_{p_1(m,k)} 
\closedcomp \cdots \closedcomp P_1 \closedcomp V_1.
\]
The result, and only the result, is revealed to \verifier.

Because each function $V_r$ is simply a set of random bits, protocol
\randomsecret suffices.  The key is to construct a protocol that computes
each $P_r$ in a $t$-resilient fashion.  In general, the functions $P_r$ may
be too complex to admit small circuits, and hence would be expensive in
terms of interaction.  In fact, however, there is no need to compute $P_r$
through circuit simulation.  Instead, the network reveals $V_r$ to \prover,
who computes $P_r$ on its own, and shares the result.  Notice that the
functions $V_r$ are private, since they are simply random bit sequences
independent of all input values; hence revealing them to $P_r$ is perfectly
tolerable.

The computation of function $V$ could be performed through circuit
simulation, but at an expense of polynomially many rounds, since there is
no guarantee that $V,$ a polynomial-time calculation, admits sub-polynomial
depth circuits.  Instead, \prover computes $V$ and shares the result, $v.$
Player \prover then provides a zero-knowledge proof on {\em secrets}, as per
\S\ref{sec-zkp-ip}, to ensure that $v$ is correct.  By verifying each step
in the computation of $V$ locally yet in parallel, the number of rounds is
kept down to a constant.  


\figstretch
\boxfig{
\noindent{\bf \provenzk}\\
\begin{tabbing}  \standtabs
\>
{\For $u=1..p_1(m,k)$ \Dopar} \\
\>\>
{\For $v=1..p_2(m,k)$ \Dopar} \\
\>\>\>
Run \randombit to generate random secret $b_{uv}.$ \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\>
{\For $r=1..p_1(m,k)$ \Do} \\
\>\>
Reconstruct $V_r = (b_{r,1},\ldots,b_{r,p_1(m,k)})$ for $\prover.$ \\
\>\>
\prover computes $M_r=P_r$ and shares it. \\
\>
\prover computes $v=V(M_{p_1(m,k)},V_r{p_1(m,k)},\ldots,M_1,V_1)$ 
and shares it.
\\
\>
Run \provepred(\prover,\verifier;$V$;
$M_{p_1(m,k)},V_r{p_1(m,k)},\ldots,M_1,V_1$;$v$). \\
\>\>
%\If output is {\em reject} or $v \not={\em accept}$ \Then  \\  %drb2020
\If output is {\em reject} or $v \not=\acc$ \Then  \\
\>\>\>
\verifier outputs {\em reject}. \\
\>\>
\Else \\
\>\>\>
\verifier outputs {\em accept}. 
\end{tabbing}
\caption{\label{fig-prove}
Protocol for $\prover$ to prove $x \in L$ to $\verifier.$
}}
\figstretchend






If $\prover$ is corrupted and fails to share the correct value of $P_r$ for
some $r$ or fails to supply a correct proof at the end, this corresponds to
its choosing, in the ideal protocol, an input $x=\Lambda.$ The prover has
the inevitable right not to participate; but the protocol we present
ensures that lack of participation is reflected properly in the final
results.  Notice that by the definition of two-party interactive proof
systems, function $V$ is robust against incorrect computations of
$P_1,\ldots,P_r,$ so that a corrupt $\prover$ who shares incorrect values
corresponds to a prover in the ideal case who chooses not to participate.

Formally speaking, we perform the composition of the following {\em ideal}
protocols.  In the first protocol, each player supplies a sequence of
$p_1(m,k)p_2(m,k)$ random bits, and the trusted host computes a string of
$p_1(m,k)p_2(m,k)$ uniformly random bits by computing the parities of each
group of $n$ bits.  It divides these into $p_1(m,k)$ strings $V_r$ of
length $p_2(m,k)$ and returns a robust and secret representation of them to
the players.  In each protocol $\idealname^{2r},$ the trusted party gives
$V_r$ to $\prover.$ In each protocol $\idealname^{2r+1},$ $\prover$
computes $P_r$ and gives it to the trusted host, who computes a robust and
secret representation of what $\prover$ supplied, and returns pieces to the
players.  In the final protocol $(2p_1(m,k)+2),$ each player provides its
pieces of the robust and private representation of all of the previous
inputs, and the trusted host computes $V$ on the reconstructed values.  It
returns the result to \verifier.

The composition of these protocols provides \verifier with the closed 
composition
\[
V \closedcomp P_{p_1(m,k)} \closedcomp V_{p_1(m,k)}
 \closedcomp \cdots \closedcomp P_1 \closedcomp V_1
\]
which reveals only the final result $V,$ as desired.  
By Theorems \ref{thm-zkp-pred-stat},
\ref{thm-zkp-pred-perf}, \ref{thm-concat}, \ref{thm-bgw}, and
\ref{thm-min}, the results are perfectly (statistically) $t$-resilient
if $3t<n$ ($2t<n$).
\end{proof}


%% When $2t<n,$ the probability of an improper run is at most
%% $\frac{1}{2^k},$ as before; when $3t<n,$ improper runs do not occur.
%% The simulator is constructed as in the proof of
%% Theorem~\ref{thm-alice}, and by induction on the number of rounds,
%% the view produced by the simulator is indistinguishable
%% from that generated during an actual run.




==> pre.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% pre.tex                    Preliminary definitions.  Protocol stuff.
%
%                            Copyright @1989  Donald Beaver.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{=======}
\typeout{pre.tex}
\typeout{=======}

\chapter{Preliminary Definitions}
\label{chap-pre}

\chapquote{
The rest of the pages he picked up from the floor, bunched together,
and threw down between his legs into the bowl.  Then he pulled the
chain.  
Down went the helping names, the influential numbers, the
addresses that could mean so much, into the round, roaring sea and
onto the rails.  
Already they were lost a mile behind, blowing over
the track now, over the glimpses of hedges into the lightning-passing
fields.

Home and help were over.  He had eight pounds ten and Lucille Harris'
address.
``Many people have begun worse,'' he said aloud.  
%% ``I am ignorant, lazy, dishonest, and sentimental, I have the pull
%% over nobody.''
}{
Dylan Thomas, {\em Adventures in the Skin Trade}
}

%% \begin{quote}
%% {\bf\tt protocol} {\em n} [MF {\em prothocole}, fr. ML {\em protocollum},
%% fr. LGk {\em protokollon} first sheet of a papyrus roll bearing data
%% of manufacture, fr. Gk {\em prot-} prot- + {\em collan} to glue
%% together, fr. {\em Kolla} glue; akin to MD {\em helen} to glue]
%% {\bf\tt 3 a:} a code prescribing strict adherence to correct etiquette
%% and precedence {\tt b:} a set of conventions governing the treatment
%% and esp. the formatting of data in an electronic communications
%% system
%% \end{quote}
%% \hspace{2.0in}--- {\em Webster's Ninth Ed.}
%% \medskip

We shall require a modest repertoire of definitions before the results of
this dissertation can be stated and proved.  Many of these definitions are
standard and we sketch them here for completeness; others have not appeared
or are unsatisfying for many reasons, and the precise and concise
formalization of their intuitive meanings is a novel, necessary, and
unifying contribution of this dissertation.  In this chapter we present
general definitions and describe the mechanical nature of a protocol --
{\em i.e.} the nature of the participants and adversaries, the network, and
the sequence of computations and communications involved.  In
Chapter~\ref{chap-def} we examine the precise nature of security and
reliability for multiparty protocols, a more subtle and significant issue.
%% In this chapter we present general
%% definitions and describe some relevant background, and then give formal
%% definitions for interactive protocols, the participants, and the properties
%% achieved by those protocols, thus providing a framework in which to prove
%% our results.

Let us emphasize once again the fundamental abstraction of a multiparty
computation:
\begin{quote}
Each of $n$ parties holds a private input value $x_i,$ and together the $n$
parties wish to compute a (finite and multi-valued ``probabilistic'')
function $F(x_1,\dots,x_n)$ without revealing anything but the result.
That is, they wish to simulate the following situation: a trusted and
reliable party receives each of their inputs privately, computes the
function $F(x_1,\dots,x_n),$ and returns the results to the players.
\end{quote}

In order to appreciate and to compare the variety of protocols under the
broad and varied set of assumptions and network models, a unifying model is
needed.  The important mechanical parameters of a model and solution can be
listed in a few dimensions.  The participants may be resource-unbounded
automata, having a finite or even an infinite number of states (the
``information-theoretic'' model), or Turing machines with limited resources
(the ``complexity-based'' model).  The network may connect the participants
completely, and it may also support a range of communication channels,
broadcast and private channels being the most important but by no means
exclusive.  Unproven complexity theoretic assumptions or cryptographic 
assumptions may be made;
often, for example, protocols are based on the unproven existence
of one-way or trapdoor functions.
Normally, one allows an adversary to observe and perhaps to change the
communications to and from various participants.  The adversary may be
unbounded or bounded, static or dynamic in its choice of participants to
corrupt, and passive or malicious in its actions.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Notation}
\label{sec-notation}
\label{sec-def-indist}

We use a vector notation\index{vector notation} to represent a labelled set
of items: $\vec{x} = \set{(1,x_1),\dots,(n,x_n)};$ we shall normally omit
the labels, writing $\vec{x} = \set{x_1,\dots,x_n}.$ A subscript denotes a
subset of those values: $\vec{x}_T = \set{x_i \mid i \in T}.$ Bars indicate
complements: $\overline{T} = [n]-T,$ where $[n] = \set{1,\dots,n}.$
The operation $a \Div b$ is defined as $b \lfloor \frac{a}{b} \rfloor.$

We adopt the standard alphabet\index{$\Sigma,$ alphabet} $\Sigma=\set{0,1}.$
We may extend it through a trivial encoding to include other characters,
especially the delimiter, \#, and a symbol $\Lambda$ indicating a null message.
Let $\Sigma^{\leq c} = \bigcup_{i=0}^c \Sigma^c.$ If $\sigma$ is a string then
$\sigma[a..b]$ denotes the substring of $\sigma$ from the $a^{th}$
character to the $b^{th},$ inclusive.  The symbol $\oplus$ denotes
exclusive or of bits, or the bitwise exclusive-or when applied to a pair of
strings.  The exclusive-or of the bits $b_i$ as $i$ ranges over a specified
set is denoted $\oplus_i b_i.$ The symbol $\circ,$ when used with strings,
denotes concatenation.  For notational convenience, we define $H_m =
(\sigstar)^m,$ the set of $m$-tuples of strings, and we let $H =
\bigcup_{i=1}^{\infty} H_i.$ We assume a uniquely decodable encoding of
$m$-tuples of strings into single strings.

We assume a natural encoding of sets of strings when written using
$\Sigma:$ if $S=\set{s_1,\dots,s_n}$ is a set of strings (where, without
loss of generality, $s_1,\ldots,s_n$ are in lexicographic order), then $S$
is written as $s_1\#s_2\#\cdots\#s_n.$ If $S'$ is a set of objects each of
which has a natural encoding as a string, then the encoding of $S'$ is the
same as the encoding of the set $S$ of encodings of each of its members.
When we speak of a set of messages or a state being written on a tape, we
implicitly assume a natural and uniquely decodable ({\em e.g.} prefix-free)
way to tag various items
such as messages (include the sender, receiver, communication channel,
contents, and time of sending) or Turing machine states.

The notation ``$i:$'' in a protocol description indicates a
local computations and variable assignments of player $i.$  
The notation ``$i\rightarrow j:m$''
indicates that $i$ sends $m$ to $j,$ and $i \rightarrow [n]:m$
means that $i$ broadcasts $m.$  The notation
$(1\leq i \leq n)$ indicates that the succeeding text is performed
in parallel for $i$ in the range from $1$ to $n.$

Let $\dist(X)$ denote the set of all distributions%
\index{$\dist(X),$ set of distributions} 
on a set $X.$ The probability of event $Y$ with respect to
distribution $P$ is denoted $\probb{P}{Y}.$ 
A {\em probabilistic function}%
\index{probabilistic function}
$F$ is a function mapping some domain $X$ to a set of {\em
distributions} on a set $Y,$ that is, $F : X \rightarrow \dist(Y).$ The
output of a probabilistic function is a distribution, but sometimes we may
abuse notation and refer to a the output as a {\em sample} taken 
according to that distribution.

The difference of two distributions $P$ and $Q$ on a set $X$ is defined by
$\abs{P-Q} = \max_{W \subseteq X} \abs{\probb{P}{W}-\probb{Q}{W}}.$ We
denote a sample $x$ taken according to $P$ by $x \leftarrow P;$ a distribution
may also be written as $P=\set{x \leftarrow P}.$
Let
$\set{x \leftarrow P \mid Y(x)}$ be a sample $x$ taken according to the
distribution $P$ subject to the condition that $Y(x)$ holds.  Let $f$ be a
function from some number $j$ of arguments to a range $X;$ we denote by
\[
\set{x_1 \leftarrow P_1; x_2 \leftarrow P_2(x_1); 
x_3 \leftarrow P_3(x_1,x_2);
\dots; x_j \leftarrow
P_j(x_1,\ldots,x_{j-1}): f(x_1,x_2,\dots,x_j)}
\]
the distribution on $X$ induced by running the $j$ experiments in order and
applying $f$ to the results. Where clear from context, we use the same
notation to describe a sample drawn from that distribution.  
The composition of two probabilistic functions $F:X \rightarrow \dist(Y)$
and $G:Y \rightarrow \dist(Z)$ is the probabilistic function 
$H:X \rightarrow \dist(Z)$ given by 
\[
H(x)=\{y \leftarrow F(x); z \leftarrow G(y) : z \}.
\]

Some often used distributions are: the uniform distribution on a set $X,$
denoted $\uniform(X);$\index{\uniform}
the uniform distribution on the set $\polyn(t,s)$ of polynomials $f(u)$ 
of degree $t$ satisfying $f(0)=s,$ denoted 
$\unifpolyn(t,s);$\index{$\unifpolyn$}
and the set of $n$ values obtained by selecting such a polynomial at 
random and evaluating it at $n$ points, defined by
\begin{eqnarray*}
\allpieces(n,t,s)\index{$\allpieces,$ pieces of polynomial} & = &
\{
\vec{y} \in E^n \mid 
(\exists f \in \polyn(t,s)) (\forall i) y_i = f(\alpha_i)
\} \\
\unifpieces(n,t,s)%
\index{$\unifpieces,$ uniform distribution on $\allpieces$} 
 & = &
\uniform(\allpieces)
\end{eqnarray*}
Here, $E$ is some finite field and the $\alpha_i$ values are implicitly fixed,
normally either $\{1,\ldots,n\}$ or $\{1,\omega,\ldots,\omega^{n-1}\}$
where $\omega$ is a primitive $n^{th}$ root of unity.
A coin biased to $0$ by $b$ is the distribution
$\bias(b)\in \dist(\set{0,1})$ given by 
$\prob{0}=\half+b.$\index{biased coin}

An ensemble\index{ensemble} is a family ${\cal P} = \set{P(z,k)}$ of
distributions on $\Sigma^{\leq p(\abs{z},k)},$ parametrized by 
%
%$l \in \nat,$
$z \in \sigstar$
and $k \in {\bf N},$
%
where $p(\cdot,\cdot)$ is polynomially bounded.  
%% When applied to
%% distributions generated by protocols, for example, $l$ describes the number
%% and size of inputs, $z$ describes the various inputs and the adversary, and
%% $k$ is a security parameter.  When applied to zero-knowledge proof systems,
%% $z$ describes the theorem to be proved and the history of previous proofs,
%% and again $k$ is a security parameter.  We sometimes omit parameters when
%% they are irrelevant to the current context.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      INDISTINGUISHABLE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}  \label{def-indist}
Ensembles $\scp$ and $\scq$ are {\defstyle
$\delta(k)$-indistinguishable}\index{indistinguishability} if
\[
%% (\forall l)
%% (\exists k_0: \nat \rightarrow \nat)
%% (\forall k \geq k_0(l))
%(\exists k_0)
%(\forall k \geq k_0)
(\forall k)
(\forall z)
\hspace{0.3in}
\abs{\scp(z,k)-\scq(z,k)} \leq \delta(k).
\]
\end{definition}
We write this as $\scp
\indistEn^{\delta(k)}\index{$\indistEn,$ indistinguishable ensemble} \scq.$
Under the standard $O$-notation, $f(k)=O(g(k))$ means $(\exists c,k_0)(k
\geq k_0 \Rightarrow f(k) \leq c \cdot g(k)).$ We call $k_0$ the
convergence parameter.\index{convergence parameter}
\begin{definition}  \label{def-o-indist}
Ensembles $\scp$ and $\scq$ are 
{\defstyle
$O(\delta(k))$-indistinguishable}\index{indistinguishable} if
\[
(\exists \Delta: \nat \rightarrow \nat) 
\mbox{\hspace{0.2in}}
\scp \indistEn^{\Delta(k)} \scq
\mbox{\hspace{0.3in} \rm and }
\Delta(k) = O(\delta(k)).
\]
\end{definition}
We use the following adjectives to delineate various abilities to
discriminate between ensembles:
\[
\begin{tabular}{lccccrcl}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      PERFECT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\defstyle perfect} &
(written $\scp \indistEn \scq$) &
if &
 &
$\scp \indistEn^0 \scq.$ \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      EXPONENTIAL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\defstyle exponential} & 
(written $\scp \indistEnE \scq$) &
if &
$(\exists c>1)$ &
$\scp \indistEn^{O(c^{-k})} \scq.$ \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      STATISTICAL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\defstyle statistical} &
(written $\scp \indistEnS \scq$) &
if &
$(\forall c)$ &
$\scp \indistEn^{O(k^{-c})} \scq.$ \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      COMPUTATIONAL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\defstyle computational} &
(written $\scp \indistEnC \scq$) &
if &
              &
(see below)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}%
\index{indistinguishability!perfect}%
\index{indistinguishability!exponential}%
\index{indistinguishability!statistical}%
\index{indistinguishability!computational}%
\index{$\indistEn,$ perfectly indistinguishable}%
\index{$\indistEnE,$ exponentially indistinguishable}%
\index{$\indistEnS,$ statistically indistinguishable}%
\index{$\indistEnC,$ computationally indistinguishable}
\]

Computational distinguishability is based on the notion of a
resource-bounded machine that tries to distinguish strings sampled from one
distribution or the other.  A {\em distinguisher} $A$ is a probabilistic
polynomial size circuit which outputs either 0 or 1.  Let $A_{\scp(z,k)}$
denote the probability that $A$ outputs a 0 on an input selected according
to $\scp(z,k).$ Let {\sc PPC}\index{PPC} denote the class of probabilistic
polynomial size circuit families.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      COMPUTATIONAL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}  \label{def-comp-indist}
Ensembles $\scp$ and $\scq$ are {\defstyle $\delta(k)$-computationally
indistinguishable}\index{indistinguishability!computational} if
\[
(\forall A \in \mbox{\sc PPC})
%% (\forall l)
%% (\exists k_0: \nat \rightarrow \nat)
%% (\forall k \geq k_0(l))
(\exists k_0)
(\forall k \geq k_0)
(\forall z)
\mbox{\hspace{0.2in}}
\abs{A_{\scp(z,k)}-A_{\scp(z,k)}} \leq \delta(k).	
\]
\end{definition}
We say they are simply {\em computationally indistinguishable} if
$\delta(k)=O(k^{-c})$ for some fixed $c,$ and write $\scp
\indistEnC\index{$\indistEnC,$ computationally indistinguishable} \scq.$

We shall soon consider ensembles induced by running a protocol with
particular parameters $n$ (number of players) and $m$ (size of inputs).
Two {\em families} of ensembles $\set{\scp(i,j)}$ and $\set{\scq(i,j)}$ are
$\delta(k)$-indistinguishable if for all $i$ and $j,$ $\scp(i,j)
\indistEn^{\delta(k)} \scq(i,j).$ We write $\set{\scp(i,j)}
\indistFa^{\delta(k)}\index{$\indistFa,$ indistinguishable ensemble family}
\set{\scq(i,j)}.$

An ensemble $\scp$ is {\em polynomially generable}%
\index{generable, polynomially} if there exists a polynomial size 
circuit family with random inputs that, on input $z$
and $k,$ produces a distribution identical to $\scp(z,k).$


\section{Two-Party Protocols}      \label{sec-twoparty}

Two-party protocols are programs for a pair of machines that must jointly
compute a result.  In its most general form, the definition of a two-party
protocol specifies only that the machines take turns computing and
communicating, eventually placing an output on each of their output tapes.
In fact, the two participants need not be machines but can be arbitrary,
even non-recursive functions mapping inputs to a random variable describing
the output.  We shall postpone discussion in full generality, however, and
for the moment consider a pair of machines.

Security for two-party protocols addresses what a given protocol accomplishes
when one of the participants is replaces by a different machine,
namely a {\em corrupted} machine.  Protocols are designed to withstand
or at least to detect such changes and to achieve the same results as
when neither party is replaced.

The two common types of machines used to model interactive computations are
Turing machines and circuits.  Depending on the degree and the nature of
the faults, one model has advantages over the other.  Non-uniform circuits
have greater computational power than Turing machines, so a protocol which
is secure against faulty circuits is stronger than one secure against
faulty Turing machines.  On the other hand, Turing machines present a more
natural model for real-world computations, in some senses, and thus the
power of nonfaulty members of a system is modelled more accurately.  The
protocols presented in this work generally require the power of a
polynomial time Turing machine at most, but they are stated with respect to
polynomial size circuits or more powerful players, to provide maximal
security.  A slightly different way to state this is that any uncorrupted
player is in general a Turing machine, whereas an adversary that corrupts
it may replace it by a more powerful, non-uniform circuit.

\subsection{Interactive Turing Machines}

An {\em interactive Turing machine} \cite{gmr89} is a probabilistic Turing 
machine
having a read-only input tape $x$ (which may be public or private),
a private work tape $W,$ a private random tape $R$ 
with a unidirectional read-head,
a read-only communication tape $C_{in}$,
and a writable communication tape $C_{out}$.
A random tape is a convenient intuitive tool to describe the generalized
computation of a probabilistic Turing machine: in particular, a probabilistic
Turing machine is a probabilistic function that maps input $x$ to the
distribution induced by choosing uniformly at random a mapping from
\nat to $\{0,1\},$ regarding this as the random tape of a standard,
deterministic, multitape 
Turing machine, and operating the machine in the usual way.
of bits, regarding this as
A machine makes a random decision, \ie\  flips a coin, by reading
its random tape.  

The interactive machine has a special {\em inactive} state, which
it enters after having performed a computation and writing on its
communication tape.  It is awoken from the inactive state when the
other machine enters its inactive state.  Local computation time is
the maximal number of steps used between entering inactive states;
total local computation is the total number of steps executed during
the interaction.

An {\em interactive protocol} is a pair of interactive Turing machines
[A,B] sharing the same public input tape and sharing 
communication tapes in the standard sense.  They take turns being active.
Normally, one or both of the machines uses polynomial local computation 
time, and often one of the machines is more powerful.
For instance, in the zero-knowledge proof
model, a machine which proves a complicated theorem may be permitted a
polynomial space computation to assist it in convincing a weak ,
polynomial-time verifier of the truth of the theorem.  

The {\em communication complexity} of a protocol is measured by two
factors: first, the number of rounds, {\em i.e.} the number of times 
each Turing machine enters its inactive state, and second, the message
complexity, {\em i.e.} the total number of bits sent during the protocol.
Each measure is a function of the size $m$ of the inputs.

\subsection{Non-Uniform Interaction}
\label{sec-nonunif-int}

For many reasons, a non-uniform model is superior to the uniform Turing
machine approach.  For instance, the security of an encryption scheme is
often stated with respect to circuits rather than Turing machines.  A
canonical example is given in \cite{gm84}.  Consider a public-key
cryptosystem in which a user A publishes his encryption key $E_A.$ In order
for the system to be secure, there should be no way for an adversary to
choose a polynomial-time Turing machine which inverts the encryption, even
if the adversary can choose the machine after the encryption key is
published.  The solution to this problem as presented in \cite{gm84} is to
allow non-uniform adversaries, such as circuits, which can have such
knowledge ``wired in.''

There are other, more important reasons to allow non-uniformity.  In order
to combine protocols in a modular way, a way to model information obtained
in earlier interactions is needed \cite{tw87,ore87,gmr89}.  Furthermore,
because external information may be available, even a protocol composed of
many subprotocols may not start with a {\em tabula rasa}.

Rather than using circuits as the model, though, it is more natural to
employ ``non-uniform'' Turing machines; the extensions to the circuit model
to allow interaction are somewhat inelegant.  Since the power of polynomial
size circuits is achieved by polynomial time Turing machines with
polynomial size advice strings (the class $\ppoly$), there is no loss of
generality in defining security and correctness with respect to Turing
machines that take advice.

A {\em non-uniform interactive Turing machine} is an interactive
Turing machine having a private read-only auxiliary input tape $\sigma.$ A
two-player {\em non-uniform interactive protocol} is a pair of non-uniform
interactive Turing machines.  Normally, each machine is taken to be a
polynomial-time machine, though for some purposes the machines may be
allowed unbounded computation time and unbounded advice.

In general, we shall use either the non-uniform Turing machine model
just described, or a more general model in which each player's
local computation is described by
some arbitrary, perhaps non-recursive function,
The former corresponds to the modern
trend of ``complexity-based'' cryptography, whereas the latter corresponds
to the classical approach of ``information-theoretic'' security, where
issues of computability and complexity are irrelevant.


\subsection{Two-Party Interactive Proof Systems}   \label{sec-def-ips}

Goldwasser, Micali, and Rackoff \cite{gmr89} and Babai \cite{bm88} pioneered
similar definitions of what it means for one machine to convince another
that a string is in a language, even when the doubting party does not have
the resources to decide the answer directly.  As defined in \cite{gmr89},
an {\em interactive proof system} [P,V] for a language $L$ is a
two-party protocol for machines called the {\em prover} (P) and the {\em
verifier} (V).  The verifier must use polynomial time, while the prover has
unbounded computation time and space.  Both machines employ probabilistic
computation.  At the end of the protocol, the verifier outputs
{\em accept} or {\em reject}.  In order to be a proof system, the protocol
must have the following properties:
\begin{itemize}
\item {\bf Completeness:}  
For $x \in L,$ if the protocol is run with correct P
and V, then for every $c>0$ and sufficiently large $n=\abs{x},$
V accepts $x$ with probability at least $1-n^{-c}.$
\item {\bf Soundness:}  
For $x \not\in L,$ if the protocol is run with any \pstar
and V, then for every $c>0$ and sufficiently large $n=\abs{x},$
V rejects $x$ with probability at least $1-n^{-c}.$
\end{itemize}

This definition generalizes in a straightforward way to cover proofs that
$f(x)=y$ for a function $f$ and values $x$ and $y.$


\subsection{Zero-Knowledge}           
\label{sec-def-zk}

It is natural to examine properties of the protocol under situations in
which one machine or the other is replaced by a different, ``faulty''
machine, which tries to obtain more information than it truly deserves.  
If
the transcript of messages send during a protocol can be generated by a
machine given only the output of the protocol, then intuitively that
machine learns nothing apart from the output by participating in the
protocol.
In an ideal case, a trusted prover would state whether or not $x \in L,$
and the verifier would accept the statement, learning only that fact
regardless of whether it were itself corrupt.  We wish to address the situation
in which the prover might be corrupt, while ensuring that  no information
is leaked beyond that of the ideal case.

Let $L \subseteq \sigstar$ be a language.  An ensemble $\scp(x,a)$ is {\em
perfectly (exponentially, statistically, computationally)
approximable\index{approximable} on $L$} if, for $x \in L,$ there is a
probabilistic expected polynomial time Turing machine $M$ whose output
$M(x,a)$ is perfectly (exponentially, statistically, computationally)
indistinguishable from $\scp(x,a).$ The machine $M$ is called a {\em
simulator}.

Notice the ``one-sidedness'' of the previous definitions.  If $x$ is not in
the language, there is no restriction that the distribution be generable by
some machine.  

Let $\vstar$ be a non-uniform interactive Turing machine with input $x$ and
auxiliary (advice) input $a.$ A protocol [P,V] is {\em perfectly
(statistically, exponentially, computationally) 
zero-knowledge\index{zero-knowledge} on
$L$ for \vstar} if the ensemble induced by the message history of the
interaction between $P$ and $\vstar$ is perfectly (statistically,
exponentially, computationally) approximable on the language
\[
\starr{L} = \set{ (x,a) \mid x \in L}.
\]
The protocol [P,V] is zero-knowledge on $L$ if it is
zero-knowledge on $L$ for any such $\vstar.$

A more powerful version of zero-knowledge considers a single, universal
simulator that simulates the conversation between $P$ and any $\vstar,$
using $\vstar$ as a ``black box''\index{black box} whose contents cannot be
examined or reset but whose input/output behavior is accessible.  A good
discussion of this and other flavors of zero-knowledge appears in
\cite{ore87}.


\subsection{Zero-Knowledge Proof Systems}      \label{sec-def-zkps}

With the definitions given above, it is easy to describe a zero-knowledge
proof system \cite{gmr89}:

A protocol [P,V] is a perfect (statistical, computational)
zero-knowledge proof system\index{zero-knowledge proof} for a
language $L$ if it is an interactive proof system for $L$ and it is
perfectly (statistically, computationally) zero-knowledge on $L.$


\section{Multiparty Protocols: The Participants}        

\subsection{Player {\em\bf ex Machina}}


A {\em player}\index{player} is an interactive automaton, namely an
automaton with an input tape, an auxiliary input tape, an output tape, and
a random tape.  Let us first consider the familiar case of interactive
Turing machines.

The definitions for the multiparty scenario are straightforward extensions
of those given for two-party protocols.
An interactive Turing machine with an input and an output communication
tape is easily regarded as one having $n-1$ input tapes and $n-1$ output 
tapes; technically, the bits of virtual tape $j$ are encoded in positions
$j+k(n-1)$ on the single tape, where $k$ ranges over the integers and 
specifies the position on the virtual tape.
As in the two-party case, each has a
read-only input tape, a private auxiliary tape, a private work tape,
and a private output tape.

A {\em multiparty Turing-machine protocol} is a set of $n$ interactive
Turing machines $\{M_1,\dots,M_n\}$ each having $n-1$ pairs of
communication tapes: the read-only communication tapes of machine $M_i$ are
labelled $\set{R_{ij}}_{j=1,..,n;j \not= i},$ and its exclusive-write tapes
are labelled $\set{W_{ij}}_{j=1,..,n;j \not= i}.$

A {\em round} in a synchronous protocol operating on a complete network
consists of the following events.  Each machine $M_i$
enters its active state, computes, and returns to its inactive state.
Each tape $W_{ij}$ is then copied to $R_{ji}.$  We shall soon
describe these mechanics in more detail, including how adversaries affect
the execution.

The computation time of machine $M_i$ is the sum of the steps it
takes while it is in an active state.  The message complexity of
the protocol is the total length of all messages sent.

%% We shall momentarily specify with more generality and formal detail the
%% sequence of events and computations occurring during the execution of a
%% protocol.  First let us specify a player in the most general terms in order
%% to have a single model within which we are able to choose the desired level
%% of complexity ({\em e.g.} bounded Turing machine {\em vs.} non-recursive
%% function) of the players and the adversaries who attempt to disrupt the
%% protocols.


\subsection{General Players}

Before specifying the sequence of events and computations occurring during
the execution of a protocol in more detail, let us first describe a player
in the most general terms.  We allow a broader model than Turing machines
for a few reasons.  Turing machines are restricted to computing recursive
functions.  If they compute a probabilistic function using a random tape,
then the resulting distribution is a recursive function of the input and
random tape.  Non-uniform functions and general distributions would not be
achievable.  In fact, even simple distributions, such as generating random
numbers modulo 3, are not computable in bounded time.  

Even though the protocols we design will not require non-recursive
functions or distributions, we would like them to be secure against the
most powerful adversary.  By using a broad computational model, we cover
all the participants --- players and adversaries --- in the protocol, and
do not need to pay attention to {\em how} a new set of messages is computed
({\em e.g.} whether by Turing machine or non-recursive function) unless we
wish to do so under particular circumstances.  This corresponds to the
``information-theoretic'' model, in which one is concerned with ``perfect''
secrecy; any distinguishable difference or dependence among distributions
on messages sent from player to player is considered to give away
information, regardless of the resources needed to detect it.  The
information-theoretic model does not restrict the power of the players and
malicious adversaries to compute recursive or even polynomial-time
functions on the messages they see; in fact, each player is defined more
generally as a probabilistic function from input messages to output
messages.%
\footnote{
Even though a function from strings to strings can be specified in a
discrete manner, a {\em distribution} on strings need not have some
discrete specification.  Often a probabilistic machine is regarded as
having a discrete and uniformly distributed input ({\em e.g.} a random tape
of bits).  Using {\em functions} rather than discrete specifications of
functions to describe the allowable transitions and distributions associated
with an ``automaton'' is more general and more powerful.
}

Thus, for full generality, we use a very general format: we describe
players as automata that may have a finite or infinite state set, and we 
set bounds on available resources only under specific circumstances.%
not set bounds on available resources.%
\footnote{
In the ``cryptographic'' model, for example, 
we may assume that players and adversaries are
polynomial-time Turing machines.  It boils down to the comment made earlier:
one can either regard a corrupted participant as a player gone awry, in which
case it is better to regard each player as powerful, or one can describe 
several different computational models, one for uncorrupted players, one
for an adversary, one for corrupted players, and so on.
}
%
Our informal use of the term ``automaton'' extends beyond the
common usage describing a finite-state machine, since we allow for infinite
state sets.  A Turing machine with infinite work and random tapes is an
automaton having an infinite general-state set, where each state describes
the finite control and the contents of the tapes.  

Each player has a state set $Q,$ a standard input set $X \subseteq
\sigstar,$ and an auxiliary input set $\auxin.$ 
For Turing machines, each input in $X$ includes a string $x$ and a security
parameter $k.$ The initial state of a player is selected according to the
input, auxiliary input, and security parameter $k;$ that is, each player has
a function $\initfn:X \times \auxin \times \nat \rightarrow Q.$

As in the case of {\em non-uniform interactive protocols}
(\S\ref{sec-nonunif-int}), the auxiliary inputs serve a few purposes.  They
introduce and encapsulate non-uniformity in a uniform model; that is, when
giving the conceptually simple specification that each player is a Turing
machine, they are a convenient means to introduce non-uniformity.  They may
also represent information held jointly by various players, such as shared
private encryption keys.  Their most common use, however, is not as part of
the protocol {\em per se} but as a record of information obtained in other
or previous computations and interactions.  For example, auxiliary input
$a_i$ may represent the history of conversations in which player $i$
participated during the previous protocol.  As in the composition of
zero-knowledge proof systems, examining resilience for arbitrary auxiliary
inputs allows one to demonstrate that secure protocols remain secure when
composed sequentially ({\em cf.}
\cite{ore87,hab88}).


During each round of a protocol, each player performs a probabilistic
computation and sends messages distributed according to the results.  The
sets of incoming and outgoing messages depend on the types of communication
channels and the number of other players in the network.  In particular,
each player is described by a {\em probabilistic} transition function
$\delta$ that produces a {\em distribution} on new states and new messages
based on the current state and incoming messages:
\[
\delta : Q \times H \rightarrow 
\dist(Q \times H).
\]
In other words, given a state and the messages of the previous round,
$\delta$ produces a distribution on new states and messages from which
distribution the subsequent state and outgoing messages of the player are
drawn.

Note that the transition function produces a {\em distribution} on outputs,
in analogy to the computation of a probabilistic Turing machine, which need
not compute a {\em function} of its inputs, but rather produces a
distribution on outputs based on its input and induced by the uniformly
random bits on its random tape.  A Turing machine can also be regarded as
producing a {\em sample} from that distribution (in particular, a Turing
machine {\em is} a function of its input and random input).  We consider a
general player in a similar, dual fashion: as producing a distribution, or
as producing a sample from that distribution.  This will allow us to
describe protocol executions in terms of the {\em distributions} on
messages as well as in terms of {\em particular message histories}
generated according to those distributions.

\begin{definition}
A {\defstyle player}\index{player} is a tuple $(Q,X,\auxin,\initfn,\delta)$
whose components are as described above.
A {\defstyle polynomial-time Turing machine player}%
\index{player!Turing machine}
is a player whose
transition function $\delta$ and initial-state function $\initfn$ are
computable in time polynomial in
the size of its input, auxiliary input, incoming messages, and an
additional parameter, $k.$
A {\defstyle polynomial-size circuit player}%
\index{player!circuit}
is a player whose
transition and initial-state functions are computable by a circuit family
of size polynomial in the above parameters.
\end{definition}

\section{Protocols}

\subsection{Networks and Communication Channels}

A {\em channel}\index{channel} is a probabilistic function $C : \sigstar
\rightarrow {\bf N} \times {\bf N} \times \sigstar$ that takes a message
$m$ as input and produces a distribution on sets of deliverable messages.
A deliverable messages is a triple of the form $(s,r,m),$ where $1 \leq s,r
\leq n$ and $m \in \sigstar.$ After all channel functions are applied and
the resulting distributions are sampled, the collection of resulting
triples forms the set ${\cal M}$ of messages to be delivered.  The subset
${\cal M}_s$ defined as $\set{(s,r,m) \mid (s,r,m) \in {\cal M}, 1 \leq r
\leq m}$ is placed on the input tape of player $r.$ If player $s$ writes
$(m,C_{sr})$ on its communication tape (meaning ``send $m$ on channel
$C_{sr}$'') then channel $C_{sr}$ is applied to $m,$ producing $(s,r,m),$
which is then placed on the communication tape of player $r.$  As mentioned
in \S\ref{sec-notation}, the set of messages appear in lexicographic order
on the tape.

For example, a private channel\index{channel!private} $C_{sr}$ from player
$s$ to player $r$ is the function that on input $m$ produces
$\set{(s,r,m)}.$ A broadcast channel\index{channel!broadcast} $C_s$ on
input $m$ produces $\set{(s,1,m),(s,2,m),\ldots,(s,n,m)}.$ An oblivious
transfer channel%
\index{channel!oblivious transfer}\index{oblivious transfer}
$C_{sr}^{\rm OT}$ gives
weight $1/2$ to messages of the form $\set{(s,r,m)}$ and $1/2$ to messages
of the form $\set{(s,r,\Lambda)}.$ 
An anonymous channel is modelled by supplying
the recipient simply with $m_j.$



\subsection{Protocols}
\label{sec-protocols}

An $n$-player protocol\index{protocol} is essentially a set of players,
channels, and output functions:
\[
\protoPi = 
\set{(P_1,\scc_1,\outfn_1,Y_1),\dots,(P_n,\scc_n,\outfn_n,Y_n)},
\]
where $\outfn_i : Q_i \rightarrow Y_i$ is an output function mapping the
(final) state of player $i$ to an output value in $Y_i.$ This can be taken
to be the contents of a work tape or output tape at the end of the
protocol.  The set of outputs depends on the purpose of the protocol but we
shall take it to be a set of $m$-bit strings.  Player $P_i$ is described by
$P_i=(Q_i,X_i,\auxin_i,\initfni,\delta_i).$ Each $\scc_i$ denotes a set
$\set{C^j}_{j \in \natsmall}$ of channels on which player $P_i$ sends its
messages.  We sometimes omit the square brackets and write $\Pi(n,m)$
instead; when other parties such as adversaries or trusted hosts are
discussed, the square brackets are intended to delimit the list of
participants.

A {\em network}\index{network} is a set of channels.  A {\em
protocol} $\Pi(n,m)$\index{protocol} is
implementable on a given network only if its channels are a subset of those
in the network.  A {\em protocol family}\index{protocol family} $\Pi=
\set{\Pi(n,m,k)}_{n,m\in \natsmall}$
specifies a protocol for each $n$ and $m.$ For each number $n$ of players
and $m$ of bits in the inputs, $\Pi(n,m)$ denotes a series of protocols
$\Pi(n,m).$ Finally, $\Pi(n)$ denotes a sequence of sets of $n$ players,
each with $m$ built in, but for purposes of asymptotic complexity analysis,
each of these players can be regarded as Turing machines that read $n$
and $m$ from its input tape.


\subsection{Protocol Compilers for Turing Machines}
\label{sec-proto-compile}

At times we may wish to regard the participants as Turing machines even
though the function $F(x_1,\dots,x_n)$ itself may not be recursive.%
\footnote{How can recursive machines compute a non-recursive function?
As we shall shortly discuss, it is often convenient to consider a universal
machine that receives a written specification of $F$ as an input.  The 
specification, which may be a circuit or formula, need not be generable
by a Turing machine.}
One
reason for regarding the players as circuits or non-uniform Turing machines
with respect to their power to ``break'' the protocol is that the
specification of a non-uniform function $F$ might itself lend power to an
otherwise uniform or polynomial-time machine.  We therefore turn our
attention to protocol ``compilers,'' which produce the specifications of
the players for the various possible network sizes, input sizes, and
security parameters.

A protocol compiler\index{protocol compiler} $\scc$ is a circuit family
$\set{C_{n,m,k}}$ where $n$ specifies network size, $m$ specifies the
number of bits in the arguments, and $k$ is a security parameter for
protocols which may ensure security and reliability with high probability,
although not certainty.  The compiler $\scc$ produces a description of $n$
Turing machines, each of which has an input $x_i$ and $n$ communication
tapes.  The computational resources of the compiler (its size and depth)
may or may not be of importance to the protocol designer, though usually
they are related to the complexity of $F.$ As with circuit families in
general, the compiler itself may be {\em uniform} (generated by a Turing
machine) or non-uniform, which would be necessary to specify protocols
computing general, perhaps non-recursive functions $F.$

A {\em universal protocol}\index{protocol!universal} specifies a single
Turing machine $M$ which takes a special input $(1^n,1^m,1^k,i,C_F),$ 
where $i$
indicates the identity of the machine in the network and $C_F$ is a
circuit description of the function $F$ for the given size and number 
of inputs.
In this case, the protocol for $n$ players consists of $n$ copies of $M,$
each of which is supplied with the appropriate parameters and a unique
identification.  Our protocols are generally of this type.

We measure the 
{\em message complexity}%
\index{complexity!communication}%
\index{complexity!message}\index{$\mesgcpx$}
$\mesgcpx(\protoname),$
(maximal number of bits in any execution), 
{\em round complexity}\index{complexity!round}\index{$\rounds$}
$\rounds(\protoname)=R,$
{\em local computational complexity}%
\index{complexity!local}\index{$\localcpx$}
$\localcpx(\protoname),$
(resources required by a Turing machine to compute the player's
transitions between rounds),
{\em computational complexity of F}%
\index{complexity!computational}\index{$\compcpx$}
$\compcpx(\protoname),$
(Turing machine
complexity of computing the outputs of all the players) 
as functions of $n,$
$m,$ and $k,$ unless otherwise specified.  Stating that a protocol uses
polynomial size messages means, for example, that it communicates at most
$p(n,m,k)$ bits in any execution, where $p(n,m,k) = O((nmk)^c)$ 
for some fixed $c.$

Usually, it is not difficult to design universal protocols in which the
communication complexity is polynomial in $n,m,k$ and the description of
$C_F.$ The trick is to design a compiler whose protocols have communication
complexity polynomial in $n,$ $m,$ and $k$ only, regardless of $F$ and its
complexity.


\subsection{Reliable Protocol Execution}
\label{sec-reliable}

Let us formally describe the sequence of steps that occur during a protocol
when all the participants are reliable.

Since our purpose is to specify {\em precisely} the nature of a protocol
and its execution rather than to become immersed in formalism, let us use
some shorthand to relieve the burden of the notation.  As mentioned, during
each round of a protocol, a player performs a computation and then sends
messages over its various channels.  Let $\mess^{\out}(U,V,r)$ denote the
set of messages sent from players in set $U$ to players in set $V$ during
round $r.$ Let $\mess(U,V,r)$\index{$\mess(i,j,r),$ messages sent}
 denote the set of messages actually delivered
from players in set $U$ to players in set $V,$ that is, those messages
drawn according to the various channel distributions acting on
$\mess^{\out}(U,V,r).$ Denote the messages received by $V$ from $U$ and $U$
from $V$ by $\mesg(U,V,r) = \mess(U,V,r) \cup \mess(V,U,r).$
(As stated in \S\ref{sec-notation}, we assume a natural and uniquely
decodable encoding of these sets of messages as strings.)  We sometimes
add a label to describe a substring of a message, so that $\mess(i,j,r;x)$
indicates the message $i$ sends to $j$ about variable $x.$

Let $\send(\set{m_1,\dots,m_k},\set{C_1,\dots,C_k})$ denote the
set of messages generated by applying each message $m_i$ to channel
$C_i.$

An execution of a synchronous $R(n,m,k)$-round protocol $\Pi(n,m,k)$ on inputs
$\vec{x}$ and auxiliary inputs $\vec{a}$ is the sequence of states and
messages obtained from the following experiment.  Initialize all states
according to $\vec{x}$ and $\vec{a}.$ At each round, select the new states
and outgoing messages using the transition functions of each player, apply
the messages to the channels, and generate the messages actually sent.
Finally, after round $R=R(n,m,k),$ allow one final computation.  The output of
player $i$ is a function of its final state; in the case of a Turing
machine, the output is written on the output tape.

More formally, but still using a somewhat loose notation, consider the case
of a network with private lines and broadcast channels.  We denote the
messages sent over private lines by $\mess_{\priv}(U,V,r)$ and those sent
over broadcast lines by $\mess_{\broad}(U,[n],r).$ Let $\scc_{\priv}$ and
$\scc_{\broad}$ denote the private and broadcast channels.  An execution of
the protocol is generated by the experiment shown in
Figure~\ref{fig-exec-reliable}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Figure:  Reliable Execution
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\figstretch
\boxfig{
\noindent{\bf \protostyle Reliable Execution}
\index{execution}
\begin{tabbing} \standtabs
%
% INITIALIZE STATES
%
{\For $i=1..n$ \Do}
\>\>\>\>\>\ccomment{initialize states} \\
\>
$\initfni \leftarrow \initfni(x_i,a_i,k).$ \\
\\
%
% ROUND BY ROUND
%
{\For $r=1..R$ \Do}
{\for $i=1..n$ \Do} 
\>\>\>\>\>  \ccomment{compute and send messages}\\
\>
$(q_i^{r},\mess_{\priv}^{\out}(i,[n],r),\mess_{\broad}^{\out}(i,[n],r)) 
 \leftarrow $ \\
\>\>\>\>\>
$\delta_i(q_i^r,\mess([n],i,r-1))$ \\
\>
$(\mess_{\priv}(i,[n],r),\mess_{\broad}(i,[n],r)) 
 \leftarrow $ \\
\>\>\>\>\> 
$\send(\mess_{\priv}^{\out}(i,[n],r) \cup \mess_{\broad}^{\out}(i,[n],r),
$ \\
\>\>\>\>\>
$\scc_{\priv} \cup \scc_{\broad})$\\
\\
%
% FINAL COMPUTATION
%
{\For $i=1..n$ \Do}
\>\>\>\>\>\ccomment{ final computation after protocol }\\
\>
$q_i^{f} \leftarrow
\delta_i(q_i^R,\mess([n],i,R))$ 
\end{tabbing}
\caption{\label{fig-exec-reliable}
Execution of protocol $[\Pi]$ with reliable players in a synchronous
network with private and broadcast channels.
}}
\figstretchend




\subsection{Views}

A global state vector\index{global state vector} is a sequence of $n$
states, one for each player.  In general, we may consider state vectors for
arbitrary subsets of the $n$ players.  Let $\playerstates$ be the set of
all partial state vectors:
\[
\playerstates = \set{ 
\vec{q}_B \mid \vec{q} \in Q_1 \times \cdots \times Q_n,
 B \subseteq [n] }.
\]
Similarly, in order to consider sets of inputs and auxiliary inputs for
arbitrary subsets of the players, we define
\[
\playerinputs = \set{ 
(\vec{x}_B,\vec{a}_B) \mid \vec{x} \in X_1 \times \cdots \times X_n,
\vec{a} \in \auxin_1 \times \cdots \times \auxin_n,
 B \subseteq [n] },
\]
and we use this notation to describe the set $\playeroutputs$ of outputs
for arbitrary subsets of the players.

We call the state vector and messages seen by
a subset $B$ of the players at a given round $r$ a {\em view}:
\[
\view_B^r = ( \vqr_B, \mesg(B,[n],r) ).
\]
The set of all possible views\index{views}\index{$\playervs,$ set of views} is
\[
\playervs = \playerstates \times H.
\]

A {\em history} or {\em execution}\index{execution} of the protocol is thus
a member of the set $\histsp$ of inputs, auxiliary inputs, initial states,
sequences of views, and final states:
\[
\histsp =
\playerinputs \times \playeraux \times \playerstates \times
(\playervs)^R \times \playerstates.
\]
A protocol induces a distribution on executions according to the experiment
described formally in \S\ref{sec-reliable}.  We may regard a protocol
as a {\em probabilistic function} from inputs to executions; the function
is the composition of several probabilistic functions as described.



\subsection{Memoryless Protocols and Players}

As described thus far, a protocol is {\em memoryless};\index{memoryless}
the current states and messages are all that matter to the execution of the
protocol.  The final states of the players do not necessarily reflect the
history of the protocol.

In practical situations it is often impossible to assure that
no record is kept of previous operations.  Backups are kept;
transactions must be rolled back to consistent states when
failures occur; and a wide variety of reasons make it extremely
risky to assume that a history of previous behavior is erased
before an adversary gains control of an installation.

In order to assure maximal security, we consider a stronger model in which
each player is replaced by a modified player that records its view of the
history of the protocol in its current state.  In other words, the state
$q_i^r$ of player $i$ at round $r$ determines the sequence
$(q_i^0,(q_i^1,\mesg(i,[n],1)),(q_i^2,\mesg(i,[n],2)),\ldots,
(q_i^r,\mesg(i,[n],r))).$ The transition function $\delta_i$ is easily
modified to accommodate this record, giving rise to a player whose behavior
is identical but whose state records the sequence of states and messages
seen by that player.  In the case of Turing machines, this means that each
Turing machine is equipped with an extra, history tape on which it records
all its computations (communications, random bits, contents of work tapes,
etc.).

We adopt this as the {\em standard} model,\index{standard model}
 and assume that all
players are transformed in this manner.  
In the standard model, the set of states of players in some coalition $T$
at round $r$ defines not only their current view, $\view_T^r,$
but the history of the protocol up to that point:
$\vec{x}_T,\vec{a}_T,\vqz_T,\view_T^1,\dots,\view_T^r.$
We distinguish the weaker model, in which players may forget 
previous state information, by specifically noting it as
the {\em memoryless} model.\index{memoryless model}
The memoryless model has advantages in {\em proving} privacy
against dynamic adversaries in cryptographic models \cite{bhy89-pc}
because it permits easier simulations of the knowledge of corrupted
players.


\section{Adversaries and Fault Models}
\label{sec-fault-models}

This dissertation examines the security and reliability of multiparty
protocols under various fault models.  The types of allowable faults are
described below.  The definitions for the multiparty case also apply to the
two-party scenario as a special case.

Failures are modelled by an adversary which ``chooses'' to substitute new
messages for the messages otherwise computed according to the protocol.  
This ``choice'' is simply an interpretation of the string output by
the adversary, which is simply a player that computes an output string 
based on some transition function and its current state; the description
of a protocol execution states how that output string is interpreted as a 
request to corrupt individual participants.

A {\em static} adversary must choose the subset it will corrupt before the
protocol is executed.  A {\em dynamic} adversary may choose at the end of a
round the set of new processors it will corrupt for the next round.  In
either case, the adversary may be allowed to {\em rush} messages, that is,
to wait for nonfaulty processors to send their messages, see the messages
to which it has access, and then specify the messages of the corrupted
processors for that round.  Finally, a {\em strongly dynamic} adversary can
rush all messages, examine them, and decide to corrupt machines of its
choice before the messages are sent; the set of corrupted machines may
encompass every player in the network over the course of the execution,
though at any particular time the current coalition must be an allowable
one.  We shall consider dynamic but not strongly dynamic adversaries.

We measure security with respect to an {\em adversary
class},\index{adversary class} namely a set of adversaries.  A typical
example is the class of all polynomial-time Turing machines.  A more
powerful class allows unlimited computing time, though still requiring
messages to be recursive functions of the inputs.  Another powerful,
non-uniform adversary class is the set of all polynomial-size circuit
families (equivalently, polynomial-time Turing machines that take advice).
The most powerful class, corresponding to ``information-theoretic''
security, allows the adversary to be a general player, namely to have an
arbitrary transition function with an arbitrary set of states.

An important parameter of the adversary is the number $t$ of machines it is
allowed to corrupt.  The three ranges of primary importance are $t < n/3,$
$n/3 \leq t < n/2,$ and $n/2 \leq t \leq n-1.$ Different levels of
fault-tolerance and security are achievable for each of these ranges.

In addition to specifying the manner in which the adversary can choose
processors to corrupt, there are various sets of restrictions on the types
of messages it is allowed to substitute.  In order of increasing power, the
types of faults are as follows.
\begin{itemize}
\item {\bf Passive:}
The adversary cannot substitute different messages for any of the original,
uncorrupted machines.  It does, however, have access to the tapes and
states of the machines it ``corrupts.''  This model is sometimes called the
{\em gossip} model.
\item {\bf Fail-Stop:}
The corrupted processors cannot write improper messages (\ie\  different from
the protocol specifications), but may halt at some round, sending only
null ($\Lambda$) messages thereafter.
\item {\bf Omission:}
The corrupted processors cannot write improper messages but may omit some
of them periodically (replacing them by $\Lambda$).  
This model is useful in examining faulty
communication lines, where occasional messages are lost.
\item {\bf Byzantine:}
The adversary may compute any message of its choice (with restrictions,
of course, if the adversary is computationally bounded), whether proper or
improper according to the protocol, and it may omit messages as well.
\end{itemize}
A protocol attacked by an adversary is formally nothing more than a
protocol with $n+1$ players, each evaluating a probabilistic transition
function and receiving and producing messages.  When a specific adversary
is concerned, the protocol is denoted $[A,\Pi];$ when an adversary may be
chosen from some adversary class $\advclass,$ the set of resulting
protocols is denoted $\anglebrack{A,\Pi}.$



\subsection{Passive Adversaries}

A {\em fault class}\index{fault class} $\sct$ is a collection of allowable
coalitions, namely a collection of subsets of $[n].$ We require that if
$T\in \sct$ and $U \subseteq T,$ then $U \in \sct.$ The standard fault
class is the $t$-{\em fault class}, $\sct = \set{T \subseteq [n] \mid
\abs{T} \leq t},$ allowing any set $T$ of size $t$ or less to be corrupted.

Formally, a passive adversary\index{passive} is a tuple
$(Q_A,\auxin_A,\initfnA,\delta_A,T),$ where $Q_A$ is a set of states,
$\initfnA$ is a function mapping auxiliary inputs in $\auxin_A$ to initial
states in $Q_A,$ $\delta_A$ is a transition function to be described
shortly, and $T$ is a function mapping $Q_A$ to $[n],$ describing the
current coalition that the adversary chooses to corrupt.  The passive
adversary does not generate messages but it does choose a new state and new
coalition based on its current state and the view of the coalition it
currently corrupts:
\[
\delta_A : Q_A \times \playervs \rightarrow \dist(Q_A).
\]
A passive adversary is {\em static} if $T$ is constant, and thus fixed
before the protocol.  A passive adversary is {\em dynamic} if $T$ varies
with the state of the adversary.  Note that if the number $n$ of players is
fixed, then there is no essential difference between static and dynamic
adversaries.  There are a finite number, ${n \choose t}$ of fixed
coalitions; the chance of selecting any one of them at random is a constant
$c_n = 1/{n \choose t}.$ Any dynamic adversary chooses some coalition $T$
with probability at least $c_n.$ Thus there is some static adversary that
starts with coalition $T$ and therefore has a constant fraction ($c_n$) of
the probability of the adversary to corrupt the protocol successfully.  We
have not yet presented definitions of security, but it turns out that
constant factors do not matter; essentially, there is a static adversary
having the same power as the dynamic one.  If $n$ grows, then the
probability of a particular coalition $T$ vanishes, and there is a
difference between static and dynamic.


A passive $\sct$-adversary for a fault class $\sct$
is a passive adversary for which
\begin{itemize}
\item[(1)] for all $q_A \in Q_A,$ $T(q_A) \in \sct,$ and 
\item[(2)] it always chooses a new coalition that is a superset of
the current one ({\em i.e.}, for all $q_A \in Q_A,$ for all partial views
$\view_{T(q_A)}^r,$ for all states $q_A'$ having nonzero probability weight
in $\delta_A(q_A,\view_{T(q_A)}^r),$ $T(q_A) \subseteq T(q_A')$).
\end{itemize}
Since we shall be concerned with fault classes containing all coalitions of
size $t$ or less, we refer simply to a passive $t$-adversary.

Figure~\ref{fig-exec-passive} shows how a $R$-round protocol is executed
synchronously in the presence of a passive adversary.  The reliable
execution of a protocol defines a view seen by a subset of players; here,
it is straightforward to include the state of the adversary and the
messages it sees in the definitions of views and histories.  For clarity,
we abuse notation for the final computation, 
omitting mention of the last messages
generated by the transition function $\delta$ because they are ignored.



\figstretch
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Figure:  Passive Execution
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\boxfig{
\noindent{\bf \protostyle Passive Execution}
\index{execution!passive}
\index{passive}
\begin{tabbing} \standtabs
%
% INITIALIZE STATES
%
{\For $i=1..n$ \Do} \\
\>
$q_i \leftarrow \initfni(x_i,a_i,k).$ \\
Set \\
\>$q_A \leftarrow \initfnA(a_A,n,m,k).$ \\
\\
%
% ROUND BY ROUND
%
{\For $r=1..R$ \Do} \\
\> {\For $i=1..n$ \Do}
 \>\>\>\ccomment{each computes and sends messages} \\
\> \>
$(q_i,\mess^{\out}(i,[n],r)) \leftarrow 
\delta_i(q_i,\mess([n],i,r-1))$ \\
\> \>
$ \mess(i,[n],r)  \leftarrow
\send(\mess^{\out}(i,[n],r),
\scc_1 \cup \cdots \cup \scc_n)$ \\
\> Set 
\>\>\>\ccomment{adversary computes} \\
\> \>
$q_A
\leftarrow
\delta_A(q_A,\view_{T(q_A)}^{r-1}). $ \\
\\
%\> Set 
%\>\>\>\ccomment{adversary computes, but its messages aren't used} \\
%\> \>
%$(q_A,\mess^{\out}(T(q_A),[n],r))
%\leftarrow
%\delta_A(q_A,\view_{T(q_A)}^{r-1}). $ \\
%\\
%
% END PROTOCOL
%
{\For $i=1..n$ \Do} 
\>\>\>\>\ccomment{final computation} \\
\>
$q_i^{f} \leftarrow
\delta_i(q_i,\mess([n],i,R))$ \\
Set \\ 
\> $q_A^f \leftarrow \delta_A(q_A,\view_{T(q_A)}^R).$
\end{tabbing}
\caption{\label{fig-exec-passive}
Execution of protocol $\protoAPi$ with a passive adversary $A.$
}
}
\figstretchend





\subsection{Byzantine Adversaries}
\label{sec-exec-prot-adv}

A Byzantine\index{Byzantine} or malicious adversary
$(Q_A,\auxin_A,\initfnA,\delta_A,T),$ has the added capability of
overwriting the messages sent by players in the coalition it has corrupted.
We thus extend its transition function to allow it to generate malicious
messages:
\[
\delta_A : Q_A \times \playervs 
\rightarrow \dist(Q_A \times H).
\]

As before, a Byzantine adversary is static if $T$ is a constant function
and dynamic if $T$ depends on the state.  A Byzantine $t$-adversary is
allowed the fault class $\sct = \set{T \mid \abs{T} \leq t}.$

The most severe sort of Byzantine adversary can {\em rush} messages,
meaning it receives the messages sent from reliable players before other
messages are delivered, allowing it to choose a larger coalition to corrupt
and to choose new messages depending on the good messages it has seen.
Rather than consider an assortment of transition functions, one of which is
used to generate new adversarial messages and others which determine new
choices of coalitions after seeing rushed messages, we simply apply the
same transition function $\delta_A$ after each set of rushed messages is
received, allowing the adversary to change its state and select new players
to corrupt.  Formally, the messages generated by the transition function
are ignored, until the point at which the adversary stops enlarging the
coalition it has chosen to corrupt.  At that point, whatever messages the
adversary generated are delivered to the appropriate recipients {\em via
the channels from the corrupted players}, and the still-unsent messages
between reliable players are also delivered.

The steps involved in an execution of the protocol with a rushing,
Byzantine adversary on inputs $\vec{x},$ auxiliary inputs $\vec{a},$ and
adversary auxiliary input $a_A$ are shown in Figure~\ref{fig-exec-byz}.
For clarity of proofs, we sometimes regard the {\bf Repeat} step
(2.1.2) as a {\bf For} loop that is repeated $t$ times; the adversary can
increase the coalition no more than $t$ times, of course.  The state of
player $i$ or the adversary at round $r$ is referred to as $q_i^r$ or as
$q_A^R,$ respectively.  If we wish to dissect the execution even further,
examining the states within the {\bf Repeat} loop, we refer to the
$\rho^{th}$ repetition of the repeat loop using the notation $(r,\rho).$
Hence we may speak of $q_A^{(r,\rho)}$ or of $q_A^r = q_A^{(r,0)}.$


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Figure:  Byzantine Execution
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\figstretch
\boxfig{
\noindent{\bf \protostyle Byzantine Execution}
\index{execution!Byzantine}
\index{Byzantine}
\begin{tabbing} \standtabs
%
% INITIALIZE STATES
%
(B1.1) \> {\For $i=1..n$ \Do} \\
\> \>
$q_i  \leftarrow  \initfni(x_i,a_i,k)$ \\
(B1.2) \> Set \\
\> \>
$q_A  \leftarrow  \initfnA(a_A,n,m,k)$ \\
\> \>
$T \leftarrow T(q_A)$ \\
\> \>
$T_{old} \leftarrow \emptyset$ \\
\> \>
$\mess([n],[n],0) \leftarrow \emptyset$ \\
\\
%
% RUN THE PROTOCOL FOR R ROUNDS
%
(B2.1) \>
{\For $r=1..R$ \Do} \\
%
% GENERATE RELIABLE MESSAGES
%
(B2.1.1) \>\>
{\For $i \in \tbar$ \Do}
\>\>\>\ccomment{nonfaulty messages}
 \\
\> \> \>
$(q_i,\mess^{\out}(i,[n],r)) \leftarrow
\delta_i(q_i,\mess([n],i,r-1))$
\\
(B2.1.2) \>\> 
{\Repeat} 
\>\>\>\ccomment{rush messages; new corruption} \\
%
% RUSH MESSAGES AND LET ADVERSARY COMPUTE
%
\>\>\>
$T_{new} \leftarrow T - T_{old}$ \\
\>\>\>
$T_{old} \leftarrow T$ \\
% SEND MORE RUSHED MESSAGES
\>\>\>
$\mess(\tbar,T_{new},r) \leftarrow
\send( \mess^{\out}(\tbar,T_{new},r),
\scc_1 \cup \cdots \cup \scc_n)$ \\
% ADVERSARY COMPUTES
\>\>\>\ccomment{adversary computes, but messages aren't}\\
\>\>\>\ccomment{actually sent until rushing is done}\\
\>\>\>
$(q_A,\mess(T,\tbar,r))
 \leftarrow \delta_A(q_A, \mess(\tbar,T_{new},r) )$ \\
\>\>\>
$T \leftarrow T(q_A)$ \\
\>\> 
{\Until} $T_{new} = \emptyset.$
\>\>\>\ccomment{until no new corruptions}\\
\\
%
% FINISHED RUSHING; SEND MESSAGES
%
(B2.1.3) \>\> 
Set  
\>\>\>\ccomment{send all pending messages} \\
\>\>\>
$\mess(T,\tbar,r) ) \leftarrow
\send( \mess^{\out}(T,\tbar,r).$ \\
\>\>\>
$\mess(\tbar,\tbar,r) ) \leftarrow
\send( \mess^{\out}(\tbar,\tbar,r).$ \\
\\
%
% FINAL COMPUTATION
%
(B3.1) \> {\For $i \in \tbar$ \Do} 
\>\>\>\>\ccomment{final computation}\\
\>\>
$q_i^f \leftarrow \delta_i(q_i, \mess([n],i,R) )$ \\
\>\>
$q_A^f \leftarrow \delta_A(q_A, \mess([n],T,R) )$
\end{tabbing}
\caption{\label{fig-exec-byz}
Execution of protocol $\protoAPi$%
\index{$<A,\protoname>,$ execution of} 
with a message-rushing Byzantine adversary.  
}}
\figstretchend


We shall have reason to speak not simply of the specific states and messages
occurring during the protocol but of the distributions on those states.%
\index{state distributions}%
\index{$\rvnames$} 
Let 
\begin{eqnarray*}
\rvnames & = & \{ x_1,\ldots,x_n,a_1,\ldots,a_n,a_A,q_1,\ldots,q_n,q_A,\\
& & 
\mess^{\out}(1,1),\ldots,\mess^{\out}(n,n),
\mess(1,1),\ldots,\mess(n,n), \\
& &
y_1,\ldots,y_n,y_A
\} .
\end{eqnarray*}
(Semantically, this is a set of ``labels'' for random variables.)
%be a set of tags (in a slight abuse of notation, ``$q_1$'' is not a state
%in $Q_1$ but a {\em label} to be used to parametrize distributions).  
The distribution on, say, the state $q_i^r$ at round $r$ will then be
described by $\rv(q_i,r).$ In general, the distribution on the state or
message $v \in \rvnames$ at round $r$ is described by $\rv(v,r).$ Each
distribution $\rv(v,r)$ is a probabilistic function of the results of
earlier samples as specified by Figure~\ref{fig-exec-byz}.  For example,
$\rv(q_i,r)$ is a probabilistic function (namely, the transition function
$\delta_i$) of $\rv(q_i,r-1),\rv(\mess(1,i),r-1), \rv(\mess(2,i),r-1),
\ldots,\rv(\mess(n,i),r-1).$ Or, for example, the variable $\rv(\mess(1,1),r)$
is in fact a probabilistic function (namely, the channel function)
$\rv(\mess^{\out}(1,1),r).$ The ``results'' or ``outputs'' of a distributed
computation are described by 
$Y_1=\rv(y_1,R),\ldots,Y_n=\rv(y_n,R),Y_A=\rv(y_A,R).$
Without loss of generality, the random variable $\rv(y_A,R)$ is 
``completely dependent''
on the variables $\rv(q_A,r)$ and $\rv(\mess(i,j),r)$ for $i,j \in
T_{\rv(q_A,R)}$ and $1 \leq r \leq R,$
in the sense that the output of the adversary specifies
every state and message it has seen.

Thus, the execution of a protocol is simply a sample taken from a set of
interdependent random variables $\rv(v,r).$ The text of this chapter shows
how to generate this joint distribution by sampling probabilistic functions
in a specified order.  Our proofs will 
fundamentally show that two probabilistic
functions are the same, where each is defined by a different sequence
of application of probabilistic functions.



\section{Outputs and Output Distributions}
\label{sec-outputs}

At the end of a general protocol the adversary and each player writes an
output string $Y_A=\outfn_A(q_A^f)$ or $Y_i=\outfn_i(q_i^f)$ (respectively)
on an output tape.  A corrupted player's tape contains $\Lambda.$

Let adversary $A$ have auxiliary input $a.$ An execution of a protocol
$\Pi(n,m)$ on inputs $\vec{x}=(x_1,\ldots,x_n),$ auxiliary inputs
$\vec{a}=(a_1,\ldots,a_n),$ and security parameter $k$ induces a {\em
distribution} on $(\sigstar)^{2n+2},$ that is, on the outputs and views
of $A$ and of the players.  The distribution is denoted:
\[
\realhist(n,m)\protoIn = 
(Y_A,Y_1,Y_2,\ldots,Y_n,\view_A,\view_1,\view_2,\ldots,\view_n).
\index{$\realpf(n,m)\protoIn$!distribution on executions}%
\index{distribution!protocol induced}
\] 
For fixed $n$ and $m,$ parametrizing over $z=\vec{x} \circ \vec{a} \circ a$
and security parameter $k$ represents an ensemble,%
\index{ensemble!protocol induced}
$\realhist(n,m).$ 
A universal protocol that computes a particular function
$F$ may include a circuit description $C_F$ in the $z$ parameter.  
For readability, we occasionally write $\realpf\protoIn$ when
$n$ and $m$ are understood in the context.
The family of ensembles when $n$ and $m$ vary is written
$\realhist=\set{\realhist(n,m)}_{n,m\in\natsmall},$ 
and is induced by the family of protocols 
$\realpf=\set{\realpf(n,m)}_{n,m\in\natsmall}.$  


When analyzed separately, the issues of privacy and correctness examine the
views apart from the outputs. We denote the output (which, without loss of
generality, includes the view) of the adversary generated in a protocol by:
\[
\realya\protoIn
= Y_A.
\]
We use a similar notation for the outputs of the players:
\[
\realyp\protoIn
= (Y_1,\ldots,Y_n).
\]
Privacy concerns $\realya,$ whereas correctness concerns $\realyp.$ The
ensemble specifying the view of the adversary and the outputs of the
players (not their views) is:
\[
\realy\protoIn
= (Y_A,Y_1,\ldots,Y_n).
\]
%Our definition for {\em resilience} (\S\ref{sec-sim-correct}) concerns
%$\realy,$ capturing privacy and correctness simultaneously.
We shall see it is advantageous to consider $\realy$ as a whole, not to
break it down into components describing privacy and correctness.




\section{The Function to Compute}
\label{sec-function}

For full generality, we wish to consider families of probabilistic
functions mapping strings to strings (equivalently, integers to integers,
encoded in a natural fashion).
Let $F=\set{F^{n,m}}_{n,m\in\natsmall}$  be a family of probabilistic functions
with $n$ inputs of length $m$ and $n$ outputs of length $m:$
\[
F^{n,m} : X_1 \times X_2 \times \cdots \times X_n \rightarrow
Y_1 \times Y_2 \times \cdots \times Y_n 
\]
where each $X_i,Y_i \subseteq \set{0,1}^m.$

Computing probabilistic functions allows us to accomplish
a wide range of tasks.  It is often the case that
a given set of inputs is not mapped in a 1-1 manner to a set of outputs
and thus is not described by a function {\em per se.}  A coin toss, useful
for tasks such as leader election and symmetry breaking, is a primary
example.

Lest our analysis become too complicated, however, we consider distributions
described by probabilistic circuits, namely distributions induced by
setting certain bits of a Boolean circuit uniformly at random.  This
covers all probabilistic Turing machine computations and is a natural
case to consider.

Let $\scf^{det,poly}$ be the set of all deterministic function families
$\hat{F}=\set{\hat{F}^{n,m}}_{n,m \in \natsmall}$ satisfying
\[
\hat{F}^{n,m} : \set{0,1}^{nm+\rho(n,m)} \rightarrow \set{0,1}^{nm}
\]
where $\rho(n,m)=O((nm)^c)$ for some $c.$  Each $F^{n,m}$
can be described as a circuit with $nm$ inputs and
a polynomial number of supplementary inputs, and $nm$ outputs
(or, if one prefers, as $nm$ such circuits each having a one-bit
output).

Let $\scf$%
\index{$\scf,$ probabilistic function}%
\index{function!to compute}
be the set of all probabilistic function families $F=\set{F^{n,m}}$
such that there exists an $\hat{F} \in \scf^{det,poly}$
satisfying
\[
F^{n,m}(\vec{x}) =
\set{ \vec{r} \leftarrow \uniform(\set{0,1}^{\rho(n,m)}) :
\hat{F}^{n,m}(\vec{x},\vec{r})}
\]
Denote the restriction of $F$ to its $i^{th}$ output bit
by $F_i(x_1,\dots,x_n).$ 

A protocol for $F \in \scf$ should compute a vector $(y_1,y_2,\dots,y_n)$
selected according to the distribution $F(x_1,x_2,\dots,x_n),$ and should
provide player $i$ with the correct value $y_i.$ 

We make two simplifying observations based on the ability of each player to
generate uniformly random bits.  First of all, we may restrict our attention
to deterministic functions by arranging that each player $i$ supply, 
as part of its input, a uniformly random sequence of $\rho(n,m)$ bits,
$\vec{r}_i=(r_{i1},\ldots,r_{i,\rho(n,m)}).$  It is easy to see that
as long as one player supplies uniformly random bits, it suffices
to compute the deterministic function 
$\check{F}((x_1,\vec{r}_1),\ldots,(x_n,\vec{r}_n))$ defined as
$\hat{F}(x_1,\ldots,x_n,R_1,\ldots,R_{\rho(n,m)})$ where
$R_j = r_{1j} \oplus r_{2j} \oplus \cdots \oplus r_{nj}.$

Secondly, it suffices to consider
functions whose single result is revealed in its entirety to all players.
Observe that if each player provides a mask, namely a sequence of random
bits $r_i,$ it suffices to compute $(y_1 \oplus r_1,\dots,y_n
\oplus r_n)$ and reveal the entire vector to all players.  Unless the
adversary specifically corrupts a given player $i,$ it gains no
information about the result $y_i$ from the publicized value 
$y_i \oplus r_i$.

Thus, without loss of generality
our protocol descriptions consider each $F$ to be
a family of deterministic functions, with one $m$-bit output
or $n$ different $m$-bit outputs as convenient.  A general protocol
compiler for families in $\scf^{det,poly}$ is also one for
$\scf.$



==> pri.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% pri.tex                      Privacy for Passive Adversaries
%
%                            Copyright @1989  Donald Beaver.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{=======}
\typeout{pri.tex}
\typeout{=======}

\chapter{Privacy for Passive Adversaries}         \label{chap-pri}

\chapquote{
``Notice all the computations, theoretical scribblings, and lab
equipment, Norm....  Yes, curiosity killed these cats.''
}{
Gary Larson}
% p 242, the PreHistory of the Far Side


Multiparty computations are generally impossible when the number of
faulty players exceeds half the network, unless additional assumptions
are made.  Chapter~\ref{chap-maj} describes how noisy channels allow
computations to proceed correctly and fairly, and
demonstrates how to achieve the same results using a cryptographic
protocol for oblivious transfer.

In order to elucidate the nature of privacy in distributed computations, we
examine protocols which tolerate very large numbers of passive faults.  We
call this the ``honest-but-curious'' model: each player is honest and never
sends a faulty message, but players may form coalitions and pool their
knowledge to try to obtain extra information to which they are not
entitled.  We may more or less ignore the issues of correctness and
fault-tolerance, focusing only on privacy.

When the bound $t$ on the number of curious parties satisfies 
$t <\lceil \frac{n}{2} \rceil,$ any function can be computed privately
in the ``honest-but-curious'' model ({\em cf.} \cite{bgw88,ccd88} and
Chapters \ref{chap-con} and \ref{chap-min}).

When $t \geq\lceil \frac{n}{2} \rceil,$ the class of privately computable
functions is restricted.  Chor and Kushilevitz \cite{ck89} characterized
the set of {\em boolean} functions that can be computed privately for $t
\geq\lceil \frac{n}{2} \rceil$ as those of the form
\[
f(x_1,x_2,\dots,x_n) = f_1(x_1) \oplus f_2(x_2) \oplus \cdots
f_n(x_n).
\]
In other words, for the boolean case, the only functions privately
computable when a majority of the parties are curious are exclusive-or's of
$n$ functions, each depending on one input.

The results of \cite{yao86,gmw87,ghy87,bg89} demonstrate that when the
participants are computationally bounded but still only curious, {\em any}
function can be privately computed for $t \leq n-1.$ Furthermore, even
functions that have non-boolean outputs are privately computable.  In an
information-theoretic sense, however, coalitions of curious parties do hold
more information than that to which they are entitled.

The complete characterization of privately computable functions when the
participants are not bounded remains an open question: 

\begin{quote}
What {\em general} functions (say from $n$ inputs to $n$-bit outputs) 
can be computed privately by $n$ parties, allowing 
$t \geq\lceil \frac{n}{2} \rceil,$ and maintaining privacy in an 
{\em information-theoretic} sense?  
\end{quote}

In this chapter, we take the penultimate step toward a complete 
characterization, by solving the following problem:
\begin{quote}
What {\em general} functions 
can be computed privately by {\em two} parties?
\end{quote}
We give a characterization of functions that are privately computable by
two parties, based on a simple property of the table for the functions.
Specifically, any function whose table can be {\em partitioned} in a
certain manner can be privately computed by two parties; and any function
that can be privately computed by two parties has a table which can be
partitioned.  (See \S\ref{sec-main} for a statement of the main theorem.)

In preliminary papers, Kushilevitz \cite{k89} and Beaver \cite{bea89-priv}
independently obtained this characterization, but the proofs appearing in
those papers contain a subtle flaw.  We present here a different proof,
which uses a different approach (see \S\ref{sec-cannot}).

Our characterization bears on the $n$-party problem in that any $n$-party
protocol that allows $t\geq\lceil \frac{n}{2} \rceil$ can be adapted to a
two-party protocol.  Thus, functions that are privately computable in the
$n$-party case must satisfy certain properties satisfied by functions that
are private in the two-party case.

We also address a different version of the $n$-party problem, in which the
output of the function is not revealed.  Instead, it is maintained in a
distributed form, using an arbitrary threshold scheme. In view of the
recent development of multiparty computation protocols based on threshold
schemes (cf. \cite{bgw88,ccd88}), as well as the protocols described in the
rest of this dissertation, all of which allow the output to be maintained
in a shared form, a characterization of the functions that can be computed
secretly is needed.  We show a strongly negative result: the only functions
that can be computed secretly, maintaining the result as a secret (for use
in further protocols), are additive functions.  This result fits neatly
with that of \cite{ck89} showing that privately computable boolean
functions are addition functions ($\mod 2$).

{\bf Assumptions made in this chapter.}  The network is complete,
with private lines, $2$ or $n$ computationally
unbounded processors.
Protocols are perfectly resilient against passive $t$-adversaries
where $t$ may be greater than $\frac{n}{2}.$



\section{Definitions}

For the two-party case, we assume that the two parties communicate
using finite strings and for a finite number of exchanges.  Neither
party is computationally bounded; the privacy of the protocols is
based on information-theoretic bounds.
Because we consider only two parties, without an active adversary,
we can make some simplifying observations.

A party can be described simply by a family of distributions on strings,
parametrized by the input and the current transcript of the protocol.
These distributions are induced by the formal transition functions,
to which we shall not refer again.
Thus, party 1 is a family of distributions 
$\set{D^1_{x,t} \mid  x\in X, t \in \Sigma^{\star}},$
where $\Sigma=\set{0,1},$ and each $D^1_{x,t}$ is a distribution
on $\Sigma^{\star}.$  The message that party 1 sends after
round $r$ is a finite string selected at random according to distribution
$D^1_{x,t_r},$ where $x$ is its input and $t_r$ is the transcript
of messages through round $r.$  Party 2 is defined similarly.
We assume that the transcripts are delimited so that the messages
are uniquely decodable from the transcripts.

Let the domain of $f$ be $X \times Y =
\set{1,\dots,\alpha} \times \set{1,\dots,\beta}.$
Let $T$ be a random variable which describes the transcript of
message exchanges between parties 1 and 2.
We say that $f$ is {\em private} if there is a protocol
such that, when party 1 holds $x \in X$ and party 2 holds $y \in Y:$
\begin{itemize}
\item
After any run of the protocol, each party knows $f(x,y).$
\item
{\bf (Privacy for party 1)}
\index{private function}
For any $x'$ such that $f(x',y)=f(x,y)$ and for any transcript $t:$
\[
\prob{ t \mid x', y} = \prob{ t \mid x, y }.
\]
\item
{\bf (Privacy for party 2)}
For any $y'$ such that $f(x,y')=f(x,y)$ and for any transcript $t:$
\[
\prob{ t \mid x, y'} = \prob{ t \mid x, y }.
\]
\end{itemize}

We shall also denote the prefix of a transcript $t$ after the $i^{th}$
round by $t_i,$ and the corresponding random variable by $T_i.$


\section{Two Party Privacy for Passive Adversaries}


\subsection{Partitions}

For any $x \in X$ and any subset $P \subseteq Y,$
we define the {\em row set} for row $x$ and columns in $P$ to be
the range of values that $f$ takes 
over that row of its table:
\[
R(x,P) = \set{ f(x,y) \mid y \in P}.
\]
Similarly, we define the {\em column set} for
$y \in Y$ and a subset of values $P \subseteq X:$
\[
C(P,y) = \set{ f(x,y) \mid x \in P}.
\]

We say that $f$ is {\em column-partitionable} into $f_P$ and $f_Q$ if
if there exists a nontrivial partition of $Y$ into blocks $P$ and $Q$
such that
\[
(\forall x \in X) R(x,P) \hspace{0.1in} \cap R(x,Q) = \emptyset,
\]
and $f_P$ and $f_Q$ are the restriction of $f$ to the sets $P$ and $Q.$
In other words, if we look at a particular row in the table for $f$
and consider the range of values which $f$ takes on
for $y \in P,$ then no such value will appear
as the output of $f$ for $y \in Q.$
Similarly, $f$ is {\em row-partitionable} 
if there exists a nontrivial partition of $X$ into blocks $P$ and $Q$
such that
\[
(\forall y \in Y) R(P,y) \hspace{0.1in} \cap R(Q,y) = \emptyset,
\]
and $f_P$ and $f_Q$ are the restriction of $f$ to the sets $P$ and $Q.$

Partitionability is recursively defined as follows.
We say that $f$ is {\em partitionable} if:
\begin{enumerate}
\item
$f$ is constant; or
\item
$f$ is column-partitionable or row-partitionable
into $f_P$ and $f_Q,$ each of which are themselves partitionable.
\end{enumerate}

For example, the AND function is not partitionable,
while the function $f(x,y) = x + y \mod 7$ is partitionable.
Functions that are not partitionable need not be based on AND
or OR, as demonstrated by the following table, which cannot
be partitioned by rows or by columns:

\setlength{\unitlength}{1pt}
\begin{picture}( 400, 100)
%\put( 107.1, 408.1){\framebox(  37.9,  17.7){}}
%\put( 107.1, 390.4){\framebox(  20.2,  17.7){}}
%\put( 127.3, 390.4){\framebox(  17.7,  17.7){}}
%\put( 127.3, 390.4){\framebox(  17.7,  17.7){}}
\put( 187.2,  58.1){\framebox(  35.4,  17.7){}}
\put( 223.4,  40.4){\framebox(  17.7,  35.4){}}
\put( 205.7,  22.7){\framebox(  35.4,  17.7){}}
\put( 187.2,  22.7){\framebox(  17.7,  35.4){}}
\small\tt
%\put( 114.0, 415.3){A}
%\put( 134.2, 415.3){A}
%\put( 115.7, 395.9){B}
%\put( 135.9, 395.9){B}
\put( 160.1,  81.6){$f(x,y)$}
\put( 194.1,  81.6){0}
\put( 212.6,  81.6){1}
\put( 231.2,  81.6){2}
\put( 194.1,  63.6){0}
\put( 212.6,  63.6){0}
\put( 231.2,  63.6){1}
\put( 231.2,  45.9){1}
\put( 231.2,  28.2){2}
\put( 212.6,  28.2){2}
\put( 212.6,  45.9){4}
\put( 194.1,  45.9){3}
\put( 194.1,  28.2){3}
\put( 176.1,  63.6){0}
\put( 176.1,  45.9){1}
\put( 176.1,  28.2){2}
\end{picture}

It is easy to see that any function that is insensitive to
$x$ or to $y$ is partitionable.

It is also straightforward to determine from an $n \times n$ table
for $f$ whether $f$ is partitionable, by using a transitive-closure algorithm,
which runs in time polynomial in $n$, to determine the columns
or rows that must fall in the same blocks of any allowable partition.

\subsection{Two Parties Cannot Compute Unpartitionable Functions}
\label{sec-cannot}

We show the following result:
\begin{lemma}     \label{lem-two-a}
If $f$ is not partitionable,
then $f$ cannot be computed privately
by two parties.
\end{lemma}

Before proceeding to the proof, let us expose the flaw in the earlier proofs
of Kushilevitz \cite{k89} and Beaver \cite{bea89-priv}.

Without loss of generality,
let party 1 send messages $m_r$ to party 2 during odd-numbered rounds $r;$
let party 2 send messages during even-numbered rounds.
This does not restrict who ``speaks'' first, since null 
or completely random messages are allowed.
We expand the probability of a transcript $t$ given $x$ and $y$
according to its prefixes $t_1,t_2,\dots,$
where $t_i = m_1 \circ m_2 \circ \cdots \circ m_i:$
\begin{eqnarray*}
\prob{t \mid x,y} & = &
\prod_r \prob{t_r \mid x,y,t_{r-1}}  \\
& = &
(\prod_{j}
\prob{t_{2j+1} \mid x,y,t_{2j}} ) 
(\prod_{j}
\prob{t_{2j} \mid x,y,t_{2j-1}} ) \\
& = & P_1(t,x) P_2(t,y)
\end{eqnarray*}
where $P_1$ and $P_2$ are defined as the parenthesized expressions.
(This notation appears literally as 
{$P_1(s~\mid~x), P_2(s~\mid~y)$} in \cite{k89},
and as $\gamma_t(x),\delta_t(y)$ in \cite{bea89-priv}.)

The faulty proof appearing in \cite{k89,bea89-priv} runs along the
following lines.  Using the privacy of $f,$ it is shown 
by induction that $\prob{t \mid x,y}$ is constant over all $x.$
The induction step fails, however, since it is based on the following
statement, which intends to show that $P_1$ is insensitive to $x:$
If $\prob{t \mid x_1,y} = \prob{t \mid x_2,y}$ then 
$P_1(t,x_1) = P_1(t,x_2).$  Unfortunately, if $P_2(t,y) = 0,$
this conclusion does not necessarily hold.  

For example, consider the function described by 
\begin{center}
\begin{tabular}{rcc}
$f(x,y)$ & $y_1$ & $y_2$ 
\\ \cline{2-3}
\multicolumn{1}{r|}{$x_1$} &
\multicolumn{1}{c|}{1} &
\multicolumn{1}{r|}{2}
\\ \cline{2-3}
\multicolumn{1}{r|}{$x_2$} &
\multicolumn{1}{c|}{1} &
\multicolumn{1}{r|}{3}
\\ \cline{2-3}
\end{tabular}
\end{center}
and the 4-round deterministic protocol where party 1 starts, and each party
sends 1 bit, described by the table of transcripts:
\begin{center}
\begin{tabular}{rcc}
 & $y_1$ & $y_2$ 
\\ \cline{2-3}
\multicolumn{1}{r|}{$x_1$} &
\multicolumn{1}{c|}{0000} &
\multicolumn{1}{r|}{0100}
\\ \cline{2-3}
\multicolumn{1}{r|}{$x_2$} &
\multicolumn{1}{c|}{0000} &
\multicolumn{1}{r|}{0110}
\\ \cline{2-3}
\end{tabular}
\end{center}
%
%% \begin{center}
%% \begin{tabular}{r|cc|cc|c}
%% \multicolumn{2}{r}{$t$} & \multicolumn{2}{c}{$y_1$} &
%% \multicolumn{2}{c}{$y_2$} 
%% \\ \cline{3-6}
%% $x_1$ & & 0000 & & 0100 & 
%% \\ \cline{5-6}
%% $x_2$ & & 0000 & & 0110 & 
%% \\ \cline{2-6}
%% \end{tabular}
%% \end{center}
%
Then $\prob{0000 \mid x_1,y_1} = P_1(0000,x_1) P_2(0000,y_1)
= \prob{0000 \mid x_2,y_1} = P_1(0000,x_2) P_2(0000,y_1),$
and we have $P_2(0000,y_1) = 1$ and $P_1(0000,x_1)=P_1(0000,x_2) = 1.$
The claim that $P_1$ is insensitive to $x$
is satisfied for this particular transcript.
On the other hand, 
$\prob{0100 \mid x_1,y_1} = \prob{0100 \mid x_2,y_1} = 0,$
but $P_1(0100,x_1)=1$ while $P_1(0100,x_2) = 0.$
Informally, transcript $0100$ is impossible given $y_1,$
but it may or may not be possible for different $x,$
a fact that cannot be determined simply by looking at the
column corresponding to $y_1.$  The claim that $P_1$ is insensitive
to $x$ fails.

It turns out that $P_1$ is indeed insensitive to $x$ when $f$ cannot be
partitioned into columns, but this is not a trivial observation, and the
proof must use the unpartitionability of $f$ by columns.  The earlier
proofs did not use this property, and thereby fail on a counterexample like the
one presented above (note that $f$ is not partitionable by rows,
but it is partitionable by columns).  Introducing the property of
unpartitionability by columns into the earlier proof techniques 
seems to be an unwieldy approach, without an easy fix;
instead, we present an alternative proof.

\medskip


\noindent {\bf Proof of Lemma~\ref{lem-two-a}:}
Since $t_{2j+1} = t_{2j} \circ m_{2j+1},$ and $m_{2j+1}$
is selected by party 1 according to distribution
$D^1_{x,t_{2j}},$ we may write:
\[
\prob{t_{2j+1} \mid x,y} = 
\prob{ t_{2j+1} \mid x,t_{2j} }
\prob{ t_{2j} \mid x,y }.
\]
Similarly,
\[
\prob{t_{2j} \mid x,y} = 
\prob{ t_{2j} \mid y,t_{2j-1} }
\prob{ t_{2j-1} \mid x,y }.
\]

First we shall show that if $f$ is privately computable but
not partitionable, then party 1 ``never speaks first.''  In other
words, all conversations are independent of $x$ until party 2 gives
away some information depending on $y.$  Then we shall show that party
2 never speaks first, leading to a contradiction.

In order to formalize the notion of not speaking first, consider the
following notations.
Let $D \subseteq X \times Y,$ 
and let $\tau(x,y)=\set{t \mid \prob{t \mid x,y} \not= 0}.$
Given a transcript $t$ and two pairs of inputs $(x,y)$ and $(u,v),$
let $\theta(t,x,y,u,v)$ be the value $r$ such that
\[
\prob{t_r \mid x,y} \not= \prob{t_r \mid u,v} \mbox{ and }
(\forall \rho < r) 
\prob{t_{\rho} \mid x,y} = \prob{t_{\rho} \mid u,v}.
\]
Clearly, such an $r$ is unique if it exists.  If no such $r$ exists,
let $\theta(t,x,y,u,v) = \infty.$
The earliest round at which the probabilities of conversations on
$(x,y)$ differ from those for {\em some} other input $(u,v)$ is denoted
\[
\phi(t,D,x,y) =
\mbox{min}_{(u,v) \in D} \hspace{0.2in} \theta(t,x,y,u,v).
\]
Now let
\[
\psi(D) = \set{ \phi(t,D,x,y) \mid (x,y) \in D, t \in \tau(x,y)}.
\]
We say that party 1 {\em does not speak first on $D$} if 
$\psi(D) \subset \set{2j \mid j \in \mbox{\bf N}} \cup \set{\infty},$
that is, if the earliest times at which conversations differ are always
even-numbered rounds, corresponding to party 2 sending a message to
party 1.

First, let us show an easy lemma:
\begin{lemma}
\label{lem-row}
(Row Lemma)
For any $x\in X$ and $y_1,y_2 \in Y,$ and for any possible transcript
$t \in \tau(x,y_1),$ if 
\[
\prob{t_r \mid x,y_1} \not= \prob{t_r \mid x,y_2} \mbox{ and }
(\forall \rho < r) 
\prob{t_{\rho} \mid x,y_1} = \prob{t_{\rho} \mid x,y_2},
\]
then $r$ is not odd.
\end{lemma}

\noindent{\bf Proof:}
If $r$ is odd, party 1 sends the message at round $r:$
\begin{eqnarray*}
\prob{t_r \mid x,y_1} 
& = & \prob{t_r \mid x, t_{r-1} } \prob{t_{r-1} \mid x,y_1} \\
& = & \prob{t_r \mid x, t_{r-1} } \prob{t_{r-1} \mid x,y_2} \\
& = & 
\prob{t_r \mid x,y_2} 
\end{eqnarray*}
which is a contradiction.
$\Box$

The crucial lemma we need is the following:

\begin{lemma}
\label{lem-speakfirst}
If $f$ is privately computable but not partitionable, then
party 1 does not speak first on $X \times Y.$
\end{lemma}

\noindent{\bf Proof:}
We show by induction that there exist
$P_1 \subset P_2 \subset \cdots \subset P_{\abs{X}} = X$
such that party 2 speaks first on each $P_i \times Y.$


Using lemma~\ref{lem-row}, we see that party 1 does not speak first on 
$P_1 \times Y,$ where $P_1 = \set{a_1}$ and $a_1 \in X$ is arbitrary.
Since party 1 only has one argument in $P_1,$ this is intuitively
clear.

Assume by way of induction that party 1 does not speak first on $P_i \times Y.$
We must demonstrate a $P_{i+1}$ such that $P_i \subset P_{i+1}$
and party 1 does not speak first on $P_{i+1}.$

Since $f$ is not partitionable, there exist values
$x_1 \in P_i, x_2 \in \overline{P}_i,$ and $y_1 \in Y$ so that
$f(x_1,y_1) = f(x_2,y_1).$  Let $P_{i+1} = P_i \cup \set{x_2}.$
To show that party 2 speaks first on $P_{i+1} \times Y,$
it suffices to show that for each $y \in Y,$ 
$\phi(t,\set{x_2} \times Y, x_2, y)$ is never odd and
$\phi(t,P_i \times Y, x_2, y)$ is never odd.  In other words,
we consider the earliest times that a meaningful message is sent for
the new inputs in $\set{x_2} \times Y$ relative to the original set
$P_i \times Y$ and relative to the new input set itself.

Lemma~\ref{lem-row} shows that 
$\phi(t,\set{x_2} \times Y, x_2, y)$ is never odd.

To obtain the claim that $\phi(t,P_i\times Y,x_2,y)$ is never odd,
let us divide the row $\set{x_2} \times Y$ into three sets,
$A = \set{(x_2,y_1)},$
$B = \set{(x_2,y) \mid (\exists a \in P_i) f(a,y) = f(x_2,y)}\backslash A,$
and
$C = \set{(x_2,y) \mid (\forall a \in P_i) f(a,y) \not= f(x_2,y)}.$

First, we show that $\phi(t,P_i \times Y, x_2,y_1)$ is even for
any possible transcript $t \in \tau(x_2,y_1).$  If $t \in
\tau(x_2,y_1)$ then by the privacy of $f,$
\[
(\forall r) 
\prob{t_r \mid x_1,y_1} = \prob{t_r \mid x_2,y_1}
\]
Then it follows easily that 
$\phi(t,P_i \times Y, x_2,y_1) = \phi(t,P_i \times Y, x_1,y_1),$
and our first claim follows.

By a similar argument, $\phi(t, P_i \times Y, x_2, y)$ is never odd
for any $y \in B$.

Thirdly, for any $(x_2,y) \in C,$ we show $\phi(t,P_i \times Y, x_2, y)$
is never odd.  We have two cases to consider: $\theta(t,x_2,y,x_1,y_1)$
is minimal or it is not.  Say it is minimal.  Again, by the privacy of
$f$ we have that
\[
(\forall r) 
\prob{t_r \mid x_1,y_1} = \prob{t_r \mid x_2,y_1}
\]
and the smallest $r$ at which 
$\prob{t_r \mid x_1,y_1} \not= \prob{t_r \mid x_2,y}$
is identical to that for which 
$\prob{t_r \mid x_2,y_1} \not= \prob{t_r \mid x_2,y}.$
Since $(x_2,y_1)$ and $(x_2,y)$ are in the same row,
$r$ must be even.

If $\theta(t,x_2,y,x_1,y_1)$ is not minimal, let
$(u,v)$ be such that
$\theta(t,x_2,y,u,v)$ is minimal.
For a given transcript $t,$ consider the probabilities
$\prob{t_r \mid u,v},$
$\prob{t_r \mid x_1,y_1},$
and $\prob{t_r \mid x_2,y}.$
At some earliest round $r,$ two or three of these differ.
Since $(u,v)$ gave the minimal value with respect to $(x_2,y)$
we see that $\prob{t_r \mid x_2,y} \not= \prob{t_r \mid u,v}.$
Since $(x_1,y_1)$ did not give the minimal value,
$\prob{t_r \mid x_2,y} = \prob{t_r \mid x_1,y_1}.$
Therefore 
$\prob{t_r \mid x_1,y_1} \not= \prob{t_r \mid u,v}.$
By the induction hypothesis, since $(x_1,y_1)$ and $(u,v)$
are in $P_i \times Y,$ we deduce $r$ is even.  $\Box$

A symmetric argument gives the corresponding lemma:
\begin{lemma}
\label{lem-speakf}
If $f$ is privately computable but not partitionable, then
party 2 does not speak first on $X \times Y.$
\end{lemma}

Combining lemmas \ref{lem-speakfirst} and \ref{lem-speakf},
we see that neither party speaks first on $X \times Y,$ implying that
$\psi(X \times Y) = \set{\infty}.$
Let $a \in X$ and $b \in Y$
be arbitrary, and let $t \in \tau(a,b).$  Then for every $x \in X$ and
$y \in Y,$ we have
$\theta(t,a,b,x,y) = \infty,$
implying $\prob{t \mid a,b} = \prob{t \mid x,y}.$  
Since $f(x,y)$ is determined by the transcript $t,$ $f$ must
be constant and hence partitionable, giving a contradiction.
$\Box$

\smallskip

\noindent{\bf Remarks:}
The proof of lemma~\ref{lem-two-a}
does not assume that the protocol is deterministic.
In the next section we observe that a deterministic protocol suffices
to compute any partitionable function.  Furthermore, even if the
protocol is only correct with probability exceeding $\half,$
the argument shows that the distributions on transcripts 
are identical regardless of the inputs, so that $f$ must be constant,
giving a contradiction.



\subsection{Two Parties Can Compute Partitionable Functions}

We now show a converse result:
\begin{lemma}     \label{lem-two-b}
If $f$ is partitionable, then there is a 
(deterministic) protocol whereby $f$ can
be computed privately by two parties.
\end{lemma}

\noindent {\bf Proof:}  
By induction on $\alpha = \abs{X}.$

\noindent{\bf (Base Case.)}
If $X=\set{x_1},$ then party 2 simply announces $f(x_1,y).$
This protocol is trivially private for party 1, and
since for all $y,y' \in Y$ such that $f(x_1,y)=f(x_1,y')$
the transcript consists exactly of $f(x_1,y),$ the protocol
is private for party 2.

\noindent{\bf (Inductive Hypothesis.)}
If $\abs{X} \leq \alpha,$ then
if $f$ is partitionable then there is a deterministic
protocol $\Pi_f$ to compute $f.$ 

\noindent{\bf (Inductive Step.)}
Let $\abs{X} = \alpha+1.$  Say that $f$ is partitionable.
If $f$ is constant there is a trivial private protocol.
Otherwise, $f$ is row-partitionable or column-partitionable.

If $f$ is row-partitionable into $f_P$ and $f_Q,$ then by the
induction hypothesis there exist private
protocols $\Pi_{f_P}$ and $\Pi_{f_Q}$ for $f_P$ and $f_Q.$
Define the protocol $\Pi_f$ as follows.  If $x \in P,$ party 1
sends a 0; then the parties execute the protocol for $\Pi_{f_P}.$
Otherwise if $x \in Q,$ party 1 sends a 1,
and the parties execute the protocol for $\Pi_{f_Q}.$

Since the protocols are deterministic, let $\Pi(x,y)$ denote
the transcript of protocol $\Pi$ on inputs $x$ and $y.$

Protocol $\Pi_f$ is private with respect to party 1.
If $f(x,y)=f(x',y),$ then either $x,x' \in P$ or
$x,x' \in Q;$ otherwise $f$ would not be row-partitionable.
If $x,x' \in P,$ then
\[
\Pi_f(x,y)= 0 \circ \Pi_{f_P}(x,y) 
= 0 \circ \Pi_{f_P}(x',y) = \Pi_f(x',y).
\]
Similarly, if
$x,x' \in Q,$ then
$\Pi_f(x,y)= \Pi_f(x',y).$ 

Protocol $\Pi_f$ is also private with respect to party 2.
If $f(x,y)=f(x,y'),$ then either $x \in P,$ in which case
\[
\Pi_f(x,y)= 0 \circ \Pi_{f_P}(x,y) 
= 0 \circ \Pi_{f_P}(x,y') = \Pi_f(x,y');
\]
or $x \in Q,$ which likewise gives
$\Pi_f(x,y)= \Pi_f(x,y').$

Now, if $f$ is not row-partitionable then it must be
column-partitionable into $P$ and $Q.$  We now prove by
induction on $\beta=\abs{Y}$ that $f$ is private.
Say $\beta=1;$ then $f$ is trivially private.  Now,
assume that the hypothesis holds for $\abs{Y} \leq \beta.$
Consider $\abs{Y} = \beta+1.$  Then $f$ is partitionable
into $f_P$ and $f_Q,$ where $\abs{P},\abs{Q} \leq \beta.$
Hence there exist private protocols $\Pi_{f_P}$ and
$\Pi_{f_Q}$ for $f_P$ and $f_Q.$  The protocol for $f$ is
straightforward:
If $y \in P,$ party 2
sends a 0; then the parties execute the protocol for $\Pi_{f_P}.$
Otherwise if $y \in Q,$ party 2 sends a 1,
and the parties execute the protocol for $\Pi_{f_Q}.$
The proof that this  
$\Pi_f$ is private follows the same lines as above.
$\Box$


\subsection{Main Result}
\label{sec-main}

We can summarize the main result of this chapter in the following theorem:

\begin{theorem}    \label{thm-main}
\index{private function}
A finite function $f(x,y)$ is 1-private if and only if
it is partitionable.
\end{theorem}

\noindent{\bf Proof:}
Follows from lemmas \ref{lem-two-a} and \ref{lem-two-b}.
$\Box$

\section{Multiparty Privacy for Modular Protocols}

As described in Chapters \ref{chap-mod}, \ref{chap-con} and \ref{chap-min},
Many of the methods for performing arbitrary secret computations follow the
method of constructing a modular library of protocols that can be selected
and combined to construct new protocols.
%These methods develop basic protocols to evaluate simple gates
%and from there to evaluate a circuit applied to the inputs
%(cf. \cite{gmw87,bgw88,ccd88,kil88-ot}).
A general library based on threshold (secret sharing) methods allows the
output of one protocol to be maintained in a secret format suitable for
input to another protocol, so that intermediate computations are not
revealed.

In this section we consider what functions can be computed given an
arbitrary threshold scheme that allows addition of secrets over the field
used for sharing, when we also require that the output of the function be
retained as a secretly shared value for potential use in further
computations.

Let $E$ be a field and let $L_0$ be a set of function families mapping
$E^n$ to $E.$ Let $L$ be the closure of functions that can be written as a
finite composition of functions in $L_0.$ For example, with
$g,f_1,\dots,f_n \in L,$ the following function is in $L.$
\[
g(f_1(x_1,\dots,x_n),\dots,f_n(x_1,\dots,x_n)).
\]
A $t$-private {\em library} ${\cal L}$ for $L$
\index{protocol!library}
is a set of protocols satisfying:
\begin{itemize}
\item
Each protocol $\Pi \in {\cal L}$ computes a function $f \in L,$ $t$-privately.
\item
For every $f \in L$ there is a protocol $\Pi \in {\cal L}$
that computes it.
%\item
%For every set of protocols $\Pi_g,\Pi_1,\dots,\Pi_n,$ there is a composite
%protocol $\Pi$ which uses the outputs of $\Pi_1,\dots,\Pi_n$ as
%the input...
%For every $f_1,\dots,f_n,g \in L,$ 
%there is a protocol which,
%using calls to protocols for $f_1,\dots,f_n,g,$
%computes the following composition $t$-privately:
%\[
%g(f_1(x_1,\dots,x_n),\dots,f_n(x_1,\dots,x_n))
%\]
\end{itemize}
%Let $\mbox{ext}(L)$ be the set of functions which are $t$-privately computed
%either directly by ${\cal L}$ or by a nesting of finitely many
%protocols in ${\cal L}.$

The protocols for multiplication and addition given in \cite{bgw88,ccd88}
satisfy these properties, and in fact are complete for any finite function
when $t< \lceil \frac{n}{2} \rceil.$ In other words, they form a $\lceil
\frac{n}{2} \rceil$-private library for the class of all finite functions.

For $t \geq\lceil \frac{n}{2} \rceil,$ however, the situation is less
optimistic.  We show that any library sufficiently powerful to compute
affine functions over $E$ can {\em only} compute affine functions over the
field $E.$
\begin{theorem}
\label{thm-library}
If ${\cal L}$ is a $t$-private library of protocols that includes all
affine functions over the field $E,$ and if $t \geq\lceil \frac{n}{2}
\rceil,$ then any function $f(x_1,\dots,x_n) \in L$ can be written
\[
f(x_1,\dots,x_n) = f_1(x_1) + f_2(x_2) + \dots + f_n(x_n).
\]
\end{theorem}

{\bf Proof:} Let $f(x_1,\dots,x_n)$ be $t$-private for some $t \geq \lceil
\frac{n}{2} \rceil,$ and let $f$ depend on $k$ variables, $1 \leq k \leq
n.$ That is, for some $j_1,\dots,j_k$ and $\hat{f},$
\[
f(x_1,\dots,x_n) = \hat{f}(x_{j_1},\dots,x_{j_k}).
\]
Then we show by induction on $k$ that 
\[
(\exists f_1,\dots,f_n,\hat{f}) \hspace{0.1in}
f(x_1,\dots,x_n) = \sum_{i=1}^n f_{i}(x_{i}).
\]
%% \[
%% (\exists f_{j_1},\dots,f_{j_k})
%% f(x_1,\dots,x_n) = \sum_{i=1}^k f_{j_i}(x_{j_i}).
%% \]

The statement is trivially true for $k=1.$
Assume that it holds for $k.$

Let $f$ be $t$-private and let $f$ depend on $k+1$ variables:
\[
(\exists j_1,\dots,j_{k+1}) \hspace{0.1in}
f(x_1,\dots,x_n) = \hat{f}(x_{j_1},\dots,x_{j_{k+1}}).
\]
Without loss of generality let $j_1=1,j_2=2,\dots,j_{k+1}=k+1.$
Fix arbitrary arguments $a_1,\dots,a_{k+1},$  
and let $l = \lceil \frac{k}{2} \rceil.$
Suppose there exist $b_1,\dots,b_{k+1}$ such that
\begin{eqnarray}
\label{eqn-suppose}
\hat{f}(b_1,\dots,b_l,b_{l+1},\dots,b_{k+1})
+ \hat{f}(a_1,\dots,a_l,a_{l+1},\dots,a_{k+1}) 
& \not= & \\
\nonumber
\hat{f}(a_1,\dots,a_l,b_{l+1},\dots,b_{k+1})
+ \hat{f}(b_1,\dots,b_l,a_{l+1},\dots,a_{k+1}).
& & 
\end{eqnarray}
It is not hard to see that there exist $r$ and $s$ with $r \not= s,$
such that $a_r \not= b_r$ and $a_s \not= b_s.$

Define the linear functions $p_r$ and $p_s$ as
%%%%%%
\begin{eqnarray*}
p_r(x_1,\dots,x_{k+1}) & = &
(x_r - a_r) (b_r - a_r)^{-1}
( \hat{f}(b_1,\dots,b_l,a_{l+1},\dots,a_{k+1}) 
\\ & &
- \hat{f}(a_1,\dots,a_l,a_{l+1},\dots,a_{k+1}) ) 
\\
& &
+ \hat{f}(a_1,\dots,a_l,a_{l+1},\dots,a_{k+1})  \\
%%%%%%
p_s(x_1,\dots,x_{k+1}) & = &
(x_s - a_s) (b_s - a_s)^{-1}
( \hat{f}(a_1,\dots,a_l,b_{l+1},\dots,b_{k+1}) 
\\ & &
- \hat{f}(a_1,\dots,a_l,a_{l+1},\dots,a_{k+1}) ) 
\\
& &
+ \hat{f}(a_1,\dots,a_l,a_{l+1},\dots,a_{k+1}) 
\end{eqnarray*}
%%%%%%
Using the assumption that the library contains all affine functions,
%and is closed under finite composition,
the function $G$ defined as follows is $t$-private:
\[
G(x_1,\dots,x_n) =
f(x_1,\dots,x_n) 
- p_r(x_1,\dots,x_{k+1})
- p_s(x_1,\dots,x_{k+1})
+ \hat{f}(a_1,\dots,a_{k+1}).
\]
Clearly,
\begin{eqnarray*}
G(a_1,\dots,a_l,a_{l+1},\dots,a_{k+1},0,0,\dots,0) & = & 0, \\
G(a_1,\dots,a_l,b_{l+1},\dots,b_{k+1},0,0,\dots,0) & = & 0, \\
G(b_1,\dots,b_l,a_{l+1},\dots,a_{k+1},0,0,\dots,0) & = & 0, \\
G(b_1,\dots,b_l,b_{l+1},\dots,b_{k+1},0,0,\dots,0) & \not= & 0.
\end{eqnarray*}

Let $\Pi_G$ be a $t$-private protocol for $G.$  We use $\Pi_G$
to construct a $1$-private protocol for two parties to compute
AND(x,y), by having party 1 simulate half the parties and
party 2 simulate the other half.  
Party 1 holds an input $x \in \set{0,1},$ and party 2 holds an
input $y \in \set{0,1},$ though when they simulate $\Pi_G$ they
will ``pretend'' to hold general arguments instead.
Let $m = \lfloor \frac{n-k-1}{2} \rfloor.$
Party 1 follows $\Pi_G,$ simulating the parties holding inputs
$x_1,\dots,x_l;x_{k+2},\dots,x_{k+1+m}.$  
%Half of these inputs influence the value of $G.$  
Party 2 follows $\Pi_G,$ simulating
the parties holding inputs
$x_{l+1},\dots,x_{k+1};x_{k+m+2},\dots,x_n.$
Notice that neither party 1 nor party 2
simulates more than $t$ parties.

If party 1 holds input $x=0,$ it selects $x_1=a_1,\dots,x_l=a_l.$
If party 1 holds input $x=1,$ it selects $x_1=b_1,\dots,x_l=b_l.$
It sets all other variables to 0.
Similarly,
if party 2 holds input $y=0,$ it selects 
$x_{l+1}=a_{l+1},\dots,x_{k+1}=a_{k+1}.$
If party 2 holds input $y=1,$ it selects 
$x_{l+1}=b_{l+1},\dots,x_{k+1}=b_{k+1}.$
It sets all other variables to 0.

Together, party 1 and party 2 simulate $\Pi_G,$ sending messages to one
another when $\Pi_G$ specifies that a player from the group simulated by
party 1 interact with a player from the group simulated by party 2.
Both party 1 and party 2 learn the value of $G$ from the simulated
protocol.  If $G = 0,$ each outputs AND(x,y)$=0$; 
if $G \not= 0,$ each outputs AND(x,y)$=1$.
It is easy to see that their outputs are correct.

Since $\Pi_G$ is $t$-private, where 
$t \geq \lceil \frac{n}{2} \rceil,$
this two-party protocol is also $1$-private.
But Theorem~\ref{thm-main} implies that
there is no two-party $1$-private protocol for AND;
hence supposition~(\ref{eqn-suppose}) is false.  Thus,
\begin{eqnarray*}
f(x_1,\dots,x_n) & = &
f(a_1,\dots,a_l,x_{l+1},\dots,x_{k+1},0,\dots,0) 
\\ & &
+ f(x_1,\dots,x_l,a_{l+1},\dots,a_{k+1},0,\dots,0) 
\\
& &
- f(a_1,\dots,a_l,a_{l+1},\dots,a_{k+1},0,\dots,0).
\end{eqnarray*}
Define
\begin{eqnarray*}
g(x_1,\dots,x_n) & = &
f(a_1,\dots,a_l,x_{l+1},\dots,x_{k+1},0,\dots,0), \\
h(x_1,\dots,x_n) & = &
f(x_1,\dots,x_l,a_{l+1},\dots,a_{k+1},0,\dots,0).
\end{eqnarray*}

Since $f$ is $t$-private, so are $g$ and $h.$
But $g$ and $h$ each depend on at most $k$ variables.
By the induction
hypothesis, there are $g_1,\dots,g_n,h_1,\dots,h_n$ such that
\begin{eqnarray*}
g(x_1,\dots,x_n) & = &
g_1(x_1)+ \cdots + g_n(x_n), \\
h(x_1,\dots,x_n) & = &
h_1(x_1)+ \cdots + h_n(x_n).
\end{eqnarray*}
Let $d = f(a_1,\dots,a_l,a_{l+1},\dots,a_{k+1},0,\dots,0).$
Then we have,
\begin{eqnarray*}
f(x_1,\dots,x_n) & = &
g(x_1,\dots,x_n) + h(x_1,\dots,x_n) - d
\\
& = &
g_1(x_1)+ \cdots + g_n(x_n) + h_1(x_1)+ \cdots + h_n(x_n) - d \\
& = &
f_1(x_1) + \cdots + f_n(x_n),
\end{eqnarray*}
where we define $f_1(x_1)=g_1(x_1)+h_1(x_1) - d$
and $f_i(x_i) = g_i(x_i)+h_i(x_i)$ for $i \geq 2.$
This completes the induction step.  

Applying the result for $k=n,$ we conclude that
for an arbitrary $t$-private function $f$ 
there exist $f_1,\dots,f_n$ such that
\[
f(x_1,\dots,x_n) = f_1(x_1)+ \cdots + f_n(x_n),
\]
completing the proof of Theorem~\ref{thm-library}.
$\Box$




==> req.tex <==

\thispagestyle{empty}

\vspace*{1.0in}

\begin{center}
\Large \bf 
Security, Fault~Tolerance, and Communication~Complexity 
in~Distributed~Systems
\end{center}

\begin{center}
A thesis presented
\end{center}

\begin{center}
by
\end{center}

\begin{center}
{\Large Donald Rozinak Beaver}
\end{center}

\begin{center}
to
\end{center}

\begin{center}
The Division of Applied Sciences
\end{center}

\begin{center}
in partial fulfillment of the requirements\\
for the degree of 
Doctor of Philosophy\\
in the subject of 
Computer Science\\
Harvard University\\
Cambridge, Massachusetts
\end{center}

\begin{center}
May 1990
\end{center}

\newpage

\vspace*{2.0in}

\thispagestyle{empty}

\begin{center}
$\copyright$ 1990 by Donald Rozinak Beaver\\
All rights reserved.
\end{center}

\newpage



==> zkp.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% zkp.tex                    Zero Knowledge Proofs on Committed Bits.
%
%                            Copyright @1989  Donald Beaver.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\typeout{=======}
\typeout{zkp.tex}
\typeout{=======}

\chapter{Zero Knowledge Proofs on Committed Bits}
\label{chap-zkp}


Notarized envelope schemes\index{envelope!notarized} are a natural
extension of the zero-knowledge proof systems introduced by Goldwasser,
Micali, and Rackoff \cite{gmr89} (see \S\ref{sec-def-zk}).  An
envelope\index{envelope} scheme is a means to commit to a string $x$ (the
contents of the envelope) in such a way that $x$ cannot later be changed.
Until the envelope is opened, the string remains secret.  It is similar to
secret-sharing in these respects: a secretly shared value remains hidden
until it is explicitly reconstructed, and its value cannot be changed in
the meantime.  In fact, threshold schemes provide a natural means to
implement envelopes in the presence of a network, an idea that will be
especially useful in Chapter~\ref{chap-mpp}.

A {\em notarized} envelope\index{envelope!notarized} provides some
additional information about the contents of the envelope.  Namely, it is
an envelope associated with a predicate $\scp$ that holds true when applied
to the contents.  The truth of the predicate may reveal information about
the contents; but nothing more is compromised.  Like zero-knowledge
proofs,\index{zero-knowledge proof!on envelopes} the bearer of the
envelope sees the simple fact that $x \in L$ --- or here, the fact that
$\scp(x)=1$ --- and whatever else it can compute given the notarized
envelope, it can compute given simply that $\scp(x)=1.$ (We shall consider
an even stronger statement: for some {\em function} $F,$ the committer
commits to $x$ and also provides a value $y$ such that $F(x)=y.$ The
example of a predicate is one-sided in that it does not apply when
$\scp(x)=0.$)

Using cryptographic assumptions, notarized envelope schemes have been
developed by, among others, Goldreich, Micali, Wigderson \cite{gmw86},
Brassard, Chaum, \crepeau\  \cite{bcc88}, and Impagliazzo, Yung \cite{iy87}.
In this model, at least one of the two players (prover and verifier) is
limited in computational power, and bit commitment is implemented using
cryptographic tools such as one-way functions.

We shall consider the {\em ideal envelope model},\index{envelope!ideal} in
which both prover and verifier have unlimited computational power, no
cryptographic assumptions are made, and bit commitment is assumed as a
primitive.  Any primitive that implements bit commitment in this model is
called an {\it envelope scheme}.  A natural question to address is whether
notarized envelope schemes exist in this model; that is, can notarized
envelopes be constructed from generic envelopes?  This question was
answered in the affirmative by Bennett, Brassard, Cr\'epeau \cite{bbc},
Ben-Or {\it et al.}~\cite{bgg88}, and Rudich \cite{ru}.

The resources measures for notarized envelope schemes are similar to those
of multiparty protocols, or for that of any interaction, for that matter.
Local computing time and space, number of rounds of interaction, 
message sizes, and number of generic envelopes (``envelope complexity'')
are of primary interest.

The notarized envelope schemes of \cite{bbc,bcc88,bgg88,gmw86,iy87,ru} are
not directly comparable, because they consider a wide variety of models,
but they have one feature in common: All have bit complexity proportional
to the circuit complexity of $\scp$.  Here, we achieve a more
communication-efficient general construction of notarized envelope schemes.
We consider the execution of an ideal generic envelope scheme to require
$O(1)$ rounds.

\begin{theorem}   \label{thm-zkp-const}
(Constant Rounds Notarization)%
\index{notarization!constant rounds}
In the ideal envelope model, every function family $F$ (and thus every
predicate family $\scp$) has an exponentially-secure notarized envelope
scheme that uses a {\em constant} number of rounds and a small polynomial
number (in $(n,M,k)$) of envelopes and bits, {\em regardless} of the
computational complexity of $F.$
\end{theorem}

By comparison, zero-knowledge proof systems are limited to languages in
$\ip=\pspace.$ Though it is unlikely that there are small circuits
describing $\pspace$ languages, the class of provable statements is limited,
and there are no proof systems requiring only a bounded number of rounds.
Our construction for notarized envelopes makes no restriction on the
predicates, and uses a bounded number of rounds.


\section{Definitions}

An {\em ideal (generic) envelope scheme}\index{envelope!generic} is the
following two-stage ideal protocol for three players, one of whom is a
trusted host.  We refer to the players as the Sender S, the Recipient R,
and the trusted Intermediary I.  In the first stage, S sends either the
message {\em refuse} or it sends a bit $b$ to I.  If it sends a bit $b,$
then I sends the message {\em accept} to R, to indicate having accepted a
bit; otherwise I sends {\em reject} to indicate refusal or misbehavior.  In
the second stage, S sends one of two messages, {\em open} or {\em retain},
to I.  If S sends {\em open}, then I sends $b$ to R.  If S sends {\em
retain}, then I sends $\Lambda$ to R.  This protocol is similar to the
Verifiable Time-Release Schemes of Chapter~\ref{chap-min}, though here we
are not concerned whether the intermediary knows the bit.

Committing to a string $x$ simply means performing $\abs{x}$ repetitions of
the ideal envelope scheme, one for each bit of $x.$ We assume a different
trusted intermediary for each committed bit.  We say that S ``opens an
envelope'' to mean that S sends {\em open} in stage 2.

An {\em ideal notarized envelope scheme} for (deterministic) function
family $F$ requires a few simple modifications.  The sender sends strings
$x$ and $y$ to I, who computes $F(x).$ If $F(x)=y,$ then I returns ({\em
accept},$y$) to R; otherwise, I sends ({\em reject},$y$).  In the second
stage, I sends either $x$ or $\Lambda$ to R, according to the request of S.

Where clear from context, we in fact refer to a notarized envelope for $F$
as one of two cases: as above, the sender S has provided a value $y$ for
$F(x);$ or secondly, the sender has also committed $y$ and is ``really''
using a notarized envelope for the function $\chi_F(x,y)$ defined as 1 iff
$F(x)=y,$ and otherwise 0.  In the latter case we implicitly assume the
sender is claiming $\chi_F(x,y)=1.$

A notarized envelope for a predicate $\scp$ has classically been defined as
the special modification in which $y=1$ always.  This weak notion does not
allow the sender to claim that the predicate does {\em not} hold.  It
corresponds to zero-knowledge in the sense that zero-knowledge proof
systems are one-sided; they show that a string $x$ is in a language, but do
not need to show $x$ is not in a language.  Thus, notarized envelopes for
predicates in NP are distinguished from notarized envelopes for coNP, or
even from notarized envelopes for NP$\cap$coNP --- which corresponds to the
more powerful definition in terms of {\em functions}.  That is, given an NP
predicate $\scp,$ if the sender is allowed to {\em choose} $y=0$ or $y=1$
then the function $F$ is an NP$\cap$coNP decision question; if the sender
were allowed only to claim $y=1,$ then the function $F$ would be an NP
decision problem, corresponding to the case of proof systems for NP.

No efficient notarized envelope schemes built on generic envelope schemes
have previously been discovered for predicates outside of NP, even with the
weaker one-sided definition.  We observe that the techniques employed to
show that $\ip=\pspace$ provide an unbounded-round method for notarized
envelopes, even with the stronger two-sided definition; and they provide an
implementation for a sender and receiver of different computational power.
In this chapter, however, we consider equally powerful parties and present
results that are not only more general but more efficient than past methods
and derivations of those methods.



\section{Notarized Envelopes from Generic Envelopes}
\label{sec-notarize}

\begin{proofof}{Theorem \ref{thm-zkp-const}}
Our goal is to construct a protocol that uses generic envelope schemes to
implement a notarized envelope scheme.  In order to construct {\em
notarized} envelopes for an arbitrary function family $F,$ we use a $(1,m)$
locally random reduction from $F$ to a family $G$ of polynomials.

We shall make use of the following important result for functions that can
be computed by logarithmic depth, polynomial size circuits.  It certainly
applies to the reduction (P) and interpolation (Q) functions of the locally
random reductions of Chapters \ref{chap-ihs} and \ref{chap-lrr}, which are
randomized $NC^1$ computations.
\begin{theorem}  \label{thm-zkp-poly}
{(Bennett et al.~\cite{bbc}, Ben-Or et al.~\cite{bgg88}, Rudich \cite{ru})}
If $F^{n,M}$ is computable by a boolean or arithmetic circuit of depth
$O(\log nM)$ and size polynomial in $nM,$ then it has a notarized envelope
scheme \notenvnc with constant round complexity, polynomial bit
complexity, and polynomial envelope complexity.
\end{theorem}

The protocol \notenv(F,x,y) for notarized envelopes for arbitrary function
$F$ is described in Figure~\ref{fig-notarized}.  Essentially, the sender
repeats the following protocol $kn^2$ times in parallel.  It first commits
to two sequences of random bits $r_1$ and $r_2$ that the reduction and
interpolation algorithms, P and Q, will use.  (Assume that the two
randomized algorithms require $p(n)$ bits on inputs of length $n;$ with
these bits, the algorithms are essentially deterministic.)  The sender uses
a notarized envelope to commit to a string containing $m$ outputs
$y_1',y_2',\ldots,y_m'$ that it claims to be the outputs of $P(r_1,x).$ The
sender also uses a notarized envelope to commit values
$z_1,z_2',\ldots,z_m$ that it claims satisify
$Q(r_2,z_1',z_2',\ldots,z_m')=y.$ These two claims are satisfied using the
notarization schemes for polynomial size circuits \cite{bbc,bgg88,ru}.

The crucial claim is the following.  The sender claims that for each $i \in
[m],$ $z_i' = G(y_i').$ Of course, the computation of $G(y_i')$ might
require a large circuit, and previous techniques will not apply without
incurring tremendous expense in terms of bits, rounds, and commitments.
The sender ``proves'' his claim by allowing the receiver to open {\em one}
of the pairs $(y_i',z_i').$ If S has behaved then indeed $z_i'=G(y_i'),$
and R will accept it.  If S has not behaved, namely if $F(x) \not= y,$ then
given that $P(r_1,x)=(y_1',y_2',\ldots,y_n')$ and
$Q(r_2,z_1',z_2',\ldots,z_n')=y,$ there must be some pair $(y_i',z_i')$ for
which $z_i' \not= y_i'.$ With probability at least $1/m,$ then, R will
detect cheating and reject.  The probability is at least $1/n$ if a $(1,n)$
LRR is used, and through amplification by repetition, the probability is at
least $1-(1-1/n)^{kn^2}$ or asymptotically $1-e^{-kn}$ that R detects
cheating if it exists.  (Locally random reductions with sharper parameters
will decrease the number of repetitions needed to amplify the
probabilities.)



\figstretch
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Figure:  Notarized Envelopes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\boxfig{
\noindent{\bf \notenv}(F,x,y)
\begin{tabbing} \standtabs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\bf Stage I (Commit):}\\
\> S computes $y=F(x)$ and sends $y$ to R.\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\> {\For $K=1..nk^2$ \Dopar:}  \\
\>\> \Begin \\
\>\> S commits two uniformly random strings $\rhat_1^K,\rhat_2^K$ of 
length $p(n).$ \\
\>\> R sends to S two uniformly random strings $\shat_1^K,\shat_2^K$ of 
length $p(n).$ \\
\>\> S sets $r_1^K=\rhat_1^K \oplus \shat_1^K, 
     r_2^K=\rhat_2^K \oplus \shat_2^K.$ \\
\>\> S computes $P(r_1^K,x) = (y_1^K,y_2^K,\ldots,y_m^K).$ \\
\>\> {\For $i=1..m:$} S computes $z_i^K=G(y_i^K).$ \\
\>\> S runs {\notenvnc}($P$;$x,r_1^K$;$y_1^K,y_2^K,\ldots,y_m^K$). \\
\>\> R assigns $P_{K}$ to be {\em accept} or {\em reject} accordingly. \\
\>\> S runs {\notenvnc}($P$;$r_2^K,z_1^K,z_2^K,\ldots,z_m^K$;$y$). \\
\>\> R assigns $Q_{K}$ to be {\em accept} or {\em reject} accordingly. \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\>\> R randomly chooses $(i_1,\ldots,i_K) \in_R [m]^K$ and sends it to S.\\
\>\> S opens the generic envelopes containing $y_i$ and $z_i$ for each $i.$\\
\>\> R receives the opened values $y_i'$ and $z_i'.$\\
\>\> R computes $G(z_i').$\\
\>\> \End \\
\> \If for all $K \in [nk^2],$ $y_i'=G(z_i')$ and $P_K=Q_K=${\em accept}, \\
\>\> \Then R outputs ({\em accept},$y$)\\
\>\> \Else  R outputs ({\em reject},$y$).\\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\bf Stage II (Open):} \\
\> S opens the generic envelopes containing $x.$
\end{tabbing}
\caption{\label{fig-notarized}
\index{\notenv}
Protocol for sender S to place $x$ in a notarized envelope claiming $F(x)=y.$
$(P,Q)$ is a $(1,m)$ locally random reduction from $F$ to $G,$ and $P$
and $Q$ are $NC^1$ computations.
}}
\figstretchend

More formally, the overall protocol computes the composition of three
functions, $F^1,$ $F^2,$ and $F^3.$ The first computes a robust and private
representation of $x$ and $\set{r_1^K,y_1^K,y_2^K,\ldots,y_m^K}_{K\in
[nk^2]},$ as well as the appropriate output {\em accept} or {\em reject}
for receiver R.  The output is clearly private: a reliable sender will
always provide inputs producing {\em accept} for R, and the output induced
by a corrupted sender depends only on the sender's information.  The second
computes a robust and private representation of $y$ and
$\set{r_2^K,z_1^K,z_2^K,\ldots,z_m^K}_{K\in [nk^2]}$ as well as the
appropriate output {\em accept} or {\em reject} for receiver R.
The third computes the function that computes {\em reject} if R has
rejected anything so far, and computes {\em reject} if any $i_j$
selects a pair $(y_i,z_i)$ that was computed incorrectly, and otherwise
computes {\em accept} for R.  Function $F^3$ is private, since if S is
reliable then the output is always {\em accept}.  It is a robust
representation of the statement that $r_1,r_2,i_1,i_2,\ldots,i_{nk^2}$
select a random reduction and a set of pairs that are consistent.  

The overall protocol runs three subprotocols in sequence, each of which
computes one of these robust and private representations of intermediate
values.  It uses a security parameter of $k'=k/4$ to ensure that the
concatenation is sufficiently resilient.

The ideal notarized envelope protocol allows no chance to cause R to output
{\em accept} improperly.  The composite interface for the three functions
$F^1,$ $F^2,$ and $F^3$ can simulate all outcomes accurately given that
cheating does not go undetected, namely that the executions of \notenvnc
for the first two phases do not run into an undetected inconsistency, and
that $r_1,r_2,i_1,i_2,\ldots,i_{nk^2}$ do not lead to an undetected
inconsistency.  The probability of such runs is at most $2^{-k'} 2^{-k'}
2^{-k'} < 2^{-k}.$ Hence the output distributions induced by the simulator
are exponentially close to that of the ideal notarized envelope protocol.
\end{proofof}



\section{Zero-Knowledge Proofs About Secrets}
\label{sec-zkmips-any}
\index{zero-knowledge proof!on secrets}

In \S\ref{sec-zkmips} we saw that any function $F_{\predicate}$ for a
predicate $\predicate$ admits a multiparty zero-knowledge interactive proof
system having constant round complexity and having message complexity
polynomial in the size of $C_{\predicate},$ a circuit for $\predicate.$

Using locally random reductions, we can show that the message complexity is
indeed independent of the circuit complexity, namely that the message
complexity is polynomial in $n,$ $m,$ and $k,$ for any $\predicate.$

Secret-sharing is indeed a method for committal, given one technical
restriction: since the committer has the option of refusing to
decommit, the reconstruction protocol must be adapted so that reliable
players give up their pieces only if the dealer requests.

A multiparty zero-knowledge proof system on secrets%
\index{zero-knowledge proof!on secrets}
(definition~\ref{def-zkmips}) is then a special case of a notarized
envelope scheme where envelopes are replaced by secret-sharing.
As a direct application of Theorem~\ref{thm-zkp-const}, we have the
following:

\begin{theorem}
(Constant Rounds ZKMIPSS) In the ideal envelope model, every function
family $F$ (and thus every predicate family $\scp$) has an
exponentially-resilient notarized envelope scheme that uses a {\em constant}
number of rounds and a small polynomial number of envelopes and bits.
\end{theorem}




